Abstract 3-Rigidity and Bivariate $C_2^1$-Splines I: Whiteley's Maximality Conjecture

A conjecture of Graver from 1991 states that the generic $3$-dimensional rigidity matroid is the unique maximal abstract $3$-rigidity matroid with respect to the weak order on matroids. Based on a close similarity between the generic $d$-dimensional rigidity matroid and the generic $C_{d-2}^{d-1}$-cofactor matroid from approximation theory, Whiteley made an analogous conjecture in 1996 that the generic $C_{d-2}^{d-1}$-cofactor matroid is the unique maximal abstract $d$-rigidity matroid for all $d\geq 2$. We verify the case $d=3$ of Whiteley's conjecture in this paper. A key step in our proof is to verify a second conjecture of Whiteley that the `double V-replacement operation' preserves independence in the generic $C_2^1$-cofactor matroid.

==> cofactor1(da_final)/badmotions.tex <==
\section{\boldmath Bad $C_2^1$-Motions} \label{sec:bad}

In this section, we show that if Theorem~\ref{thm:doubleV} does not hold for some graph $G$, then every generic realization of $G$ in $\mathbb{R}^2$ has a special kind of motion, and  derive some properties of such `bad' motions.
%Motivated by the form of the motion, we define a class of "bad" motions.
We use these properties in Section~\ref{sec:well-behaved}, to prove that no 
%1-dof 
generic framework can have a bad motion.

The following notation will be used throughout the remainder of this paper.
Suppose $p_i=(x_i, y_i)$ is a point in the plane for $i=0,1,2,3$. 
For any three of these points, we let 
$$\Delta(p_i, p_j, p_k)=\begin{vmatrix} x_i & y_i & 1 \\ x_j & y_j & 1 \\ x_k & y_k & 1 \end{vmatrix},$$
which is twice the signed area of the triangle defined by the three points.
%When the points belong to a framework $(G,\bp)$, we simply denote $\Delta(\bp(v_i), \bp(v_j), \bp(v_k))$ by $\Delta(v_i,v_j,v_k)$ or $\Delta_{i,j,k}$.
%For all four points, 
The formula for the determinant of a Vandermonde matrix implies that
\begin{align}
\left|
\begin{array}{c}
D(p_0, p_1) \\ D(p_0 , p_2) \\ D(p_0, p_3)
\end{array}\right|
&=-\left|
\begin{array}{ccc}
x_0 & y_0 & 1 \\
x_1 & y_1 & 1 \\
x_2 & y_2 & 1
\end{array}\right|
\left|
\begin{array}{ccc}
x_0 & y_0 & 1 \\
x_2 & y_2 & 1 \\
x_3 & y_3 & 1
\end{array}\right|
\left|
\begin{array}{ccc}
x_0 & y_0 & 1 \\
x_3 & y_3 & 1 \\
x_1 & y_1 & 1
\end{array}\right| \\
&=-\Delta(p_0, p_1, p_2) \Delta(p_0, p_2, p_3) \Delta(p_0, p_3, p_1). \label{eq:Vandermonde}
\end{align}
See, e.g., \cite[page~15]{W90} for further details.
%Further details are given in Appendix \ref{app:Delta}.

\subsection{Bad local behavior}
%In the proof of Theorem~\ref{thm:doubleV} we use the following projective invariance of the rank of  $C_2^1$-cofactor matrices.
%
%Let $(G,p)$ be a two dimensional framework.
%We say that a two dimensional framework $(G,p')$ is a {\em projective image} of $(G,p)$ if there are nonsingular $A\in \mathbb{R}^{3\times 3}$ and a non-zero $k_v\in \mathbb{R}$ for each $v\in V$ such that
%%$\begin{pmatrix} q_v  \\ 1\end{pmatrix}=k_v A \begin{pmatrix} p_v \\  1\end{pmatrix}$ 
%$\begin{pmatrix}p'(v)\\ 1\end{pmatrix}=k_v A\begin{pmatrix} p(v)\\ 1\end{pmatrix}$
%for every $v\in V$.
%\begin{lemma}(Whiteley~\cite[Theorem 11.3.2.]{Wsurvey}) \label{lem:projective}
%Let $(G,p)$ be a two dimensional framework, and $(G,q)$ be a projective image of $(G,p)$.
%Then $\rank C_2^1(G,p)=\rank C_2^1(G,q)$.
%\end{lemma}

%If the underlying framework $(G,p)$ is clear, we simply denote $\Delta(p(v_i), p(v_j), p(v_k))$ by $\Delta(v_i,v_j,v_k)$.
The following key lemma states that if Theorem~\ref{thm:doubleV} does not hold for some vertex $v_0$ of type ($\star$) in a  graph $G$, then every generic framework $(G,\bp)$ has a non-trivial $C_2^1$-motion $\bq$ with the property that each coordinate  of $\bq(v_i)$,  for $v_i\in \hat N_G(v_0)$, can be expressed as a polynomial in the coordinates of the points $\bp(v_j)$, for $v_j\in \hat N_G(v_0)$.  
We  note that the precise formulae of Lemma~\ref{lem:motion} are not important in the remaining proof, and only the fact  that each coordinate is written as a polynomial in the coordinates of $\bp(v_0), \bp(v_1),\dots, \bp(v_5)$ will be important.
\begin{lemma}
\label{lem:motion}
Let $(G,\bp)$ be a generic framework,
%with $|E|=3|V|-6$  and
 $v_0$ be a vertex of type $(\star)$ in $G$
with $N_G(v_0)=\{v_1,\dots, v_5\}$,  $H=G-v_0$
and $\bp|_H$ be the restriction of $\bp$ to $H$. 
Suppose that 
%${\rm cl}(E(G-v_0))$ forms a star on $N_G(v_0)$ centered at $v_5$. If 
$G$ is not $C_2^1$-rigid. Then there exist non-trivial $C_2^1$-motions $\bq_1$ of $(H+v_1v_2, \bp|_H)$ and 
$\bq_2$ of $(H+v_1v_3, \bp|_H)$ satisfying
\begin{align*}
\bq_1(v_1)&=\bq_1(v_2)=\bq_1(v_5)=0, \\ 
\bq_1(v_3)&=\Delta(\bp(v_1),\bp(v_2),\bp(v_3)) D(v_3, v_4) \times D(v_3, v_5),  \\
\bq_1(v_4)&=\Delta(\bp(v_1),\bp(v_2),\bp(v_4)) D(v_3, v_4)\times D(v_4, v_5),
\end{align*}
and
\begin{align*}
\bq_2(v_1)&=\bq_2(v_3)=\bq_2(v_5)=0, \\
\bq_2(v_2)&=\Delta(\bp(v_1), \bp(v_3), \bp(v_2)) D(v_2, v_4)\times D(v_2, v_5), \\
\bq_2(v_4)&=\Delta(\bp(v_1), \bp(v_3), \bp(v_4)) D(v_2, v_4)\times D(v_4, v_5),
\end{align*}
where $\times$ denotes the 
%exterior 
cross product of two vectors.
Moreover, $G$ has a non-trivial motion $\bq$ such that $\bq|_{V-v_0} = \alpha \bq_1 + \beta \bq_2$, where
\begin{align*}
\alpha=\begin{vmatrix} D(v_0, v_2) \\ D(v_2, v_4) \\ D(v_2,v_5) \end{vmatrix} \begin{vmatrix} D(v_0, v_3) \\ D(v_0, v_1) \\ D(v_0, v_5) \end{vmatrix}, 
\quad
\beta=-\begin{vmatrix} D(v_0, v_3) \\ D(v_3, v_4) \\ D(v_3, v_5) \end{vmatrix} \begin{vmatrix} D(v_0, v_2) \\ D(v_0, v_1) \\ D(v_0, v_5) \end{vmatrix},
\end{align*}
and $\bq(v_0)$ is given by 
\[
\bq(v_0)=\Delta(\bp(v_1), \bp(v_2) \bp(v_3))\begin{vmatrix} D(v_0, v_3) \\ D(v_3, v_4) \\ D(v_3, v_5) \end{vmatrix} 
\begin{vmatrix} D(v_0, v_2) \\ D(v_2, v_4) \\ D(v_2, v_5) \end{vmatrix}
 D(v_0, v_1)\times D(v_0, v_5).
\]
\end{lemma}
\begin{proof}
For simplicity, put $D_{i,j}=D(v_i,v_j)$ and $\Delta_{i, j, k}=\Delta(\bp(v_i), \bp(v_j), \bp(v_k))$.

Since $v_0$ is of type $(\star)$ in $G$, 
%$H+v_1v_2+v_1v_3$ and $H+v_2v_3+v_3v_4$ are both $C_2^1$-rigid. Hence   
$(H+v_1v_2+v_1v_3,\bp|_H)$ and $(H+v_1v_3+v_3v_4,\bp|_H)$ are both  $C_2^1$-rigid.
Also ${\rm cl}(E(H))$ forms a star on $N_G(v_0)$ centered at $v_5$.
%, 
% \begin{equation}
% \label{eq:coordinates}
% \bp|_H(v_1)=(0,0), \quad \bp|_H(v_2)=(0,1),  \quad \bp|_H(v_3)=(1,0), \quad \bp|_H(v_5)=(1,1),
% \end{equation}
%  and $\{\bp|_H(v_i)\,:\, i\neq 1,3,4,5\}$ is generic. 
 We first prove a result concerning the $C_2^1$-motions of $(H,\bp|_H)$.

\begin{claim}\label{claim:Hbase}  There exist non-trivial $C_2^1$-motions $\bq_1$ of $(H+v_1v_2,\bp|_H)$ and $\bq_2$ of $(H+v_1v_3,\bp|_H)$ such that:\\
(a) $\bq_1(v_1)=\bq_1(v_2)=\bq_1(v_5)=0$, $D_{3,4}\cdot [\bq_1(v_3)-\bq_1(v_4)]=0$, and
$D_{1,3}\cdot \bq_1(v_3)\neq 0$;\\
(b) $\bq_2(v_1)=\bq_2(v_3)=\bq_2(v_5)=0$, $D_{2,4}\cdot [\bq_2(v_2)-\bq_2(v_4)]=0$, and
$D_{1,2}\cdot \bq_2(v_2)\neq 0$;\\
%(c) $D_{1,3}\cdot \bq_1(v_3)\neq 0 \neq D_{1,2}\cdot q_2(v_2)$.
(c) $Z(H,\bp|_H)=Z_0(H,\bp|_H)\oplus\langle \bq_1,\bq_2 \rangle$.
%where $\langle \bq_1,\bq_2 \rangle$ denotes the linear  span of $\bq_1$ and $\bq_2$.
\end{claim}
\begin{proof}
Since  ${\rm cl}(E(H))$ forms a star on $N_G(v_0)$ centered at $v_5$, 
${\rm cl}(E(H)+v_1v_2)$ contains the triangle $K(v_1,v_2,v_5)$.
%Hence by  $\dim Z(H+v_1v_2,\bp|_H)=7$, 
Since $G$ contains a $1$-extension of $H+v_1v_2$ and  is not $C_2^1$-rigid, $H+v_1v_2$ is not $C_2^1$-rigid. Hence we can choose a non-trivial motion $\bq_1$ of $(H+v_1v_2,\bp|_H)$ such that  $\bq_1(v_1)=\bq_1(v_2)=\bq_1(v_5)=0$ (by pinning the triangle on $\{v_1,v_2,v_5\}$).
The fact that $(H+v_1v_2+v_1v_3,\bp|_H)$ is  $C_2^1$-rigid implies that
$D_{1,3}\cdot [\bq_1(v_3)-\bq_1(v_1)]=D_{1,3}\cdot \bq_1(v_3)\neq 0$. 
If  $D_{3,4}\cdot [\bq_1(v_3)-\bq_1(v_4)]\neq 0$ then $H+v_1v_2+v_3v_4$ would be $C_2^1$-rigid, and $G$ would also be $C_2^1$-rigid since it can be obtained from $H+v_1v_2+v_3v_4$ by an X-replacement. Thus $D_{3,4}\cdot [\bq_1(v_3)-\bq_1(v_4)]= 0$. 
This completes the proof of (a). Part (b) can be proved analogously.

The facts that  $D_{1,2}\cdot [\bq_1(v_1)-\bq_1(v_2)]=0\neq D_{1,2}\cdot [\bq_2(v_1)-\bq_2(v_2)]$ and
$D_{1,3}\cdot [\bq_1(v_1)-\bq_1(v_3)]\neq 0= D_{1,3}\cdot [\bq_2(v_1)-\bq_2(v_3)]$ imply that $\bq_1,\bq_2$ are linearly independent and can be extended to a base of $Z(H,\bp|_H)$ by adding the vectors in a base of $Z_0(H,\bp|_H)$. Hence $Z(H,\bp|_H)=Z_0(H,\bp|_H)\oplus\langle \bq_1,\bq_2 \rangle$.
\end{proof}

%Since $(G,p)$ is a generic framework, we may suppose that $p(v_0)=(x_0,y_0)$ is algebraically independent over
%$\rat(p|_H,\bq_1,\bq_2)$.


\begin{claim}\label{claim:Gmotion}  There exists a non-trivial $C_2^1$-motion $\bq$ of $(G,\bp)$ such that $\bq|_H=\alpha \bq_1+\beta \bq_2$ for some $\alpha, \beta\in \R$ with $\beta\neq 0$.
\end{claim}
\begin{proof}
Since $G$ is not $C_2^1$-rigid, we may choose a non-trivial $C_2^1$-motion $\bq$ of $(G,\bp)$. Since $d_G(v_0)=5$, $\bq|_H$ is a non-trivial $C_2^1$-motion of $(H,\bp|_H)$. By Claim \ref{claim:Hbase}(c),
$\bq|_H=\bq_0+\alpha \bq_1+\beta \bq_2$ for some $\bq_0\in Z_0(H,\bp|_H)$ and $\alpha,\beta\in \R$. We may choose $\tilde \bq\in Z_0(G,\bp)$ such that $\tilde \bq|_H=\bq_0$. Then $\hat \bq=\bq-\tilde \bq$ is a non-trivial $C_2^1$-motion of $(G,\bp)$ and  $\hat \bq|_H=\alpha \bq_1+\beta \bq_2$.
Since $(G+v_1v_2,\bp)$ can be obtained from  $(H+v_1v_2+v_1v_3,\bp|_H)$ by first performing a 1-extension operation and then adding the edge $v_0v_5$, $(G+v_1v_2,\bp)$ is $C_2^1$-rigid. This tells us that $D_{1,2}\cdot [\hat \bq(v_1)- \hat \bq(v_2)]\neq 0$ and hence $\beta\neq 0$. %Thus $\beta^{-1}\hat q$ is the required $C_2^1$-motion of $(G,\bp)$.
\end{proof}

Let  $\alpha, \beta$ be as described in Claim~\ref{claim:Gmotion}, and put $\gamma=\alpha/\beta$.
For all $1\leq i\leq 5$, $G$ contains the edge $v_0v_i$, and so
$D_{0,i}\cdot [\bq(v_0)-\bq(v_i)]=0$. Since
%$\bq(v_0)=(a_0,b_0,c_0)$ and
$\bq(v_i)=\alpha \bq_1(v_i)+\beta \bq_2(v_i)$ for $1\leq i\leq 5$,
% and $\bp(v_i)=(x_i,y_i,z_i)$ for $0\leq i\leq 5$,
we obtain the system of equations
$$ D_{0,i}\cdot [\bq(v_0)/\beta-\gamma \bq_1(v_i)]=D_{0,i}\cdot \bq_2(v_i) \mbox{ for $1\leq i\leq 5$}.$$
Putting $\bq(v_0)/\beta=(a_0,b_0,c_0)$, and using the facts that $\bq_1$ is zero on $v_1,v_2,v_5$ and $\bq_2$ is zero on $v_1,v_3,v_5$, we may rewrite this system as the matrix equation

\begin{equation}
\label{eq:dV2}
\left(
\begin{array}{ccc}
D_{0,1} &0 \\
D_{0,2} & 0\\
D_{0,3} & -D_{0,3}\cdot \bq_1(v_3)\\
D_{0,4} & -D_{0,4}\cdot \bq_1(v_4)\\
D_{0,5} & 0
\end{array}
\right) \left(
\begin{array}{c}
a_0\\ b_0\\ c_0\\ \gamma
\end{array}
\right) =
\left(
\begin{array}{c}
0 \\
D_{0,2}\cdot \bq_2(v_2)\\
0\\
D_{0,4}\cdot \bq_2(v_4)\\
0
\end{array}
\right)\,.
\end{equation}

\bigskip\noindent
Since this equation has a solution for $a_0,b_0,c_0,\gamma$ we have
\begin{equation}\label{eq:dV3}
\left|
\begin{array}{ccc}
D_{0,1} &0 & 0\\
D_{0,2} & 0 & D_{0,2}\cdot \bq_2(v_2)\\
D_{0,3} & -D_{0,3}\cdot \bq_1(v_3) & 0\\
D_{0,4} & -D_{0,4}\cdot \bq_1(v_4) & D_{0,4}\cdot \bq_2(v_4)\\
D_{0,5} & 0 & 0
\end{array}
\right| = 0\,.
\end{equation}

Let $\bp(v_0)=(x_0,y_0)$.
The left hand side of (\ref{eq:dV3}) is a polynomial in $x_0,y_0$ with coefficients in $\mathbb{Q}(\bp|_H, \bq_1, \bq_2)$. Since it is equal to zero for all generic values of $x_0,y_0$, each coefficient is zero. This implies that (\ref{eq:dV3}) will hold for {\em all} values of $x_0$ and $y_0$, including  non-generic choices of $\bp(v_0)$.

\begin{claim}\label{cllm:dV4-1}
%\begin{equation}
%\label{eq:dV4-1}
$D_{3,4}\cdot \bq_1(v_3)=0.$
%\end{equation}
\end{claim}
\begin{proof}
We choose $\bp(v_0)$ to be a point on the interior of the line segment joining  $\bp(v_3)$ and $\bp(v_4)$.
Then $D_{0,3}$ and $D_{0,4}$ are scalar multiples of $D_{3,4}$.
We can now use elementary row and column operations to convert (\ref{eq:dV3}) to
\begin{equation}
\label{eq:dV3-2}
\left|
\begin{array}{ccc}
D_{0,1} &0 & 0\\
D_{0,2} & 0 & D_{0,2}\cdot \bq_2(v_2)\\
D_{3,4} & D_{3,4}\cdot \bq_1(v_3) & 0\\
0 & D_{3,4}\cdot (\bq_1(v_4)-\bq_1(v_3)) & D_{3,4}\cdot \bq_2(v_4)\\
D_{0,5} & 0 & 0
\end{array}
\right| = 0.\,
\end{equation}
Since $D_{3,4}\cdot (\bq_1(v_4)-\bq_1(v_3))=0$ by Claim \ref{claim:Hbase}(a), this gives
\begin{equation}
\label{eq:dV3-3}
\left|
\begin{array}{ccc}
D_{0,1} &0 & 0\\
D_{0,2} & 0 & D_{0,2}\cdot \bq_2(v_2)\\
D_{3,4} & D_{3,4}\cdot \bq_1(v_3) & 0\\
0 &0 & D_{3,4}\cdot \bq_2(v_4)\\
D_{0,5} & 0 & 0
\end{array}
\right| = 0.\,
\end{equation}
Hence
\begin{equation}\label{eq:dV3-4}
\left|
\begin{array}{c}
D_{0,1} \\ D_{0,2} \\ D_{0,5}
\end{array}\right|
(D_{3,4}\cdot \bq_1(v_3)) \,
%(D_{3,4}\cdot (\bq_2(v_4)-\bq_2(v_3)))=0.
(D_{3,4}\cdot \bq_2(v_4))=0.
\end{equation}
As long as $\bp(v_0)$ is generic on the line through $\bp(v_3)$ and $\bp(v_4)$, the first term is non-zero. Since $\bq_2$ is a non-trivial $C_2^1$-motion of $(H+v_1v_3,\bp|_H)$ and $(H+v_1v_3+v_3v_4,\bp|_H)$ is  $C_2^1$-rigid, we also have
$D_{3,4}\cdot \bq_2(v_4)=D_{3,4}\cdot (\bq_2(v_4)-\bq_2(v_3))\neq 0$.
Hence (\ref{eq:dV3-4}) gives $D_{3,4}\cdot \bq_1(v_3)=0$. 
\end{proof}
%On the other hand, since 

Since the edge $v_3v_5$ exists in ${\rm cl}(E(H))$ and $\bq_1(v_5)=0$,
we also have
\begin{equation}
\label{eq:dV4-2}
D_{3,5}\cdot \bq_1(v_3)=0.
\end{equation}
Claim~\ref{cllm:dV4-1} and (\ref{eq:dV4-2}) imply that $\bq_1(v_3)$ is a vector in the orthogonal complement of the span of $D_{3,4}$ and $D_{3,5}$.
Hence, scaling $\bq_1$ appropriately, we may assume that 
\begin{equation}
\label{eq:dV4-3}
\bq_1(v_3) = \Delta_{1,2,3} \,D_{3,4}\times D_{3,5}.
\end{equation}
%(Here we put a scalar $\Delta_{1,2,3} D_{3,4}$ just to get the formula of the statement.)
By an analogous argument on the line through $\bp(v_2)$ and $\bp(v_4)$, we obtain
\begin{equation}
\label{eq:dV4-4}
\bq_2(v_2) = \Delta_{1,3,2} D_{2,4}\times D_{2,5}.
\end{equation}

We next calculate $\bq_1(v_4)$. 
Since the edge $v_4v_5$ exists in ${\rm cl}(E(H))$ and $\bq_1(v_5)=0$, we have 
$D_{4,5}\cdot \bq_1(v_4)=0$.
Also the edge $v_3v_4$ exists in ${\rm cl}(E(H)+v_1v_2)$, since otherwise we could perform an X-replacement on $H+v_1v_2+v_3v_4$ and deduce that $G$ is $C_2^1$-rigid.
Hence $D_{3,4}\cdot (\bq_1(v_4)-\bq_1(v_3))=0$. Since $D_{3,4}\cdot \bq_1(v_3)=0$ by Claim \ref{cllm:dV4-1}, we have $D_{3,4}\cdot \bq_1(v_4)=0$.
Thus $\bq_1(v_4)$ is in the orthogonal complement of the span of $D_{4,5}$ and $D_{3,4}$,
and $\bq_1(v_4)=s D_{3,4}\times D_{4,5}$ for some $s\in\mathbb{R}$.
The next claim determines the value of $s$:
\begin{claim}
%$s=\begin{vmatrix} x_1 & y_1 & 1 \\ x_2 & y_2 & 1 \\ x_4 & y_4 & 1 \end{vmatrix} /\begin{vmatrix} x_1 & y_1 & 1 \\ x_2 & y_2 & 1 \\ x_3 & y_3 & 1 \end{vmatrix}$.
$s=\Delta_{1,2,4}$.
%\begin{equation}
%\label{eq:dV6}
%\left|
%\begin{array}{c}
%D_{0,1} \\ D_{0,5} \\ D_{0,3}
%\end{array}\right|
%(D_{0,4}\cdot q_1(v_4) )
%-
%\left|
%\begin{array}{c}
%D_{0,1} \\ D_{0,5} \\ D_{0,4}
%\end{array}\right|
%(D_{0,3}\cdot q_1(v_3) )
%=0
%\end{equation}
\end{claim}
\begin{proof}
We put $\bp(v_0)$ on the interior of the line segment joining  $\bp(v_1)$ and $\bp(v_2)$.
Then $D_{0,1}$ is a scalar multiple of  $D_{0,2}$.
With this choice of $\bp(v_0)$, we may expand the determinant in (\ref{eq:dV3})
%and use the fact that $p(v_0)$ is on the line through $p(v_1)$ and $p(v_2)$,
to obtain
\begin{equation}
\label{eq:dV5}
\left|
\begin{array}{c}
D_{0,1} \\ D_{0,5} \\ D_{0,3}
\end{array}\right|
(D_{0,4}\cdot \bq_1(v_4) )
(D_{0,2}\cdot \bq_2(v_2))
-
\left|
\begin{array}{c}
D_{0,1} \\ D_{0,5} \\ D_{0,4}
\end{array}\right|
(D_{0,3}\cdot \bq_1(v_3) )
(D_{0,2}\cdot \bq_2(v_2))
=0.
\end{equation}
%The formula for the determinant of a Vandermonde matrix implies that
%\[
%\left|
%\begin{array}{c}
%D_{0,i} \\ D_{0,j} \\ D_{0,k}
%\end{array}\right|
%=\left|
%\begin{array}{ccc}
%x_0 & y_0 & 1 \\
%x_i & y_i & 1 \\
%x_j & y_j & 1
%\end{array}\right|
%\left|
%\begin{array}{ccc}
%x_0 & y_0 & 1 \\
%x_j & y_j & 1 \\
%x_k & y_k & 1
%\end{array}\right|
%\left|
%\begin{array}{ccc}
%x_0 & y_0 & 1 \\
%x_k & y_k & 1 \\
%x_i & y_i & 1
%\end{array}\right|.
%\]
We may use the fact that $D_{1,2}\cdot \bq_2(v_2)\neq 0$ by Claim \ref{claim:Hbase}(b) to deduce that $D_{0,2}\cdot \bq_2(v_2)\neq 0$ and  then rewrite (\ref{eq:dV5}) as
\begin{equation}
\label{eq:dV6}
\left|
\begin{array}{c}
D_{0,1} \\ D_{0,5} \\ D_{0,3}
\end{array}\right|
(D_{0,4}\cdot \bq_1(v_4) )
-
\left|
\begin{array}{c}
D_{0,1} \\ D_{0,5} \\ D_{0,4}
\end{array}\right| 
%\Delta_{1,2,3}
(D_{0,3}\cdot \bq_1(v_3) )
=0.
\end{equation}
Using $\bq_1(v_4)=s D_{3,4}\times D_{4,5}$, and substituting $\bq_1(v_3)$ with \eqref{eq:dV4-3}, we obtain 
\begin{equation}\label{eq:dV7}
s = \frac{
\left|
\begin{array}{c}
D_{0,1} \\ D_{0,5} \\ D_{0,4}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,3} \\ D_{3,4} \\ D_{3,5}
\end{array}\right|}{ 
\left|
\begin{array}{c}
D_{0,1} \\ D_{0,5} \\ D_{0,3}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,4} \\ D_{3,4} \\ D_{4,5}
\end{array}\right|}\Delta_{1,2,3}.
\end{equation}

By using the identity (\ref{eq:Vandermonde}) and the fact $D_{i,j} = D_{j,i}$, (\ref{eq:dV7}) becomes 
\begin{equation}
s=\frac{\Delta_{0, 1, 5} \Delta_{0, 5, 4} \Delta_{0, 4, 1} \Delta_{3, 0, 4} \Delta_{3, 4, 5} \Delta_{3, 5, 0}}{\Delta_{0, 1, 5} \Delta_{0, 5, 3} \Delta_{0, 3, 1} \Delta_{4, 0, 3} \Delta_{4, 3, 5} \Delta_{4, 5, 0}}\Delta_{1,2,3}
=\frac{\Delta_{0,4,1}}{\Delta_{0,3,1}}\Delta_{1,2,3}.
\end{equation}
Finally since $\bp(v_0)$ is on the interior of the line segment joining $\bp(v_1)$ and $\bp(v_2)$, 
we get 
\[
s=\frac{\Delta_{0,4,1}}{\Delta_{0,3,1}}\Delta_{1,2,3}=\frac{\Delta_{1,2,4}}{\Delta_{1,2,3}}\Delta_{1,2,3}=\Delta_{1,2,4}.\qedhere
\]
\end{proof}
This completes the derivation  of the formula for $\bq_1$  in the statement of the lemma. 
The formula for $\bq_2$ can be obtained using a symmetric argument by changing the role of $v_2$ and $v_3$.

It remains to compute $\bq(v_0)$. By (\ref{eq:dV2}), $\bq(v_0)/\beta$ is in the orthogonal complement of the span of $D_{0,1}$ and $D_{0,5}$. Hence $\bq(v_0)/\beta = k D_{0,1} \times D_{0,5}$ for some $k\in \mathbb{R}$.
By the second equation in (\ref{eq:dV2}), we also have $D_{0,2}\cdot \bq_2(v_2) = D_{0,2}\cdot (\bq(v_0)/\beta) = k D_{0,2}\cdot(D_{0,1} \times D_{0,5})$. 
Combining this with (\ref{eq:dV4-4}), we get 
\begin{equation}
\label{eq:dV8}
k = \Delta_{1,3,2} \frac{D_{0,2}\cdot (D_{2,4}\times D_{2,5})}{D_{0,2}\cdot(D_{0,1} \times D_{0,5})}.
\end{equation}
By the third equation in (\ref{eq:dV2}), $(D_{0,3}\cdot \bq_1(v_3))\gamma = D_{0,3}\cdot \bq(v_0)/\beta= k D_{0,3}\cdot (D_{0,1} \times D_{0,5})$. Hence by  (\ref{eq:dV8}) and \eqref{eq:dV4-3} we get 
\begin{align*}
\frac{\alpha}{\beta}=\gamma &= \frac{k D_{0,3}\cdot (D_{0,1} \times D_{0,5})}{D_{0,3}\cdot \bq_1(v_3)}
=\frac{\Delta_{1,3,2} D_{02}\cdot(D_{24}\times D_{25}) D_{03}\cdot (D_{01}\times D_{05})}{\Delta_{1,2,3} D_{03}\cdot(D_{34}\times D_{35}) D_{02}\cdot (D_{01}\times D_{05})} \\
&=-\frac{
\left|
\begin{array}{c}
D_{0,2} \\ D_{2,4} \\ D_{2,5}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,3} \\ D_{0,1} \\ D_{0,5}
\end{array}\right|}{
\left|
\begin{array}{c}
D_{0,3} \\ D_{3,4} \\ D_{3,5}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,2} \\ D_{0,1} \\ D_{0,5}
\end{array}\right|}.
\end{align*}
By scaling $\bq$ appropriately, we may take
$$\alpha = \left|
\begin{array}{c}
D_{0,2} \\ D_{2,4} \\ D_{2,5}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,3} \\ D_{0,1} \\ D_{0,5}
\end{array}\right|
\mbox{ and }
\beta = -
\left|
\begin{array}{c}
D_{0,3} \\ D_{3,4} \\ D_{3,5}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,2} \\ D_{0,1} \\ D_{0,5}
\end{array}\right|.$$ 
%$\alpha=D_{02}\cdot(D_{24}\times D_{25}) D_{03}\cdot (D_{01}\times D_{05})$ and 
%$\beta=-D_{03}\cdot(D_{34}\times D_{35}) D_{02}\cdot (D_{01}\times D_{05})$ as given in the statement.
Since $\bq(v_0)= \beta k D_{0,1} \times D_{0,5}$, we can now use (\ref{eq:dV8}) to obtain the formula for $\bq(v_0)$ given in the statement of the lemma.
\end{proof}

%\subsection{$b$-motions}
\subsection{Bad motions and proof of Theorem \ref{thm:doubleV}}
Let $(G,\bp)$ be a generic framework and $v_0$ be a vertex of type $(\star)$ in $G$ with $N_G(v_0)=\{v_1,\dots, v_5\}$. Lemma~\ref{lem:motion} shows that, if $G$ is not $C_2^1$-rigid, then $(G,\bp)$ is a 1-dof framework and has a non-trivial motion $\bq$ with the property that the coordinates of $\bq$ at each vertex  of $\hat{N}_G(v_0)$ are three polynomials in the coordinates of $\bp(\hat{N}_G(v_0))$ with coefficients in $\rat$.
%, when regarding the coordinates of $\bp(\hat{N}_G(v_0))$ as variables. 
This seems unlikely as the graph on $N_G(v_0)$ induced by $\cl(E(G-v_0))$ 
%the restriction of $(G,\bp)$ to $\hat{N}(v_0)$ has more than one degree of freedom (since $v_0$ is of type $(\star)$). 
is a star on the five vertices  (since $v_0$ is of type $(\star)$), which has a large degree of freedom as a subframework.
%but the entries of a non-trivial motion is determined by  $\bp(\hat{N}_G(v_0))$.
Our goal is to give a rigorous proof that this cannot happen. 
The following concepts will be useful 
%of $b$-motions will come up naturally 
for this purpose.



 
Let $G=(V,E)$ be a graph with $V=\{v_1,v_2,\ldots, v_n\}$. For $U\subseteq V$, let 
\[
b:U\to \rat[X_1,Y_1,X_2, Y_2,\ldots,X_n,Y_n]^3
\]
be a map which associates a 3-tuple $b_{i}$ of polynomials in $2n$ variables to each $v_i\in U$.

For a given framework $(G,\bp)$ with $\bp(v_i)=(x_i,y_i)$ for all $1\leq i\leq n$, the substitution of $(X_i, Y_i)$ with $(x_i,y_i)$ in $b_{i}$ for all $1\leq i\leq n$ gives a vector $b_{i}(\bp)$ in $\R^3$
for each $v_i\in U$.
We say that a $C_2^1$-motion $\bq$ of  $(G,\bp)$ is a {\em $b$-motion}  if $\bq(v_i)=b_{i}(\bp)$  for all $v_i\in U$.

%Our next result uses Lemma \ref{lem:abstract_bad_pinning} to deduce that the property 
The following lemma states that the property of having  a $b$-motion is stable over a large set $S$ of realisations. (In particular, it will imply that this  property is generic). Since we will need the realisations in $S$ to satisfy the hypotheses of Lemma \ref{lem:1dof_motion1} it will be convenient to say that the realisation $\bp$ is {\em non-degenerate on $U$} if there exist three distinct vertices in $U$ which have distinct `$y$-coordinates' in $(G,\bp)$.
%at vertices $v_a,v_b,v_c$} if $\bp(v_m)=(x_m,y_m)$ for $m=a,b,c$ and $(y_a-y_b)(y_b-y_c)(y_c-y_a)\neq 0$. 



\begin{lemma}\label{lem:bad_pinning}
Let $G=(V,E)$ be a $C_2^1$-independent graph with $V=\{v_1,\dots,v_n\}$, 
%$v_a,v_b,v_c\in V$, 
$U
%=\{v_1,\dots,v_t\}
\subseteq V$, $F
%=\{f_1,\ldots,f_k\}
\subseteq K(U)$, 
%be a set of edges on $U$
and
%\begin{equation}\label{eq:bad_pinning}
$
S=\{\bp:\mbox{$(G+F,\bp)$ is minimally $C_2^1$-rigid and $\bp$ is non-degenerate on $U$}\}.
%\text{$\bp$ is non-degenerate at $v_a,v_b,v_c$ and $(G+F,\bp)$ is minimally $C_2^1$-rigid}
$
%\end{equation}
Suppose that $b:U\to \rat[X_1,Y_1,\ldots,X_n,Y_n]^3$ and $(G,\bp)$ has a $b$-motion for some generic $\bp$. Then $(G, \bp)$ has a $b$-motion for all $ \bp\in S$.
\end{lemma}
%\begin{proof}
%Suppose $\bar \bp\in S$. Since $\bar \bp$ is non-degenerate on $U$ we can choose three distinct vertices $v_a,v_b,v_c\in U$ which have distinct `$y$-coordinates' in $(G,\bar \bp)$ and let $\tilde{C}(G+F,\bar \bp)$ be the extended $C_2^1$-cofactor matrix with respect to $v_a,v_b,v_c$.
%We can then deduce that $(G,\bar \bp)$ has a $b$-motion  by  applying Lemma \ref{lem:abstract_bad_pinning} to 
%$\tilde{C}(G+F,\bar \bp)$, taking the rows indexed by $D$ to be the rows indexed by  $F$ together with the  six rows 
%%of  $\tilde{C}(G+F,\bar \bp)$ 
%which are not rows of ${C}(G+F,\bar \bp)$. (More precisely, we define $M$ to be the matrix obtained from $\tilde{C}(G+F,\bar \bp)$ by replacing each of the coordinates $x_i,y_i$ in the definition of $\tilde{C}(G+F,\bar \bp)$ by indeterminates $X_i,Y_i$. We then  put $
%%\begin{equation}\label{eq:abstract_bad_pinning}
%T=\{\bar \bp\in \R^{2n}: 
% \text{$M(\bar \bp)$ is non-singular}
% % and $M_{D}(x)$ is row independent
% \}$. 
% Lemma~\ref{lem:1dof_motion1} implies that $\tilde{C}(G+F,\bar \bp)$ is non-singular for all $\bar \bp\in S$ so $S\subseteq T$.)
%\end{proof}
%

Lemma~\ref{lem:bad_pinning} can be understood as follows.
Since each entry of $C(G,\bp)$ is a polynomial function of the coordinates of $\bp$, we can choose a base of the space of $C_2^1$-motions of $(G,\bp)$ such that 
each entry of the vectors in the base is a polynomial function of the coordinates of $\bp$.
By the assumption of the lemma, $(G,{\bp})$ has a $b$-motion for some generic ${\bp}$, which is spanned by  this base.
Since this holds for some generic ${\bp}$ and $b$ is a polynomial function, it will hold for all generic $\bp$. 
The statement of Lemma~\ref{lem:bad_pinning} follows for all generic $\bp$.
We need a slightly more involved argument to verify the statement for {all} $\bp\in S$. This is given in Appendix~\ref{sec:bad_pinning}. 




Suppose $v_0$ is a vertex of type $(\star)$ in a generic framework $(G,\bp)$ and $(G,\bp)$ is not $C_2^1$-rigid. Then 
%$(G,\bp)$ will have exactly one degree of freedom and, since $\cl(E(G-v_0)$ induces a star on $N_G(v_0)$, every 
Lemma \ref{lem:motion} tells us that $(G,\bp)$ has a 
non-trivial motion $\bq$ 
with the property that the value of $\bq$ at each vertex  of $\hat{N}_G(v_0)$ can be described by three polynomials in the coordinates of $\bp(\hat{N}_G(v_0))$ with coefficients in $\rat$. We will see in Lemma~\ref{lem:bad_motion} below that $\bq$ also has the property that the graph on $N_G(v_0)$ with edge set $\{v_iv_j\,:\,D(v_i,v_j)\cdot (\bq(v_i)-\bq(v_j))=0\}$ is a star. 
We will concentrate on $b$-motions which share these properties.
%This motivates our next definition.
 
Formally, let $(G,\bp)$ be a framework and  $v_0$ be a vertex of degree five in $G$ with $N_G(v_0)=\{v_1,v_2,\ldots,v_5\}$. We say that a $C_2^1$-motion $\bq$ of $(G,\bp)$ is {\em bad at $v_0$} if $\bq$ is a $b$-motion for some $b:\hat N_G(v_0)\to \rat[X_0,Y_0,X_1, Y_1,\ldots,X_5,Y_5]^3$ for which 
\begin{equation}\label{eq:bad}
\text{the graph on $N_G(v_0)$ with edge set 
$\{v_iv_j: 
D_{i,j}\cdot (b(v_i)-b(v_j))=0 \}$
 is a star,}
\end{equation}
where $D_{i,j}=((X_i-X_j)^2, (X_i-X_j)(Y_i-Y_j), (Y_i-Y_j)^2)$.
(Here $D_{i,j}\cdot (b(v_i)-b(v_j))=0$ means that polynomial $D_{i,j}\cdot (b(v_i)-b(v_j))$ is identically zero.)

Our next result verifies that the motion defined in Lemma \ref{lem:motion} is indeed a bad motion.
 

\begin{lemma}
\label{lem:bad_motion}
Let $(G,\bp)$ be a generic framework and $v_0$ be a vertex of type $(\star)$ 
with $N_G(v_0)=\{v_1,\dots, v_5\}$.
Suppose that $G$ is not $C_2^1$-rigid. 
Then $(G,\bp)$ has a bad motion at $v_0$.
\end{lemma}
\begin{proof}
%Let $(G,\bp)$ be a framework and $v_0$ be a vertex of degree five with $N_G(v_0)=\{v_1,\dots, v_5\}$.
%Suppose further that 
%$\hat{N}_G(v_0)$ is a locally 1-dof part in $G$. 
Motivated by Lemma~\ref{lem:motion}, we define $b:\hat{N}_G(v_0)\rightarrow\rat[X_0,Y_0,X_1,\ldots,Y_5]^3$ by
\begin{align}
b(v_0)&=\Delta_{1,2,3} \left|
\begin{array}{c} D_{0,3} \\ D_{3,4} \\ D_{3,5}
 \end{array} \right|
\left|
\begin{array}{c} D_{0,2} \\ D_{2,4} \\ D_{2,5}
 \end{array} \right|
 D_{0,1}\times D_{0,5}, \label{eq:bad1}\\
b(v_1)&=0,\\
b(v_2)&=\beta \Delta_{1,3,2} D_{2,4}\times D_{2,5}, \\
b(v_3)&=\alpha \Delta_{1,2,3} D_{3,4} \times D_{3,5}, \\
b(v_4)&=\alpha\Delta_{1,2,4} D_{3,4}\times D_{4,5} +\beta \Delta_{1,3,4}D_{2,4}\times D_{4,5}, \\
b(v_5)&=0;  \label{eq:bad6}
\end{align}
where
 $\Delta_{i,j,k}=\left|
\begin{array}{ccc}
X_i & Y_i & 1 \\ X_j & Y_j & 1 \\ X_k & Y_k & 1
\end{array}\right|$,
$\alpha = \left|
\begin{array}{c}
D_{0,2} \\ D_{2,4} \\ D_{2,5}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,3} \\ D_{0,1} \\ D_{0,5}
\end{array}\right|$,
$\beta = -
\left|
\begin{array}{c}
D_{0,3} \\ D_{3,4} \\ D_{3,5}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,2} \\ D_{0,1} \\ D_{0,5}
\end{array}\right|$
%where each $\Delta(v_i, v_j, v_k)$ and $D(v_i,v_j)$ 
are 
regarded as 
polynomials in $X_0,Y_0,X_1,\ldots,Y_5$.
Then, by Lemma~\ref{lem:motion}, $(G,\bp)$ has a $b$-motion at $v_0$.

It remains to show that $b$ satisfies (\ref{eq:bad}) symbolically.
This can be done by a hand computation using the explicit formulae,
see Appendix \ref{app:bad} for the details.
\end{proof}

Our next result asserts that  no generic framework with one degree of freedom can have a bad motion.
\begin{theorem}\label{thm:well-behaved0}
Let $(G,\bp)$ be a generic 1-dof framework and $v_0$ be a vertex of degree five.
Then $(G,\bp)$ has no bad motion  at $v_0$.
\end{theorem}
%\begin{theorem}\label{thm:well-behaved}
%Let $(G,\bp)$ be a generic framework and $v_0$ be a vertex of degree five such that 
%$\hat{N}_G(v_0)$ is a locally $k$-dof part in $G$ with $k=1$ or $k=2$.
%Then $(G,\bp)$ has no bad motion  at $v_0$.
%\end{theorem}

We will delay the proof of Theorem \ref{thm:well-behaved0} until  Section \ref{sec:well-behaved}. Instead we show how it can be used to deduce Theorem~\ref{thm:doubleV}.

\medskip
\noindent
{\bf Proof of Theorem~\ref{thm:doubleV}.}
Suppose the theorem is false. Let $G$ be a counterexample and $\bp$ be a generic realisation of $G$. 
%Since $v_0$ is type $(\star)$, $G-v_0+v_1v_2+v_1v_3$ is rigid. The fact that 1-extension preserves $C^1_2$-rigidity now implies that  $(G,\bp)$ has one degree of freedom. 
Then Lemma~\ref{lem:bad_motion} implies that $(G,\bp)$ has a bad motion at $v_0$ and this contradicts Theorem~\ref{thm:well-behaved0}. 
(Note that $(G,\bp)$ is a 1-dof framework since $v_0$ is type $(\star)$.)
%) and hence every subset of the vertices of $G$ is either a locally rigid part or a locally 1-dof part of $G$.)
\qed

%\medskip
%Theorem~\ref{thm:doubleV} follows from  Theorem~\ref{thm:well-behaved} and Lemma~\ref{lem:bad_motion}, since the hypothesis of Theorem~\ref{thm:doubleV} that $v_0$ is a vertex of type $(\star)$ in $G$  implies that every generic framework $(G,p)$ will have at most one degree of freedom. 

%The reader may wonder why we include the case $k=2$ in Theorem \ref{thm:well-behaved}, since our proof of  Theorem~\ref{thm:doubleV} only uses the case $k=1$.
%%Although this deduction only requires the special case of Theorem~\ref{thm:well-behaved} when $k=1$,
%%$\hat{N}_G(v_0)$ is a locally $1$-dof part in $G$,  
%The reason is that
%we need the case $k=2$
%%$\hat{N}_G(v_0)$ is a locally $2$-dof part 
%for our inductive proof of 
%Theorem~\ref{thm:well-behaved}.  
%%We will delay this proof until  Section \ref{sec:well-behaved}.

%
%In the proof of Theorem~\ref{thm:well-behaved0}, we  sometimes use the technique of pinning described in Section~\ref{subsec:pinning}. The following technical on lemma follows easily by the argument of the proof of Lemma~\ref{lem:canonical}.
%\begin{lemma}\label{lem:bad_pinned}
%Let $(G,\bp)$ be a 
% framework with $\bp(v_i)=(x_i,y_i)\in \mathbb{R}^2$ for all $v_i\in V(G)$. Let $v_0$ be a vertex of $G$ of degree five and $v_a,v_b,v_c\in \hat N_G(v_0)$  such that $(y_a-y_b)(y_a-y_c)(y_b-y_c)\neq 0$. 
%Let  $\tilde{C}(G,\bp)$ be the extended cofactor matrix of $(G,\bp)$ with respect to $(v_a, v_b, v_c)$.
% Suppose $\bq$ is a bad $C^1_2$-motion of $(G,\bp)$ at $v_0$. Then there exists a bad motion $\bq'$ of $(G,\bp)$ at $v_0$ such that $\bq'\in \ker\tilde C(G,\bp)$.
% \end{lemma}
%\begin{proof} We adopt the notation used in Section \ref{subsec:pinning}. It will suffice to find a trivial $C^1_2$-motion $\bq^*\in Z_0(G,p)$ such that 
%$\bq^*$ is a $b^*$-motion of $(G,p)$ for some $b^*:\hat N_G(v_0)\to \Q[X_0,Y_0,X_1,\ldots,Y_5]^3$ and 
%\begin{equation}\label{eq:pin}
%\bq^* \cdot {\bf e}_{s,t}=\bq \cdot {\bf e}_{s,t} \text{ for all } (s,t)\in \{(a,1), (a, 2), (a,3), (b,1), (b,2), (c,1)\}.
%\end{equation}
%(We can then put $\bq'=\bq-\bq^*$.)
%
%Let $\{\bq_i^*:1\leq i\leq 6\}$ be the basis for $Z_0(G,p)$ given in Section \ref{subsec:pinning}. Taking $\bq^*=\sum_{i=1}^6\lambda_i \bq_i^*$,   the  system of equations (\ref{eq:pin}) can be expressed as
%\begin{equation}\label{eq:pin1}
%\begin{pmatrix}
%1 & 0 & 0 & y_a & 0 & y_a^2 \\ 
%0 & 1 & 0 & -x_a & -y_a & -2x_ay_a \\ 
%0 & 0 & 1 & 0 & x_a & x_a^2 \\
%1 & 0 & 0 & y_b & 0 & y_b^2 \\ 
%0 & 1 & 0 & -x_b & -y_b & -2x_by_b \\
%1 & 0 & 0 & y_c & 0 & y_c^2 
%\end{pmatrix}
%\begin{pmatrix}
%\lambda_1 \\
%\lambda_2 \\
%\lambda_3 \\
%\lambda_4 \\
%\lambda_5 \\
%\lambda_6 
%\end{pmatrix}
%=
%\begin{pmatrix}
%\bq \cdot {\bf e}_{a,1} \\
%\bq \cdot {\bf e}_{a,2} \\
%\bq \cdot {\bf e}_{a,3} \\
%\bq \cdot {\bf e}_{b,1} \\
%\bq \cdot {\bf e}_{b,2} \\
%\bq \cdot {\bf e}_{c,1}
%\end{pmatrix}.
%\end{equation}
%Let $Q$ denote the matrix of coefficients of this system. 
%Then $\det Q=(y_a-y_b)^2(y_c-y_a)(y_b-y_c)\neq 0$.
%Hence $Q$ is non-singular, and  (\ref{eq:pin1}) has a unique solution ${\boldmath \lambda}^*=(\lambda_1^*,\ldots \lambda_6^*)$.  In addition, the facts that each entry in $Q$ is a polynomial in $p(\hat N_G(v_0))$ and $q$ is a $b$-motion for some $b:\hat N_G(v_0)\to \Q[X_0,Y_0,X_1,\ldots,Y_5]^3$ implies that, for all $1\leq i\leq 6$, $\lambda_i^*=f_i(p(\hat N_G(v_0)) $  for some rational functions $f_i\in \Q(X_0,Y_0,X_1,\ldots,Y_5)$. By choosing an appropriate scaling of $\boldmath \lambda$ we may assume that  each $f_i\in \Q[X_0,Y_0,X_1,\ldots,Y_5]$. Then $\bq^*=\sum_{i=1}^6\lambda_i^*\bq_i^*$ is the required trivial $C^1_2$-motion for $(G,p)$.
%\end{proof}

\subsection{Projective transformations}
Recall that each point $p=(x,y)\in \R^2$ can be associated to a point $p^\uparrow=[x,y,1]^T$ in 2-dimensional real projective space. 
%$\bP^2$. 
A map $f:\R^2\to \R^2$ is a {\em projective transformation} if there exists a $3\times 3$ non-singular matrix $M$ such that, for all $p\in\R^2$, 
%$[f(p),1]=Mp^\uparrow$ 
$f(p)^\uparrow=\lambda_pMp^\uparrow$ for some non-zero $\lambda_p\in \R$.
We say that a framework $(G,\bp')$ is a {\em projective image} of a framework $(G,\bp)$ if there is a 
projective transformation $f:\mathbb{R}^2\rightarrow \mathbb{R}^2$ such that $\bp'(v_i)=f(\bp(v_i))$ for all $v_i\in V(G)$.
Whiteley~\cite[Theorem 11.3.2.]{Wsurvey} showed that $C_2^1$-rigidity is invariant under projective transformations. 
We shall use the following lemma, which implies that a certain projective transformation preserves the existence of a bad motion, to simplify our calculations in the proof of Theorem \ref{thm:well-behaved0}. 
%claiming that a certain projective transformation keeps the existence of bad motions.
Its statement  implicitly uses the fact that, for any two ordered sets $S$ and $T$ of four points in general position in $\R^2$, 
%such that no three points in each set are colinear 
there is a unique projective transformation that maps $S$ onto $T$.
\begin{lemma}\label{lem:projective_bad}
Let $(G,\bp)$ be a generic framework, $v_0$ be a vertex of degree five with $N_G(v_0)=\{v_1,\dots, v_5\}$ 
%Suppose that 
and $(G, \bp')$ be a projective image of $(G,\bp)$ such that 
$\bp'(v_1)=(1, 0)$, $\ \bp'(v_2)=(0, 0)$, $\bp'(v_3)=(0,1)$, and  $\bp'(v_4)=(1,1)$.
If $(G, \bp')$ has a bad motion at $v_0$, then $(G, \bp)$ has a bad motion at $v_0$.
\end{lemma}
Lemma~\ref{lem:projective_bad} will follow from the fact that the entries in the matrix which defines the projective transformation given in the lemma are  determined by  
the coordinates of $\bp(v_i)$ for $1\leq i\leq 4$. However, a rigorous proof seems to
%seems to 
require a precise understanding of how the projective transformation changes the motion space of the framework. Whiteley's proof of projective invariance does not provide this as it uses a  self-stress argument.
%, and there seems no exposition  from the view point of $C_2^1$-motions.
We develop a new proof technique for the projective invariance of $C_2^1$-rigidity in Appendix~\ref{sec:projective},
and then use it to derive Lemma~\ref{lem:projective_bad}.



==> cofactor1(da_final)/inductive_26_6_20.tex <==
\section{Inductive Construction and Proof of Theorem~\ref{thm:cofactor}}
\label{sec:inductive}
\subsection{Inductive Construction}\label{subsec:inductive}
Our proof of Theorem~\ref{thm:cofactor} 
uses the following  3-dimensional versions of standard graph operations from rigidity theory. 
%In their most general form, these definitions depend on the underlying dimension $d$, but here we only describe the operations for 3-rigidity.)
Given a graph $H$:
\begin{itemize}
\item the \emph{$0$-extension} operation adds a new vertex $v$ and three new edges from $v$ to vertices in $H$; 
\item the {\em $1$-extension} operation chooses an edge $e$ of $H$ and adds a new vertex $v$ and four new edges from $v$ to vertices in $H-e$ with the proviso that two of the new edges join $v$ to the end-vertices of $e$;
\item the {\em X-replacement} operation chooses two non-adjacent edges $e$ and $f$ of $H$ and adds a new vertex $v$ and five new edges from $v$ to vertices in $H-\{e,f\}$ with the proviso that four of the new edges join $v$ to the end-vertices of $e$ and $f$;
\item the {\em  V-replacement} operation chooses two adjacent edges $e$ and $f$ of $H$ and adds a new vertex $v$ and five new edges from $v$ to vertices in $H-\{e,f\}$ with the proviso that three of the new edges join $v$ to the end-vertices of $e$ and $f$;
\item the {\em  vertex splitting} operation chooses a vertex $u$ of $H$ and pairwise disjoint sets  $U_1,U_2,U_3$ with $U_1\cup U_2\cup U_3=N_H(u)$ and $|U_2|=2$, deletes all edges from $u$ to $U_3$, and then adds a new vertex $v$ and $|U_3|+3$ new edges from $v$ to each vertex in $U_2\cup U_3\cup \{u\}$.
\end{itemize}
Whiteley~\cite[Lemmas 10.1.5 and 10.2.1, Theorems 10.2.7 and 10.3.1]{Wsurvey} showed that all but one of these operations preserve  $C_2^1$-independence:
\begin{lemma}
%(Whiteley~\cite[Lemmas 10.1.5 and 10.2.1, Theorems 10.2.7 and %10.3.1]{Wsurvey})
\label{lem:cofactor_ind}
The  $0$-extension, $1$-extension, X-replacement, and vertex splitting operations  preserve $C_{2}^{1}$-independence.
%The following properties hold for $C_2^1$-rigidity.
%\begin{itemize}
%\item (0-extension property) three-dimensional $0$-extension preserves $C_2^1$-rigidity.
%\item (1-extension property) three-dimensional $1$-extension preserves $C_2^1$-rigidity.
%\item (vertex-splitting property) vertex 2-splitting preserves $C_2^1$-rigidity
%\item (X-replacement property) three-dimensional $X$-replacement preserves $C_2^1$-rigidity
%\end{itemize}
\end{lemma}

In general V-replacement may not preserve $C_2^1$-independence, but there is an important special case when it does.
%Namely, suppose the V-replacement removes two edges $e=v_1v_2, f=v_1v_3$
% and adds a new vertex $v_0$ with fives edges $v_0v_i$ for $i=1,\dots, 5$.
% If the original graph has edges $v_1v_4$ and $v_1v_5$, then this V-replacement is a special case of vertex splitting, and hence preserves $C_2^1$-independence. 
 % See Figure~\ref{fig:vertexsplitting}.


\begin{lemma}
\label{lem:V} Suppose that $v_1,v_2,v_3,v_4,v_5$ are vertices of a $C_2^1$-independent graph $H=(V,E)$, $e=v_1v_2,f=v_1v_3$ are edges of $H$ and  $v_1v_4,v_1v_5$ belong to the closure of $E-e-f$ in the $C^1_{2}$-cofactor matroid on $K(V)$. Then the graph $G$ obtained from $H-e-f$ by adding a new vertex $v$ and new edges $vv_1,vv_2,vv_3,vv_4,vv_5$ is $C_2^1$-independent.
\end{lemma}
\begin{proof}
 Let $\cl(.)$ denote the closure operator in the $C^1_{2}$-cofactor matroid on $K(V)$. Since  $v_1v_4,v_1v_5\in \cl(E-e-f)$,  we may choose a base $B$ of $\cl(E-e-f)$ with $v_1v_4,v_1v_5\in B$. Then the graph $H'=(B,B+e+f)$ is $C_2^1$-independent and we can now apply the vertex splitting operation at $v_1$ to deduce that the graph $G'$ obtained from $H'-e-f$ by adding a new vertex $v$ and new edges $vv_1,vv_2,vv_3,vv_4,vv_5$ is $C_2^1$-independent, see Figure~\ref{fig:vertexsplitting}. This and the fact that $\cl(B)=\cl(E-e-f)$ imply that $G$ is $C_2^1$-independent.
 \end{proof}
 
 \noindent
Lemma \ref{lem:V} will be used several times in our proofs 
 
Whiteley~\cite{Wsurvey} conjectured that another special case of V-replacement preserves $C_2^1$-independence: if $H\cup \{e_1,e_2\}$ and $H\cup \{e_1',e_2'\}$ are both $C_2^1$-independent for two pairs of adjacent edges $e_1,e_2$ and $e_1',e_2'$ with the property that the common endvertex of $e_1,e_2$ is distinct from that of $e_1',e_2'$, then the graph $G$ obtained by adding a new vertex $v_0$ of degree five to $H$ in such a way that the endvertices of $e_1,e_2,e_1',e_2'$ are all neighbours of $v_0$, is $C_2^1$-independent. See Figure~\ref{fig:doubleV}. This operation is referred to as  {\em double V-replacement} since $G$ can be constructed from both $G-v_0+e_1+e_2$ and $G-v_0+e_1'+e_2'$ by a V-replacement.
%
% Although V-replacement may not preserves $C_2^1$-rigidity in general, Whiteley conjectured that "double V-replacement" does in general. 
We will verify Whiteley's conjecture:

\begin{figure}[t]
\centering
\includegraphics[scale=0.8]{vertexsplitting.pdf}
\caption{An extension operation which can be considered as a special case of both V-replacement and vertex splitting. }
\label{fig:vertexsplitting}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[scale=0.8]{doubleV.pdf}
\caption{An example of double V-replacement.}
\label{fig:doubleV}
\end{figure}


\begin{theorem}\label{thm:doubleVconj}
%Let $G=(V,E)$ be a graph that has a vertex  $v_0$ of degree five,
%and let $\{e_1,e_2\}$ and  $\{e_1',e_2'\}$ be two pairs of adjacent edges on $N_G(v_0)$.
%Suppose that $G-v_0+e_1+e_2$ and $G-v_0+e_1'+e_2'$ are both $C_2^1$-independent,
%and that the common endvertex of $e_1$ and $e_2$ is distinct from that of $e_1'$ and $e_2'$.
%Then $G$ is $C_2^1$-independent.
The  double V-replacement operation  preserves $C_{2}^{1}$-independence.

\end{theorem}

Lemma \ref{lem:cofactor_ind} and Theorem~\ref{thm:doubleVconj} imply that we can construct all minimally $C_2^1$-rigid graphs from copies of $K_4$ with a `Henneberg tree construction' using the 0-, 1-, X- and double V-extension operations. We refer the reader to \cite{TW85,Wsurvey} for more details.



The proof of Theorem \ref{thm:doubleVconj} will be spread over  Sections \ref{sec:doubleV}, \ref{sec:bad} and \ref{sec:well-behaved} of this paper. To motivate this rather long and technical proof we show in the remainder of this section how (a generalisation of) our main result, Theorem ~\ref{thm:cofactor}, can be deduced easily from Lemma \ref{lem:cofactor_ind} and Theorem \ref{thm:doubleVconj}. 

\subsection{\boldmath $K_t$-matroids
% and proof of Theorem ~\ref{thm:cofactor}
}
\label{subsec:K_d matroid}
Let $n$ and $t$ be positive integers with $t\leq n$.
A matroid ${\cal M}$ on the edge set of a complete graph $K_n$ is said to be a {\em $K_t$-matroid} if  the edge set of every copy of $K_t$ in $K_n$ is a circuit in ${\cal M}$.  The following simple characterization of abstract $d$-rigidity matroids due to Nguyen{\cite[Theorem 2.2]{N10}} 
implies that every abstract $d$-rigidity matroid is a $K_{d+2}$-matroid.
\begin{theorem}
%[Nguyen{\cite[Theorem 2.2]{N10}}]
\label{thm:hang}
Let $n,d$ be positive integers with $n\geq d+2$ and ${\cal M}$ be a matroid on 
%the edge set of the complete graph 
$E(K_n)$. 
Then ${\cal M}$ is an abstract $d$-rigidity matroid if and only if 
${\cal M}$ is a $K_{d+2}$-matroid with rank $dn-{d+1\choose 2}$.
\end{theorem}
%The family of $K_t$-matroids extends the family of abstract $d$-rigidity matroids when we take $t=d+2$. 
We will prove a stronger version of Theorem~\ref{thm:cofactor} by showing that the $C^1_2$-cofactor matroid is the unique maximal matroid in the family of  $K_5$-matroids. (This strengthening will be needed in our companion paper \cite{CJT1}.)

Our next lemma shows that $dn-{d+1\choose 2}$ is an upper bound on the rank of any $K_{d+2}$-matroid on $E(K_n)$ when $n$ is sufficiently large. 

\begin{lemma}\label{lem:rank_upper_bound} Suppose that ${\cal M}$ is a $K_{d+2}$-matroid on $E(K_n)$ for $n\geq d+2$. Then ${\cal M}$ has rank at most  $dn-{{d+1}\choose{2}}$.
\end{lemma}
\begin{proof}
We proceed  by induction on $n$.
The claim is trivial when $n=d+2$.

Suppose $n>d+2$, and denote   the vertex set of $K_n$ by $\{v_1,\dots, v_n\}$. 
Let $K$ be the edge set of the complete graph on $\{v_1,\dots, v_{n-1}\}$.
 Since ${\cal M}|_{K}$ is a $K_{d+2}$-matroid, the rank of $K$ in ${\cal M}$ is at most $d(n-1)-{d+1\choose 2}$ by induction.
 Let $K'=K+\{v_1v_n,v_2v_n,\dots, v_dv_n\}$. We show $K'$ spans $E(K_n)$.
 
For each $i=d+1,\dots, n-1$, let $C_i$ be the edge set of the complete graph on $\{v_1, v_2,\dots, v_{d-1}, v_d, v_n,v_i\}$.
Note that $K'$ contains all edges of $C_i$ except $v_iv_n$. Since ${\cal M}$ is a $K_{d+2}$-matroid, $v_iv_n$ is spanned by $K'$. 
Hence $K'$ spans $E(K_n)$, and the rank of ${\cal M}$ is at most $|K'| =|K|+d=dn-{d+1\choose 2}$.
\end{proof}

Theorem~\ref{thm:hang} and Lemma~\ref{lem:rank_upper_bound} imply that an abstract $d$-rigidity matroid is a $K_{d+2}$-matroid which attains the maximum possible rank. 

\subsection{\boldmath Maximality of the generic $C_2^1$-cofactor matroid} \label{subsec:proof_of_thm12}
We show that 
%the abstract $3$-rigidity matroid 
${\cal C}_{2,n}^1$ is the unique maximal element, with respect to the weak order, in the set of all $K_5$-matroids on $E(K_n)$. Since every abstract $3$-rigidity matroid is a $K_{5}$-matroid, this immediately implies 
% 
%\subsection{Proof of Theorem~\ref{thm:cofactor}}
%\label{subsec:proof2}
%
%By Theorem~\ref{thm:hang},  
Theorem~\ref{thm:cofactor}.
% that ${\cal C}_n={\cal C}_{2,n}^{1}$ is the unique maximal $K_5$-matroid on $E(K_n)$.

 \begin{theorem}\label{thm:K_d+2matroid}
  The generic $C_2^1$-cofactor matroid ${\cal C}_{2,n}^{1}$ is the unique maximal $K_5$-matroid on $E(K_n)$ for all $n\geq 1$.
  \end{theorem}

\begin{proof}
The theorem is trivially true when $n\leq 5$ so we may assume that $n\geq 6$.
   Let  ${\cal M}$ be an arbitrary $K_5$-matroid on $E(K_n)$ and $F\subseteq E(K_n)$ be an independent set in $\cal M$. We will show that $F$ is independent in ${\cal C}_{2,n}^{1}$ by induction on $|F|$.  
   %put ${\cal C}={\cal C}_{2,n}^{1}$.
 %It will suffice to show that every base 
 %$B$ 
 %of ${\cal M}$ is independent in ${\cal C}_n$. 
 We will abuse notation throughout this proof and use the same letter for both a subgraph of $K_n$ and its edge set. 
 %In particular we will often consider $B$ to be a subgraph of $K_n$ as well as a base of ${\cal M}$.

 Since ${\cal M}$ is a $K_5$-matroid,  Lemma \ref{lem:rank_upper_bound} implies that $|F|=r(F)\leq 3|V(F)|-6$, and hence  
 %we may modify our choice of $v_0$ if necessary to ensure that $v_0$ 
 %the minimum degree of $B$ is at most five.
 %
 %Let $v_0$ be a vertex of 
 there exists a vertex $v_0$ of degree at most five in $F$. 
 Let $N_F(v_0)=\{v_1,\dots, v_k\}$ (where $k$ is the degree of $v_0$) and
  let $K$ be the complete graph on $N_F(v_0)$.
  
  Suppose $d_F(v_0)\leq 3$. Since $F-v_0$ is independent in ${\cal M}$, $F-v_0$ is independent in ${\cal C}^1_{2,n}$ by induction.  Then $F$ is independent in ${\cal C}^1_{2,n}$ by the $0$-extension property in Lemma~\ref{lem:cofactor_ind}.
  %This contradicts our assumption that $F$ is dependent in ${\cal C}_n$.
  Hence we may suppose $d_F(v_0)\in\{4,5\}$.
  
 \begin{claim}\label{claim:spline1} %Neither
 ${\rm cl}_{{\cal M}}(F-v_0)\cap K$
 %nor ${\rm cl}_{{\cal C}_{n-1}}(F-v_0)\cap K$ 
does not contain a copy of $K_4$.
  \end{claim}
  \begin{proof}
  Suppose, for a contradiction, that  ${\rm cl}_{{\cal M}}(F-v_0)$ contains a copy of $K_4$.
  We may assume that  ${\rm cl}_{{\cal M}}(F-v_0)$ contains $K(v_1, v_2, v_3, v_4)$. 
  Let $e_i =v_0v_i$ for $1\leq i\leq 4$.
  Since ${\cal M}$ is a $K_5$-matroid, $e_4\in \cl_{\cal M}(F-v_0+e_1+e_2+e_3)$. This contradicts the fact that $F$ is independent in ${\cal M}$.
 % Hence ${\rm cl}_{{\cal M}'}(F-v_0)\cap K$ contains no $K_4$.
%  
%  Claim~\ref{claim:spline-1} and the fact that $F-v_0$ is independent in ${\cal M}'$, now imply that  ${\rm cl}_{{\cal C}_{n-1}}(F-v_0)\cap K$ contains no copy of $K_4$.
  \end{proof}
 
%  Assume that some base $F$ of $M$ is not independent in ${\cal C}_n$ and that $F$ has been chosen amongst all such bases of $M$ so that  ${\rm cl}_{{\cal C}_{n-1}}(F-v_0)\cap K$ contains as many edges of $F-v_0$ as possible.
%  
%\begin{claim}\label{claim:spline-1}  
%  ${\rm cl}_{{\cal C}_{n-1}}(F-v_0)\cap K\subset F-v_0$.
%\end{claim} 
%\begin{proof} Suppose $e\in ({\rm cl}_{{\cal C}_{n-1}}(F-v_0)\cap K)\setminus (F-v_0)$. Then $e\in  {\rm cl}_{{M'}}(F-v_0)$ by (\ref{eq:spline0}) and hence $e$ belongs to a circuit $C$ of 
%$M'|_{F-v_0+e}$. The facts that $M$ is a $K_5$-matroid and $F$ is a base of $M$ imply that $C\not\subseteq K$ and hence we can choose $f\in C\setminus K$.  Then $F'=F-f+e$ is a base of $M$. Since $r_{{\cal C}_{n}}(F)<|F|$ and $e\in {\rm cl}_{{\cal C}_{n-1}}(F-v_0)$ we have
%$r_{{\cal C}_{n}}(F')<|F'|$ and hence $F'$ is dependent in ${\cal C}_{n}$. This contradicts the choice of $F$ since $F'$ contains more edges of $K$ than $F$.
%\end{proof}
% 
  

 Suppose that  $d_F(v_0)=4$.  Claim \ref{claim:spline1} 
 %and the fact that $F$ is independent in ${\cal M}$ 
 implies that $F-v_0+v_1v_2$ is independent in ${\cal M}$ for two non-adjacent neighbors $v_1v_2$ of $v_0$ in $F$.
 % (otherwise all edges between the neighbours of $v_0$ would belong to $\clo_{M}(F-v_0)$ and the fact that $K_5$ is dependent in $M$ would imply that $F$ is dependent in $M$). 
 We can now apply induction to deduce that $F-v_0+v_1v_2$ is independent in ${\cal C}^1_{2,n}$ and then use the 1-extension property in Lemma~\ref{lem:cofactor_ind} to deduce that $F$ is independent in ${\cal C}^1_{2,n}$.
Hence we may assume that $d_F(v_0)=5$.

\begin{claim}\label{claim:spline2-0}
$K\not\subseteq {\rm cl}_{\MM}(F-v_0+e)$ for all $e\in K$.
  \end{claim}
  \begin{proof} Suppose, for a contradiction, that $K\subseteq {\rm cl}_{\MM}(F-v_0+e)$ for some $e\in K$. 
  %Fy Claim~\ref{claim:spline1} we may assume $F-v_0+e$ is independent.
  Then  $F-v_0+e$ is independent in ${\cal M}$ by Claim \ref{claim:spline1}.
  Combining this with the fact  ${\cal M}$ is a $K_5$-matroid, we obtain
  $r_{\cal M}(F)\leq r_{\cal M}(F-v_0+e)+3$. 
  On the other hand, the fact that $F$ is independent in ${\cal M}$ tells us that $r_{\cal M}(F)= r_{\cal M}(F-v_0)+5= r_{\cal M}(F-v_0+e)+4$.
  This is a contradiction.
  \end{proof}


Claims \ref{claim:spline1} and \ref{claim:spline2-0} imply that we can choose $e_1,e_2\in K\setminus F$ such that $(F-v_0)+e_1+e_2$ is independent in $\MM$. The induction hypothesis now tells us that $(F-v_0)+e_1+e_2$ is independent in ${\cal C}^1_{2,n}$.
If $e_1,e_2$ have no common endvertices, then  $F$ can be obtained from $F-v_0+e_1+e_2$ by X-replacement and $F$ would be independent in ${\cal C}^1_{2,n}$ by Lemma~\ref{lem:cofactor_ind}, a contradiction. Hence we may suppose that $v_1$ is a common endvertex of $e_1,e_2$.  Claim  \ref{claim:spline1} now tells us that $F-v_0+e_1'$ is independent in ${\cal M}$ for some $e_1'\in K(v_2,v_3,v_4,v_5)\setminus F$, and Claim  \ref{claim:spline2-0} in turn gives an edge $e_2'\in K\setminus F$ such that $F-v_0+e_1'+e_2'$ is independent in ${\cal M}$. Then $F-v_0+e_1'+e_2'$ is independent in ${\cal C}^1_{2,n}$ by induction. 
Since $F$ can be obtained from $F-v_0+e_1+e_2$ and $F-v_0+e_1'+e_2'$ by a double V-replacement,   Theorem \ref{thm:doubleVconj} tells us that  $F$ is independent in ${\cal C}^1_{2,n}$.
This contradiction completes the proof.
\end{proof}





 
\section{Double V-replacement}\label{sec:doubleV}
The remainder of the paper is dedicated to proving Theorem~\ref{thm:doubleVconj}. Since we will only be concerned with the $C_2^1$-cofactor matroid we will often suppress specific mention of this matroid. In particular we  will 
say that a set of edges $F\subseteq E(K_n)$  is {\em independent} if it is independent in ${\cal C}^1_{2,n}$  and 
use $\cl(F)$ to denote the closure of $F$ in ${\cal C}^1_{2,n}$.
We will continue to use the terms $C^1_2$-independent and $C^1_2$-rigid for graphs.

In this section, we will formulate a special case of Theorem \ref{thm:doubleVconj},  Theorem~\ref{thm:doubleV} below, 
and then show that the general result will follow from this special case. The proof of Theorem~\ref{thm:doubleV} is delayed until Sections~\ref{sec:bad} and~\ref{sec:well-behaved}. 

We first need to establish a structural result for $C^1_2$-independent graphs.
%Recall that $K(U)$ denotes the edge set of the complete graph on $U$.

\begin{lemma}\label{lem:combinatorial}
Let $H=(V,E)$ be a $C^1_2$-independent graph, $U=\{v_1,\dots, v_5\}$ be a set of five vertices in $G$, and $K=K(U)$. 
%be the set of edges on the complete graph on $V'$.
Then at least one of the following holds:
\begin{itemize}
\item[(i)] ${\rm cl}(E)\cap K$ contains a copy of $K_4$. 
\item[(ii)] $K\subseteq {\rm cl}(E+e)$  for some edge $e\in K$.
\item[(iii)] there are two non-adjacent edges $e_1$ and $e_2$ in $K$ such that 
$H+e_1+e_2$ is $C^1_2$-independent.
\item[(iv)] there are two adjacent edges $e_1$ and $e_2$ in $K$ such that 
$H+e_1+e_2$ is $C^1_2$-independent and 
%$d_{{\rm cl}(E)\cap K}(w)=2$ at 
the common end-vertex of $e_1$ and $e_2$ is incident to two edges in ${\rm cl}(E)\cap K$. 
\item[(v)] ${\cl}(E)\cap K$ forms a star on five vertices, and ${\rm cl}(E+e)\cap K$ contains no copy of $K_4$ for all $e\in K$.
\end{itemize}
\end{lemma}
\begin{proof}
We assume that  (i) - (iv) do not hold and prove that (v) must hold.

Since (iii) does not hold, we have:
\begin{equation}\label{eq:combinatorial1}
\text{for all $e=v_iv_j\in K\setminus {\rm cl}(E)$, ${\rm cl}(E+e)$ contains a triangle on $U\setminus \{v_i,v_j\}$. }  
\end{equation}



  \begin{claim}\label{claim:spline2}
 For all $e\in K$, ${\rm cl}(E+e)\cap K$ contains no copy of $K_4$.
  \end{claim}
  \begin{proof}
  Since (i) does not occur, the claim follows if $e\in {\rm cl}(E)$.
  Thus we suppose that $e\notin {\rm cl}(E)$, and hence $E+e$ is independent.
  
  Relabeling if necessary, we may suppose $e=v_1v_2$.
 By (\ref{eq:combinatorial1}),
 ${\rm cl}(E+e)$ contains the triangle $K(v_3,v_4,v_5)$ on $\{v_3,v_4,v_5\}$.
 Since (ii) does not hold,  ${\rm cl}(E+e)\cap K$ does not contain two copies of $K_4$ (since the union of two distinct copies of $K_4$ on $U$ would form a $C_2^1$-rigid graph on $U$.)
We consider two cases.


\medskip
\noindent \emph{Case 1:} 
 Suppose that
 ${\rm cl}(E+e)\cap K$ contains a $K_4$ which includes $e=v_1v_2$. 
 By symmetry we may assume that this is a $K_4$ on $\{v_1, v_2, v_3, v_4\}$.
 Since ${\rm cl}(E+e)\cap K$ contains $K(v_3,v_4,v_5)$ and contains at most one $K_4$, 
 %we may further assume
 $v_1v_5, v_2v_5\notin {\rm cl}(E+e)$.
We will show that:
\begin{equation}
\label{eq:claim3}
%\text{all edges on $\{v_1,v_2,v_3,v_4\}$ except for $v_1v_2$ are in ${\rm cl}(E)$.}
\{v_2v_3,v_2v_4\}\subset {\rm cl}(E).
 \end{equation}

Suppose  $v_2v_3\notin {\rm cl}(E)$. 
Since   $v_2v_3\in {\rm cl}(E+e)\setminus {\rm cl}(E)$,
$E+v_2v_3$ is independent and ${\rm cl}(E+e)={\rm cl}(E+v_2v_3)$.
Since $v_1v_5 \notin {\rm cl}(E+e)$, this in turn implies $v_1v_5\notin {\rm cl}(E+v_2v_3)$. Hence $E+v_2v_3+v_1v_5$ is independent, contradicting that (iii) does not hold.
Thus $v_2v_3\in {\rm cl}(E)$. 
The same argument for $v_2v_4$ implies (\ref{eq:claim3}).

Since $v_2v_5\notin {\rm cl}(E+e)$, $E+v_1v_2+v_2v_5$ is independent. Combined with  (\ref{eq:claim3}), this contradicts the assumption that (iv) does not hold.

\medskip
\noindent \emph{Case 2:} Suppose that
 ${\rm cl}(E+e)\cap K$ contains a $K_4$ which avoids $e=v_1v_2$. 
 By symmetry we may assume that this is a $K_4$ on $\{v_1, v_3, v_4,v_5\}$. Since ${\rm cl}(E+e)\cap K$ contains at most one $K_4$, there is at most one edge from $v_2$ to $\{v_3,v_4,v_5\}$ in ${\rm cl}(E+e)\cap K$ and we may assume by symmetry that
  $v_2v_4, v_2v_5\notin {\rm cl}(E+e)$.
We will show that this case cannot occur by showing that
\begin{equation}
\label{eq:claim3.5}
\text{all edges on $\{v_1,v_3,v_4,v_5\}$  are in ${\rm cl}(E)$}
 \end{equation}
and hence that (i) holds.


Suppose $v_1v_3\notin {\rm cl}(E)$.
Then, since  $v_1v_3\in {\rm cl}(E+e)\setminus {\rm cl}(E)$,
$E+v_1v_3$ is independent and ${\rm cl}(E+v_1v_2)={\rm cl}(E+v_1v_3)$.
Since $v_2v_4\notin {\rm cl}(E+v_1v_2)$, we have  $v_2v_4\notin {\rm cl}(E+v_1v_3)$. Hence $E+v_1v_3+v_2v_4$ is independent and (iii) holds.
This contradiction implies  that $v_1v_3\in {\rm cl}(E)$. 
The same argument holds for all the other edges on $\{v_1,v_3,v_4,v_5\}$ except $v_4v_5$.
If $v_4v_5\notin {\rm cl}(E)$ then, since  $v_4v_5\in {\rm cl}(E+v_1v_2)\setminus {\rm cl}(E)$,
$E+v_4v_5$ is independent and ${\rm cl}(E+v_1v_2)={\rm cl}(E+v_4v_5)$.
This in turn implies $v_2v_4\notin {\rm cl}(E+v_4v_5)$,
and $E+v_2v_4+v_4v_5$ is independent. 
This and the fact $v_1v_4,v_3v_4\in {\rm cl}(E)$ contradicts the assumption that (iv) does not hold.
Hence $v_4v_5\notin {\rm cl}(E)$ and (\ref{eq:claim3.5}) holds.
%
%Now (\ref{eq:claim3.5}) implies that (i). This contradiction completes the proof.
\end{proof}

Claim \ref{claim:spline2} implies that the second part of condition (v) in the statement holds. It remains to show that ${\rm cl}(E)\cap K$ forms a star on $U$.
This will follow by combining Claims~\ref{claim:spline5} and \ref{claim:spline6}, below.
We first derive an auxiliary claim.
 \begin{claim}
 \label{claim:spline4}
 Suppose that $E+v_1v_2$ is independent.
 Then ${\rm cl}(E)$ has at least two edges on $\{v_3, v_4, v_5\}$.
 \end{claim}
 \begin{proof}
 Recall that ${\rm cl}(E+v_1v_2)$ contains a complete graph  on $\{v_3,v_4,v_5\}$ by (\ref{eq:combinatorial1}).
 
 We first consider the complete graph on $\{v_1, v_2, v_3, v_4\}$.
 By Claim~\ref{claim:spline2}, we may assume without loss of generality that $v_1v_3\not\in {\rm cl}(E+v_1v_2)$.
 If $v_4v_5\notin {\rm cl}(E)$, then $v_4v_5\in {\rm cl}(E+v_1v_2)\setminus {\rm cl}(E)$, and so
 ${\rm cl}(E+v_4v_5) = {\rm cl}(E+v_1v_2)$. Hence $v_1v_3\notin {\rm cl}(E+v_4v_5)$.
 This gives a contradiction as  $E+v_4v_5+v_1v_3$ would be independent  and (iii) would hold.
 Thus we obtain $v_4v_5\in {\rm cl}(E)$.

We next  consider the complete graph on $\{v_1,v_2,v_4,v_5\}$.
 By Claim~\ref{claim:spline2},   we may assume without loss of generality that either $v_1v_4\notin {\rm cl}(E+v_1v_2)$ or $v_2v_4\notin {\rm cl}(E+v_1v_2)$.
% (In the subsequent discussion we will not use $v_1v_3\notin {\rm cl}(B-v_0+v_1v_2)$, so this assumption can be done without loss of generality.)
  If $v_3v_5\notin {\rm cl}(E)$, then $v_3v_5\in {\rm cl}(E+v_1v_2)\setminus {\rm cl}(E)$, and so ${\rm cl}(E+v_1v_2)={\rm cl}(E+v_3v_5)$. Hence $v_1v_4\notin {\rm cl}(E+v_3v_5)$ or $v_2v_4\notin {\rm cl}(E+v_3v_5)$ respectively.
 This gives a contradiction as (iii) would hold.
 Thus we obtain $v_3v_5\in {\rm cl}(E)$.
 \end{proof}

 \begin{claim}
 \label{claim:spline5}
 For all $i$ with $1\leq i\leq 5$, $d_{{\rm cl}(E)\cap K}(v_i)\geq 1$.
 And if $d_{{\rm cl}(E)\cap K}(v_i)=1$, then the vertex $v_j$ adjacent to $v_i$ in ${\rm cl}(E)\cap K$ satisfies $d_{{\rm cl}(E)\cap K}(v_j)=4$.
 \end{claim}
 \begin{proof}
 Suppose that $d_{{\rm cl}(E)\cap K}(v_5)=0$.
 Since ${\rm cl}(E)$ has no copy of $K_4$, we may assume $v_1v_2\not\in {\rm cl}(E)$.
 Then $E+v_1v_2$ is independent, and ${\rm cl}(E)$ has at most one edge on $\{v_3, v_4, v_5\}$ since  $d_{{\rm cl}(E)\cap K}(v_5)=0$.
 This contradicts  Claim~\ref{claim:spline4}.

 Suppose that $d_{{\rm cl}(E)\cap K}(v_5)=1$.  We may assume without loss of generality that $v_5$ is adjacent to $v_1$ in ${\rm cl}(E)$.
 Suppose further that ${\rm cl}(E)$ does not contain $v_1v_2$.
 Then $E+v_1v_2$ is independent. On the other hand,  ${\rm cl}(E)$ has at most one edge on $\{v_3, v_4, v_5\}$ because $v_5$ is incident only to $v_1$ in ${\rm cl}(E)\cap K$.
 This again contradicts  Claim~\ref{claim:spline4}.
 \end{proof}

 \begin{claim}
 \label{claim:spline6}
 ${\rm cl}(E)\cap K$ is cycle free.
 \end{claim}
 \begin{proof}
 Suppose that ${\rm cl}(E)\cap K$ contains a cycle of length five.
 By Claim \ref{claim:spline2} we may choose two chords $e_1, e_2$ of this cycle such that $E+e_1+e_2$ is independent.
 This would contradict the assumption that (iii) and (iv) do not hold since either $e_1$ and $e_2$ are non-adjacent or  their common end-vertex has degree two in ${\rm cl}(E)\cap K$.


 Suppose that ${\rm cl}(E)\cap K$ contains a cycle of length four, say $v_1v_2v_3v_4v_1$.
% Assume that the cycle enumerate the vertices in the order of $v_1,\dots, v_4$.
 Since ${\rm cl}(E)\cap K$ has no $K_4$, we may suppose that $v_1v_3\notin {\rm cl}(E)$. Then Claim~\ref{claim:spline2} implies that $E+v_1v_3+v_2v_4$ is independent and (iii) holds, a contradiction. 
% for some $e_2\in K$. 
%This is again a contradiction.


 Suppose that ${\rm cl}(E)\cap K$ contains a triangle, say $K(v_1,v_2,v_3)$.
 Claim~\ref{claim:spline5} and the fact that ${\rm cl}(E)\cap K$ contains no cycle of length four tells us that there is exactly one edge in ${\rm cl}(E)\cap K$ from each of $v_4,v_5$  to $\{v_1,v_2,v_3\}$, and that both of these edges have a common end-vertex, say $v_1$. Hence $E+v_2v_4$ is independent. 
 We can now use (\ref{eq:combinatorial1}) to deduce that $v_3v_5\in \clo(E+v_2v_4)$.  Claim~\ref{claim:spline2} now implies that $v_2v_5\not\in \clo(E+v_2v_4)$ and hence $E+v_2v_4+v_2v_5$ is independent. This gives a contradiction since $v_2$ has degree two in ${\rm cl}(E)\cap K$ and hence (iv) holds.
 \end{proof}

 Claims \ref{claim:spline5} and \ref{claim:spline6} imply that
 ${\rm cl}(E)\cap K$ forms a star on $\{v_1,v_2,\dots, v_5\}$ and hence (v) holds.
 \end{proof}

\medskip

Let $G=(V,E)$ be a graph.
A vertex $v_0$ in $G$ is said to be of {\em type $(\star)$} if 
\begin{itemize}
\item $v_0$ has degree five with  $N_G(v_0)=\{v_1,v_2,v_3,v_4,v_5\}$,  
\item $G-v_0+v_1v_2+v_1v_3$ and $G-v_0+v_1v_3+v_3v_4$ are both $C_2^1$-rigid, and
\item ${\rm cl}(E(G-v_0))\cap K(N_G(v_0))$ forms a star on five vertices centered on $v_5$,
\end{itemize}
%cf.~the statment of the double V-replacement in Theorem~\ref{thm:doubleVconj}.
See Figure~\ref{fig:type_star}.

\begin{figure}[t]
\centering
%\begin{minipage}{0.35\textwidth}
%\centering
%\includegraphics[scale=0.8]{star1.pdf}
%\par
%(a)
%\end{minipage}
%\begin{minipage}{0.6\textwidth}
%\centering
\includegraphics[scale=0.8]{star2.pdf}
%\par
%(b)
%\end{minipage}
\caption{The double V-replacement that creates a vertex $v_0$ of type ($\star$). 
The dashed lines represent the edges in ${\rm cl}(E(G-v_0))\cap K(N_G(v_0))$, which form a star on five vertices centered on $v_5$.}
\label{fig:type_star}
\end{figure}




The following theorem implies that double V-replacement preserves 
%minimal 
minimal $C_2^1$-rigidity in the special case when the new vertex is of type $(\star)$.

\begin{theorem}\label{thm:doubleV}
Let $G=(V,E)$ be a graph with $|E|=3|V|-6$ 
and suppose that $G$ has a vertex  $v_0$  of type $(\star)$.
Then $G$ is minimally $C_2^1$-rigid.
\end{theorem}

As noted above, we delay the proof of this theorem to Sections~\ref{sec:bad} and~\ref{sec:well-behaved} and instead use it to  verify Theorem \ref{thm:doubleVconj}.

%Double V-Replacement Conjecture.
%Proving Theorem~\ref{thm:doubleV} turns out to be the most difficult step, and so we delay its proof until Sections~\ref{sec:bad} and~\ref{sec:well-behaved}.
%
%The following theorem verifies the double V-replacement conjecture posed by Whiteley~\cite{Wsurvey}. (The statement was called the double V-replacement conjecture since $G$ can be constructed from $G-v_0+e_1+e_2$ and $G-v_0+e_1'+e_2'$ by V-replacement.)
%\begin{theorem}\label{thm:doubleVconj}
%Let $G=(V,E)$ be a graph that has a vertex  $v_0$ of degree five,
%and let $\{e_1,e_2\}$ and  $\{e_1',e_2'\}$ be two pairs of adjacent edges on $N_G(v_0)$.
%Suppose that $G-v_0+e_1+e_2$ and $G-v_0+e_1'+e_2'$ are both $C_2^1$-independent,
%and that the common endvertex of $e_1$ and $e_2$ is distinct from that of $e_1'$ and $e_2'$.
%Then $G$ is $C_2^1$-independent.
%\end{theorem}
%\begin{proof}

%\subsection*{Proof of Theorem \ref{thm:doubleVconj}}
\paragraph{Proof of Theorem \ref{thm:doubleVconj}} Let $G=(V,E)$ be a graph that has a vertex  $v_0$ of degree five,
and let $\{e_1,e_2\}$ and  $\{e_1',e_2'\}$ be two pairs of adjacent edges on $N_G(v_0)$.
Suppose that  $G-v_0+e_1+e_2$ and $G-v_0+e_1'+e_2'$ are both $C^1_2$-independent,
and the common endvertex of $e_1$ and $e_2$ is distinct from that of $e_1'$ and $e_2'$.
%Then $G$ is $C_2^1$-independent.
Let $N_G(v_0)=\{v_1,\dots, v_5\}$.
We need to show that $G$ is $C_2^1$-independent.

We apply Lemma~\ref{lem:combinatorial} to $H:=G-v_0$ and $U:=N_G(v_0)$.
(Note that $H$ is $C^1_2$-independent.)
Neither (i) nor (ii) of Lemma~\ref{lem:combinatorial}  hold since otherwise $G-v_0+e_1+e_2$ or $G-v_0+e_1'+e_2'$ would be dependent.
If (iii)  holds, then we can construct $G$ from a $C^1_2$-independent graph by X-replacement, and hence $G$ is $C^1_2$-independent by Lemma~\ref{lem:cofactor_ind}.
Similarly, if  (iv) holds, then $G$ can be  constructed from a $C^1_2$-independent graph by a V-replacement satisfying the hypotheses of 
Lemma~\ref{lem:V} so is $C^1_2$-independent.
Hence we may assume (v) of Lemma~\ref{lem:combinatorial} holds,
and, without loss of generality, that  ${\rm cl}(E(H))\cap K(U)$ forms a star whose center is $v_5$.
Then $E(H)+v_1v_2$ and $E(H)+v_3v_4$ are both independent.
If $v_3v_4\notin {\rm cl}(E(H)+v_1v_2)$, then $G$ can be obtained from the $C^1_2$-independent graph $H+v_1v_2+v_3v_4$ by X-replacement.
Hence we may assume that $v_3v_4\in {\rm cl}(E(H)+v_1v_2)$, 
and thus ${\rm cl}(E(H)+v_1v_2)={\rm cl}(E(H)+v_3v_4)$ by the independence of $H+v_3v_4$.
Since (v) of Lemma~\ref{lem:combinatorial} holds, 
we may further suppose that $v_1v_3\notin {\rm cl}(E(H)+v_1v_2)$.
Therefore both $H+v_1v_2+v_1v_3$ and $H+v_3v_4+v_1v_3$ are $C^1_2$-independent.

Let $k=3|V|-6-|E|$. We complete the proof by induction on $k$.
If $k=0$ then $H+v_1v_2+v_1v_3$ and $H+v_3v_4+v_1v_3$ are both minimally $C_2^1$-rigid,
and $v_0$ is of type $(\star)$.
Theorem~\ref{thm:doubleV} now implies that $G$ is minimally $C_2^1$-rigid.

For the induction step, we assume that $k>0$.
Since  ${\rm cl}(E(H)+v_1v_2)={\rm cl}(E(H)+v_3v_4)$,
we have  ${\rm cl}(E(H)+v_1v_2+v_1v_3)={\rm cl}(E(H)+v_3v_4+v_1v_3)$.
As $H+v_1v_2+v_1v_3$ is a $k$-dof graph with $k>0$, there is an edge $f\in K(V-v_0)$ such that 
$H+v_1v_2+v_1v_3+f$ and $H+v_3v_4+v_1v_3+f$ are both $C^1_2$-independent.
Applying the induction hypothesis to $H+f$, we find that
$G+f$ is $C^1_2$-independent.
Therefore $G$ is $C^1_2$-independent.
\qed


==> cofactor1(da_final)/introduction.tex <==
\section{Introduction}\label{sec:cofactor}
The statics of skeletal structures strongly depends on their underlying graphs. This connection has been studied since the seminal work of James Clerk Maxwell \cite{Max} in 1864, and combinatorial rigidity theory is now a fundamental topic in structural rigidity~\cite{GSS93,Wsurvey}.

We will consider a {\em $d$-dimensional (bar-joint) framework},  which is a pair $(G,\bp)$ consisting of a finite graph $G=(V,E)$ and a map $\bp:V\rightarrow \mathbb{R}^d$. 
Asimow and Roth~\cite{AR78} and Gluck~\cite{Glu} observed that the properties of rigidity and infinitesimal rigidity   coincide when $\bp$ is  generic (i.e., the set of coordinates in $\bp$ is algebraically independent over the rational field),  
and  are completely determined by $G$ and $d$. This fact enables us to define the generic $d$-dimensional rigidity matroid ${\cal R}_d(G)$ on the edge set of $G$, whose rank characterizes the rigidity of any generic framework $(G,\bp)$. 
(See, e.g.,~\cite{GSS93,SW,Wsurvey} for more details.)

The generic $1$-dimensional rigidity matroid ${\cal R}_1(G)$ is equal to the graphic matroid of $G$, and a celebrated theorem of Pollaczek-Geiringer \cite{P-G} and Laman~\cite{Lam} can be used to obtain a concise combinatorial formula for the rank function of the generic $2$-dimensional rigidity matroid ${\cal R}_2(G)$, see \cite{LY82}. Finding a combinatorial description for ${\cal R}_3(G)$ remains a fundamental open problem in the field which has inspired a significant amount of research.

In 1991, Graver~\cite{G91} suggested the approach of  abstracting representative properties of the $d$-dimensional rigidity matroid and recasting rigidity as a matroid property.
Suppose that $(G,\bp)$, $(G_1, \bp_1)$ and $(G_2, \bp_2)$ are generic $d$-dimensional frameworks such that $G=G_1\cup G_2$
%$V(G_1)\cap V(G_2)\neq \emptyset$ 
and $\bp_i$ is the restriction of $\bp$ to  $V(G_i)$ for $i=1,2$. 
%Then along $V(G_1)\cap V(G_2)$ one can glue them together to get a framework $(G,\bp)$. 
It is intuitively clear that: 
\begin{itemize}
\item if $|V(G_1)\cap V(G_2)|\leq d-1$ then adding any edge between $V(G_1)\setminus V(G_2)$ and $V(G_2)\setminus V(G_1)$ will restrict the `flexibility' of $(G,\bp)$, see  Figure~\ref{fig:glueing}(a); 
\item if $|V(G_1)\cap V(G_2)|\geq d$ and $(G_1,\bp_1)$ and $(G_2,\bp_2)$ are both rigid then $(G,\bp)$ will be rigid, see Figure~\ref{fig:glueing}(b).
\end{itemize}
%the glued framework 
%$(G,\bp)$ is rigid if and only if each $(G_i,\bp_i)$ is rigid and $|V(G_1)\cap V(G_2)|\geq d$. 
Graver~\cite{G91} observed that these physical properties can be 
%completely 
described in terms of matroid closure,  and proposed to investigate all matroids which satisfy these properties.  More precisely, 
%for a finite set $V$, 
he defined a matroid $M$ on the edge set $K(V)$ of the complete graph with vertex set $V$ 
%$K(V))$ 
to be an {\em abstract $d$-rigidity matroid}  if the following two properties hold:
\begin{description}
\item[(R1)] If $E_1, E_2\subseteq K(V)$ with $|V(E_1)\cap V(E_2)|\leq d-1$, then ${\rm cl}_M(E_1\cup E_2)\subseteq K(V(E_1))\cup K(V(E_2))$;
\item[(R2)] If $E_1, E_2\subseteq K(V)$ with ${\rm cl}_M(E_1)=K(V(E_1)), {\rm cl}_M(E_2)=K(V(E_2))$, and $|V(E_1)\cap V(E_2)|\geq d$, then ${\rm cl}_M(E_1\cup E_2)=K(V(E_1\cup E_2))$,
\end{description}
where 
%$K(X)$ denotes the complete graph with vertex set  $X$ and 
${\rm cl}_M$ denotes the closure operator of $M$.
The generic $d$-dimensional rigidity matroid for $K(V)$, ${\cal R}_d(V)$,  is an example of an abstract $d$-rigidity matroid.
Graver~\cite{G91} conjectured that, for all $d\geq 1$, there is a unique maximal abstract $d$-rigidity matroid on $K(V)$ with respect to the weak order of matroids, and further that ${\cal R}_d(V)$ is this maximal matroid. 
He verified his conjecture for $d=1,2$ but N.~J.~Thurston (see, \cite[page 150]{GSS93}) subsequently showed that ${\cal R}_d(V)$ is not the unique maximal abstract $d$-rigidity matroid when $d\geq 4$.
%However the conjecture is false for $d\geq 4$, as first pointed out by 
We will verify the first part of Graver's conjecture when $d=3$.\footnote{The first part of Graver's conjecture, that there exists a unique maximal abstract $d$-rigidity matroid on $K(V)$, would follow for all $d$ as a special case of the main result in a preprint of Sitharam and Vince~\cite{SV}. Unfortunately this more general result  is false, see \cite{PAP, JT}.}
The second part 
%of Graver's conjecture for $d=3$ still 
remains as a long-standing open problem.

\begin{conjecture}[Maximality conjecture]\label{conj:max}
The generic $3$-dimensional rigidity matroid  on $K(V)$ is the unique maximal abstract $3$-rigidity matroid on $K(V)$.
\end{conjecture}

\begin{figure}[t]
\centering
\begin{minipage}{0.45\textwidth}
\centering
\includegraphics[scale=0.65]{glueing1.pdf}
\par
(a)
\end{minipage}
\begin{minipage}{0.45\textwidth}
\centering
\includegraphics[scale=0.65]{glueing2.pdf}
\par
(b)
\end{minipage}
\caption{Examples in $d=3$: (a) When $|V(G_1)\cap V(G_2)|=2$, 
$(G_1,\bp_1)$ and $(G_2,\bp_2)$ can rotate about the line through the points of $V(G_1)\cap V(G_2)$, and adding any edge between $V(G_1)\setminus V(G_2)$ and $V(G_2)\setminus V(G_1)$ will restrict this motion.
(b)  Rigid frameworks $(G_1,\bp_1)$ and $(G_2,\bp_2)$ are glued together along three vertices, and the resulting framework is rigid.}
\label{fig:glueing}
\end{figure}

%Sitharam and Vince recently released a preprint on arXiv~\cite{SV} in
%which they announce the uniqueness of the maximal abstract 3-rigidity
%matroid on $E(K_n)$.

Whiteley~\cite{Wsurvey} found another candidate for a maximal abstract $d$-rigidity matroid 
%when $d\geq 4$ 
from approximation theory.
Consider a plane polygonal domain $D$ which has been subdivided into  a set of polygonal faces $\Delta$. 
A {\em bivariate $C_s^r$-spline} over $\Delta$ is a function on $D$ which is continuously differentiable $r$ times and is given by a polynomial of degree $s$ over each face of $\Delta$. The set of all $C_s^r$-splines over $\Delta$ forms a vector space $S_s^r(\Delta)$, 
and 
%evaluating the tight bound of the 
determining the dimension of $S_s^r(\Delta)$ is a major question in this area.
When $r=0$ and $d=1$, $S_1^0(\Delta)$ is the space of piecewise linear functions, 
and {\em Maxwell's reciprocal diagram } gives a concrete correspondence between $S_1^0(\Delta)$ and  the self-stresses of the $1$-skeleton of $\Delta$, regarded  as a 2-dimensional framework $(G,\bp)$.
Whiteley~\cite{W90,W91,Wsurvey} extended this connection further and demonstrated  how the dimension of $S_s^r(\Delta)$ can be computed from the rank of the  {\em $C_s^r$-cofactor matrix $C_s^r(G,\bp)$},  which is a variant of the incidence matrix of $G$ in which the entries are replaced by block matrices whose entries are polynomials in $\bp$.
Billera~\cite{B88} used Whiteley's approach to solve a conjecture of Strang on the generic dimension of $S_s^1(\Delta)$.

The definition of  $C_s^r(G,\bp)$ is not dependent on the fact that  $(G,\bp)$ is a realisation of $G$ in the plane without crossing edges and is equally valid for  any 2-dimensional framework $(G,\bp)$. Moreover,
%for an arbitrary 2-dimensional framework $(G,\bp)$ (see Section \ref{subsec:generic_cofactor} for a formal definition). 
in the case when $r=s-1$, each row of $C_s^{s-1}(G,\bp)$ is associated with a distinct edge of $G$,
and hence the row matroid of $C_s^{s-1}(G,\bp)$ is a matroid defined on $E(G)$. We refer to this matroid  as the {\em $C_s^{s-1}$-cofactor  matroid}
for $(G,\bp)$ and denote it by 
${\cal C}_s^{s-1}(G,\bp)$.
Since the matroids ${\cal C}_s^{s-1}(G,\bp)$ are the same for all generic $\bp$, the {\em generic $C_s^{s-1}$-cofactor  matroid} of $G$, denoted  by ${\cal C}_s^{s-1}(G)$, is defined to be ${\cal C}_s^{s-1}(G,\bp)$ for any generic $\bp$. (See Section \ref{subsec:generic_cofactor} for a formal definition).
Let ${\cal C}_{d-1}^{d-2}(V)={\cal C}_{d-1}^{d-2}(K(V))$.
Whiteley~\cite{Wsurvey} showed that  ${\cal C}_{d-1}^{d-2} (V)$ is an example of an abstract $d$-rigidity matroid and pointed out that  ${\cal C}_{d-1}^{d-2} (V)={\cal R}_{d} (V)$ when $d=2$. He also showed that ${\cal C}_{d-1}^{d-2} (V)$ is a counterexample to Graver's original maximality conjecture for all $d\geq 4$ and conjectured further that  ${\cal C}_{d-1}^{d-2} (V)$  is the maximal abstract $d$-rigidity matroid for all $d\geq 2$.

In this paper we verify Whiteley's conjecture for $d=3$, and hence prove the cofactor counterpart of Conjecture~\ref{conj:max}:
\begin{theorem}\label{thm:cofactor}
The generic $C_2^1$-cofactor matroid ${\cal C}_2^1(V)$
%on the edge set of a complete graph 
is the unique maximal abstract 3-rigidity matroid on $K(V)$.  
\end{theorem}

The most difficult part of the proof of Theorem~\ref{thm:cofactor} is to show that a certain graph operation (called the double V-replacement operation) preserves independence in the generic $C_2^1$-cofactor  matroid. This is related to another long-standing conjecture on the generic 3-dimensional rigidity matroid, known as the {\em Henneberg construction conjecture},  which asks if every base of the generic 3-dimensional rigidity matroid ${\cal R}_3(V)$ can be constructed from $K_4$  by a sequence of simple graph operations (see~\cite{TW85,C14} for more details). 
%It is a classical conjecture due to Tay and Whiteley~\cite{TW85}, and  extensive efforts have been done so far to have partial solutions, see~\cite{C14} for a recent result. 
Based on a strong similarity between rigidity matroids and cofactor matroids, Whiteley~\cite[page 55]{W90} posed a corresponding Henneberg construction conjecture for the generic $C_2^1$-cofactor  matroid. 
%In this paper 
We will verify this conjecture.
% (Theorem \ref{thm:doubleVconj}).
%Our proof is not short, but the method is new, and may still be of interest as it overcomes a known technical difficulty which appears in previous work.

In his survey on generic rigidity and cofactor matroids, Whiteley gave a table of properties and conjectures for the generic $3$-dimensional rigidity and $C_2^1$-cofactor matroids
% with several conjectured items
~\cite[page 65]{Wsurvey}. The table below updates Whiteley's table with results from  \cite{JJ05} and the current paper. 
%results of this paper complete the list as follows:

\begin{center}
\begin{tabular}{|l||c|c|} \hline
 & Generic $3$-dim rigidity &Generic $C_2^1$-cofactor \\ \hline\hline
 rank $K_n$, $n \geq 3$ & $3n-6$ & $3n-6$ \\\hline
0-extension (vertex addition) & YES & YES \\\hline
1-extension (edge split) & YES & YES \\\hline
abstract 3-rigidity & YES & YES  \\\hline
vertex splitting & YES & YES  \\\hline
simplicial 2-surfaces & Rigid
~\cite{Glu} 
& Rigid
~\cite{B88} 
\\\hline
coning & YES & YES  \\\hline
X-replacement & Conjectured & YES 
\cite{Wsurvey} 
\\\hline
double V-replacement & Conjectured & YES (Theorem~\ref{thm:doubleVconj}) \\\hline
Dress conjecture & NO \cite{JJ05} & NO \cite{JJ05} \\\hline
$K_{4,6}$ & Base & Base \\\hline
$K_{5,5}$ & Circuit & Circuit \\\hline
maximal abstract 3-rigidity matroid & Conjectured & YES  (Theorem~\ref{thm:cofactor}) \\\hline
\end{tabular}
\end{center}

%This is the first paper in a series on maximal abstract rigidity and cofactor matroids. 
%In the second paper 
We will give a combinatorial characterization of the rank function of the maximal abstract 3-rigidity matroid ${\cal C}_2^1(V)$ in a companion paper~\cite{CJT1} to this one, and hence solve the cofactor counterpart to  the combinatorial characterization problem for $3$-dimensional rigidity. 
Theorem~\ref{thm:cofactor} is a key ingredient of the proof in this companion paper.

This paper focuses on proving Theorem~\ref{thm:cofactor}, and hence we restrict our attention to $C_2^1$-cofactor matroids. 
In Section~\ref{sec:preliminaries}, we first provide a brief introduction to $C_2^1$-cofactor matroids, and then give a detailed roadmap for the proof of Theorem~\ref{thm:cofactor}. 
%TODO KC - "... and provide formal definitions for terms above." eg. weak order, extension
%In Section~\ref{sec:inductive} we show that 
%%describe the proofs of 
%%our main result, 
%Theorem~\ref{thm:cofactor} will follow from the statement that double V-replacement preserves independence in the $C^1_2$-cofactor matroid. %conjecture. 
%We give a special case of this statement, Theorem~\ref{thm:doubleV}, in Section \ref{sec:doubleV} and then show that the general statement on double V-replacement will follow from the special case.
%The most difficult part of the paper is the proof of Theorem~\ref{thm:doubleV}, %which forms the core of our proof that double V-replacement preserves independence in the $C_2^1$-matroid (Theorem~\ref{thm:doubleVconj}).
%which  is given in Sections~\ref{sec:bad} and \ref{sec:well-behaved}. 
%are devoted to proving Theorem~\ref{thm:doubleV}.


==> cofactor1(da_final)/lemma46.tex <==
\section{Proof of  Lemma~\ref{lem:bad_pinning} and statement (\ref{eq:special})}\label{sec:bad_pinning}
We deduce both Lemma~\ref{lem:bad_pinning}  and statement (\ref{eq:special}) from Lemma \ref{lem:abstract_bad_pinning} below, which is a general result on matrices with polynomial entries. 
%This more general result, Lemma~\label{lem:abstract_bad_pinning}, is also required  at one point in the proof of Claim~\ref{claim:2mechanism4} when we apply it to a matrix which is not a cofactor matrix.
%For the proof of Lemma~\ref{lem:bad_pinning}, we first prove one technical lemma, Lemma~\ref{lem:abstract_bad_pinning}.


Given a matrix $M$ with entries in $\mathbb{R}[X_1,X_2,\ldots,X_m]$ and $x=(x_1,x_2,\ldots,x_m)\in \R^m$ we use $M(x)$ to denote the real matrix obtained by substituting the values $X_i=x_i$ into $M$. 
We assume that the rows and columns of $M$ are indexed by two disjoint sets $R$ and $C$ respectively. For $D\subseteq R$ and $U\subseteq C$, we use $M_D$ to denote the submatrix of $M$ with rows indexed by $D$, and $M_{D,U}$ to denote the submatrix  of $M_D$ with columns indexed by $U$. We also set $\overline{D}=R\setminus D$ and $\overline{U}=C\setminus U$.  For $x\in \R^m$, we consider the components of each vector  $z(x)\in \ker M(x)$ to be indexed by $C$ and use $z_i(x)$ to denote the $i$'th component of $z(x)$ for $i\in C$.

%We will deduce Lemma~\ref{lem:bad_pinning} from the following lemma by taking $M$ be the extended cofactor matrix for an `arbitrary' realisation of the graph $G+F$ in the statement of Lemma~\ref{lem:bad_pinning}.
%
%
%The following technical lemmas are motivated by the idea of setting $M(x)=C^1_2(G,\bp)$, $U=\hat N_G(v_0)$ and $D=E(G)$
%for our generic framework $(G,\bp)$ in the proof of Lemma~\ref{lem:bad_pinning}. %In other words, by appending suitable rows to $C(G)$, we hope to better understand the motions of G

\begin{lemma}\label{lem:abstract_bad_pinning}
Let $\F$ be a subfield of $\R$, 
$M$ be a square matrix with entries in $\F[X_1,\ldots,X_m]$, and 
$
%\begin{equation}\label{eq:abstract_bad_pinning}
T=\left\{x\in \R^m: 
 \text{$M(x)$ is non-singular}
 % and $M_{D}(x)$ is row independent
 \right\}.
$
%\end{equation}
Let
$D\subseteq R$ and $U\subseteq C$ such that every entry of $M_{D,\overline{U}}$ is zero, and let
%$
%%\begin{equation}\label{eq:abstract_bad_pinning}
%T=\left\{x\in \R^m: 
% \text{$M(x)$ is non-singular}
% % and $M_{D}(x)$ is row independent
% \right\}.
%$
%\end{equation}
%Also let 
$b:U\to \F[X_1,X_2,\ldots,X_m]$.
Suppose that,  for some $\tilde x\in T$ which is generic over $\F$, 
there is a vector $z(\tilde x)\in \ker M_{\overline{D}}(\tilde x)$ such that $z_i(\tilde x)=b_i(\tilde x)$ for all $i\in U$.
Then, for  all $x\in T$, there is a vector $z(x)\in \ker M_{\overline{D}}(x)$ such that $z_i(x)=b_i(x)$
for all $i\in U$.
\end{lemma}
\begin{proof}
 Choose any $x\in T$.
As $M(x)$ is non-singular, it is row independent and hence $M_{R-d}(x)$ is  row independent for all $d\in D$.
 Since each entry of $M_{R-d}(x)$ is a polynomial function of the coordinates of $x$, 
Cramer's rule implies that we can choose a non-zero $z_d\in \ker M_{R-d}(x)$ in such a way that 
each of its coordinates is a polynomial function of the coordinates of $x$.
%Let $z_\ell$ and $w_\ell$ be the endvertices of the edge $f_\ell$.
%Observe that $D(z_\ell,w_\ell)\cdot (q_\ell(z_\ell)-q_\ell(w_\ell))\neq 0$, since otherwise $f_{\ell}\in {\rm cl}(G+F-f_\ell)$ and this would would contradict the fact that $(G+F,p)$ is $C^1_2$-independent.
%This and the fact that $\dim Z(G,p)=t+6$  imply that 
%\begin{equation}\label{eq:bad_pinning}
If  for some $d_1\in D$, the vector $z_{d_1}$ is spanned by $\{z_d\,:\,d\in D-d_1\}$ then we would have $\ker M_{\overline{D}}(x)= \ker M_{\overline{D-d_1}}(x)$ and this would contradict the row independence of $M(x)$. Thus  
 $\{z_d:d\in D\}$ is linearly independent, and so $\dim \ker M_{\overline{D}}(x)\geq|D|$. The independence of $M(x)$ implies this holds with equality. Hence $\{z_d:d\in D\}$ is  a base for $\ker M_{\overline{D}}(x)$ and each $z\in \ker M_{\overline{D}}(x)$ can be expressed as $z=\sum_{d\in D} \lambda_d z_d$ for some $\lambda_d\in \R$.

Let  $z_d|_U$ denote the restriction of $z_d$ to $U$ for each $d\in D$. We will show that 
\begin{equation}\label{eq:abstract_bad_pinning2}
\text{
%For any $\bp\in S$, 
$\{ z_d|_U\,:\,d\in D\}$ is linearly independent.}
\end{equation}
Suppose to the contrary that, for some  
 some $d_1\in D$, $z_{d_1}|_U$ is spanned by $\{z_d|_U:d\in D-d_1\}$. Then  the hypothesis that every entry of $M_{D,\overline{U}}$ is zero implies that we again have $\ker M_{\overline{D}}(x)= \ker M_{\overline{D-d_1}}(x)$ and contradict the row independence of $M(x)$.
Hence (\ref{eq:abstract_bad_pinning2}) holds.

We next consider the matrix equation $A_x\,\lambda=b_x$ with variable $\lambda$, where $A_x$ is the $|U|\times |D|$ matrix with columns $z_d|_U$ for $d\in D$, 
$\lambda=(\lambda_1,\ldots,\lambda_{|D|})^\top$, and   $b_x\in \R^{|U|}$ is the column vector with entries given by the coordinates of
$b_{i}(x)$ for $i\in U$. 
By (\ref{eq:abstract_bad_pinning2}), $\rank A_x=|D|$ for all $x\in T$.

Since, for some generic $\tilde x\in T$,   
there is a vector $z(\tilde x)\in \ker M_{\overline{D}}(\tilde x)$ such that $z_i(\tilde x)=b_i(\tilde x)$ for all $i\in U$, the equation $A_{\tilde x}\,\lambda=b_{\tilde x}$ has a solution, and hence $\rank (A_{\tilde x},b_{\tilde x})=\rank A_{\tilde x}=|D|$ for this generic $\tilde x$.
Since each entry in $(A_x,b_x)$ is a polynomial function of the coordinates of $x$, this implies that $\rank (A_x,b_x)\leq |D|$ for all $x\in T$.
On the other hand we have seen that $\rank A_x=|D|$ for all $x\in T$.
Hence $\rank (A_x,b_x)=\rank A_x$ holds for all $x\in T$, and as a result, the equation $A_x\,\lambda=b_x$ has a solution for all $x\in T$.
This solution will give us a vector $z(x)\in \ker M_{\overline{D}}(x)$ such that $z_i(x)=b_i(x)$ for all $i\in U$ and all $x\in T$.
\end{proof}
 
%Let $G=(V,E)$ be a graph with $V=\{v_1,v_2,\ldots, v_n\}$. For $U\subseteq V$, let 
%\[
%b:U\to \R[X_1,Y_1,X_2, Y_2,\ldots,X_n,Y_n]^3
%\]
%be a map which associates a 3-tuple $b_{i}$ of polynomials in $2n$ variables to each $v_i\in U$.
%%i.e. 
%% be a subset of $t+1$ vertices in $G=(V,E)$,and let 
%%$b:U\to \R[X_1,Y_1,X_2, Y_2,\ldots,X_n,Y_n]^3$. 
%
%%Then $b_{u}$ is a $3$-tuple of polynomials with $2t$ variables for all $u\in U$.
%% representing the coordinates of the vertices of $\hat{N}_G(v_0)$.  
%For a given framework $(G,\bp)$ with $\bp(v_j)=(x_j,y_j)$ for all $1\leq j\leq n$, the substitution of $(X_j, Y_j)$ with $(x_j,y_j)$ in $b_{i}$ for all $1\leq j\leq n$ gives a vector $b_{i}(\bp)$ in $\R^3$
%%, which is simply denoted by $b_{v_i}(\bp)$ 
%for each $v_i\in U$.
%%, which we denote by $b_{u}(\bp)$.  
%%Motivated by Lemma~\ref{lem:motion}, 
%We say that a $C_2^1$-motion $\bq$ of  $(G,\bp)$ is a {\em $b$-motion}  if $\bq(v_i)=b_{i}(\bp)$  for all $v_i\in U$.
%
%Our next result uses Lemma \ref{lem:abstract_bad_pinning} to deduce that the property that $(G,\bp)$ has a $b$-motion is stable over a set  of realisations $S$. (In particular the property is generic). Since we will need the realisations in $S$ to satisfy the hypotheses of Lemma \ref{lem:1dof_motion1} it will be convenient to say that the realisation $\bp$ is {\em non-degenerate on $U$} if there exist three distinct vertices in $U$ which have distinct `$y$-coordinates' in $(G,\bp)$.
%%at vertices $v_a,v_b,v_c$} if $\bp(v_m)=(x_m,y_m)$ for $m=a,b,c$ and $(y_a-y_b)(y_b-y_c)(y_c-y_a)\neq 0$. 

%
%
%\begin{lemma}\label{lem:bad_pinning}
%Let $G=(V,E)$ be an independent graph, 
%%$v_a,v_b,v_c\in V$, 
%$U
%%=\{u_1,\dots,u_t\}
%\subseteq V$, $F
%%=\{f_1,\ldots,f_k\}
%\subseteq K(U)$, 
%%be a set of edges on $U$
%and
%\begin{equation}\label{eq:bad_pinning}
%S=\{\bar \bp:\mbox{$(G+F,\bar \bp)$ is minimally $C_2^1$-rigid and $\bar \bp$ is non-degenerate on $U$}\}.
%%\text{$\bp$ is non-degenerate at $v_a,v_b,v_c$ and $(G+F,\bp)$ is minimally $C_2^1$-rigid}
%\end{equation}
%Suppose that $b:U\to \R[X_1,Y_1,\ldots,X_n,Y_n]^3$ and $(G,\bp)$ has a $b$-motion for some generic $\bp\in S$. Then $(G,\bar \bp)$ has a $b$-motion for all $\bar \bp\in S$.
%\end{lemma}

We are now ready to prove Lemma~\ref{lem:bad_pinning}. For convenience we repeat the statement.

\newtheorem*{slemma}{Lemma~\ref{lem:bad_pinning}}
\begin{slemma}
Let $G=(V,E)$ be a $C_2^1$-independent graph with $V=\{v_1,\dots,v_n\}$, 
%$v_a,v_b,v_c\in V$, 
$U
%=\{v_1,\dots,v_t\}
\subseteq V$, $F
%=\{f_1,\ldots,f_k\}
\subseteq K(U)$, 
%be a set of edges on $U$
and
%\begin{equation}\label{eq:bad_pinning}
$
S=\{\bp:\mbox{$(G+F,\bp)$ is minimally $C_2^1$-rigid and $\bp$ is non-degenerate on $U$}\}.
%\text{$\bp$ is non-degenerate at $v_a,v_b,v_c$ and $(G+F,\bp)$ is minimally $C_2^1$-rigid}
$
%\end{equation}
Suppose that $b:U\to \rat[X_1,Y_1,\ldots,X_n,Y_n]^3$ and $(G,\bp)$ has a $b$-motion for some generic $\bp$. Then $(G, \bp)$ has a $b$-motion for all $ \bp\in S$.
\end{slemma}
\begin{proof}
Choose $ \bp_1\in S$ and let $\bp_1(v_i)=(x_i,y_i)$ for all $v_i\in V$. Since $\bp_1$ is non-degenerate on $U$, we can choose three distinct vertices $v_a,v_b,v_c\in U$ which have distinct `$y$-coordinates' in $(G, \bp_1)$. Let $\tilde{C}(G+F, \bp_1)$ be the extended $C_2^1$-cofactor matrix with respect to $v_a,v_b,v_c$ and let $M$ be the matrix obtained from $\tilde{C}(G+F, \bp_1)$ by replacing each of the coordinates $x_i,y_i$ in the definition of $\tilde{C}(G+F, \bp_1)$ by indeterminates $X_i,Y_i$ for all $v_i\in V$. Then each entry in $M$ belongs to $\rat[X_1,Y_1,\ldots,X_n,Y_n]$.
We will deduce that $(G, \bp_1)$ has a $b$-motion  at $v_0$ by  applying Lemma 
%\ref{lem:bad_pinned} and 
\ref{lem:abstract_bad_pinning} to 
$M$.

%Let $\bp_1(v_i)=(x_i,y_i)$ for all $v_i\in V$ and let $U=\{v_0,v_1,\ldots,v_5\}$.  Let $M$ be the matrix obtained from $\tilde{C}(G+F, \bp_1)$ by replacing each of the coordinates $x_i,y_i$ in the definition of $\tilde{C}(G+F, \bp_1)$ by indeterminates $X_i,Y_i$ for all $0\leq i\leq 5$.
Let
$
%\begin{equation}\label{eq:abstract_bad_pinning}
T=\{ \bp: 
 \text{$M( \bp)$ is non-singular}
 % and $M_{D}(x)$ is row independent
 \}$ and let $S_1$ be the set of all $\bp\in S$ such that $\bp(v_a)$, $\bp(v_b)$ and $\bp(v_c)$ have distinct $y$-coordinates. 
 Lemma~\ref{lem:1dof_motion1} implies that $\tilde{C}(G+F, \bp)$ is non-singular for all $ \bp\in S_1$ so $S_1\subseteq T$.
Let $D$ be the set of rows of $M$ indexed by  
$$F\cup \{\be_{s,t}:(s,t)\in \{(a,1), (a, 2), (a,3), (b,1), (b,2), (c,1)\},$$
%of  $\tilde{C}(G+F, \bp)$ 
%which do not correspond to rows of ${C}(G+F, \bp_1)$.
using the row labelling defined in Section \ref{subsec:pinning}. 
Then every entry of $M_{D,\overline{U}}$ is zero, and  $M_{\overline{D}}(\bp)=C(G,\bp)$ for all realisations $\bp$. Since $(G,\bp)$ has a $b$-motion for some  generic $\bp$,  Lemma  
\ref{lem:abstract_bad_pinning} tells us that 
$(G,\bp)$ has a $b$-motion for all $\bp\in T$. In particular $(G,\bp_1)$ has a $b$-motion. 
\end{proof}

\paragraph{Proof of statement (\ref{eq:special}).}
Since $q_{\rm bad}$ is a bad motion of $(G,\bp)$ at $v_0$, there exists $b:\hat N(v_0)\to \rat[X_0,Y_0,\ldots,X_5,Y_5]^3$ which satisfies (\ref{eq:bad}) and has $q_{\rm bad}(v)=b(v)$ for all $v\in \hat N_G(v_0)$. 

Consider the family of realisations $\bp_t$ of $G$ parametrized by $t\in \mathbb{R}$ defined by 
 $\bp_t(w)=\bp(w)$ for $w\in V_0$
and $\bp_t(u_0)=t\bp(u_0)+(1-t)\bp(u_1)$. (This family was used in the proof of \cite[Theorem 10.2.7]{Wsurvey} to show that 
vertex-splitting preserves $C_2^1$-independence.) 
Since $\bp$ is generic and $\bp_t|_{V_0}=\bp|_{V_0}$, 
%$\bp_t$ is non-degenerate on $\hat N_G(V_0)$ and hence 
we can choose three distinct vertices $v_a,v_b,v_c\in \hat N_G(v_0)$ which have distinct `$y$-coordinates' in $(G,\bp_t)$ for all $t\in \mathbb R$.  
Let $\tilde{C}(G+F,\bp_t)$ be the extended $C_2^1$-cofactor matrix for $(G+F,\bp_t)$ with respect to  $v_a,v_b,v_c$, and  let ${C}^*(G+F,\bp_t)$ be obtained from $\tilde{C}(G+F,\bp_t)$
by replacing the row indexed by the edge $u_0u_1$ with a row of the form 
$$
%\begin{equation}\label{eq:special_row}
\kbordermatrix{
 & & u_0 & & u_1 & \\
 e=u_0u_1 & 0\dots 0 & D(\bp(u_0),\bp(u_1)) & 0 \dots 0 & -D(\bp(u_0),\bp(u_1)) & 0\dots 0 
}.
%\end{equation}
$$
Since  $D(\bp_t(u_0),\bp_t(u_1))=t^2 D(\bp(u_0), \bp_t(u_1))$,
$\ker  \tilde{C}(G,\bp_t)=\ker {C}^*(G,\bp_t)$ for $t\neq 0$.
Moreover, when $t=0$,  the  argument for vertex splitting  in 
\cite[Theorem 10.2.7]{Wsurvey}
%\cite{Wsurvey} or \cite{W90vertexsplit} 
can be applied directly to show that ${C}^*(G+F,\bp_0)$ is non-singular.\footnote{
Since $(G_0+F+e_1+e_2,\bp|_{V_0})$ is minimally $C_2^1$-rigid, Lemma~\ref{lem:1dof_motion1}  implies that  $\tilde{C}(G_0+F+e_1+e_2,\bp|_{V_0})$ is row independent. 
We may now use elementary matrix manipulations and the fact that $\bp_0(u_0)=\bp(u_1)$ 
to deduce that 
${C}^*(G+F,\bp_0)$ is row independent and hence non-singular, see the proof 
of  \cite[Theorem 10.2.7]{Wsurvey}
%\cite{Wsurvey} or \cite{W90vertexsplit} 
for more details.}

Observe that $\bp_t$ is generic over $\rat$ whenever $t$ is taken to be generic over $\mathbb{Q}(\bp(V))$.
%%\footnote{This can be checked easily by looking at the following simpler situation.
%Suppose $x, y, t$ are three generic numbers over $\mathbb{Q}$, and 
%consider two numbers $x, ty+(1-t)x$. If the two numbers are not generic, then there is a non-zero polynomial $f(a,b)$ such that $f(x, ty+(1-t)x)$ is identically zero as a polynomial in $x, y, t$. Let $d$ be the maximum degree of $f$ in $b$. Then $f(a,b)=g(a)b^d+\text{(lower degree monomials in $b$)}$ for some non-zero polynomial $g$ in $a$. 
%Then $f(x,ty+(1-t)x)=g(x)t^d y^d+\text{(lower degree monomials in $y$)}$, which cannot be identically zero by $g(x)\neq 0$, a contradiction.}.
Together with Lemma~\ref{lem:bad_pinning} and the facts that $\bp$ is generic over $\rat$ and $(G,\bp)$ has a $b$-motion, this implies that  $(G, \bp_t)$ has a $b$-motion for any  $t$ which is generic over $\mathbb{Q}(\bp(V))$. 

We next consider $M:={C}^*(G+F,\bp_t)$ to be a matrix with entries in $\F[t]$ where $\F=\rat(p(V))$ and $t$ is an indeterminate. 
Let $T=\{t\in \mathbb{R} : \mbox{$M(t)$ is non-singular}\}$.
Then $0\in T$ and $t\in T$ for any generic $t$ over $\mathbb{Q}(\bp(V))$.
Let $U=\hat N_G(v_0)$ and $D$ be the set of rows of $M$ indexed by  
$F\cup \{\be_{h,k}:(h,k)\in \{(a,1), (a, 2), (a,3), (b,1), (b,2), (c,1)\}$,
%of  $\tilde{C}(G+F, \bp)$ 
%which do not correspond to rows of ${C}(G+F, \bp_1)$.
using the row labelling defined in Section \ref{subsec:pinning}. 
Then every entry of $M_{D,\overline{U}}$ is zero, and  $M_{\overline{D}}(t)=C^*(G,\bp_t)$ for all  $t\in \R$. Since $(G,\bp_t)$ has a $b$-motion and $\bp_t\in T$ for any  $t$ which is generic over $\mathbb{Q}(\bp(V))$, and $0\in T$,  Lemma  
\ref{lem:abstract_bad_pinning} implies that there exists a $z\in \ker M(0)$ such that $z(v)=b(v)$ for all $v\in U=\hat N_G(v_0)$. The fact that 
$M_{\overline{D}}(0)=C^*(G,\bp_0)$ and the defininition of $\bp_0$ now imply that
 $z|_{V_0}$ is a bad motion of $(G_0+e_1+e_2,\bp|_{V_0})$  so (\ref{eq:special}) holds.
\qed
%
%Also, by $\ker  \tilde{C}(G,\bp_t)=\ker {C}^*(G,\bp_t)$ for $t\neq 0$, 
%$\ker {C}^*(G,\bp_t)$ contains a bad motion of $(G,\bp_t)$ for any generic $t$ over $\mathbb{Q}(\bp(V))$.
%By Lemma A.1 applied to $M(t):={C}^*(G+F,\bp_t)$, 
%$\ker {C}^*(G,\bp_0)$ contains a bad motion $\bq_{\rm bad}'$  of $(G, \bp_0)$.
%The definition of $\bp_0$ implies that $\bq_{\rm bad}'(u_0)=\bq_{\rm bad}'(u_1)$,
%and hence $\bq_{\rm bad}'|_{V_0}$ is a motion of $(G_0+e_1+e_2,\bp|_{V_0})$.  
%Since $(G_0+e_1+e_2,\bp|_{V_0})$ is a generic 2-dof framework, $\bq_{\rm bad}'|_{V_0}$ is bad at $v_0$ and this
%contradicts the minimality of $|V|$.
%\qed







%\begin{slemma}
%Let $G=(V,E)$ be a $C^1_2$-independent graph, 
%%$v_a,v_b,v_c\in V$, 
%$U
%%=\{u_1,\dots,u_t\}
%\subseteq V$, $F
%%=\{f_1,\ldots,f_k\}
%\subseteq K(U)$, 
%%be a set of edges on $U$
%and
%\begin{equation}\label{eq:bad_pinning}
%S=\{\bar \bp:\mbox{$(G+F,\bar \bp)$ is minimally $C_2^1$-rigid and $\bar \bp$ is non-degenerate on $U$}\}.
%%\text{$\bp$ is non-degenerate at $v_a,v_b,v_c$ and $(G+F,\bp)$ is minimally $C_2^1$-rigid}
%\end{equation}
%Suppose that $b:U\to \R[X_1,Y_1,\ldots,X_n,Y_n]^3$ and $(G,\bp)$ has a $b$-motion for some generic $\bp\in S$. Then $(G,\bar \bp)$ has a $b$-motion for all $\bar \bp\in S$.
%\end{slemma}
%\begin{proof}%[Proof of Lemma~\ref{lem:bad_pinning}]
%Suppose $\bar \bp\in S$. Since $\bar \bp$ is non-degenerate on $U$ we can choose three distinct vertices $v_a,v_b,v_c\in U$ which have distinct `$y$-coordinates' in $(G,\bar \bp)$ and let $\tilde{C}(G+F,\bar \bp)$ be the extended $C_2^1$-cofactor matrix with respect to $v_a,v_b,v_c$. (See Section~\ref{subsec:pinning}.)
%We can then deduce that $(G,\bar \bp)$ has a $b$-motion  by  applying Lemma \ref{lem:abstract_bad_pinning} to 
%$\tilde{C}(G+F,\bar \bp)$, taking the rows indexed by $D$ to be the rows indexed by  $F$ together with the  six rows 
%%of  $\tilde{C}(G+F,\bar \bp)$ 
%which are not rows of ${C}(G+F,\bar \bp)$. 
%(More precisely, we define $M$ to be the matrix obtained from $\tilde{C}(G+F, \bp)$ by replacing each of the coordinates $x_i,y_i$ in the definition of $\tilde{C}(G+F, \bp)$ by indeterminates $X_i,Y_i$. We then  put $
%%\begin{equation}\label{eq:abstract_bad_pinning}
%T=\{\bp\in \R^{2n}: 
% \text{$M(\bp)$ is non-singular}
% % and $M_{D}(x)$ is row independent
% \}$. 
% Lemma~\ref{lem:1dof_motion1} implies that $\tilde{C}(G+F,\bar \bp)$ is non-singular for all $\bar \bp\in S$ so $S\subseteq T$.)
%\end{proof}



\section{Calculation in the proof of Lemma~\ref{lem:bad_motion}}\label{app:bad}
We use the same notation for the polynomials $D_{i,j}$ and $\Delta_{i,j,k}$, and the polynomial map $b$ as in the proof of Lemma~\ref{lem:bad_motion}. 
%Since $\bp$ is generic we can check that $b$ satisfies (\ref{eq:bad}) by performing the substitution $(X_i,Y_i):=\bp(v_i)$ for all $v_i\in  N_G(v_0)$ and checking that:
We need to show that:
%\begin{equation}\label{eq:badnew}
$$\text{the graph on $N_G(v_0)$ with edge set 
$\{v_iv_j: 
D_{v_i,v_j}\cdot (b(v_i)-b(v_j))=0 \}$
 is a star.}
$$
%\end{equation}
%where $q$ takes the specific values given in Lemma \ref{lem:motion}. 
Since $\bp$ is generic   and the $C^1_2$-motion $\bq$ of $(G,p)$ defined in the conclusion of  Lemma~\ref{lem:motion} satisfies $\bq(v_i)=b(v_i)$ for all $v_i\in N_G(v_0$), it will suffice to show that 
%\begin{equation}\label{eq:badnew}
$$\text{the graph on $N_G(v_0)$ with edge set 
$\{v_iv_j: 
D_{v_i,v_j}\cdot (\bq(v_i)-\bq(v_j))=0 \}$
 is a star,}
$$
%\end{equation}
%where $q$ takes the specific values given in Lemma \ref{lem:motion}. 
where we are abusing notation by continuing to use  $D_{ij}$ for the real number obtained from the polynomial $D(i,j)$ by the  substitution $(X_i,Y_i)\to (x_i,y_i)=\bp(v_i)$ for all $v_i\in \hat N_G(v_0)$. 
The hypotheses that $\bq$ is a $C^1_2$-motion of $(G,\bp)$ and $v_0$ is a type $(\star)$ vertex in $G$ imply that
  $D_{v_i,v_5}\cdot (\bq(v_i)-\bq(v_5))=0$ for all $1\leq i\leq 4$. Hence it only remains to check that $\delta_{ij}:=D_{v_i,v_j}\cdot (\bq(v_i)-\bq(v_j))\neq 0$ for all $1\leq i<j\leq 4$.  We can do this for each $\delta_{i,j}$ as follows, where we use $c_{ij}$ and $c_{ij}'$ to denote non-zero constants.
%Let $\delta_{ij}=D_{ij}\cdot (b(v_i)-b(v_j))$ for $0\leq i<j\leq 5$. 
%We check the value of $\delta_{ij}$ below, 
%by putting the explicit value of $q(v_i)$ for $0\leq i<j<5$:
%(We use 
%To simplify notation we  
%switch to using $D_{i,j}$ and $\Delta_{i,j,k}$ to represent the evaluations of the corresponding polynomials at $\bp(N_G(v_0))$, and use  
%use $c_{ij}$ and $c_{ij}'$ to denote some non-zero constants.
%\begin{align*}
%\delta_{01}&=D_{01}\cdot (q(v_0)-q(v_1))=c_{01} D_{0,1}\cdot  D_{01}\times D_{05}=0. \\
%\delta_{02}&=D_{02}\cdot (q(v_0)-q(v_2))\\
%&=c_{02} D_{0,2}\cdot 
%\left(
%\left|
%\begin{array}{c}
%D_{0,3} \\ D_{3,4} \\ D_{3,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{2,4} \\  D_{2,5}
%\end{array}\right|
%D_{0,1}\times D_{0,5}
%-
%\left|
%\begin{array}{c}
%D_{0,3} \\ D_{3,4} \\ D_{3,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{0,1} \\  D_{0,5}
%\end{array}\right|
%D_{2,4}\times D_{2,5}
%\right) \\
%&=
%c_{02}' \left( 
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{2,4} \\  D_{2,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{0,1} \\  D_{0,5}
%\end{array}\right|
%-
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{0,1} \\  D_{0,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{2,4} \\  D_{2,5}
%\end{array}\right|
%\right)=0 \\
%\delta_{0,3}&=0 \quad \text{(by a symmetric argument)} \\
%\delta_{0,4}&=D_{0,4}\cdot (q(v_0)-q(v_4))\\
%&=
%%D_{0,4}\cdot 
%\Delta_{1,2,3} \left|
%\begin{array}{c}
%D_{0,3} \\ D_{3,4} \\ D_{3,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{2,4} \\  D_{2,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,4} \\ D_{0,1} \\ D_{0,5}
%\end{array}\right|
%-
%\Delta_{1,2,4} \left|
%\begin{array}{c}
%D_{0,2} \\ D_{2,4} \\ D_{2,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,3} \\ D_{0,1} \\  D_{0,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,4} \\ D_{3,4} \\ D_{4,5}
%\end{array}\right|
%-\Delta_{1,3,4} \left|
%\begin{array}{c}
%D_{0,3} \\ D_{3,4} \\ D_{3,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{0,1} \\  D_{0,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,4} \\ D_{2,4} \\ D_{4,5}
%\end{array}\right| \\
%&=c_{04}(\Delta_{1,2,3}\Delta_{0,4,1}-\Delta_{1,2,4}\Delta_{0,3,1}+\Delta_{1,3,4}\Delta_{0,2,1}) \\
%&=0, 
%\end{align*}
%where the second equation follows from the Vandermonde identity and the last equation can be checked by expanding each determinant symbolically.
\begin{align*}
%\delta_{0,5}&=D_{0,5}\cdot (q(v_0)-q(v_5))=c_{0,5} D_{0,5}\cdot (D_{0,1}\times D_{0,5})=0 \\
\delta_{1,2}&=D_{1,2}\cdot (\bq(v_1)-\bq(v_2))=c_{1,2} D_{1,2}\cdot (D_{2,4}\times D_{2,5}) 
=c_{1,2}\left|
\begin{array}{c}
D_{1,2} \\ D_{2,4} \\ D_{2,5}
\end{array}\right| \neq 0. \\
\delta_{1,3}&\neq 0 \quad \text{(by a symmetric argument)}. \\
\delta_{1,4}&=D_{1,4}\cdot (\bq(v_1)-\bq(v_4))=-\alpha\Delta_{1,2,4} D_{1,4}\cdot (D_{3,4}\times D_{4,5})-\beta\Delta_{1,3,4} D_{1,4}\cdot (D_{2,4}\times D_{4,5}) \\
&=-\alpha \Delta_{1,2,4} \left|
\begin{array}{c}
D_{1,4} \\ D_{3,4} \\ D_{4,5}
\end{array}\right| 
-
\beta
\Delta_{1,3,4} \left|
\begin{array}{c}
D_{1,4} \\ D_{2,4} \\ D_{4,5}
\end{array}\right| \\
&=-\Delta_{2,5,0}\Delta_{0,1,5}\Delta_{0,5,3}\Delta_{4,5,1}\Delta_{2,4,5}\Delta_{1,2,4}\Delta_{4,3,5}\Delta_{4,1,3}(\Delta_{2,0,4}\Delta_{0,3,1}-\Delta_{3,0,4}\Delta_{0,2,1})\\
&\neq 0,
\end{align*}
where the third equation follows from the Vandermonde identity and the last relation holds since
% can be checked symbolically.
%(Symbolically 
$\Delta_{2,0,4}\Delta_{0,3,1}\neq \Delta_{3,0,4}\Delta_{0,2,1}$. 
(To see this, consider the special position where $\bp(v_3)$ is on the line through $\bp(v_0)$ and $\bp(v_1)$. 
%for an example. 
Then the left term is zero while the right term is non-zero when the other points are in a generic position.) 
\begin{align*}
%\delta_{1,5}&=0 \\
\delta_{2,3}&=D_{2,3}\cdot (\bq(v_2)-\bq(v_3)) =D_{2,3}\cdot (\beta \Delta_{1,3,2} D_{2,4}\times D_{2,5} - \alpha \Delta_{1,2,3}D_{3,4} \times D_{3,5}) \\
&=-\Delta_{1,2,3}\left( 
\beta\left|
\begin{array}{c}
D_{2,3} \\ D_{2,4} \\ D_{2,5}
\end{array}\right|
+\alpha\left|
\begin{array}{c}
D_{3,2} \\ D_{3,4} \\ D_{3,5}
\end{array}\right|
\right) \\
&=\Delta_{1,2,3} \Delta_{2,3,4}\Delta_{2,4,5}\Delta_{2,5,3}\Delta_{3,4,5}\Delta_{2,5,0}\Delta_{0,1,5}\Delta_{0,5,3}(\Delta_{3,0,4} \Delta_{0,2,1} -\Delta_{2,0,4} \Delta_{0,3,1}) \neq 0.\\
\delta_{2,4}&=D_{2,4}\cdot (\bq(v_2)-\bq(v_4))\\
&=D_{2,4} \cdot (c_{24} D_{2,4}\times D_{2,5} -\alpha \Delta_{1,2,4} D_{3,4} \times D_{4,5} - c_{24}' D_{2,4} \times D_{4,5}) \\
&=-\alpha \Delta_{1,2,4}  \left|
\begin{array}{c}
D_{2,4} \\ D_{3,4} \\  D_{4,5}
\end{array}\right| \neq 0. \\
\delta_{3,4}&\neq 0 \quad \text{(by a symmetric argument)}. 
%\\
%\delta_{4,5}&=D_{4,5}\cdot (q(v_4)-q(v_5))=D_{4,5}\cdot (c_{45} D_{3,4}\times D_{4,5} +c_{34}' D_{2,4}\times D_{4,5})=0.
\end{align*}  


==> cofactor1(da_final)/preliminaries.tex <==

\section{Preliminaries}\label{sec:preliminaries}
In this section we give a formal definition of $C_2^1$-cofactor matroids and describe their fundamental properties. 
We then give a roadmap for the proof of Theorem~\ref{thm:cofactor}.
% We also prove a few preliminary lemmas, which will be frequently used in the subsequent discussion, in Sections~\ref{subsec:pinning} and \ref{subsec:kdof}.

 We use the following notation throughout this paper.
For a finite set $V=\{v_1,v_2,\ldots,v_n\}$, let $K(V)$, or $K(v_1,v_2,\ldots,v_n)$, denote the edge set of the complete graph with vertex set  $V$.
%If $V=\{u,v,w\}$, then we sometimes denote $K(V)$ by $K(u,v,w)$.
For a graph $G=(V,E)$ and $v\in V$, let $N_G(v)$ be the set of neighbors of $v$ in $G$ and $\hat{N}_G(v)=N_G(v)\cup \{v\}$ be the closed neighborhood of $v$ in $G$.
For an edge set $F$ and a vertex $v$, let $d_F(v)$ denote the number of edges of $F$ incident to $v$. 
A {\em star on $n$ vertices} is a tree with $n$ vertices in which one vertex is adjacent to all other vertices.

We often regard a map $\bp:V\to \R^k$ as a $k|V|$-dimensional vector. 
The inner product $\bp\cdot \bq$ of two maps $\bp, \bq:V\to \R^k$ is given by this identification.

For vectors $\bv_1,\dots, \bv_k$ in a Euclidean space, let $\langle \bv_1,\dots, \bv_k\rangle$ be their linear span.

For a set $Z$ of real numbers, let $\mathbb{Q}(Z)$ denote the smallest subfield of $\mathbb{R}$ that contains the rationals and $Z$.

The closure operator and the rank function of a matroid ${\cal M}$ are 
denoted by ${\rm cl}_{{\cal M}}$ and $r_{{\cal M}}$, respectively.
The {\em weak order for matroids} is a partial order over all matroids with the same groundset $E$, where
for two matroids ${\cal M}_i=(E, r_{{\cal M}_i})\ (i=1,2)$ 
we have 
${\cal M}_1\preceq {\cal M}_2$ if $r_{{\cal M}_1}(X)\leq r_{{\cal M}_2}(X)$ holds
for all $X\subseteq E$. 

\subsection{\boldmath The $C_2^1$-cofactor Matrix}\label{subsec:generic_cofactor}

Given two points $p_i=(x_i,y_i)$ and $p_j=(x_j,y_j)$ in $\R^2$, we define $D(p_i,p_j)\in \mathbb{R}^{3}$ by
\[D(p_i,p_j)=((x_i-x_j)^2, (x_i-x_j)(y_i-y_j), (y_i-y_j)^2).
\] 
For a 2-dimensional framework $(G,\bp)$ with vertex set $V=\{v_1,v_2,\ldots,v_n\}$, we simply write $D(v_i,v_j)$ for  $D(\bp(v_i),\bp(v_j))$ when $\bp$ is clear from the context.


We define the {\em $C^{1}_2$-cofactor matrix} of a 2-dimensional framework $(G,\bp)$  to be the matrix $C_2^{1}(G,\bp)$ of size 
$|E|\times 3|V|$ in which each vertex is associated with a set of three consecutive  columns,
%is associated with a vertex, 
each edge is associated with a row,
and the row associated with the  edge $e=v_iv_j$ with $i<j$ is 
\[
\kbordermatrix{
 & & v_i & & v_j & \\
 e=v_iv_j & 0\cdots 0 & D(v_i,v_j) & 0 \cdots 0 & -D(v_i,v_j) & 0\cdots 0 
}.
\]
%where  
%\[D_s(v_i,v_j)=((x_i-x_j)^s, (x_i-x_j)^{s-1}(y_i-y_j),\dots, (x_i-x_j)(y_i-y_j)^{s-1}, (y_i-y_j)^s)\in \mathbb{R}^{s+1}.
%\]
%=((x_i-x_j)^s, (x_i-x_j)^{s-1}(y_i-y_j),\dots, (x_i-x_j)(y_i-y_j)^{s-1}, (y_i-y_j)^s)\in \mathbb{R}^{s+1}$.
For example, for $(K_4,\bp)$ with $\bp(v_1)=(0,0)$, $\bp(v_2)=(1,0)$, $\bp(v_3)=(0,1)$ and $\bp(v_4)=(-1,-1)$, 
\[
C_2^1(K_4,\bp)=
\kbordermatrix{
 & & v_1 &  & & & v_2 & & & & v_3 & & & & v_4 & \\
v_1v_2 & 1 & 0 & 0 & & -1 & 0 & 0 & & 0 & 0 & 0 & & 0 & 0 & 0 \\ 
v_1v_3 & 0 & 0 & 1 & & 0 & 0 & 0 & & 0 & 0 & -1 & & 0 & 0 & 0 \\ 
v_1v_4 & 1 & 1 & 1 & & 0 & 0 & 0 & & 0 & 0 & 0 & & -1 & -1 & -1 \\
v_2v_3 & 0 & 0 & 0 & & 1 & -1 & 1 & & -1 & 1 & -1 & & 0 & 0 & 0 \\
v_2v_4 & 0 & 0 & 0 & & 4 & 2 & 1 & & 0 & 0 & 0 & & -4 & -2 & -1 \\
v_3v_4 & 0 & 0 & 0 & & 0 & 0 & 0 & & 1 & 2 & 4 & & -1 & -2 & -4 
}.
\]
(Our definition is slightly different to that given by Whiteley \cite{Wsurvey}, but the two definitions are equivalent up to elementary column operations.)
It is known that 
the space $S_2^{1}(\Delta)$ of bivariate $C_2^{1}$-splines over a subdivision $\Delta$ of a polygonal domain in the plane is linearly isomorphic to the left kernel of  $C_2^{1}(G,\bp)$ if $(G,\bp)$ is the 1-skeleton of $\Delta$.
See, \cite{Wsurvey} for more details.

% and
%made the following conjecture. 
%\begin{conjecture}[Maximality conjecture for cofactor matroids] \cite[Conjecture 11.5.1]{Wsurvey}\label{conj:max_cofactor}
%The generic  $C_2^{1}$-cofactor matroid ${\cal C}_{2,n}^{1}$ is the unique maximal abstract $3$-rigidity matroid on $E(K_n)$ for all $n\geq 1$.
%\end{conjecture}
%For $s=1$, the conjecture follows from the result of Graver \cite{G91} that the generic $2$-dimensional rigidity matroid is the maximal abstract 2-rigidity matroid by observing that $C_1^0(G,\bp)=R(G,\bp)$ for any 2-dimensional framework $(G,\bp)$.
%% from the fact that the generic $2$-rigidity matroid is the maximal abstract 2-rigidity matroid
%%and  ${\cal C}_{1,n}^0={\cal R}_{2,n}$ by $C_1^0(G,p)=R(G,p)$ for any 2-dimensional frame.
%In this paper we solve the conjecture for $s=2$.
% \begin{theorem}\label{thm:cofactor}
%  The generic $C_2^1$-cofactor matroid ${\cal C}_{2,n}^{1}$ is the unique maximal abstract $3$-rigidity matroid on $E(K_n)$ for all $n\geq 1$.
%  \end{theorem}
  

%\subsection{Notation}
%Throughout the paper we will focus on the case when $s=2$. Hence we often suppress specific mention of $s$. In particular, we will write $D(v_i,v_j)$ for $D_2(v_i,v_j)$ and $C(G,\bp)$ for $C_2^{1}(G,{\bm p})$.
%The generic $C_2^1$-cofactor matroid ${\cal C}_{2,n}^1$ is denoted by ${\cal C}_n$ or simply by ${\cal C}$ if $n$ is clear from the context.
%%We will also assume that $n$ is a large fixed integer, that all graphs considered are subgraphs of $K_n$, and  suppress specific mention of $n$. (Note that if Conjecture \ref{conj:max_cofactor} is true for $K_n$ then it is true for $K_m$ for all $m<n$.)  and $\MC$ for $\MC_{2,n}^1$.  DO YOU THINK THIS IS A GOOD IDEA?
%
%%Also, for two points $p_i=(x_i,y_i)\in \mathbb{R}^2$, $i=1,2$ 
%%%in the plane, 
%%let 
%%\[
%%D(p_1, p_2)=((x_i-x_j)^2, (x_i-x_j)(y_i-y_j), (y_i-y_j)^2)\in \mathbb{R}^{3}.
%%\]
%




\subsection{\boldmath $C_2^1$-motions} \label{subsec:C_2^1-motions}
As mentioned above, the left kernel of the $C_2^1$-cofactor matrix $C_2^1(G,\bp)$ has an important role in the analysis of $C_2^1$-splines. An analogous situation occurs in 
%In terms of 
rigidity theory
%, each element in 
where the left kernel of the rigidity matrix is the space of {\em self-stresses} of the framework. 
%In graph rigidity, the dual concept (right kernel) has an equally important physical meaning, that is, it 
%In order to apply the analysis from graph rigidity, in this paper we shall look at 
The right kernel of the rigidity matrix plays an equally important role in %graph 
rigidity theory since it is the space of {\em infinitesimal motions} of the framework. 
%$C_2^1$-cofactor matrices. 
In order to apply techniques from rigidity theory to cofactor matrices, 
%in this paper 
we will also consider the right kernel of the $C_2^1$-cofactor matrix.

Let $G=(V,E)$ be a graph and $\bp:V\to \R^2$ such that $\bp(v_i)=(x_i,y_i)\in \mathbb{R}^2$ for all $v_i\in V$.
% and $\bp(V)$ affinely spans $\R^2$.
%and $p(v_1)=(0,0)$ and $p|_{V-v_1}$ generic.
%Let $p(v_i)=(x_i,y_i)$ for all $v_i\in V$.
A {\em $C_2^1$-motion} (or simply, a {\em motion}) of $(G,\bp)$ is a map $\bq:V\rightarrow \mathbb{R}^3$ satisfying
\begin{equation}\label{eq:cofactor_inf}
D(v_i,v_j)\cdot ( \bq(v_i)-\bq(v_j))=0\qquad (v_iv_j\in E).
\end{equation}
%where $D(v_i,v_j)=((x_i-x_j)^2, (x_i-x_j)(y_i-y_j), (y_i-y_j)^2)$ is as given in the definition of $C_2^1(G,\bp)$. 
The $C_2^1$-cofactor matrix
$C_2^1(G,\bp)$ defined in Section~\ref{subsec:generic_cofactor} is the matrix of coefficients of this system 
%(\ref{eq:cofactor_inf}) 
of linear equations in the variable $\bq$,
and hence each $C_2^1$-motion $\bq$ is a vector in the right kernel $Z(G,\bp)$ of $C_2^1(G,\bp)$.


Whiteley \cite{Wsurvey} showed that $Z(G,\bp)$  
has dimension at least six  when $\bp(V)$ affinely spans $\R^2$ by showing that  the $C_2^1$-motions $\bq_i^*:V\rightarrow \mathbb{R}^3$, $1\leq i\leq 6$, defined by
\begin{align}
%\label{eq:rigid_motions}
\bq_1^*(v_i)&=(1,0,0), &  \bq_2^*(v_i)&=(0,1,0), &  \bq_3^*(v_i)&=(0,0,1),\label{eq:rigid_motions1} \\ 
\bq_4^*(v_i)&=(y_i,-x_i,0), & \bq_5^*(v_i)&=(0,-y_i,x_i) &  \bq_6^*(v_i)&=(y_i^2,-2x_iy_i,x_i^2) \label{eq:rigid_motions2}
\end{align}  
for each $v_i\in V$,
are linearly independent  vectors in $Z(G,\bp)$ for all $G$. (We have adjusted the values of the $\bq_i^*$ given in \cite{Wsurvey} to fit our modified definition of $C_2^1(G,\bp)$.)
We will refer to a $C_2^1$-motion that can be described as a linear combination of the $\bq_i^*, 1\leq i\leq 6$ as a {\em trivial} $C_2^1$-motion,
and let $Z_0(G,\bp)$ be the space of all trivial $C_2^1$-motions.
%Then $q_1^*, \dots, q_6^*$ are called the {\em canonical base} for $Z_0(G,\bp)$.
 
 The following terminologies are $C_2^1$-cofactor analogues of standard terminologies in rigidity theory.
 We say that a framework $(G,\bp)$ is: {\em $C_2^1$-rigid} if $Z(G,\bp)= Z_0(G,\bp)$;  {\em $C_2^1$-independent} if
 the rows of $C_2^1(G,\bp)$ are linearly independent;  {\em minimally $C_2^1$-rigid} if $(G,\bp)$ is both $C_2^1$-rigid and $C_2^1$-independent; a {\em $k$-degree of freedom framework}, or {\em $k$-dof framework} for short, if $\dim Z(G,\bp)=6+k$.
We will use the same terms for the graph $G$ if  $(G,\bp)$ has the corresponding properties for some (or equivalently, every) generic $\bp$.
 
% and that  $G$ is {\em $C_2^1$-rigid} if $(G,p)$ is $C_2^1$-rigid for some $p$.
%
%We say that $(G,p)$ is a {\em $k$-degree of freedom framework}, or {\em $k$-dof framework} for short, if $\dim Z(G,p)=6+k$, and that $G$ is a {\em $k$-dof graph} if $(G,p)$ is a $k$-dof framework for some (or equivalently, every) generic $p$.

\subsection{\boldmath Generic ${C}_2^1$-cofactor Matroids}
The generic {\em $C_2^{1}$-cofactor matroid}, ${\cal C}_{2,n}^{1}$, is the matroid on $E(K_n)$ in which independence is given by the linear independence of the  rows  of $C_2^{1}(K_n,\bp)$ for any generic $\bp$. 
We will sometimes simplify ${\cal C}_{2,n}^1$ to ${\cal C}_n$ or even ${\cal C}$ when it is clear from the context.
Note that a graph $G$ with $n$ vertices is minimally $C_2^1$-rigid (resp., $C_2^1$-independent) if and only if $E(G)$ is a base (resp., an independent set) of 
${\cal C}_{2,n}^1$. 

Since $\dim Z(K_n,\bp)\geq \dim Z_0(K_n,\bp)=6$ holds when $n\geq 3$ and  $\bp$ is generic, the rank of ${\cal C}_{2,n}^1$ is at most $3n-6$ for all $n\geq 3$.
Whiteley~\cite[Corollary 11.3.15]{Wsurvey} showed that the rank of ${\cal C}_{2,n}^1$ is equal to $3n-6$ when $n\geq 3$, and, more significantly,  that ${\cal C}_{2,n}^{1}$ is an abstract $3$-rigidity matroid.
Our main result, Theorem~\ref{thm:cofactor},  verifies that ${\cal C}_{2,n}^{1}$ is the unique maximal abstract $3$-rigidity matroid on $E(K_n)$.

\subsection{Pinning}\label{subsec:pinning}
 
The technique of {\em pinning}, i.e.\ specifying the value of a motion at one or more vertices, is frequently used when dealing with a $k$-dof framework $(G,\bp)$ in rigidity theory,
and we will also use this technique in our analysis. 
The following technical lemmas will be used only in Sections~\ref{sec:bad} and~\ref{sec:well-behaved}, so the reader may wish to skip this subsection and refer back to it later.


For $v_s\in V(G)$ and $t\in \{1,2,3\}$, let ${\bf e}_{s,t}: V\rightarrow \R^3$ be such that ${\bf e}_{s,t}(v_s)$ is the unit vector with $1$ at the $t$-coordinate and zeros elsewhere, and ${\bf e}_{s,t}(v_i)=0$ for  $i\neq s$.


\begin{lemma}\label{lem:canonical}
Let $(G,\bp)$ be a 
$k$-dof framework such that $\bp(v_i)=(x_i,y_i)\in \mathbb{R}^2$ for all $v_i\in V(G)$; $v_a, v_b, v_c$ be three distinct vertices such that $(y_a-y_b)(y_a-y_c)(y_b-y_c)\neq 0$;  $\bq_0, \bq_1, \dots, \bq_k$ be motions of $(G,\bp)$ such that 
$\bq_1, \dots, \bq_k$ are linearly independent and 
%$Z(G,\bp)=Z_0(G,\bp)\oplus \langle q_1, \dots, q_k\rangle$.
%Suppose that
\begin{equation}
\label{eq:canonical1}
\bq_i\cdot {\bf e}_{s,t}=0 \text{ for all } (s,t)\in \{(a,1), (a, 2), (a,3), (b,1), (b,2), (c,1)\}
\end{equation}
for every $i\in \{0,1,\ldots,k\}$.
%If $Z(G,\bp)=Z_0(G,\bp)\oplus \langle \bq_1, \dots, \bq_k\rangle$, 
Then  $Z(G,\bp)=Z_0(G,\bp)\oplus \langle \bq_1, \dots, \bq_k\rangle$ and $\bq_0\in \langle \bq_1, \dots, \bq_k\rangle$.
%\begin{equation}
%\label{eq:canonical}
%\begin{split}
%&q(v_i)-q'(v_i)=(0,0,0) \\
%&q(v_j)-q'(v_j)=(0, 0, a) \\
%&q(v_k)-q'(v_k)=(0, b, c) \\
%\end{split}
%\end{equation}
%for some $a, b, c\in \R$.
%Then, $q$ is a scaler multiple of $q'$.
\end{lemma}
\begin{proof}
Suppose $\sum_{i=1}^k \mu_i \bq_i =\sum_{j=1}^6 \lambda_j\bq^*_j$ for some  $\mu_i, \lambda_j\in \mathbb{R}$. Then (\ref{eq:canonical1}) gives
\[
\sum_{j=1}^6 \lambda_j(\bq^*_j \cdot {\bf e}_{s,t})=0 \text{ for every } (s,t)\in \{(a,1), (a, 2), (a,3), (b,1), (b,2), (c,1)\}.
\] By the definition of $q_i^*$ in (\ref{eq:rigid_motions1}) and (\ref{eq:rigid_motions2}), this system of equations can be written as 
\[
\begin{pmatrix}
1 & 0 & 0 & y_a & 0 & y_a^2 \\ 
0 & 1 & 0 & -x_a & -y_a & -2x_ay_a \\ 
0 & 0 & 1 & 0 & x_a & x_a^2 \\
1 & 0 & 0 & y_b & 0 & y_b^2 \\ 
0 & 1 & 0 & -x_b & -y_b & -2x_by_b \\
1 & 0 & 0 & y_c & 0 & y_c^2 
\end{pmatrix}
\begin{pmatrix}
\lambda_1 \\
\lambda_2 \\
\lambda_3 \\
\lambda_4 \\
\lambda_5 \\
\lambda_6 
\end{pmatrix}
=
\begin{pmatrix}
0 \\
0 \\
0 \\
0 \\
0 \\
0
\end{pmatrix}.
\]
Let $Q$ denote the matrix of coefficients of this system. 
Then $\det Q=(y_a-y_b)^2(y_c-y_a)(y_b-y_c)\neq 0$.
Hence $Q$ is non-singular, and   $\lambda_j=0$ for all $1\leq j\leq 6$. Thus $Z_0(G,\bp)\cap \langle \bq_1, \dots, \bq_k\rangle=\{0\}$. The fact that $(G,\bp)$ is a $k$-dof framework now gives $Z(G,\bp)=Z_0(G,\bp)\oplus \langle \bq_1, \dots, \bq_k\rangle$.


Since $\bq_0$ is a motion, we have
$\bq_0=\sum_{i=1}^k \mu_i' \bq_i +\sum_{j=1}^6 \lambda_j'\bq^*_j$ for some  $\mu_i', \lambda_j'\in \mathbb{R}$.
We can  use (\ref{eq:canonical1}) to obtain 
\[
\sum_{j=1}^6 \lambda_j'(\bq^*_j \cdot {\bf e}_{s,t})=0 \text{ for every } (s,t)\in \{(a,1), (a, 2), (a,3), (b,1), (b,2), (c,1)\}.
\] The same argument as in the previous paragraph now gives 
%\] In a matrix form, this gives 
%\[
%\begin{pmatrix}
%1 & 0 & 0 & y_a & 0 & y_a^2 \\ 
%0 & 1 & 0 & -x_a & -y_a & -2x_ay_a \\ 
%0 & 0 & 1 & 0 & x_a & x_a^2 \\
%1 & 0 & 0 & y_b & 0 & y_b^2 \\ 
%0 & 1 & 0 & -x_b & -y_b & -2x_by_b \\
%1 & 0 & 0 & y_c & 0 & y_c^2 
%\end{pmatrix}
%\begin{pmatrix}
%\lambda_1 \\
%\lambda_2 \\
%\lambda_3 \\
%\lambda_4 \\
%\lambda_5 \\
%\lambda_6 
%\end{pmatrix}
%=
%\begin{pmatrix}
%0 \\
%0 \\
%0 \\
%0 \\
%0 \\
%0
%\end{pmatrix}.
%\]
%Let $Q$ denote the matrix of coefficients of this system. 
%Since $(y_a-y_b)(y_a-y_c)(y_b-y_c)\neq 0$,
%%Then 
%$Q$ is nonsingular  
%%(i.e., the determinant is a nonzero polynomial in $x_a, y_a, x_b, y_b, y_c$),
$\lambda_j'=0$ for all $1\leq j\leq 6$. 
In other words, $\bq_0$ is a linear combination of $\bq_1, \dots, \bq_k$.
\end{proof}


Suppose $v_a, v_b, v_c$ are distinct vertices in a framework $(G,\bp)$. 
We define the {\em extended $C_2^1$-cofactor matrix} $\tilde{C}(G,\bp)$ (with respect to  $(v_a, v_b, v_c)$) 
to be the matrix of size $3|V|\times (|E|+6)$ obtained from $C(G,\bp)$ by adding the six rows,
${\bf e}_{a,1}, {\bf e}_{a,2}, {\bf e}_{a,3}, {\bf e}_{b,1}, {\bf e}_{b,2}, {\bf e}_{c,1}$.

For example, for $(K_4,\bp)$ with $\bp(v_1)=(0,0)$, $\bp(v_2)=(1,0)$, $\bp(v_3)=(0,1)$ and $\bp(v_4)=(-1,-1)$, 
the extended $C_2^1$-cofactor matrix with respect to $(v_1,v_2,v_3)$ is
\[
\kbordermatrix{
 & & v_1 &  & & & v_2 & & & & v_3 & & & & v_4 & \\
 & 1 & 0 & 0 & & 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\ 
 & 0 & 1 & 0 & & 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\ 
 & 0 & 0 & 1 & & 0 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\ 
 & 0 & 0 & 0 & & 1 & 0 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\ 
 & 0 & 0 & 0 & & 0 & 1 & 0 && 0 & 0 & 0 && 0 & 0 & 0 \\ 
 & 0 & 0 & 0 & & 0 & 0 & 0 && 1 & 0 & 0 && 0 & 0 & 0 \\ 
v_1v_2 & 1 & 0 & 0 & & -1 & 0 & 0 & & 0 & 0 & 0 & & 0 & 0 & 0 \\ 
v_1v_3 & 0 & 0 & 1 & & 0 & 0 & 0 & & 0 & 0 & -1 & & 0 & 0 & 0 \\ 
v_1v_4 & 1 & 1 & 1 & & 0 & 0 & 0 & & 0 & 0 & 0 & & -1 & -1 & -1 \\
v_2v_3 & 0 & 0 & 0 & & 1 & -1 & 1 & & -1 & 1 & -1 & & 0 & 0 & 0 \\
v_2v_4 & 0 & 0 & 0 & & 4 & 2 & 1 & & 0 & 0 & 0 & & -4 & -2 & -1 \\
v_3v_4 & 0 & 0 & 0 & & 0 & 0 & 0 & & 1 & 2 & 4 & & -1 & -2 & -4 
}.
\]

\medskip


\begin{lemma}
\label{lem:1dof_motion1}
Let $(G,\bp)$ be a framework with $|E(G)|=3|V(G)|-(6+k)$, and denote $\bp(v_i)=(x_i,y_i)$ for each $v_i\in V$. Let $\tilde{C}(G,\bp)$ be the
extended $C_2^1$-cofactor matrix  with respect to three vertices $(v_a, v_b, v_c)$ and suppose that 
%$\bp(v_f)=(x_f,y_f)$ for all $v_f\in V$ and  
$(y_a-y_b)(y_a-y_c)(y_b-y_c)\neq 0$.
Then $\tilde{C}(G,\bp)$ is row independent if and only if $\dim Z(G,\bp)=6+k$.
\end{lemma}
\begin{proof}
If $\tilde{C}(G,\bp)$ is row independent, then $C(G,\bp)$ is row independent and hence $$\dim Z(G,\bp)=3|V(G)|-|E(G)|=6+k.$$
To see the converse, suppose $\dim Z(G,\bp)=6+k$ but $\tilde{C}(G,\bp)$ is row dependent.
We can choose $k+1$ linearly independent $C_2^1$-motions $\bq_0, \bq_1,\dots, \bq_k$ of $(G,\bp)$ from the kernel of $\tilde{C}(G,\bp)$. 
Then each $\bq_i$ 
%is taken from the kernel of $\tilde{C}(G,\bp)$, it 
satisfies (\ref{eq:canonical1}). Hence, by Lemma~\ref{lem:canonical}, $\bq_0\in\langle \bq_1,\dots, \bq_k\rangle$, which is a contradiction.
\end{proof}



\subsection{Roadmap for  the proof of Theorem~\ref{thm:cofactor}}
The proof of Theorem~\ref{thm:cofactor} is structured as follows:
{\footnotesize
\[
\text{Theorem~\ref{thm:cofactor} $\overset{\mathrm{Sec~\ref{subsec:K_d matroid}}}\Longleftarrow$
Theorem~\ref{thm:K_d+2matroid} $\overset{\mathrm{Sec~\ref{subsec:proof_of_thm12}}}\Longleftarrow$
Theorem~\ref{thm:doubleVconj} $\overset{\mathrm{Sec~\ref{sec:doubleV}}}\Longleftarrow$
Theorem~\ref{thm:doubleV} $\overset{\mathrm{Sec~\ref{sec:bad}}}\Longleftarrow$
Theorem~\ref{thm:well-behaved0}$\overset{\mathrm{Sec~\ref{sec:well-behaved}}}\Longleftarrow$
Theorem~\ref{thm:well-behaved}}.
\]
}
Below we briefly explain each theorem and step.

\paragraph{Section~\ref{subsec:K_d matroid}:} 
%We prove Theorem~\ref{thm:K_d+2matroid}, which is a slightly stronger statement than Theorem~\ref{thm:cofactor} in the following sense.
It is known that the edge set of $K_5$ is a circuit  in any abstract 3-rigidity matroid (see, e.g., \cite{GSS93} or Theorem~\ref{thm:hang}).
A matroid satisfying this circuit property is called a $K_5$-matroid.
The class of $K_5$-matroids is slightly larger  than the set of abstract 3-rigidity matroids.
Theorem~\ref{thm:K_d+2matroid} states that the generic $C_2^1$-cofactor matroid ${\cal C}_2^1(K_n)$ is the unique maximal matroid in the poset of all  $K_5$-matroids on $E(K_n)$.
Thus Theorem~\ref{thm:K_d+2matroid} is a stronger version of Theorem~\ref{thm:cofactor}.

\paragraph{Section~\ref{subsec:proof_of_thm12}:}
 Graver~\cite{G91} proved that the generic 2-dimensional rigidity matroid is the unique maximal abstract 2-rigidity matroid based on that fact that 
 any base of the generic 2-dimensional rigidity matroid  can be constructed from $K_3$ by a sequence of two simple graph operations, called the Henneberg constructions. 
% We follow the same approach.
 Following the same approach as that of Graver~\cite{G91}, 
 we show that Theorem~\ref{thm:K_d+2matroid} will follow from an inductive construction of the bases of the  ${\cal C}_2^1$-cofactor matroid. 
For this purpose, Whiteley~\cite{Wsurvey} already verified that  various graph operations preserve $C_2^1$-independence. 
However, there remained one operation, double V-replacement, that Whiteley could not show preserved independence. (See Figure~\ref{fig:doubleV} for an example of double V-replacement.).
We confirm that it does preserve independence in Theorem~\ref{thm:doubleVconj}. The remainder of the paper is devoted to proving this result.

\paragraph{Section~\ref{sec:doubleV}:}
By combining existing results from~\cite{Wsurvey} and a simple combinatorial argument in  Section~\ref{sec:doubleV}, we prove that Theorem~\ref{thm:doubleVconj} holds in all but  one special case.
This remaining special case is when ${\rm cl}(E(G-v_0))\cap K(N_G(v_0))$ forms a star on five vertices as shown in Figure~\ref{fig:type_star},
where $v_0$ denotes the vertex created by the double $V$-replacement.
We formulate a new result, Theorem~\ref{thm:doubleV}, to  deal with  this remaining special case.


\paragraph{Section~\ref{sec:bad}:}

 In Section~\ref{sec:bad}, we first show that, if the statement of  Theorem~\ref{thm:doubleV} fails, then the framework created by  the double V-replacement operation has a very special $C_2^1$-motion.
 Theorem~\ref{thm:well-behaved0} states that such a motion cannot exist in any generic $1$-dof framework.
 
 
 \paragraph{Section~\ref{sec:well-behaved}:}
 We prove Theorem~\ref{thm:well-behaved0}. Our inductive proof requires a more general inductive statement, Theorem~\ref{thm:well-behaved}, which  concerns frameworks with at most two degrees of freedom. The proof is rather long so we first outline the main ideas in Section~\ref{subsec:outline}.
 






 

%In Section~\ref{sec:inductive} we show that 
%%describe the proofs of 
%%our main result, 
%Theorem~\ref{thm:cofactor} will follow from the statement that double V-replacement preserves independence in the $C^1_2$-cofactor matroid. %conjecture. 
%We give a special case of this statement, Theorem~\ref{thm:doubleV}, in Section \ref{sec:doubleV} and then show that the general statement on double V-replacement will follow from the special case.
%The most difficult part of the paper is the proof of Theorem~\ref{thm:doubleV}, %which forms the core of our proof that double V-replacement preserves independence in the $C_2^1$-matroid (Theorem~\ref{thm:doubleVconj}).
%which  is given in Sections~\ref{sec:bad} and \ref{sec:well-behaved}. 



%\subsection{Locally $k$-dof parts}\label{subsec:kdof}
%Let $G=(V,E)$ be a graph.
%A set $X\subseteq V$ is said to be a {\em locally rigid part} in $G$ if 
%every edge in $K(X)$ is in ${\rm cl}_{{\cal C}}(E(G))$. 
%The set $X$ is said to be a {\em locally $k$-dof part} in $G$ if 
%there is a set $F$ of $k$ edges in $K(V)$ such that 
%$X$ is locally rigid part in $G+F$, but 
%%there is 
%no smaller edge set has this property.
%
%\begin{lemma}\label{lem:local1}
%Let $G=(V,E)$ be a graph and $X$ be a locally $k$-dof part in $G$.
%Then  there exists a set of edges $D$ of $K(V)$ such that  $H=G+D$ is a $k$-dof graph and $X$ is still a locally $k$-dof part in $H$.
%Moreover, for any generic framework $(G,\bp)$ and any motion $\bq$ of $(G,\bp)$, $(H,\bp)$ has a motion $\bq'$ satisfying $\bq'(v)=\bq(v)$ for all $v\in X$.
%\end{lemma}
%\begin{proof} 
%%We first consider the case when $(G,p)$ is generic. 
%%Let $E'$ be a maximal subset of $E$ which is independent in $\MC^1_2(G,p)$,
%% put $G'=(V,E')$. 
%Let 
%$F$ be a set of $k$ edges in $K(V)$ such that $X$ is a locally rigid part in $G+F$, and $D$ be a minimal set of edges in $K(V)$ such that $G+F+D$ is $C^1_2$-rigid. For each $e\in F\cup D$, $G+F+D-e$ is a 1-dof graph and we can choose a non-trivial $C^1_2$-motion $\bq_e$ of  $(G+F+D-e,\bp)$. Then $B_1=\{\bq_i^*\,:\,1\leq i\leq 6\}\cup
%\{\bq_e\,:\,e\in F\cup D\}$ is a base for $Z(G,\bp)$ and 
%$B_2=\{\bq_i^*\,:\,1\leq i\leq 6\}\cup
%\{\bq_e\,:\,e\in F\}$ is a base for $Z(G+D,\bp)$. The facts that the motions in $B_1$ are linearly independent and that, for each $e\in F$, we have $D(u,v)\cdot (\bq_e(u)-\bq_e(v))\neq 0$ for some $u,v\in X$ now implies that we must add at least $k$ edges to $G+D$ to make $X$ locally rigid. Hence $X$ is a locally $k$-dof part in $G+D$.
%
%Since $\bq$ is a motion of $(G,\bp)$ and $B_1$ is a base for $Z(G,\bp)$, we have $\bq=\sum_{i=1}^6 \lambda_i \bq_i^*+\sum_{e\in  F\cup D}\mu_e \bq_e$ for some $\lambda_i, \mu_e\in \R$. Since $X$ is a locally rigid part of $G+F$, $\bq_e|_X$ is a trivial motion of $(K(X),\bp|_X)$ for all $e\in D$. Hence $\bq_e|_X=\bq_e^*|_X$ for some trivial motion $\bq_e^*$ of $(G,\bp)$. Let $\bq'=\sum_{i=1}^6 \lambda_i' \bq_i^*+\sum_{e\in  F}\mu_e \bq_e+\sum_{e\in D}\mu'_e \bq_e^*$. Then $\bq'|_X=\bq^*|_X+\sum_{e\in F}\mu_e \bq_e|_X $ for some $\bq^*\in Z_0(G,\bp)$. For the right choices of $\lambda_i'$ and $\mu_e'$, this gives $\bq'|_X=\bq|_X$.  Since $B_2$ is a base for $Z(G+D,\bp)$, we have $\bq'\in Z(G+D,\bp)$. 
%\end{proof}


==> cofactor1(da_final)/projective.tex <==
\section{Projective Transformations}\label{sec:projective}

%We say that a framework $(G,\bq)$ is a projective image of a framework $(G,p)$ if there is a projective transformation $f$ such that 
%$\bq(v_i)=f(\bp(v_i))$ for every $v_i\in V$.
%It was shown by Whiteley that $C_2^1$-rigidity is invariant by projective transformations. 
%The proof of Whiteley for the projective invariance is based on a self-stress argument, 
We give a new analysis of the projective invariance of $C_2^1$-rigidity from the viewpoint of $C_2^1$-motions, and then use this to prove Lemma~\ref{lem:projective_bad}.


Let $\mathbb{S}^{3\times 3}$ be the set of symmetric $3\times 3$ matrices. We will use the fact  that ${\rm Trace}(AB)=\sum_{1\leq i, j\leq 3} a_{ij}b_{ij}$ holds for any $A=(a_{ij}), B=(b_{ij})\in \mathbb{S}^{3\times 3}$.

\subsection{\boldmath $C_2^1$-motions in the projective setting}
Recall that each point $p_i=(x_i,y_i)^\top\in \R^2$ is associated with the point $p_i^{\uparrow}=[x_i,y_i,1]^\top$ in 2-dimensional real projective space $\bP^2$. This allows us to associate a framework $(G,\bp^{\uparrow})$ in $\bP^2$ with any framework $(G,\bp)$ in $\R^2$.   
We will consider $(G,\bp^{\uparrow})$ to be a framework in $\R^3$ in which the `$z$-component' of every vertex is non-zero and  define a projective  $C_2^1$-motion as a new kind of motion of such a framework.
  
Let $G=(V,E)$ be a graph and $\tilde{\bp}:V \to \mathbb{R}^3$ such that $\tilde \bp(v_i)=(x_i, y_i, z_i)^{\top}$ and
%.For simplicity of description, throughout this paper we shall focus on the case when 
$z_i\neq 0$ for all $v_i\in V$. 
We say that $\bQ:V\rightarrow \mathbb{S}^{3\times 3}$ is a {\em projective  $C_2^1$-motion} of $(G, \tilde{\bp})$ if 
\begin{equation}\label{eq:projective}
{\rm Trace}\left((\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))(\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))^{\top} (\bQ(v_i)-\bQ(v_j))\right)=0 
\end{equation}
for all $v_iv_j\in E$, where $(\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))$ denotes the cross product of $\tilde{\bp}(v_i)$ and $\tilde{\bp}(v_j)$.
%, i.e. 
%$$\tilde{\bp}(v_i)\times \tilde{\bp}(v_j) = 
%\left( 
%\left|\begin{array}{cc} y_i & z_i \\ y_j & z_j \end{array}\right|,
%\left|\begin{array}{cc} z_i & x_i \\ z_j & x_j \end{array}\right|,
%\left|\begin{array}{cc} x_i & y_i \\ x_j & y_j \end{array}\right|
%\right)^{\top}.$$
A projective $C^1_2$-motion $\bQ$ is \emph{trivial} if \eqref{eq:projective} holds for all $v_i,v_j\in V$. 
These definitions are inspired by the following observation (and Lemma~\ref{lem:projective2} below).





\begin{lemma}\label{lem:projective1}
For a framework $(G,\bp)$ in $\R^2$, 
define $\bp^{\uparrow}:V\rightarrow \mathbb{R}^3$ by 
$\bp^{\uparrow}(v_i)=(\bp(v_i), 1)^\top$.
For $\bq:V\rightarrow \mathbb{R}^3$, define $\bQ:V\rightarrow \mathbb{S}^{3\times 3}$ by 
\begin{equation}\label{eq:lifting}
\bq(v_i)=\begin{pmatrix} 
q_1(v_i) \\ q_2(v_i)\\ q_3(v_i)
\end{pmatrix}
%\in \mathbb{R}^3 
\mapsto
\bQ(v_i)=\begin{pmatrix}
2q_3(v_i) & -q_2(v_i) & 0 \\
-q_2(v_i) & 2q_1(v_i) & 0 \\
0 & 0 & 0
\end{pmatrix} \mbox{for all $v_i\in V$.}
%\in \mathbb{S}^{3\times 3}.
\end{equation}
Then $\bq$ is a $C^1_2$-motion of $(G,\bp)$ if and only if $\bQ$ is a projective  $C_2^1$-motion of $(G,\bp^{\uparrow})$.
\end{lemma}
\begin{proof}
Denote $\bp(v_i)=(x_i ,y_i )^\top$ for all $v_i\in V$. Then
\[
(\bp^{\uparrow}(v_i)\times \bp^{\uparrow}(v_j))(\bp^{\uparrow}(v_i)\times \bp^{\uparrow}(v_j))^{\top}
=\begin{pmatrix}
(y_i-y_j)^2 & -(x_i-x_j)(y_i-y_j) & \ast \\
-(x_i-x_j)(y_i-y_j) & (x_i-x_j)^2 & \ast \\
\ast & \ast & \ast
\end{pmatrix}.
\]
It is now straightforward to check that  
%(\ref{eq:projective}) holds for $\bQ$ 
%(of the form of (\ref{eq:lifting}) 
%if and only if 
%$D(p(v_i), p(v_j))\cdot (\bq(v_i)-\bq(v_j))=0$ holds for $\bq$.
$${\rm Trace}\left((\bp^{\uparrow}(v_i)\times \bp^{\uparrow}(v_i))(\bp^{\uparrow}(v_i)\times \bp^{\uparrow}(v_i))^{\top} (\bQ(v_i)-\bQ(v_j))\right)=2D(\bp(v_i), \bp(v_j))\cdot (\bq(v_i)-\bq(v_j))$$
for all $v_i,v_j\in V$.
\end{proof}

Lemma~\ref{lem:projective1} gives a linear isomorphism between the $C_2^1$-motions $\bq$ of $(G,\bp)$ and the projective $C_2^1$-motions $\bQ$ of $(G,\bp^{\uparrow})$
with the property  that the right column and bottom row of $\bQ$ are both zero. 


\subsection{\boldmath Projective $C_2^1$-rigidity}
We show that every framework $(G,\tilde \bp)$ in $\R^3$ has at least $3|V|+6$ linearly independent projective $C_2^1$-motions.
% and hence the dmension of its space of projective $C_2^1$-motions is at least $3|V|+6$. 
We use this to define projective $C_2^1$-rigidity and then show that a given framework $(G,\bp)$ in $\R^2$ is $C_2^1$-rigid if and only if the corresponding framework
$(G,\bp^\uparrow)$ in $\R^3$ is projective $C_2^1$-rigid.

%Given $(G,\hat{p})$ with $\hat{p}:V\rightarrow \mathbb{R}^3$, a motion of $(G,\hat{p})$ was defined to be a map $\bQ:V\rightarrow \mathbb{S}^{3\times 3}$ satisfying (\ref{eq:projective}).
%Since $\mathbb{S}^{3\times 3}$ is a six-dimensional space, the set of maps $\bQ:V\rightarrow \mathbb{S}^{3\times 3}$ forms a $6|V|$-dimensional space, which is much bigger than the set of maps $q:V\rightarrow \mathbb{R}^3$ for an ordinary framework $(G,p)$. We now explain how to understand that extra $3|V|$-dimensional space.
%  
%We next investigate the trivial motions of $(G,\tilde{p})$.
We defined six linearly independent (trivial) $C_2^1$-motions $\bq_i^*$ for an arbitrary 2-dimensional framework in (\ref{eq:rigid_motions1}) and (\ref{eq:rigid_motions2}).
We may apply Lemma \ref{lem:projective1} to each of these to obtain the following 
six linearly independent  projective $C_2^1$-motions for any framework $(G,\tilde \bp)$ in $\R^3$.
%
%we have defined trivial motions of a 2-dimensional framework $(G,\bp)$. The corresponding motions for $(G,\tilde{p})$ are defined by 
%$Q_i^*:V\rightarrow \mathbb{S}^{3\times 3}$, where 
\begin{equation}\label{eq:projective_trivial}
\begin{gathered}
\bQ_1^*(v_i)=\begin{pmatrix}
0 & 0 & 0 \\
0 & 2 & 0 \\
0 & 0 & 0 
\end{pmatrix}, 
\bQ_2^*(v_i)=\begin{pmatrix}
0 & -1 & 0 \\
-1 & 0 & 0 \\
0 & 0 & 0 
\end{pmatrix}, 
\bQ_3^*(v_i)=\begin{pmatrix}
2 & 0 & 0 \\
0 & 0 & 0 \\
0 & 0 & 0 
\end{pmatrix}, \\
\bQ_4^*(v_i)=\begin{pmatrix}
0 & x_i/z_i & 0 \\
x_i/z_i & 2 y_i/z_i & 0 \\
0 & 0 & 0 
\end{pmatrix}, 
\bQ_5^*(v_i)=\begin{pmatrix}
2x_i/z_i & y_i/z_i & 0 \\
y_i/z_i & 0 & 0 \\
0 & 0 & 0 
\end{pmatrix}, \\
\bQ_6^*(v_i)=\begin{pmatrix}
2x_i^2/z_i^2 & 2x_iy_i/z_i^2 & 0 \\
2x_iy_i/z_i^2 & 2y_i^2/z_i^2 & 0 \\
0 & 0 & 0 
\end{pmatrix}.
\end{gathered}
\end{equation}
It is straightforward to check that each $\bQ_k^*$, $1\leq k\leq 6$, satisfies (\ref{eq:projective}) for every pair of vertices $v_i, v_j\in V$, and hence is a trivial projective $C_2^1$-motion of $(G,\tilde{\bp})$.
%(Notice also that the trivial motions (\ref{eq:rigid_motions1}) and (\ref{eq:rigid_motions2}) for an ordinary framework are obtained from (\ref{eq:projective_trivial}) via the correspondence given in Lemma~\ref{lem:projective1}.)
We may define a further $3|V|$ linearly independent projective $C_2^1$-motions for any $(G,\tilde \bp)$, three for each vertex, as follows.
For each $v_i\in V$, let $\bQ_{i,1}^*, \bQ_{i,2}^*, \bQ_{i,3}^*: V\rightarrow \mathbb{S}^{3\times 3}$ by: 
\begin{equation}\label{eq:trivial_vertex}
\begin{gathered}
\bQ_{i,1}^*(v_i)= \begin{pmatrix} 0 & x_i & 0 \\ x_i & 2y_i & z_i \\ 0 & z_i & 0 \end{pmatrix}, 
\text{ and } \bQ_{i,1}^*(v_j)=\begin{pmatrix} 0 & 0 & 0 \\ 0 & 0 & 0 \\ 0 & 0 & 0 \end{pmatrix} \text{ for all } v_j\neq v_i; \\
\bQ_{i,2}^*(v_i)= \begin{pmatrix} 2x_i & y_i & z_i \\ y_i & 0 & 0 \\ z_i & 0 & 0 \end{pmatrix}, \text{ and } 
\bQ_{i,2}^*(v_j)=\begin{pmatrix} 0 & 0 & 0 \\ 0 & 0 & 0 \\ 0 & 0 & 0 \end{pmatrix} \text{ for all } v_j\neq v_i; \\
\bQ_{i,3}^*(v_i)= \begin{pmatrix} -x_i^2 & -x_iy_i & 0 \\ -x_iy_i & -y_i^2 & 0 \\ 0 & 0 & z_i^2 \end{pmatrix}, \text{ and } 
\bQ_{i,3}^*(v_j)=\begin{pmatrix} 0 & 0 & 0 \\ 0 & 0 & 0 \\ 0 & 0 & 0 \end{pmatrix} \text{ for all  } v_j\neq v_i. 
\end{gathered}
\end{equation}
It is straightforward to check that each  $\bQ_{i,j}^*$ satisfies (\ref{eq:projective}) for all pairs of vertices $v_i, v_j\in V$, and hence is a trivial motion of $(G,\tilde{\bp})$.
We will refer to the space of projective $C_2^1$-motions generated by these $3|V|+6$ motions as the {\em space of trivial motions}, and say that a projective $C_2^1$-motion of $(G,\tilde \bp)$ is {\em non-trivial} if it does not belong to this space.
We define $(G,\tilde{\bp})$ to be {\em projectively $C_2^1$-rigid} if every projective $C_2^1$-motion of $(G,\tilde{\bp})$ is a trivial motion, or equivalently, if its space of projective $C_2^1$-motions has dimension $3|V|+6$.

The following lemma follows from Lemma~\ref{lem:projective1} (and the formulae for $\bQ_{i,j}^*$ given above).
\begin{lemma}\label{lem:projective2}
Let $(G,\bp)$ be a two-dimensional framework, and let $(G,\bp^{\uparrow})$ be as defined in Lemma~\ref{lem:projective1}.
Then $(G,\bp)$ is $C_2^1$-rigid if and only if $(G,\bp^{\uparrow})$ is projectively $C_2^1$-rigid.
\end{lemma}

\subsection{Projective invariance} \label{subsec:projective_motion}
In this subsection we show that 
the projective $C_2^1$-rigidity of a framework $(G,\tilde \bp)$ is invariant under a pointwise scaling and a non-singular linear transformation of $\mathbb{R}^3$.
These two facts combined with Lemma~\ref{lem:projective2} 
will imply the projective invariance of $C_2^1$-rigidity for 2-dimensional frameworks. 
 
We first show that the projective $C_2^1$-rigidity of $(G,\tilde \bp)$ is invariant by the scaling of each point.
Choose a non-zero scalar
$\lambda_i\in \R$ for each $v_i\in V$, and let $\lambda \tilde{\bp}$ be the point configuration in $\mathbb{R}^3$ defined by $(\lambda \tilde{\bp})(v_i)=\lambda_i \tilde{\bp}(v_i)$ for each $v_i\in V$.
Then $\bQ:V\rightarrow \mathbb{S}^{3\times 3}$ is a (non-trivial) motion of $(G,\tilde{\bp})$ if and only if 
$\bQ$ is a (non-trivial) motion of $(G,\lambda \tilde{\bp})$ since
\begin{align*}
&{\rm Trace}\left(((\lambda\tilde{\bp})(v_i)\times (\lambda\tilde{\bp})(v_j))((\lambda\tilde{\bp})(v_i)\times (\lambda\tilde{\bp})(v_j))^{\top} (\bQ(v_i)-\bQ(v_j))\right) \\
&=\lambda_i^2\lambda_j^2{\rm Trace}\left((\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))(\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))^{\top} (\bQ(v_i)-\bQ(v_j))\right).
\end{align*}
Thus projective $C_2^1$-rigidity is invariant by the scaling of each point.

To see the invariance under non-singular linear transformations, choose any non-singular matrix $A\in \mathbb{R}^{3\times 3}$ and let $C_A$ be its cofactor matrix.
% of $A$, that is a $3\times 3$-matrix whose 
%$(i,j)$-th entry is the determinant of  the $2\times 2$-matrix obtained from $A$ by removing the $i$-th row and $j$-th column. 
It is well-known that $(Ax)\times (Ay)=C_A(x\times y)$ for any $x,y\in \mathbb{R}^3$.
Moreover, $C_A$ is non-singular if and only if $A$ is non-singular.
Given $\bQ:V\to  \mathbb{S}^{3\times 3}$
%a (non-trivial) projective $C_2^1$-motion $\bQ$ of $(G,\tilde{\bp})$,
%framework $(G,\tilde{\bp})$ and a nonsingular linear map $A\in \mathbb{R}^{3\times 3}$, 
we let $\bQ_A:V\rightarrow \mathbb{S}^{3\times 3}$ by $\bQ_A(v_i)=C_A^{-\top} \bQ(v_i) C_A^{-1}$, where $C_A^{-\top}=(C_A^{-1})^{\top}$.
Then, for any $v_i, v_j\in V$,
\begin{align*} 
&{\rm Trace}\left((A\tilde{\bp}(v_i)\times A\tilde{\bp}(v_j))(A\tilde{\bp}(v_i)\times A\tilde{\bp}(v_j))^{\top} (\bQ_A(v_i)-\bQ_A(v_j))\right) \\
&= {\rm Trace}\left(C_A(\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))(\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))^{\top} C_A^{\top} C_A^{-\top}(\bQ(v_i)-\bQ(v_j)) C_A^{-1}\right) \\
&= {\rm Trace}\left(C_A\left((\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))(\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))^{\top} (\bQ(v_i)-\bQ(v_j)) \right) C_A^{-1} \right)\\
&= {\rm Trace}\left((\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))(\tilde{\bp}(v_i)\times \tilde{\bp}(v_j))^{\top} (\bQ(v_i)-\bQ(v_j)) \right).
\end{align*} 
Thus $\bQ$ is a (non-trivial) projective $C_2^1$-motion of $(G, \tilde{\bp})$ if and only if $\bQ_A$ is a (non-trivial) projective $C_2^1$-motion of $(G, A\tilde{\bp})$.
%, and the projective $C_2^1$-rigidity of $(G,\tilde p)$ is invariant under the linear transformation defined by $A$.

Hence projective $C_2^1$-rigidity is invariant under both pointwise scaling and  non-singular linear transformations. This implies that the $C_2^1$-rigidity of 2-dimensional frameworks is projectively invariant.
 
\subsection{Proof of Lemma~\ref{lem:projective_bad}}
%We say that a framework $(G,p')$ is {\em quasi-generic} (with respect to $(v_1, \dots, v_4)$) if 
%$p'(v_1)=(1, 0), p'(v_2)=(0, 0), p'(v_3)=(0,1), p'(v_4)=(1,1)$,
%and the set of coordinates at other vertices are algebraically independent.
%(Hence the framework $(G,p')$ in the statement (obtained from a generic framework $(G,p)$ by a projective transformation) is quasi-generic.

%For quasi-generic frameworks one can prove the corresponding claim to Lemma~\ref{lem:bad_pinning} by the same proof:
%\begin{lemma}
%\label{lem:bad_pinning_quasi}
%Let $G=(V,E)$ be a graph, $U=\{v_0,v_1,\dots, v_5\}$ be six vertices, and $b':U\rightarrow \rat[X_0,\dots, Y_5]^3$.
%Suppose that $(G,p')$ has a $b'$-motion at some quasi-generic $p'$, then $(G,p')$ has a $b'$-motion at any quasi-generic $p'$.
%\end{lemma}

\newtheorem*{tlemma}{Lemma~\ref{lem:projective_bad}}

\begin{tlemma}
Let $(G,\bp)$ be a generic framework, $v_0$ be a vertex of degree five with $N_G(v_0)=\{v_1,\dots, v_5\}$, 
and $(G, \bp')$ be a projective image of $(G,\bp)$ such that 
$\bp'(v_1)=(1, 0),\ \bp'(v_2)=(0, 0),\ \bp'(v_3)=(0,1), \text{and } \bp'(v_4)=(1,1)$.
If $(G, \bp')$ has a bad motion at $v_0$, then $(G, \bp)$ has a bad motion at $v_0$.
\end{tlemma}
\begin{proof}
Since $\bp$ is generic,  the set of coordinates of the other vertices of $(G,\bp')$ is algebraically independent over $\rat$.
Suppose that $(G,\bp')$ has a bad motion $\bq'$ at $v_0$, i.e., there is a map $b':\hat N_G(v_0)\rightarrow \rat[X_0,\dots, Y_5]^3$ satisfying (\ref{eq:bad}) and such that $b'_{i}(\bp')=\bq'(v_i)$ for all $v_i\in \hat N_G(v_0)$, where $b'_{i}(\bp')$ denotes the evaluation of $b'(v_i)$ at $p'(\hat N_G(v_0))$.
Suppose also that the inverse of the projective map from $(G,\bp)$ to $(G,\bp')$ is represented by the matrix $A\in \mathbb{R}^{3\times 3}$. Note that each entry of $A$ can be expressed  as a rational function of $\bp(v_1),\dots, \bp(v_4)$ over $\mathbb{Q}$.
We consider the following procedure for converting the motion $\bq'$ to a motion $\bq$ of $(G,\bp)$:
\begin{align*}
\text{$C_2^1$-motion $\bq'$ of $(G,\bp')$} &\overset{\raise0.2ex\hbox{\textcircled{\scriptsize{1}}}}{\longrightarrow} \text{projective $C_2^1$-motion $\bQ'$ of $(G,(\bp')^{\uparrow})$} \\
&\overset{\raise0.2ex\hbox{\textcircled{\scriptsize{2}}}}{\longrightarrow} \text{projective $C_2^1$-motion $\bQ'_A$ of $(G,A(\bp')^{\uparrow})$} \\
&\overset{\raise0.2ex\hbox{\textcircled{\scriptsize{3}}}}{\longrightarrow} \text{projective $C_2^1$-motion $\bQ'_A$ of $(G,\bp^{\uparrow})$} \\
&\overset{\raise0.2ex\hbox{\textcircled{\scriptsize{4}}}}{\longrightarrow} \text{projective $C_2^1$-motion $\bQ$ of $(G,\bp^{\uparrow})$} \\
&\overset{\raise0.2ex\hbox{\textcircled{\scriptsize{5}}}}{\longrightarrow} \text{$C_2^1$-motion $\bq$ of $(G,\bp)$}.
\end{align*}
An explanation of each step in this procedure is given below.
\begin{itemize}
\item[\raise0.2ex\hbox{\textcircled{\scriptsize{1}}}] We construct the projective $C_2^1$-motion $\bQ'$ of $(G,(\bp')^{\uparrow})$ from $\bq'$ as in (\ref{eq:lifting}).
\item[\raise0.2ex\hbox{\textcircled{\scriptsize{2}}}] $\bQ'_A$ is a projective $C_2^1$-motion of $(G,A(\bp')^{\uparrow})$
as explained in Subsection~\ref{subsec:projective_motion}.
\item[\raise0.2ex\hbox{\textcircled{\scriptsize{3}}}] Since $A$ represents the projective transformation from $(G,\bp')$ to $(G,\bp)$, we can scale each point of $(G,A(\bp')^{\uparrow})$ to obtain $(G, \bp^{\uparrow})$. As explained in Subsection~\ref{subsec:projective_motion}, $\bQ'_A$ remains a projective $C_2^1$-motion after this pointwise scaling.
\item[\raise0.2ex\hbox{\textcircled{\scriptsize{4}}}] We eliminate non-zero entries in the right column and the bottom row in $\bQ'_A(v_i)$ by adding (scaled) trivial motions $\bQ_{i,1}^*, \bQ_{i,2}^*, \bQ_{i,3}^*$ for each $v_i\in V$.
This is always possible since $\bQ_{i,1}^*, \bQ_{i,2}^*, \bQ_{i,3}^*$ are of the form, 
$
\begin{pmatrix}
* & * & 0 \\ * & * & 1 \\ 0 & 1 & 0
\end{pmatrix},
\begin{pmatrix}
* & * & 1 \\ * & * & 0 \\ 1 & 0 & 0
\end{pmatrix},
\begin{pmatrix}
* & * & 0 \\ * & * & 0 \\ 0 & 0 & 1
\end{pmatrix}
$
respectively, 
by (\ref{eq:trivial_vertex}). (Note that $z_i=1$ in $\bp^{\uparrow}(v_i)$.)
Since we only add  trivial motions, the resulting $\bQ:V\rightarrow \mathbb{S}^{3\times 3}$ is still a projective $C_2^1$-motion of $(G,\bp^{\uparrow})$.
\item[\raise0.2ex\hbox{\textcircled{\scriptsize{5}}}] We construct the $C_2^1$-motion $\bq$ of $(G,\bp)$ from $\bQ$ as in  (\ref{eq:lifting}).
\end{itemize}
We can compute each $\bq(v_i)$ from $\bq'(v_i)$ by following the above procedure.
For each $v_i\in \hat N_G(v_0)$, the procedure can be performed at a symbolic level starting from $\bq'(v_i)=b_{i}'(\bp')$,
and  returning a map $b:\hat N_G(v_0)\rightarrow \rat(X_0,Y_0,X_1,\dots, Y_5)^3$ with $\bq(v_i)=b_{i}(\bp)$ for each $v_i\in N_G(v_0)$.
By scaling appropriately, we may suppose that $b(v_i)$ is a polynomial map for each $v_i\in N_G(v_0)$. 
Then $\bq$ is a $b$-motion of $(G,\bp)$.
In addition, for all $v_i, v_j\in V$, 
$D(\bp'(v_i),\bp'(v_j))\cdot (b_{i}'(\bp')-b_{j}'(\bp'))=0$ if and only if 
$D(\bp(v_i),\bp(v_j))\cdot (b_{i}(\bp)-b_{j}(\bp))=0$.
This can be verified by checking the corresponding formulae in each step of the above procedure.
Since $p$ is generic, this implies that $b$ satisfies (\ref{eq:bad}), and hence $\bq$ is a bad motion of $(G,\bp)$ at $v_0$.
\end{proof}
 

  



==> cofactor1(da_final)/well_balanced.tex <==
\section{Proof of Theorem~\ref{thm:well-behaved0}}\label{sec:well-behaved}
\subsection{Locally $k$-dof parts}\label{subsec:kdof}\label{subsec:kdof_parts}
Let $G=(V,E)$ be a graph.
A set $X\subseteq V$ is said to be a {\em locally $C_2^1$-rigid part} in $G$ if every edge in $K(X)$ is in ${\rm cl}(E(G))$. 
The set $X$ is said to be a {\em locally $k$-dof part} in $G$ if 
there is a set $F$ of $k$ edges in $K(V)$ such that 
$X$ is a locally $C_2^1$-rigid part in $G+F$, but 
%there is 
no smaller edge set has this property.

Our inductive proof of Theorem~\ref{thm:well-behaved0} requires the following more general  inductive hypothesis. 
\begin{theorem}\label{thm:well-behaved}
Let $(G,\bp)$ be a generic framework and $v_0$ be a vertex of degree five such that 
$\hat{N}_G(v_0)$ is a locally $k$-dof part in $G$ with $k=1$ or $k=2$.
Then $(G,\bp)$ has no bad motion  at $v_0$.
\end{theorem}
%The reader may wonder why we include the case $k=2$ in Theorem \ref{thm:well-behaved}, since our proof of  Theorem~\ref{thm:doubleV} only uses the case $k=1$.
%%Although this deduction only requires the special case of Theorem~\ref{thm:well-behaved} when $k=1$,
%%$\hat{N}_G(v_0)$ is a locally $1$-dof part in $G$,  
%The reason is that
%we need the case $k=2$
%%$\hat{N}_G(v_0)$ is a locally $2$-dof part 
%for our inductive proof of 
%Theorem~\ref{thm:well-behaved}.  
%%We will delay this proof until  Section \ref{sec:well-behaved}.

We give an outline of the proof of Theorem~\ref{thm:well-behaved} in Section~\ref{subsec:outline}, 
and delay the full proof to Section~\ref{subsec:final}.
%We first prove a lemma on locally $k$-dof parts.
%It implies that, if $X$ is a locally $k$-dof part in an arbitrary graph $G$, then we can extend $G$ to a $k$-dof graph in such a way that we preserve the motions of the vertices in $X$.

%\begin{lemma}\label{lem:local1}
%Let $G=(V,E)$ be a graph and $X$ be a locally $k$-dof part in $G$.
%Then  there exists a set of edges $D$ of $K(V)$ such that  $G+D$ is a $k$-dof graph and $X$ is still a locally $k$-dof part in $G+D$.
%Moreover, for any generic framework $(G,\bp)$ and any motion $\bq$ of $(G,\bp)$, $(G+D,\bp)$ has a motion $\bq'$ satisfying $\bq'(v)=\bq(v)$ for all $v\in X$.
%\end{lemma}
%\begin{proof} 
%%We first consider the case when $(G,p)$ is generic. 
%%Let $E'$ be a maximal subset of $E$ which is independent in $\MC^1_2(G,p)$,
%% put $G'=(V,E')$. 
%Let 
%$F$ be a set of $k$ edges in $K(V)$ such that $X$ is a locally $C_2^1$-rigid part in $G+F$, and $D$ be a minimal set of edges in $K(V)$ such that $G+F+D$ is $C^1_2$-rigid. For each $e\in F\cup D$, $G+F+D-e$ is a 1-dof graph and we can choose a non-trivial $C^1_2$-motion $\bq_e$ of  $(G+F+D-e,\bp)$. 
%Then $B_1:=\{\bq_i^*\,:\,1\leq i\leq 6\}\cup
%\{\bq_e\,:\,e\in F\cup D\}$ is a base for $Z(G,\bp)$ and 
%$B_2:=\{\bq_i^*\,:\,1\leq i\leq 6\}\cup
%\{\bq_e\,:\,e\in F\}$ is a base for $Z(G+D,\bp)$,
%where $\{q_i^*:1\leq i\leq 6\}$ is the basis for  $Z_0(G,p)$ given in Section~\ref{subsec:C_2^1-motions}.
% The facts that the motions in $B_1$ are linearly independent and that, for each $e\in F$, we have $D(u,v)\cdot (\bq_e(u)-\bq_e(v))\neq 0$ for some $u,v\in X$ now imply that we must add at least $k$ edges to $G+D$ to make $X$ locally $C_2^1$-rigid. Hence $X$ is a locally $k$-dof part in $G+D$.
%
%Let $\bq$ be a motion of $(G,\bp)$. Since $B_1$ is a base for $Z(G,\bp)$, we have $\bq=\sum_{i=1}^6 \lambda_i \bq_i^*+\sum_{e\in  F\cup D}\mu_e \bq_e$ for some $\lambda_i, \mu_e\in \R$. Since $X$ is a locally $C_2^1$-rigid part of $G+F$, $\bq_e|_X$ is a trivial motion of $(K(X),\bp|_X)$ for all $e\in D$. Hence $\bq_e|_X=\bq_e^*|_X$ for some trivial motion $\bq_e^*$ of $(G,\bp)$. Let $\bq'=\sum_{i=1}^6 \lambda_i \bq_i^*+\sum_{e\in  F}\mu_e \bq_e+\sum_{e\in D}\mu_e \bq_e^*$. Then $\bq'\in Z(G+D,\bp)$.  Since $\bq_e|_X=\bq_e^*|_X$ for $e\in D$, we also have $\bq'|_X=\bq|_X$.
%\end{proof}



\subsection{Outline of the proof of  Theorem~\ref{thm:well-behaved}}
 \label{subsec:outline}
Theorem~\ref{thm:well-behaved} is proved by contradiction. 
We choose a counterexample $(G,\bp)$ with $G=(V,E)$ and $|V|$ as small  as possible and, subject to this condition, $k$ as small as possible. 
The proof proceeds as follows.
\begin{description}
\item[Section~\ref{subsubsec:1}.] The first step  is to prove that $G$ is a 2-dof graph (Claim~\ref{claim:k=2}) and  $G$ has a vertex $u_0$ of degree five with $u_0\notin \hat{N}_G(v_0)$ (Claim~\ref{claim:2d4}).

\item[Sections~\ref{subsubsec:2} and~\ref{subsubsec:3}.] 
Let $G_0=(V_0, E_0)=G-u_0$.
We prove statement (46): ${\rm cl}(E_0)\cap K(N_G(u_0))$ is a star on five vertices.
The proof of (\ref{eq:star}) proceeds as in that of Lemma~\ref{lem:combinatorial}, but to apply a similar argument  we need to prepare several preliminary claims in Section~\ref{subsubsec:2}.

\item[Section~\ref{subsubsec:4}.] The final goal of the proof is to contradict the minimal choice of $(G,\bp)$ by showing that 
  $(G_0+e_1+e_2, \bp|_{V_0})$ is a 2-dof framework with a bad motion at $v_0$   
  for two edges $e_1,e_2\in K(N_G(u_0))$.
To do this we prove the existence of distinct  edges $f_1, f_2\in K(N_G(v_0))$ 
such that $G+f_1+f_2$ is $C_2^1$-rigid and distinct edges  $e_{j,1}, e_{j,2}\in K(N_G(u_0))$ for $j=1,2,3$ such that $(G_0+f_i+e_{j,1}+e_{j,2},\bp)$ has a non-trivial motion $\bq_j^i$ for all $i=1,2$ and $j=1,2,3$ so that   $Z(G_0+f_i, \bp|_{V_0})=Z_0(G_0+f_i, \bp|_{V_0})\oplus \langle \bq_1^i, \bq_2^i, \bq_3^i\rangle$.

\item[Section~\ref{subsubsec:5}.] Let $\bq^i$ be a nontrivial motion of $(G+f_i,\bp)$ for $i=1,2$. 
Since  $G+f_1+f_2$ is $C_2^1$-rigid, we have $Z(G, \bp)=Z_0(G, \bp)\oplus \langle \bq^1, \bq^2 \rangle$.
By $Z(G_0+f_i, \bp|_{V_0})=Z_0(G_0+f_i, \bp|_{V_0})\oplus \langle \bq_1^i, \bq_2^i, \bq_3^i\rangle$, we may suppose (by subtracting a suitable trivial motion) that, for both $i=1,2$,   
$\bq^i|_{V_0}=\sum_{j=1}^3\alpha_j^i\bq_j^i$ for some scalars $\alpha_j^i$.

Since  ${\rm cl}(E_0)\cap K(N_G(u_0))$ forms a star on five vertices,  
we can use the proof technique of Lemma~\ref{lem:motion} to derive an explicit formula for the scalars $\alpha^i_j$.


\item[Section~\ref{subsubsec:6}.] 
The original framework $(G,\bp)$ has a bad motion $\bq_{\rm bad}$ at $v_0$, and its restriction to $V_0$ is a motion of $(G_0, \bp|_{V_0})$.
Since  $Z(G, \bp)=Z_0(G, \bp)\oplus \langle \bq^1, \bq^2 \rangle$, we have 
\[
\bq_{\rm bad}|_{\hat{N}(v_0)}\in \left\langle \sum_{j=1}^3\alpha_j^1\, \bq_j^1|_{\hat{N}(v_0)}, \sum_{j=1}^3\alpha_j^2\, \bq_j^2|_{\hat{N}(v_0)}\right\rangle.
\]
We can use the explicit formulae for the scalars $\alpha_j^i$ derived in Section~\ref{subsubsec:5} and the facts that the entries of $\bq_{\rm bad}|_{\hat{N}(v_0)}$ are contained in $\mathbb{Q}(\bp(V_0))$ and $p(u_0)$ is generic over $\mathbb{Q}(\bp(V_0))$
to show  that
%, for a generic choice of $u_0$, 
 \[
\bq_{\rm bad}|_{\hat{N}(v_0)}\in \left\langle  \bq_j^1|_{\hat{N}(v_0)},  \bq_j^2|_{\hat{N}(v_0)}\right\rangle
\]
for some $j\in \{1,2,3\}$.
Since any linear combination of $\bq_j^1$ and $\bq_j^2$ is a motion of $(G_0+e_{j,1}+e_{j,2},\bp|_{V_0})$,
this implies that  $(G_0+e_{j,1}+e_{j,2},\bp|_{V_0})$ has a bad motion at $v_0$. This contradiction to the minimal choice of $(G,\bp)$ completes the proof.
 \end{description}

\subsection{Proof of Theorem~\ref{thm:well-behaved}}\label{subsec:final}
%We proceed by an inductive argument. 
We assume the statement of Theorem~\ref{thm:well-behaved} is false and choose a counterexample $(G,\bp)$ with $G=(V,E)$ and $v_0\in V$ such that the $G$ is minimal under the lexicographic ordering given by $(|V|,k, \mbox{dof } G,|E|)$.
%and $|V|$ as small  as possible and, subject to this condition, $k$ as small as possible. 
Then $(G,\bp)$ has a bad motion at $v_0$,  
 $d_G(v_0)=5$ 
 %is a vertex of degree five 
 and $\hat{N}_G(v_0)$ is a locally $k$-dof part in $G$.
%We may assume that $k=2$ since, if $k=1$, we can delete edges from $G$ which are not incident to $v_0$ until $\hat N_G(v_0)$ becomes a 2-dof part in $G$, and edge deletion will not destroy the bad motion at $v_0$.
%Our goal is to contradict this choice of $(G,\bp)$ by showing that 
%  $(G-u_0+e_1+e_2,\bp|_{V-u_0})$ is a $k$-dof framework with a bad motion at $v_0$   for some vertex $u_0\in V\setminus \hat N_G(v_0)$ of degree five in $G$ and  some edges $e_1,e_2$ joining the neighbors of $u_0$.


\subsubsection{\boldmath %Existence of a vertex $u_0$ of degree five in $G$ with $u_0\notin \hat{N}_G(v_0)$
Preliminary results on the structure of $G$}\label{subsubsec:1}
The first step of the proof is to show that $G$ is a  ${C}_2^1$-independent, 2-dof graph (statement (\ref{eq:Kv}) and Claims~\ref{claim:Gkdof} and \ref{claim:k=2}) and  $G$ has a vertex $u_0$ of degree five with $u_0\notin \hat{N}_G(v_0)$ (Claim~\ref{claim:2d4}).

%By Lemma~\ref{lem:local1},  we may assume that $(G,\bp)$ is a  $k$-dof framework with $k=1$ or $2$. Choose a base $E'$ of $E$ in ${\cal C}_2^1$ and let $G'$ be the subgraph of $G$ induced by $E'$. Then $(G,\bp)$ and $(G',\bp)$ will have the same space of motions. By this observation, we may also assume that $G$ is $C_2^1$-independent. 

Let $N_G(v_0)=\{v_1,\dots,v_5\}$ and denote for simplicity $K_v=K(N_G(v_0))$.
Since $(G,\bp)$ is a counterexample,  $(G,\bp)$ has a $b$-motion $\bq_{\rm bad}$ for some  $b:\hat{N}_G(v_0)\rightarrow \mathbb{Q}[X_0, Y_0, \dots,Y_5]$ which satisfies (\ref{eq:bad}).
Relabeling $N_G(v_0)$ if necessary, we may suppose that, for all $v_i,v_j\in N_G(v_0)$ with $i<j$,
\begin{equation}\label{eq:star1}
%\text{for $1\leq i<j\leq 5$, 
\text{$D(v_i,v_j)\cdot (\bq_{\rm bad}(v_i)-\bq_{\rm bad}(v_j))=0$ holds if and only if $j=5$.}
\end{equation}
%Let $E_v$ be the set of edges incident to $v$ in $G$.
%Then, by (\ref{eq:star1}), $E_v\cup (





By (\ref{eq:star1}),  $v_iv_j\notin {\rm cl}(E)$ for all $1\leq i<j\leq 4$.
If $v_iv_5\notin {\rm cl}(E)$ for some $1\leq i\leq 4$, then again by (\ref{eq:star1}), $(G+v_iv_5,\bp)$ would be a $(k-1)$-dof framework having the bad motion $\bq_{\rm bad}$, 
which would contradict either the fact that $(G+v_iv_5,\bp)$ is $C^1_2$-rigid (when $k=1$) or the minimality of $k$ (when $k=2$).
%By the proof of Subsection~\ref{subsec:1dof}, this does not hold.
Hence, for all $v_i,v_j\in N_G(v_0)$,
 we have $v_iv_j\in {\rm cl}(E)$ if and only if $j=5$. 
 Then $\cl(E)\cap K_v$ induces a star on five vertices so is ${C}_2^1$-independent. This implies that
%Hence, 
we may choose a base $E'$ of $\cl(E)$ in ${\cal C}_2^1$ with $\cl(E)\cap K_v\subseteq E'$ and $N_E(v_0)=N_{E'}(v_0)$. Let $G'$ be the subgraph of $K(V)$ induced by $E'$. Then $(G,\bp)$ and $(G',\bp)$ have the same space of motions. The minimality of $|E|$ now implies that $|E|=|E'|$ and $G$ is ${C}_2^1$-independent. Replacing $G$ by $G'$ if necessary, we may assume that
\begin{equation}\label{eq:Kv}
\text{$G$ is ${C}_2^1$-independent and $E\cap  K_v={\rm cl}(E)\cap K_v$ is a star on five vertices centred on $v_5$.}
\end{equation}
 
 
% I MERGED EQUATIONS eq:Kv AND eq:2Kv. IF YOU THINK THIS IS A GOOD IDEA THEN WE SHOULD REPLACE ref{eq:2Kv} BY ref{eq:Kv} IN WHAT FOLLOWS.
 
 
% This and (\ref{eq:Kv}) now give
%\begin{equation}\label{eq:Kv}
%\text{$E\cap K_v$  is a star on five vertices centred on $v_5$.}
%\end{equation}
%Then by (\ref{eq:star})
%\begin{equation}\label{eq:2Kv}
%\text{$f\in K_v$ is in ${\rm cl}(E(G))$ if and only if $f\in E(G)$.}
%\end{equation}


 \begin{claim}\label{claim:Gkdof} $G$ is a $k$-dof graph.
 \end{claim}
\begin{proof}
Suppose that $G$ has $k'$ degrees of freedom. We show that  there exists a set of $(k'-k)$ edges $D$ of $K(V-v_0)$ such that  $G+D$ is a $k$-dof graph,  $X:=\hat N_G(v_0)$ is a locally $k$-dof part in $G+D$ and, for any generic framework $(G,\bp)$ and any motion $\bq$ of $(G,\bp)$, $(G+D,\bp)$ has a motion $\bq'$ satisfying $\bq'(v)=\bq(v)$ for all $v\in X$.
%We first consider the case when $(G,p)$ is generic. 
%Let $E'$ be a maximal subset of $E$ which is independent in $\MC^1_2(G,p)$,
% put $G'=(V,E')$. 

Let 
$F$ be a set of $k$ edges in $K(V)$ such that $X$ is a locally $C_2^1$-rigid part in $G+F$, and $D$ be a minimal set of edges in $K(V-v_0)$ such that $G+F+D$ is $C^1_2$-rigid. (Note that $D$ exists since $d_G(v_0)=5$.) For each $e\in F\cup D$, $G+F+D-e$ is a 1-dof graph and we can choose a non-trivial $C^1_2$-motion $\bq_e$ of  $(G+F+D-e,\bp)$. 
Then $B_1:=\{\bq_i^*\,:\,1\leq i\leq 6\}\cup
\{\bq_e\,:\,e\in F\cup D\}$ is a base for $Z(G,\bp)$ and 
$B_2:=\{\bq_i^*\,:\,1\leq i\leq 6\}\cup
\{\bq_e\,:\,e\in F\}$ is a base for $Z(G+D,\bp)$,
where $\{q_i^*:1\leq i\leq 6\}$ is the basis for  $Z_0(G,p)$ given in Section~\ref{subsec:C_2^1-motions}.
 The facts that the motions in $B_1$ are linearly independent and that, for each $e\in F$, we have $D(u,v)\cdot (\bq_e(u)-\bq_e(v))\neq 0$ for some $u,v\in X$ now imply that we must add at least $k$ edges to $G+D$ to make $X$ locally $C_2^1$-rigid. Hence $X$ is a locally $k$-dof part in $G+D$.

Let $\bq$ be a motion of $(G,\bp)$. Since $B_1$ is a base for $Z(G,\bp)$, we have $\bq=\sum_{i=1}^6 \lambda_i \bq_i^*+\sum_{e\in  F\cup D}\mu_e \bq_e$ for some $\lambda_i, \mu_e\in \R$. Since $X$ is a locally $C_2^1$-rigid part of $G+F$, $\bq_e|_X$ is a trivial motion of $(K(X),\bp|_X)$ for all $e\in D$. Hence $\bq_e|_X=\bq_e^*|_X$ for some trivial motion $\bq_e^*$ of $(G,\bp)$. Let $\bq'=\sum_{i=1}^6 \lambda_i \bq_i^*+\sum_{e\in  F}\mu_e \bq_e+\sum_{e\in D}\mu_e \bq_e^*$. Then $\bq'\in Z(G+D,\bp)$.  Since $\bq_e|_X=\bq_e^*|_X$ for $e\in D$, we also have $\bq'|_X=\bq|_X$.

Hence $(G+D,\bp)$ is a counterexample. The minimality of dof $G$ now implies that $k'=k$ and $D=\emptyset$. Hence $G$ is a $k$-dof graph.
\end{proof}








As $G$ is a $k$-dof graph for some $1\leq k\leq 2$, (\ref{eq:Kv}) implies that $|V|\geq 7$.

\begin{claim}\label{claim:well-behaved2}
$G$ has a vertex $u_0$ of degree at most five with $u_0\notin\hat N_G(v_0)$.
\end{claim}
\begin{proof}
Put $G-\hat{N}_G(v_0)=G'=(V',E')$ and let
% $n=|V|, n'=|V\setminus \hat{N}_G(v_0)|$, $E'$ be the set of edges of $G\setminus \hat{N}_G(v_0)$, and 
$F$ be the set of edges of $G$ from $\hat{N}_G(v_0)$ to $V'$.
Since $|V|\geq 7$, we have $|V'|\geq 1$.
By (\ref{eq:Kv}) we have 
\begin{equation}
\label{eq:degree1}
9+|F|+|E'|=|E|=3|V|-6-k=3(|V'|+6)-6-k.
\end{equation}

Suppose every vertex in $V'$ has degree at least six in $G$.
Then 
\begin{equation}
\label{eq:degree3}
\sum_{v'\in V'} d_G(v') = |F|+2|E'|\geq 6|V'|.
\end{equation}
We can now use (\ref{eq:degree1}) and (\ref{eq:degree3}) to deduce that $|E'|\geq 3|V'|-3+k\geq 3|V'|-2$. This contradicts the fact that $G$ is $C_2^1$-independent.
\end{proof}

Let $u_0\in V\setminus \hat{N}_G(v_0)$ be a vertex of degree at most five in $G$,
% and put $N_G(u_0)=\{u_1,\dots, u_{d}\}$.
%, where $d=d_G(u_0)$.
%To simplify notation, we 
$K_u=K(N_G(u_0))$ and put $G-u_0=G_0=(V_0,E_0)$.
%We also denote ${\rm cl}_{\cal C}$ by ${\rm cl}$ in the remainder of this section.
Let ${\cal C}_{n-1}$ be the generic $C_2^1$-cofactor matroid on $K(V_0)$ and let ${\cal C}_{n-1}/{\rm cl}(E_0)$ be the matroid obtained from ${\cal C}_{n-1}$ by contracting ${\rm cl}(E_0)$.


\begin{claim}
\label{claim:2mechanism1}
$F_v:=\{v_1v_2, v_1v_3, v_1v_4\}$ is a base of $K_v\setminus {\rm cl}(E_0)$ in ${\cal C}_{n-1}/{\rm cl}(E_0)$ (and hence
$K_v\setminus {\rm cl}(E_0)$ has rank three in ${\cal C}_{n-1}/{\rm cl}(E_0)$).
\end{claim}
\begin{proof}
By (\ref{eq:Kv}) the subgraph of $G+F_v$
induced by $\hat N_G(v_0)$ is $C_2^1$-rigid. Hence $F_v$ spans $K_v\setminus {\rm cl}(E_0)$ in ${\cal C}_{n-1}/{\rm cl}(E_0)$.
%we have
%
%$G$ has $K_{2,4}^+$ (the complete bipartite graph $K_{2,4}$ plus one edge on the class of two vertices) on $\hat{N}_G(v_0)$.
%The union of $K_{2,4}^+$ and $F_v$ forms a rigid subgraph on $\hat{N}_G(v_0)$, implying that 
%$K_v\setminus {\rm cl}(E_0)\subseteq [F_v]$. Hence $K_v\setminus {\rm cl}(E_0)$ has rank at most three.
Choose
a base $F'$ of $F_v$ in ${\cal C}_{n-1}/{\rm cl}(E_0)$.
% has size at most two.
Since the closure of $F'$ contains $F_v$, 
%which means that 
${\rm cl}(E_0\cup F')$ contains a $C^1_2$-rigid subgraph on $\hat{N}_G(v_0)$.
Hence  $\hat{N}_G(v_0)$ is a locally $t$-dof part in $G_0$ with $t = |F'|$.
Since $\bq_{\rm bad}|_{V_0}$ is a  bad motion of $(G_0, \bp|_{V_0})$  at $v_0$ and $G_0$ is not a counterexample by the minimality of $|V|$, we must have  $t=|F'|=3$ and $F'=F_v$.
\end{proof}

\begin{claim}\label{claim:degree4or5}
$d_G(u_0)\in\{4,5\}$.
\end{claim}

\begin{proof}
If $d_G(u_0)\leq 3$, then $G_0$ would be a $t$-dof graph for some $t\leq 2$. This would contradict Claim~\ref{claim:2mechanism1}.
\end{proof}

\begin{claim}\label{claim:k=2} $k=2$.
\end{claim}
\begin{proof}
Suppose for a contradiction that $k=1$. If $d_G(u_0)=4$ then 
$G_0$ would be a $t$-dof graph for some $t\leq 2$ and this would contradict Claim \ref{claim:2mechanism1}.
%$(G_0,\bp|_{V_0})$ would be a $t$-dof framework for some $t\leq 2$ and $\bq|_{V_0}$ would be a bad motion at $v_0$, contradicitng the minimality of $|V|$. 
Hence we may suppose $d_G(u_0)=5$. Let  $N_G(u_0)=\{u_1,u_2,\ldots,u_5\}$. We will obtain a contradiction by showing that $(G_0+u_iu_j,\bp|_{V_0})$ has a bad motion at $v_0$ for some $1\leq i<j\leq 5$.

Since $G$ is a 1-dof graph, $G_0$ is a 3-dof graph and hence, by Claim \ref{claim:2mechanism1}, $G_0+F_v$ is minimally $C_2^1$-rigid. 
As $G+F_v-u_0u_4-u_0u_5$  is obtained from $G_0+F_v$ by a 0-extension, 
Lemma \ref{lem:cofactor_ind} now implies that $G+F_v-u_0u_4-u_0u_5$ is minimally $C_2^1$-rigid. Since $G$ is $C_2^1$-independent,
$G+F-u_0u_5$ is minimally $C_2^1$-rigid for some $F\subset F_v$ with $|F|=2$. 
We may now deduce that  $G_0+F+u_iu_j$ is minimally $C_2^1$-rigid for some $1\leq i<j\leq 4$, and hence that $G_0+u_iu_j$ is a 2-dof graph. 
It remains to show that there is a bad motion for $(G_0+u_iu_j,\bp|_{V_0})$ at $v_0$. 

Let $G'=G-u_0u_5$. Observe that $G'$ is obtained from $G_0+u_iu_j$ by a 1-extension. 
We shall consider the following non-generic realisation $\bp'$ of $G'$, 
which was used in the proof of \cite[Theorem 10.2.1]{Wsurvey} to show that 
1-extension preserves independence. For $w\in V$, let
\[
\bp'(w)=\begin{cases}
\bp(w) & (\text{if } w\in V\setminus \{u_0\}) \\
\text{the mid-point of the line segment joining $\bp(u_i)$ and $\bp(u_j)$} & (\text{if } w=u_0).
\end{cases}
\]
%and $(G',\bp')$ be the framework obtained by setting $\bp'(w)=\bp(w)$ for $w\in V\setminus \{u_0\}$
%and $\bp'(u_0)$ to be the mid-point of the line segment joining $\bp(u_i)$ and $\bp(u_j)$.
%We can use the  $C_2^1$-rigidity of $G_0+F+u_iu_j$ and the fact 
%that $u_0,u_i, u_j$ are colinear in $(G'+F+u_iu_j,\bp')$, 
%to deduce  that $(G'+F,\bp')$ is $C_2^1$-rigid. 
See Figure~\ref{fig:claim5-3}.
\begin{figure}[h]
\centering
\begin{minipage}{0.45\textwidth}
\centering
\includegraphics[scale=0.6]{1extension1.pdf}
\par(a)
\end{minipage}
\begin{minipage}{0.45\textwidth}
\centering
\includegraphics[scale=0.6]{1extension2.pdf}
\par(b)
\end{minipage}
\caption{(a) $(G',\bp')$ and (b) $(G_0+u_iu_j,\bp_{|V_0})$.}
\label{fig:claim5-3}
\end{figure}

We now use Lemma~\ref{lem:bad_pinning} to show that $(G',\bp')$ has a bad motion at $v_0$. Let
\[
S=\left\{\bar \bp: 
 \text{$(G'+F,\bar \bp)$ is minimally $C_2^1$-rigid and $\bar \bp$ is non-degenerate on $\hat N_{G'}(v_0)$}
%\text{$\bp$ is non-degenerate at $v_a,v_b,v_c$ and $(G+F,\bp)$ is minimally $C_2^1$-rigid}
\right\}.
\]
We may use  the minimal $C_2^1$-rigidity of $(G_0+F+u_iu_j,\bp|_{V_0})$, 
and the fact that $\{u_0,u_i,u_j\}$ is collinear in $(G'+F+u_iu_j,\bp')$ to deduce that 
$(G'+F,\bp')$ is minimally $C_2^1$-rigid, see the proof of \cite[Theorem 10.2.1]{Wsurvey} for more details. 
Since $\bp$ is generic, $\bp'$ is non-degenerate  on $\hat N_{G'}(v_0)$ and hence $\bp'\in S$.
Since $\bq_{\rm bad}$ is a bad motion of $(G',\bp)$  at $v_0$,
% for a generic $\bp$, 
Lemma~\ref{lem:bad_pinning} now implies that $(G',\bp')$ has a bad motion $\bq_{\rm bad}'$ at $v_0$.
%
%Consider the restriction $\bq''$ of $\bq'$ to $V_0$. 
The definition of $\bp'$ implies that 
%and observe that 
$\bq_{\rm bad}'|_{V_0}$ is a motion of $(G_0+u_iu_j,\bp|_{V_0})$.  
%(ADD MORE EXPOSITION.) Moreover, 
Since $(G_0+u_iu_j,\bp|_{V_0})$ is a generic 2-dof framework, $\bq_{\rm bad}'|_{V_0}$ is bad at $v_0$ and this
%the existence of a bad motion at $v_0$ in  $(G_0+e_1+e_2,\bp|_{V_0})$ 
contradicts the minimality of $G$.
\end{proof}

 
Recall that $F_v=\{v_1v_2,v_1v_3,v_1v_4\}$.
We will denote the set of all pairs of edges in $F_v$ by ${F_v\choose 2}$.
%Let $F=\{u_1u_i, u_1u_j\}$ be a pair of edges in $F_v$.
We say that $F\in {F_v\choose 2}$ is {\em good} if $G+F$ is $C_2^1$-independent (and hence minimally $C_2^1$-rigid by $k=2$).
We say that an edge $f\in F_v$ is {\em very good} if $\{f, f'\}$ is good for any $f'\in F_v\setminus \{f\}$.
\begin{claim}\label{claim:good}
There is at least one very good edge in $F_v$. (Equivalently,  at most one pair in ${F_v\choose 2}$ is not good).
\end{claim}
\begin{proof}
Let $F_v=\{f_1, f_2, f_3\}$, and suppose that $\{f_1, f_2\}$ and $\{f_1, f_3\}$ are not good.
By  (\ref{eq:Kv}),
% and (\ref{eq:Kv}), 
 $f_1\notin {\rm cl}(E)$. Hence $G+f_1$ is $C_2^1$-independent and $f_2,f_3\in {\rm cl}(E+f_1)$.
% and  $f_3\in {\rm cl}(E(G)+f_1)$.
This in turn implies that $K_v\subseteq {\rm cl}(E+f_1)$ 
%since the union of $F_v$ and $K_{2,4}^+$ on $\hat{N}(v_0)$ forms a rigid subgraph on $\hat{N}_G(v_0)$.
%This however implies that 
and hence $\hat{N}_G(v_0)$ is a locally 1-dof part in $G$. 
This is a contradiction as $\hat{N}_G(v_0)$ is a locally $k$-dof part with $k=2$ by Claim~\ref{claim:k=2}.
%Hence there is at most one bad pair in $F_v$, and there is a very good edge.
\end{proof}
%
%\begin{claim}\label{claim:mechanism1}
%For $f\in K_v\setminus {\rm cl}(E_0)$, $[f]$ does not contain $K_v\setminus {\rm cl}(E_0)$.
%\end{claim}
%\begin{proof}
%If $[f]$ contains $K_v\setminus {\rm cl}(E_0)$, then $K_v\subset {\rm cl}(E_0+f)$.
%In other words, $N_G(v_0)$ (and $\hat{N}_G(v_0)$) is a locally 1-dof part in $G_0$.
%By induction $(G_0,p)$ has no bad motion at $v_0$.
%Since the restriction of any motion of $(G,p)$ to $V(G)-u_0$ is a motion of $(G_0,p)$, $(G,p)$ has no bad motion at $v_0$, which is a contradiction. 
%\end{proof}

\begin{claim}\label{claim:2mechanism2}
Let $F\in {F_v\choose 2}$ be a good pair.
Then ${\rm cl}(E_0\cup F)\cap K_u$ does not contain a copy of $K_4$.
\end{claim}
\begin{proof}
Suppose that ${\rm cl}(E_0\cup F)\cap K_u$  contains a copy of $K_4$, say on $\{u_1,\dots, u_4\}\subseteq N_G(u_0)$.
Then $u_0u_4\in \cl((E_0\cup F)+u_0u_1+u_0u_2+u_0u_3)$.
% implies $u_0u_4$.
This in turn implies that $E\cup F$ is dependent and  contradicts the hypothesis that $F$ is good.
\end{proof}

\begin{claim}\label{claim:2d4}
$d_G(u_0)=5$.
\end{claim}
\begin{proof}
Assume this is false. Then by Claim \ref{claim:degree4or5}, $d_G(u_0)=4$.
Choose a good pair $F\in {F_v\choose 2}$. 
By Claim~\ref{claim:2mechanism2}, there is an edge $e=u_iu_j\in K_u$ such that 
$G_0+F+u_iu_j$ is $C_2^1$-independent. Since $d_G(u_0)=4$, it is minimally $C_2^1$-rigid.
%By Claim~\ref{claim:mechanism0} we may assume that $f=v_1v_2$.
We can now proceed as in the last paragraph of the proof of Claim \ref{claim:k=2} (with $G'$ replaced by $G$) to show that $(G_0+u_iu_j,\bp|_{V_0})$ has a bad motion at $v_0$ and hence
%Since $(G_0+u_iu_j, \bp)$.
%Let $(G,\bp')$ be a framework obtained by setting $\bp'(w)=\bp(w)$ for $w\in V\setminus \{u_0\}$
%and $\bp'(u_0)$ to be the mid-point of the line segment joining $\bp(u_i)$ and $\bp(u_j)$.
%We can use the  $C_2^1$-rigidity of $G_0+F+u_iu_j$ and the fact 
%that $u_0,u_i, u_j$ are colinear in $(G+F+u_iu_j,\bp')$, 
%to deduce  that $(G+F,\bp')$ is $C_2^1$-rigid. The remainder of the \bproof is similar to that of Claim \ref{claim:mechanism3}. We use Lemma \ref{lem:bad_pinning} to show that  $(G+F,p')$ has a bad motion $\bq'$ at $v_0$, then show that $\bq'|_{V_0}$ is a bad motion of $(G_0+u_iu_j,p|_{V_0})$ at $v_0$.
%
%
%
%The proof is identical to that of Claim~\ref{claim:mechanism3}, but we repeat it form completeness.
%Define
%\[
%S_f=\left\{\bar{p}: 
%\begin{array}{l} \text{$(G+f,\bar{p})$ is independent and $C_2^1$-rigid} \\ 
%\text{$(\bar{y}_i-\bar{y}_j)(\bar{y}_j-\bar{y}_k)(\bar{y}_k-\bar{y}_i)\neq 0$ at some distinct vertices $v_i,v_j,v_k$}
%\end{array}
%\right\}
%\]
%where we denote $\bar{p}(v_i)=(\bar{x}_i, \bar{y}_i)\in \mathbb{R}^2$.
%
%(ADD MORE EXPOSITION.)
%In other words, $p'\in {\cal S}(G+F)$.
%As $(G,p)$ has a bad motion $\bq$ for a generic $p$, 
%Lemma~\ref{lem:bad_pinning} now imply that $(G,p')$ has a bad motion $\bq'$ on $\hat{N}(v_0)$.
%Consider the restriction $\bq'|_{V_0}$ of $q$ to $V_0$,
%and observe that $q'|_{V_0}$ is still a motion of $(G_0+u_iu_j,p|_{V_0})$. (ADD MORE EXPOSITION.)
%Moreover, $q'|_{V_0}$ is still bad on $\hat{N}(v_0)$. 
%Since $(G_0+u_iu_j, p)$ is a generic 2-dof framework, the existence of a bad motion in  $(G_0+u_iu_j,p)$ 
contradict the minimality of $|V|$.
\end{proof}


\subsubsection{\boldmath Preliminary results on $\cl(E_0)\cap K_u$}\label{subsubsec:2}
 Our next goal is to show that 
 ${\rm cl}(E_0)\cap K_u$ is a star on five vertices
 (statement (\ref{eq:star}) in the next section). 
In this section we verify some preliminary claims.
Let $N_G(u_0)=\{u_1,u_2,\ldots,u_5\}$.

%For this, we prepare several preliminary claims.

%Our next two claims can be proved in a similar way to Claims \ref{claim:mechanism3} and \ref{claim:mechanism4}.

%\begin{claim}\label{claim:2mechanism3}
%For $F\in {F_v\choose 2}$, there is no pair of two distinct edges $e_1, e_2$ in $K_u$ such that 
%\begin{itemize}
%\item[(X1)] $e_1$ and $e_2$ do not share an end-vertex, and
%\item[(X2)] $E_0+F+e_1+e_2$ is independent.
%\end{itemize}
%\end{claim}
%\begin{proof}
%The same idea as the proof of Claim~\ref{claim:2d4}.
%Use X-replacement instead.
%\end{proof}

\begin{claim}\label{claim:2mechanism3}
$G_0+F+e_1+e_2$ is $C_2^1$-dependent for all $F\in {F_v\choose 2}$
and all  pairs of non-adjacent edges  $e_1, e_2\in K_u\setminus E_0$.
\end{claim}
\begin{proof}
Suppose that 
%there are two non-adjacent edges $e_1=u_1u_2$ and $e_2=u_3u_4$ such that $G_0+e_1+e_2$ is $C_2^1$-independent.
%By Claim~\ref{claim:1dof1}, $K_v$ contains an edge $f$ such that 
$G_0+F+e_1+e_2$ is $C_2^1$-independent (and hence  minimally $C_2^1$-rigid) for $e_1=u_1u_2$ and $e_2=u_3u_4$. We will contradict the minimality of $G$ by showing that $(G_0+e_1+e_2,\bp|_{V_0})$ has a bad motion at $v_0$. 

%where we denote $\bar{\bp}(v_i)=(\bar{x}_i, \bar{y}_i)\in \mathbb{R}^2$.

Observe that $G+F$ is obtained from $G_0+F+e_1+e_2$ by an X-replacement. 
We shall consider the following non-generic realisation $\bp'$ of $G$, 
which was used in the proof of \cite[Theorem 10.3.1]{Wsurvey} to show that 
X-replacement preserves $C_2^1$-independence. For $w\in V$, let 
$\bp'(w)=\bp(w)$ for $w\in V_0$ and $\bp'(u_0)$ be the point of intersection of the  line  through $\bp(u_1)$ and $\bp(u_2)$, and the line  through $\bp(u_3)$ and $\bp(u_4)$.
%Let $(G,\bp')$ be the framework obtained by setting $\bp'(w)=\bp(w)$ for $w\in V_0$
%and $\bp'(u_0)$ to be the point of intersection of the  line  through $\bp(u_1)$ and $\bp(u_2)$, and the line  through $\bp(u_3)$ and $\bp(u_4)$.
We first use Lemma~\ref{lem:bad_pinning} to show that $(G,\bp')$ has a bad motion at $v_0$. To do this, let
\[
S=\left\{\bar \bp: 
 \text{$(G+F,\bar \bp)$ is minimally $C_2^1$-rigid and $\bar \bp$ is non-degenerate on $\hat N_G(v_0)$}
%\text{$\bp$ is non-degenerate at $v_a,v_b,v_c$ and $(G+F,\bp)$ is minimally $C_2^1$-rigid}
\right\}.
\]
We may use  the minimal $C_2^1$-rigidity of $(G_0+F+e_1+e_2,\bp|_{V_0})$, 
and the fact the vertex sets $\{u_0,u_1,u_2\}$ and $\{u_0,u_3,u_4\}$ are collinear in $(G+F+e_1+e_2,\bp')$ to deduce that 
$(G+F,\bp')$ is minimally $C_2^1$-rigid, see the proof of \cite[Theorem 10.3.1]{Wsurvey} for more details. Since $\bp$ is generic, $\bp'$ is non-degenerate  on $\hat N_G(v_0)$ and hence $\bp'\in S$.
Since $(G,\bp)$ has a bad motion at $v_0$,
% for a generic $\bp$, 
Lemma~\ref{lem:bad_pinning} now implies that $(G,\bp')$ has a bad motion $\bq_{\rm bad}'$ at $v_0$.
%
%Consider the restriction $q''$ of $q'$ to $V_0$. 
The definition of $\bp'$ implies  that 
%and observe that 
$\bq_{\rm bad}'|_{V_0}$ is a motion of $(G_0+e_1+e_2,\bp|_{V_0})$.  
%(ADD MORE EXPOSITION.) Moreover, 
Since $(G_0+e_1+e_2,\bp|_{V_0})$ is a generic 2-dof framework, 
$\bq_{\rm bad}'|_{V_0}$ is bad at $v_0$ and this
%the existence of a bad motion at $v_0$ in  $(G_0+e_1+e_2,\bp|_{V_0})$ 
contradicts the minimality of $G$.
\end{proof}

Claim~\ref{claim:2mechanism3} implies the following.

\begin{claim}\label{smallclaim2}
Let $F\in {F_v\choose 2}$ and let $e=u_iu_j\in K_u\setminus E_0$ such that $G_0+F+e$ is $C_2^1$-independent.
Then ${\rm cl}((E_0\cup F)+e)$ contains a triangle on $N_G(u_0)\setminus \{u_i, u_j\}$.
\end{claim}
\begin{proof}
If not, then we can choose an edge $e'$ on $N_G(u_0)\setminus \{u_i, u_j\}$ such that $G_0+F+e+e'$ is $C_2^1$-independent. 
%Then $F$, $e$ and $e'$ 
%satisfy (X1) and (X2), which 
This contradicts Claim~\ref{claim:2mechanism3}.
\end{proof}


%\begin{claim}\label{claim:2mechanism4}
%For $F\in {F_v\choose 2}$, there is no pair of two distinct edges $e_1, e_2$ in $K_u$ such that 
%\begin{itemize}
%\item[(V1)] $e_1$ and $e_2$ share an endpoint $w$, 
%\item[(V2)] $d_{{\rm cl}(E_0)\cap K_u}(w)=2$, and
%\item[(V3)] $E_0+F+e_1+e_2$ is independent.
%\end{itemize}
%\end{claim}
%\begin{proof}
%The same idea as the proof of Claim~\ref{claim:2d4}.
%Use vertex-spliting instead.
%\end{proof}

\begin{claim}\label{claim:2mechanism4}
$G_0+F+e_1+e_2$ is $C_2^1$-dependent for all $F\in {F_v\choose 2}$
and all pairs of adjacent edges  $e_1, e_2\in K_u\setminus E_0$ whose common end-vertex has degree two in ${\rm cl}(E_0)\cap K_u$.
\end{claim}
\begin{proof}
Suppose that 
%there are two adjacent edges $e_1=u_1u_2$ and $e_2=u_1u_3$ such that their common end-vertex $u_1$ has degree two in $\cl(E_0)\cap K_u$ and $G_0+e_1+e_2$ is $C_2^1$-independent.
%By Claim~\ref{claim:1dof1}, $K_v$ contains an edge $f$ such that 
$G_0+F+e_1+e_2$ is $C^1_2$-independent (and hence minimally $C_2^1$-rigid). Our aim is to contradict the minimality of $G$ by showing that $(G_0+e_1+e_2,\bp|_{V_0})$ has a bad motion at $v_0$. 
%where we denote $\bar{\bp}(v_i)=(\bar{x}_i, \bar{y}_i)\in \mathbb{R}^2$.

Let $u_1$ be the common endvertex of $e_1$ and $e_2$. Since $u_1$ has degree two in $\cl(E_0)\cap K_u$ we may
choose a base $E_0'$ of $\cl(E_0)$ such that
$u_1$ has degree two in $E_0'\cap K_u$ and $v_0$ is incident with the same set of edges in $E_0$ and $E_0'$. Let $G_0'$ be the graph induced by $E_0'$ and $G'$ be the graph obtained from $G_0'$ by adding $u$ and the edges of $G$ incident to $u$. Then $G_0'+F+e_1+e_2$ is $C^1_2$-independent and hence $G'+F$ is $C^1_2$-independent by Lemma \ref{lem:V}. In addition, the fact that $\cl(E_0)=\cl(E_0')$ implies that $(G,p)$ and $(G',p)$ will have the same space of motions. Relabelling $G'$ by $G$, we may assume that  $u_1$  has degree two in $E_0\cap K_u$ and
%Observe that 
$G+F$ is obtained from $G_0+F+e_1+e_2$ by a vertex splitting. 

Consider the realisation $\bp_0$ of $G$ 
%parametrized by $t\in \mathbb{R}$ 
defined by 
$\bp_0(w)=\bp(w)$ for $w\in V_0$
and $\bp_0(u_0)=\bp(u_1)$. 
%(This family was used in the proof of \cite[Theorem 10.2.7]{Wsurvey} to show that 
%vertex-splitting preserves $C_2^1$-independence.) 
%We shall consider the family of realisations $\bp_t$ of $G$ parametrized by $t\in \mathbb{R}$ defined by 
% $\bp_t(w)=\bp(w)$ for $w\in V_0$
%and $\bp_t(u_0)=t\bp(u_0)+(1-t)\bp(u_1)$. (This family was used in the proof of \cite[Theorem 10.2.7]{Wsurvey} to show that 
%vertex-splitting preserves $C_2^1$-independence.) 
Let
${C}^*(G+F,\bp_0)$ be obtained from the cofactor matrix ${C}(G+F,\bp_0)$
by replacing the zero-row indexed by the edge $u_0u_1$ with a row of the form 
$$
%\begin{equation}\label{eq:special_row}
\kbordermatrix{
 & & u_0 & & u_1 & \\
 e=u_0u_1 & 0\dots 0 & D(\bp(u_0),\bp(u_1)) & 0 \dots 0 & -D(\bp(u_0),\bp(u_1)) & 0\dots 0 
}.
%\end{equation}
$$
%Since  $D(\bp_t(u_0),\bp_t(u_1))=t^2 D(\bp(u_0), \bp_t(u_1))$,
%$\ker {C}(G,\bp_t)=\ker {C}^*(G,\bp_t)$ for all $t\neq 0$.
%Moreover, when $t=0$,  
The  argument used to show that vertex splitting  preserves $C^1_2$-independence in  \cite[Theorem 10.2.7]{Wsurvey} implies that ${C}^*(G+F,\bp_0)$ is row independent.
%\footnote{
%Since $(G_0+F+e_1+e_2,\bp|_{V_0})$ is minimally $C_2^1$-rigid, ${C}(G_0+F+e_1+e_2,\bp|_{V_0})$ is row independent. 
%We may now use elementary matrix manipulations and the fact that $\bp_0(u_0)=\bp(u_1)$ 
%to deduce that 
%${C}^*(G+F,\bp_0)$ is row independent,
%% and hence non-singular, 
%see the proof technique in \cite[Theorem 10.2.7]{Wsurvey} for more details.}
If ${C}^*(G+F,\bp_0)$ were the $C^1_2$-cofactor matrix of $(G+F,\bp_0)$ then we could find a bad motion for $(G_0+e_1+e_2,\bp|_{V_0})$ by applying Lemma~\ref{lem:bad_pinning} to $(G+F,\bp_0)$ as in the last paragraph of Claim \ref{claim:2mechanism3}, and this would contradict the minimality of $G$.  Since ${C}^*(G+F,\bp_0)$ is not a $C^1_2$-cofactor matrix 
%of $(G+F,\bp_0)$ 
we instead apply the proof technique of Lemma~\ref{lem:bad_pinning} directly to ${C}^*(G+F,\bp_0)$ to show that
\begin{equation}\label{eq:special}
\mbox{$z|_{V_0}$ is a bad motion of $(G_0+e_1+e_2,\bp|_{V_0})$ for some $z\in \ker {C}^*(G,\bp_0)$}
\end{equation}
and obtain the same contradiction. We give the proof of (\ref{eq:special}) immediately after the proof of  Lemma~\ref{lem:bad_pinning} in Appendix
\ref{sec:bad_pinning}.
%
%Since $\bp$ is generic and $\bP_t|_{V_0}=\bp|_{V_0}$, 
%%$\bp_t$ is non-degenerate on $\hat N_G(V_0)$ and hence 
%we can choose three distinct vertices $v_a,v_b,v_c\in \hat N_G(v_0)$ which have distinct `$y$-coordinates' in $(G,\bp_t)$ for all $t\in \mathbb R$.  
%Let $\tilde{C}(G+F,\bp')$ be the extended $C_2^1$-cofactor matrix for $(G+F,\bp_t)$ with respect to  $v_a,v_b,v_c$, and  let ${C}^*(G+F,\bp_t)$ be obtained from $\tilde{C}(G+F,\bp_t)$
%by replacing the zero-row associated to the edge $u_0u_1$ with a row of the form 
%$$
%%\begin{equation}\label{eq:special_row}
%\kbordermatrix{
% & & u_0 & & u_1 & \\
% e=u_0u_1 & 0\dots 0 & D(\bp(u_0),\bp(u_1)) & 0 \dots 0 & -D(\bp(u_0),\bp(u_1)) & 0\dots 0 
%}.
%%\end{equation}
%$$
%Since  $D(\bp_t(u_0),\bp_t(u_1))=t^2 D(\bp(u_0), \bp_t(u_1))$,
%$\ker  \tilde{C}(G,\bp_t)=\ker {C}^*(G,\bp_t)$ for $t\neq 0$.
%Moreover, when $t=0$,  the  argument for vertex splitting  in \cite{Wsurvey} or \cite{W90vertexsplit} can be applied directly to show that $\tilde{C}(G+F,\bp_0)$ is non-singular\footnote{
%Since $(G_0+F+e_1+e_2,\bp|_{V_0})$ is minimally $C_2^1$-rigid, Lemma~\ref{lem:1dof_motion1}  implies that  $\tilde{C}(G_0+F+e_1+e_2,\bp|_{V_0})$ is row independent. 
%We may now use elementary matrix manipulations and the fact that $\bp_0(u_0)=\bp(u_1)$ 
%to deduce that 
%${C}^*(G+F,\bp_0)$ is row independent and hence non-singular, see the proof technique in \cite{Wsurvey} or \cite{W90vertexsplit} for more details.}.
%
%Observe that $\bp_t$ is generic if $t$ is taken to be generic over $\mathbb{Q}(\bp(V))$\footnote{This can be checked easily by looking at the following simpler situation.
%Suppose $x, y, t$ are three generic numbers over $\mathbb{Q}$, and 
%consider two numbers $x, ty+(1-t)x$. If the two numbers are not generic, then there is a non-zero polynomial $f(a,b)$ such that $f(x, ty+(1-t)x)$ is identically zero as a polynomial in $x, y, t$. Let $d$ be the maximum degree of $f$ in $b$. Then $f(a,b)=g(a)b^d+\text{(lower degree monomials in $b$)}$ for some non-zero polynomial $g$ in $a$. 
%Then $f(x,ty+(1-t)x)=g(x)t^d y^d+\text{(lower degree monomials in $y$)}$, which cannot be identically zero by $g(x)\neq 0$, a contradiction.}.
%By Lemma~\ref{lem:bad_pinning} and the fact that $(G,\bp_1)$ has a bad motion,  $(G, \bp_t)$ has a bad motion for any generic $t$ over $\mathbb{Q}(\bp(V))$. 
%
%Define $S=\{\bp_t: t\in \mathbb{R}, C^*(G+F, \bp_t) \text{ is non-singular}\}$.
%Then $\bp_0\in S$ and $\bp_t\in S$ for any generic $t$ over $\mathbb{Q}(\bp(V))$.
%Also, by $\ker  \tilde{C}(G,\bp_t)=\ker {C}^*(G,\bp_t)$ for $t\neq 0$, 
%$\ker {C}^*(G,\bp_t)$ contains a bad motion of $(G,\bp_t)$ for any generic $t$ over $\mathbb{Q}(\bp(V))$.
%By Lemma A.1 applied to $M(t):={C}^*(G+F,\bp_t)$, 
%$\ker {C}^*(G,\bp_0)$ contains a bad motion $\bq_{\rm bad}'$  of $(G, \bp_0)$.
%The definition of $\bp_0$ implies that $\bq_{\rm bad}'(u_0)=\bq_{\rm bad}'(u_1)$,
%and hence $\bq_{\rm bad}'|_{V_0}$ is a motion of $(G_0+e_1+e_2,\bp|_{V_0})$.  
%Since $(G_0+e_1+e_2,\bp|_{V_0})$ is a generic 2-dof framework, $\bq_{\rm bad}'|_{V_0}$ is bad at $v_0$ and this
%contradicts the minimality of $|V|$.
\end{proof}


%(NOTE: Using Claim~\ref{claim:mechanism3} and Claim~\ref{claim:mechanism4} the next goal is to prove 
%that ${\rm cl}(E_0)\cap K$ forms a star.
%We apply our familiar argument that is used for proving the maximality. 
%However, we have one new issue:
%the previous argument can only show that ${\rm cl}(E_0+f)\cap K$ forms a star for some $f\in K_v$.
%We hence need extra arguments.)



\subsubsection{\boldmath The structure of  ${\rm cl}(E_0)\cap K_u$}\label{subsubsec:3}
%Using the claims above, our next goal is to determine the shape of ${\rm cl}(E_0)\cap K_u$.
%The goal of this subsection is to 
We show that ${\rm cl}(E_0)\cap K_u$ is a star on $N_G(u_0)$.
The proof proceeds as in that of Lemma~\ref{lem:combinatorial}.
%For the 1-dof case this fact straightforwardly follows from Lemma~\ref{lem:combinatorial},
%but the 2-dof case we need to give a stronger statement. 
%Although there are tedious extra case analysis, the proof story essentially follow that of Lemma~\ref{lem:combinatorial}.

 
\begin{claim}\label{claim:2mechanism5}
For every good pair $F\in {F_v\choose 2}$ and every $e\in K_u$ such that $(E_0\cup F)+e$ is independent,
${\rm cl}((E_0\cup F)+e)\cap K_u$ does not contain a $C_2^1$-rigid subgraph spanning $N_G(u_0)$.
\end{claim}
\begin{proof}
Suppose ${\rm cl}((E_0\cup F)+e)\cap K_u$ contains a $C_2^1$-rigid subgraph spanning $N_G(u_0)$. Then 
$K_u\subseteq {\rm cl}((E_0\cup F)+e)$
%, that is, a complete graph on $N(u_0)$.
and hence $u_0u_4, u_0u_5\in \cl((E_0\cup F)+e+u_0u_1+u_0u_2+u_0u_3)$. 
%implies $u_0u_4$ and $u_0u_5$.
%Note that $E(G)=E_0\cup \{u_0u_i: 1\leq i\leq 5\})$.
Since $G$ is $C_2^1$-independent,  we can use two base exchanges to show that $\cl((E_0\cup F)+e+u_0u_1+u_0u_2+u_0u_3)=\cl(E+e')$ for some $e'\in F+e$. Then  $F\subseteq \cl(E+e')$. This contradicts the hypothesis that $F$ is good. 
%However, since $F$ is good, $E+e''$ cannot imply $F$ for any edge $e''$.
%This contradiction proves the claim.  
\end{proof}

For $F\subseteq K(V_0)\setminus \cl(E_0)$, we use
%To simplify notation, we let $K_u=K(N_G(u_0))$, $V_0=V(G)-u_0$, and $E_0=E(G)-u_0$, again.
%Recall also that ${\cal C}/{\rm cl}(E_0)$ denotes the matroid obtained from ${\cal C}$ by contracting ${\rm cl}(E_0)$.
%Since $G_0$ has four degree of freedom, ${\cal C}/{\rm cl}(E_0)$ has rank four.
$[F]$ to denote the closure of $F$ in ${\cal C}_{n-1}/{\rm cl}(E_0)$.
Thus an edge $e\in K(V_0)\setminus {\rm cl}(E_0)$ belongs to $[F]$ if and only if we have $e\in C\subseteq (E_0\cup F)+e$ for some circuit $C$ of ${\cal C}_{n-1}$.
If $F$ is a singleton $\{f\}$, then we denote $[\{f\}]$ by $[f]$.

We say that a set $F\subset F_v$ is {\em influential} if $[F]\cap K_u\neq \emptyset$.
%Similarly, an edge $e\in K_u\setminus {\rm cl}(E_0)$ is said to be {\em influential} if $[e]\cap K_v\neq \emptyset$.
A set $F+e$ with $F\in {F_v\choose 2}$ and $e\in K_u\setminus {\rm cl}(E_0)$ is said to be a {\em stabilizer} if $\hat{N}(v_0)$ is a locally $C_2^1$-rigid part of $G_0+F+e$.
By Claim~\ref{claim:2mechanism1}, $F+e$ is a stabilizer if and only if 
${\rm cl}((E_0\cup F)+e)={\rm cl}(E_0\cup F_v)$.
This fact will be used frequently.

\begin{claim}\label{claim:2mechanism6}
Let $F\in {F_v\choose 2}$ be a good pair and $e\in K_u\setminus {\rm cl}(E_0)$ such that $(E_0\cup F)+e$ is independent.
Suppose that  either $F$ is not influential or $F+e$ is a stabilizer. 
Then ${\rm cl}((E_0\cup F)+e)\cap K_u$ contains no copy of $K_4$.
\end{claim}
\begin{proof}
%By $e\notin [F]$, $E_0+f+e$ is independent.
Without loss of generality, let $e=u_1u_2$.

Suppose that ${\rm cl}((E_0\cup F)+e)\cap K_u$ contains a copy of $K_4$.
If ${\rm cl}((E_0\cup F)+e)\cap K_u$ contains two distinct copies of $K_4$, then
%Since $|V(K_u)|=5$, two copies of $K_4$ would share three vertices and hence 
their union would be a $C^1_2$-rigid subgraph of $K_u$. This would contradict 
%However 
Claim~\ref{claim:2mechanism5}.
% states that there is no rigid subgraph in ${\rm cl}(E_0+f+e)\cap K_u$.
Hence ${\rm cl}((E_0\cup F)+e)\cap K_u$ contains exactly one copy of $K_4$.
We consider two cases depending on the position of the copy of $K_4$.

\medskip
\noindent
\emph{Case 1:} The copy of $K_4$ in ${\rm cl}((E_0\cup F)+e)\cap K_u$ contains $e=u_1u_2$.\\
By symmetry we may assume that this is a $K_4$ on $\{u_1, u_2, u_3, u_4\}$.
By Claim~\ref{smallclaim2}, ${\rm cl}((E_0\cup F)+e)\cap K_u$ also contains $\{u_3u_5, u_4u_5\}$.
Hence, by Claim~\ref{claim:2mechanism5}, 
$$u_1u_5, u_2u_5\notin {\rm cl}((E_0\cup F)+e)\cap K_u.$$

We next show that:
\begin{equation}
\label{eq:2-6-1}
u_1u_3, u_1u_4\in {\rm cl}(E_0\cup F).
\end{equation}
To see this, suppose $u_1u_3\notin {\rm cl}(E_0\cup F)$. Since $u_1u_3\in {\rm cl}((E_0\cup F)+e)$, we have that
$(E_0\cup F)+u_1u_3$ is independent and $u_2u_5\not\in{\rm cl}((E_0\cup F)+e)={\rm cl}((E_0\cup F)+u_1u_3)$.
Hence $(E_0\cup F)+u_1u_3+u_2u_5$ is independent.
%, and $u_1u_3$ and $u_2u_5$ satisfy (X1)(X2). 
This contradicts Claim~\ref{claim:2mechanism3} so  $u_1u_3\in {\rm cl}(E_0\cup F)$. The same argument for $u_1u_4$ gives (\ref{eq:2-6-1}).  

%Next suppose that both $u_1u_3$ and $u_1u_4$ are contained in ${\rm cl}(E_0)$.
Since $(E_0\cup F)+e+u_1u_5$ is independent,
% $e=u_1u_2$ and $u_1u_5$ satisfy (V1)(V2)(V3),
%which contradicts 
Claim~\ref{claim:2mechanism4} implies that $\{u_1u_3,u_1u_4\}\not \subseteq {\rm cl}(E_0)$.
By symmetry, we may suppose that $u_1u_3\notin {\rm cl}(E_0)$, i.e., $u_1u_3\in {\rm cl}((E_0\cup F))\setminus {\rm cl}(E_0)=[F]$.
This implies that $F$ is influential, and hence (by an hypothesis of the claim) $F+e$ is a stabilizer.
Thus, for the unique edge  $f_e\in F_v\setminus F$, we have ${\rm cl}((E_0\cup F)+e)={\rm cl}((E_0\cup F)+f_e)$. 
Since $u_1u_3\in [F]$, we also have 
$u_2u_5\not\in{\rm cl}((E_0\cup F)+e)={\rm cl}((E_0\cup F)+f_e)={\rm cl}(E_0+f+u_1u_3+f_e)$ for some edge $f\in F$. 
%Thus $u_2u_5\notin {\rm cl}(E_0+f+u_1u_3+f_e)$.
%Finally observe that $u_1u_3$ and $u_2u_5$ satisfy (X1)(X2) in $E_0+f+f_e$. 
Then $(E_0\cup \{f,f_e\})+u_1u_3+u_2u_5$ is independent.
This contradicts Claim~\ref{claim:2mechanism3}.
% completes the proof of Case 1.

\medskip
\noindent
\emph{Case 2:} ${\rm cl}((E_0\cup F)+e)\cap K_u$ contains a copy of $K_4$ which avoids  $e=u_1u_2$.\\
By symmetry we may assume that this is a $K_4$ on $\{u_1, u_3, u_4, u_5\}$.
Since there is no other copy of $K_4$ in ${\rm cl}((E_0\cup F)+e)\cap K_u$, 
%without loss of generality 
we may also assume 
$$u_2u_3, u_2u_4\notin {\rm cl}((E_0\cup F)+e).$$

We proceed in a similar way to Case 1. We first show: %(\ref{eq:2-6-2}) and then (\ref{eq:2-6-3}):
\begin{equation}
\label{eq:2-6-2}
\{u_1u_3, u_1u_4, u_1u_5, u_3u_5, u_4u_5\}\subseteq  {\rm cl}(E_0\cup F).
\end{equation}
To see this, suppose $u_1u_3\notin {\rm cl}(E_0\cup F)$. 
Since $u_1u_3\in {\rm cl}((E_0\cup F)+e)$, 
$(E_0\cup F)+u_1u_3$ is independent and  $u_2u_4\notin {\rm cl}((E_0\cup F)+e)={\rm cl}((E_0\cup F)+u_1u_3)$.
Hence $(E_0\cup F)+u_1u_3+u_2u_4$ is independent.
%, and $u_1u_3$ and $u_2u_4$ satisfy (X1)(X2). 
This contradicts Claim~\ref{claim:2mechanism3}.
The same proof can be applied to the other edges to give (\ref{eq:2-6-2}).

We next show that:
\begin{equation}
\label{eq:2-6-3}
\{u_1u_3, u_1u_4, u_1u_5, u_3u_5, u_4u_5\}\subseteq {\rm cl}(E_0).
\end{equation}
To see this, suppose $u_1u_3\notin {\rm cl}(E_0)$. Then $u_1u_3\in {\rm cl}((E_0\cup F))\setminus {\rm cl}(E_0)=[F]$.
This implies that $F$ is influential, and hence (by an hypothesis of the claim) $F+e$ is a stabilizer.
Thus, for the unique edge  $f_e\in F_v\setminus F$, ${\rm cl}((E_0\cup F)+e)={\rm cl}((E_0\cup F)+f_e)$ holds, and we have 
$u_2u_4\not\in {\rm cl}((E_0\cup F)+e)={\rm cl}((E_0\cup F)+f_e)={\rm cl}(E_0+f+u_1u_3+f_e)$ for some edge $f\in F$. 
%Thus $u_2u_4\notin {\rm cl}(E_0+f+u_1u_3+f_e)$.
Hence $(E_0\cup \{f,f_e\})+u_1u_3+u_2u_4$ is independent.
%Finally observe that $u_1u_3$ and $u_2u_4$ satisfy (X1)(X2) in $E_0+f+f_e$, which 
This contradicts Claim~\ref{claim:2mechanism3}.
 The same argument can be applied to the other edges to give  (\ref{eq:2-6-3}).
 
Suppose that $u_3u_4\notin {\rm cl}(E_0 \cup F)$.
As $u_3u_4\in {\rm cl}((E_0\cup F)+e)$, 
$(E_0\cup F)+u_3u_4$ is independent and $u_2u_4\not\in {\rm cl}((E_0\cup F)+e)={\rm cl}((E_0\cup F)+u_3u_4)$.
Hence $(E_0\cup F)+u_3u_4+u_2u_4$ is independent. Since $u_4$ has degree two in ${\rm cl}(E_0)\cap K_u$ by
%and $u_3u_4$ and $u_2u_4$ satisfy (V1)(V2)(V3), where (V2) follows from  
(\ref{eq:2-6-3}),
this contradicts Claim~\ref{claim:2mechanism4}. Hence $u_3u_4\in {\rm cl}(E_0 \cup F)$.
This and (\ref{eq:2-6-2})  imply that ${\rm cl}(E_0 \cup F)$ contains a copy of $K_4$ on 
$\{u_1, u_3, u_4, u_5\}$, contradicting Claim~\ref{claim:2mechanism2}.
%This completes the proof.
\end{proof}



\begin{claim}\label{claim:mechanism7}
Let $F\in {F_v\choose 2}$ be a good pair  and $e=u_iu_j\in K_u$ be such that $(E_0\cup F)+e$ is independent.
Suppose that either $F$ is not influential or $F+e$ is a stabilizer.
Then ${\rm cl}(E_0)$ contains at least two edges of the triangle on $N_G(u_0)\setminus \{u_i, u_j\}$.
\end{claim}
\begin{proof}
Without loss of generality suppose $e=u_1u_2$.
By Claim~\ref{smallclaim2}, ${\rm cl}(E_0+F+e)$ contains a triangle on $\{u_3,u_4,u_5\}$.

We first consider the complete graph on $\{u_1, u_2, u_3, u_4\}$.
By Claim~\ref{claim:2mechanism6} we may assume without loss of generality that 
${\rm cl}((E_0\cup F)+e)$ does not contain $u_1u_3$.
If $u_4u_5\in {\rm cl}((E_0\cup F)+e)\setminus {\rm cl}(E_0\cup F)$, then 
$(E_0\cup F)+u_4u_5$ is independent and  ${\rm cl}((E_0\cup F)+u_4u_5)={\rm cl}((E_0\cup F)+e)$. This would imply that $(E_0\cup F)+u_1u_3+u_4u_5$ is independent and 
%and $u_4u_5$ and $u_1u_3$ satisfy (X1)(X2), which 
contradict Claim~\ref{claim:2mechanism3}.
Hence $u_4u_5\in {\rm cl}(E_0\cup F)$.

Suppose next that $u_4u_5\in {\rm cl}(E_0\cup F)\setminus {\rm cl}(E_0)$, i.e., $u_4u_5\in [F]$.
Then $F$ is influential and so, by the hypothesis, $F+e$ is a stabilizer. 
Hence ${\rm cl}((E_0\cup F)+e)={\rm cl}(E_0\cup F_v)={\rm cl}(E_0+f_1+f_2+u_4u_5)$ holds for some edges  $f_1, f_2\in F_v$.
Then $E_0+f_1+f_2+u_4u_5+u_1u_3$ is independent and we again %satisfy (X1)(X2) in $E_0+f+f_e$, which 
contradict Claim~\ref{claim:2mechanism3}.
Hence $u_4u_5\in {\rm cl}(E_0)$.

By applying the 
%exactly 
same argument to the complete graph on $\{u_1, u_2, u_4, u_5\}$, 
we also get $u_3u_4\in {\rm cl}(E_0)$ or $u_3u_5\in {\rm cl}(E_0)$.
(Specifically, we have $u_3u_4\in {\rm cl}(E_0)$ 
when  $u_1u_5\notin {\rm cl}(E_0+f+e)$ or $u_2u_5\notin {\rm cl}((E_0\cup F)+e)$ holds,
and we have $u_3u_5\in {\rm cl}(E_0)$ when  $u_1u_4\notin {\rm cl}((E_0\cup F)+e)$ or $u_2u_4\notin {\rm cl}((E_0\cup F)+e)$ holds.)
\end{proof}

Recall that an edge $f\in F_v$ is said to be very good if $\{f, f'\}$ is a good pair for every $f'\in F_v\setminus \{f\}$.
In order to apply Claim~\ref{claim:2mechanism5} for a given edge $e\in K_u$, we need to find 
a good pair $F\subset F_v$ such that $(E_0\cup F)+e$ is independent.
The following claim shows we can do this under a mild assumption.

\begin{claim}\label{claim:verygood}
Let  $e\in K_u\setminus {\rm cl}(E_0)$, and suppose that $e\notin [f]$ for some very good edge $f\in F_v$.
Then there is a good pair $F\in {F_v\choose 2}$ such that $(E_0\cup F)+e$ is independent.
\end{claim}
\begin{proof}
Let $F_v=\{f_1, f_2, f_3\}$, and suppose that an edge $e\in K_u\setminus {\rm cl}(E_0)$ satisfies $e\notin [f_1]$ for a very good edge $f_1$.
Since $e\notin [f_1]$, $E_0+f_1+e$ is independent.
As $f_1$ is very good, $\{f_1, f_2\}$ and $\{f_1, f_3\}$ are both good.
Hence, if no good pair has the desired property, then $\{f_2, f_3\}\subset {\rm cl}(E_0+f_1+e)$.
By Claim~\ref{claim:2mechanism1}, $E_0+f_1+f_2$ is independent. Since $f_2\in {\rm cl}(E_0+f_1+e)$,
this gives ${\rm cl}(E_0+f_1+e)={\rm cl}(E_0+f_1+f_2)$,
and $f_3\in {\rm cl}(E_0+f_1+f_2)$ follows since $f_3\in {\rm cl}(E_0+f_1+e)$.
This would contradict Claim~\ref{claim:2mechanism1}. 
\end{proof}

Our next claim extends  Claim~\ref{claim:2mechanism6}.
(Note that $F$ is not required to be a good pair in the following claim.)
\begin{claim}\label{claim:2K4}
${\rm cl}(E_0\cup F_v)\cap K_u$ has no copy of $K_4$ and, for any stabilizer $F+e$, 
${\rm cl}((E_0\cup F)+e)\cap K_u$ has no copy of $K_4$.
%  with $F\in {F_v\choose 2}$ and $e\in K_u$.
\end{claim}
\begin{proof}
Suppose that a copy of $K_4$ exists in ${\rm cl}(E_0\cup F_v)\cap K_u$.
By Claim~\ref{claim:good} we can choose a very good edge $f$ from $F_v$.
Then Claim~\ref{claim:2mechanism2} implies that ${\rm cl}(E_0+f)\cap K_u$ has no copy of $K_4$.
Hence there is an edge $e$ in the copy of $K_4$ with $e\notin {\rm cl}(E_0+f)$.
By Claim~\ref{claim:verygood}, there exists a good pair $F$ of edges in $F_v$ such that $(E_0\cup F)+e$ is independent.
Since $e\in {\rm cl}(E_0\cup F_v)$ and $(E_0\cup F)+e$ is independent,
we have $F_v\subset {\rm cl}(E_0\cup F_v)={\rm cl}((E_0\cup F)+e)$. (Note that $E_0\cup F_v$ is independent by Claim~\ref{claim:2mechanism1}.)
Now $F_v\subset {\rm cl}((E_0\cup F)+e)$ implies that $F+e$ is a stabilizer while 
${\rm cl}(E_0\cup F_v)={\rm cl}((E_0\cup F)+e)$ implies that  ${\rm cl}((E_0\cup F)+e)$ has a copy of $K_4$.
This contradicts Claim~\ref{claim:2mechanism6}, and completes the proof of the first part of the claim.
The second part now follows from the fact that ${\rm cl}(E_0\cup F_v)={\rm cl}((E_0\cup F)+e)$ when $F+e$ is a stabilizer. 
\end{proof}


\begin{claim}\label{claim:2mechanism8}
Let $e=u_iu_j\in K_u\setminus {\rm cl}(E_0)$ be such that $e\notin [f]$ for some very good edge $f\in F_v$.
%Let $F$ be a good pair of edges in $F_v$ and $e=u_iu_j\in K_u$ such that $E_0+F+e$ is independent.
Then ${\rm cl}(E_0)$ contains at least two edges of the triangle on $N_G(u_0)\setminus \{u_i, u_j\}$.
\end{claim}
\begin{proof}
We may assume, without loss of generality, that $e=u_1u_2$.
Suppose that two edges on $\{u_3,u_4,u_5\}$ are missing in ${\rm cl}(E_0)$.
By symmetry, we may assume that $u_3u_5$ and $u_4u_5$ are missing.

We first show that for any  $F\in {F_v\choose 2}$ with $(E_0\cup F)+e$ independent, we have
\begin{equation}\label{eq:2-8-1}
\{u_1u_2, u_1u_3, u_1u_4, u_2u_3, u_2u_4, u_3u_4, u_3u_5, u_4u_5\}\subset {\rm cl}((E_0\cup F)+e).
\end{equation}
To see this, choose an $F\in {F_v\choose 2}$ such that $(E_0\cup F)+e$ is independent.
By Claim~\ref{smallclaim2}, ${\rm cl}((E_0\cup F)+e)$ contains a triangle on $\{u_3,u_4,u_5\}$.
To show that $\{u_1u_2,u_1u_3, u_1u_4, u_2u_3, u_2u_4\}$ is contained in  ${\rm cl}((E_0\cup F)+e)$, we first prove:
\begin{equation}
\label{eq:2-8-2}
\begin{split}
&\text{ if $u_ku_l\notin {\rm cl}(E_0)$ for some  $k,l \in \{3,4,5\}$, then} \\
&\text{${\rm cl}((E_0\cup F)+e)$ contains a triangle on $N(u_0)\setminus \{u_k,u_l\}$.}
\end{split}
\end{equation}
This follows from Claim~\ref{smallclaim2} if $u_ku_l\not\in {\rm cl}(E_0\cup F)$.
Hence we assume $u_ku_l\in {\rm cl}(E_0\cup F)\setminus {\rm cl}(E_0)=[F]$.
By Claim~\ref{claim:2mechanism1}, the unique edge $f'$ in $F_v\setminus F$ satisfies $f'\notin [F]$.
Also, since $u_ku_l\in [F]$, we can choose $f''\in F$ such that  ${\rm cl}(E_0\cup F)={\rm cl}(E_0+f''+u_ku_l)$. Since $f'\notin {\rm cl}(E_0\cup F)$, this implies that $(E_0\cup \{f',f''\})+u_ku_l$ is independent.
If $e=u_1u_2\notin {\rm cl}((E_0\cup \{f',f''\})+u_ku_l)$, then $(E_0\cup \{f',f''\})+u_ku_l+e$ would be independent, which  contradicts Claim \ref{claim:2mechanism3}.
Hence $e\in  {\rm cl}((E_0\cup \{f',f''\})+u_ku_l)$. 
As $[\{f'',u_ku_l\}]=[F]$ and $(E_0\cup F)+e$ is independent, 
we have ${\rm cl}((E_0\cup \{f',f''\})+u_ku_l)={\rm cl}((E_0\cup F)+e)$.
By Claim~\ref{smallclaim2}, ${\rm cl}((E_0\cup \{f',f''\})+u_ku_l)$ contains a triangle on $N_G(u_0)\setminus \{u_k, u_l\}$. This
in turn implies (\ref{eq:2-8-2}), since ${\rm cl}((E_0\cup \{f',f''\})+u_ku_l)={\rm cl}((E_0\cup F)+e)$.

The assumption that $u_3u_5\not\in{\rm cl}(E_0)$ and  (\ref{eq:2-8-2}) imply that 
$u_1u_2, u_1u_4, u_2u_4\in {\rm cl}((E_0\cup F)+e)$. 
Similarly, $u_4u_5\not\in{\rm cl}(E_0)$ and  (\ref{eq:2-8-2}) imply that 
$u_1u_3, u_2u_3\in {\rm cl}((E_0\cup F)+e)$. 
Hence (\ref{eq:2-8-1}) holds.
In particular, ${\rm cl}((E_0\cup F)+e)$ contains a copy of $K_4$, and 
Claim~\ref{claim:2K4} now gives:
\begin{equation}\label{eq:2-8-3}
\mbox{for any $F\in {F_v\choose 2}$ such that $(E_0\cup F)+e$ is independent, $F+e$ is not a stabilizer.}
\end{equation}

Let $F_v=\{f_1,f_2,f_3\}$. 
By Claim~\ref{claim:verygood} there is a good pair $F$ such that $(E_0\cup F)+e$ is independent.
We may assume without loss of generality that  $F=\{f_1, f_2\}$.
We next prove:
\begin{equation}\label{eq:2-8-3-2}
%\text{for any $F\in {F_v\choose 2}$, $(E_0\cup F)+e$ is independent.}
\text{$E_0+f_1+f_3+e$ and $E_0+f_2+f_3+e$ are both independent.}
\end{equation}

%We show that both $E_0+f_1+f_3+e$ and $E_0+f_2+f_3+e$ are independent.
Suppose $E_0+f_1+f_3+e$ is dependent. Then, since $E_0+f_1+e$ is independent,  $f_3\in {\rm cl}(E_0+f_1+e)$.
This in turn implies that $f_1+f_2+e$ is a stabilizer, contradicting (\ref{eq:2-8-3}).
Hence $E_0+f_1+f_3+e$ is independent. A similar argument for 
$E_0+f_2+f_3+e$ 
%is dependent, then as $E_0+f_3+e$ is indepdent we have $f_2\in {\rm cl}(E_0+f_3+e)$.
%This in turn implies that $f_1+f_3+e$ is a stabilizer, cotradicting (\ref{eq:2-8-3}).
%Thus 
gives (\ref{eq:2-8-3-2}).

We next show that:
\begin{equation}\label{eq:2-8-4}
S:=\{u_1u_2, u_1u_3, u_1u_4, u_2u_3, u_2u_4, u_3u_4, u_3u_5, u_4u_5\}\subset {\rm cl}(E_0+e).
\end{equation}
To see this suppose $u_iu_j\notin {\rm cl}(E_0+e)$ for some edge $u_iu_j\in S$.
Since $u_iu_j\in {\rm cl}(E_0+f_1+f_2+e)$ by (\ref{eq:2-8-1})  but $u_iu_j\notin {\rm cl}(E_0+e)$, 
we may assume without loss of generality that ${\rm cl}(E_0+f_1+f_2+e)={\rm cl}(E_0+f_1+e+u_iu_j)$.
Then $f_2\in {\rm cl}(E_0+f_1+e+u_iu_j)$.
We also have $u_iu_j\in {\rm cl}(E_0+f_1+f_3+e)$ by (\ref{eq:2-8-1}) and (\ref{eq:2-8-3-2}).
This gives ${\rm cl}(E_0+f_1+f_3+e)={\rm cl}(E_0+f_1+f_3+e+u_iu_j)$.
Since $f_2\in {\rm cl}(E_0+f_1+f_3+e+u_iu_j)$, this in turn implies that $f_1+f_3+e$ is a stabilizer, contradicting (\ref{eq:2-8-3}).
Thus (\ref{eq:2-8-4}) holds.

%By Claim~\ref{claim:verygood} there is a good pair $F\subseteq F_v$ such that $E_0+F+e$ is independent.
Since $F$ is a good pair,
Claim~\ref{claim:2mechanism5} implies that ${\rm cl}((E_0\cup F)+e)\cap K_u$ cannot contain a $C_2^1$-rigid graph which spans $N_G(u_0)$. 
Combining this fact with (\ref{eq:2-8-4}), we have 
\begin{equation}\label{eq:2-8-5}
{\rm cl}((E_0\cup F)+e)\cap K_u= {\rm cl}(E_0+e)\cap K_u=S.
%\{u_1u_2, u_1u_3, u_1u_4, u_2u_3, u_2u_4, u_3u_4, u_3u_5, u_4u_5\}.
\end{equation}
In particular, $u_1u_5$ and $u_2u_5$ are missing in ${\rm cl}((E_0\cup F)+e)$.
If $u_1u_3, u_1u_4\in {\rm cl}(E_0)$, then the fact that
$(E_0\cup F)+e+u_1u_5$ is independent would 
%$e$ and $u_1u_5$ satisfy (V1)(V2)(V3) in $E_0\cup F$, 
contradict Claim~\ref{claim:2mechanism4}.
Thus we may assume $u_1u_3\notin {\rm cl}(E_0)$.
Then $u_1u_3\in [e]$ by (\ref{eq:2-8-5}).
This implies that ${\rm cl}((E_0\cup F)+e)={\rm cl}((E_0\cup F)+u_1u_3)$, and hence $(E_0\cup F)+u_1u_3+u_2u_5$ is independent as $u_2u_5\notin {\rm cl}((E_0\cup F)+e)$.
%and $u_1u_3$ and $u_2u_5$ satisfy (X1)(X2) in $E_0\cup F$, 
This  contradicts Claim~\ref{claim:2mechanism3}.
%This completes the proof.
\end{proof}

\begin{claim}\label{claim:2mechanism9}
For all $i$ with $1\leq i\leq 5$, $d_{{\rm cl}(E_0)\cap K_u}(u_i)\geq 1$.
And if $d_{{\rm cl}(E_0)\cap K_u}(u_i)=1$, then the vertex $u_j$ adjacent to $u_i$ in ${\rm cl}(E_0)\cap K_u$ satisfies 
$d_{{\rm cl}(E_0)\cap K_u}(u_j)=4$.
\end{claim}
\begin{proof}
Let $F_v=\{f_1, f_2, f_3\}$. By Claim~\ref{claim:good}, we may assume that $f_1$ is a very good edge.

 Suppose that $d_{{\rm cl}(E_0)\cap K_u}(u_5)=0$.
 By Claim~\ref{claim:2mechanism2}, ${\rm cl}(E_0+f_1)\cap K_u$ has no copy of $K_4$.
 Hence we can choose an edge $e$ on  $\{u_1,u_2,u_3,u_4\}$ such that $e\notin {\rm cl}(E_0+f_1)$.
We can then apply Claim~\ref{claim:2mechanism8} to $e$ to deduce that
 ${\rm cl}(E_0)$ has an edge incident to $u_5$. This gives a contradiction and completes the proof of first part of the claim.

 To prove the second part we assume that $d_{{\rm cl}(E_0)\cap K_u}(u_5)=1$ and
% .  We may assume without loss of generality 
 that $u_5$ is adjacent to $u_1$ in ${\rm cl}(E_0)$. We will show that 
 $u_1u_2,u_1u_3,u_1u_4\in {\rm cl}(E_0)$.
 %and that 
 Suppose,  for a contradiction, that 
 $u_1u_2\not\in {\rm cl}(E_0)$.
 If $u_1u_2\notin [f_1]$, then Claim~\ref{claim:2mechanism8} would imply that $u_5$ has degree at least two in ${\rm cl}(E_0)$, a contradiction.
 Hence $u_1u_2\in [f_1]$ which gives $u_1u_2\in {\rm cl}(E_0+f_1)$. 
 %By the same reasoning, 
 We aslo have $u_1u_3, u_1u_4\in {\rm cl}(E_0+f_1)$ since, if $u_1u_i\not\in {\rm cl}(E_0)$ for some $i=1,2$, then we can use the same argument as for $u_1u_2$ to deduce that $u_1u_i\in [f_1]$.
 The facts that $u_1u_2\in [f_1]$ and  $F_v$ is independent in ${\cal C}_{n-1}/{\rm cl}(E_0)$ imply that  $E_0+f_2+f_3+u_1u_2$ is independent and  ${\rm cl}(E_0\cup F_v)={\rm cl}(E_0+f_2+f_3+u_1u_2)$.
Since $u_3u_4, u_4u_5, u_5u_3\in {\rm cl}(E_0+f_2+f_3+u_1u_2)$  by Claim~\ref{smallclaim2},
${\rm cl}(E_0\cup F_v)$ contains a copy of $K_4$ on $\{u_1,u_3,u_4,u_5\}$.
This contradicts Claim~\ref{claim:2K4}.
 \end{proof}

 \begin{claim}
 \label{claim:2mechanism10}
 ${\rm cl}(E_0)\cap K_u$ is cycle free.
 \end{claim}
 \begin{proof}
We choose $F\in {F_v\choose 2}$ and $e\in K_u$ as follows.
\\[-6mm]
\begin{itemize}
\item When $[F_v]\cap K_u\neq \emptyset$, we first choose $e\in [F_v]\cap K_u$
and then choose $F$ such that $F+e$ is independent. Such a choice of $F$ is possible by Claim \ref{claim:2mechanism1} and will ensure that $F+e$ is a stabilizer.
\\[-4mm]
\item
When  $[F_v]\cap K_u= \emptyset$, we first choose $F$ to be good and then choose $e\in K_u\setminus {\rm cl}(E_0)$. This choice will ensure that  $(E_0\cup F)+e$ is independent and $F$ is good but not influential.
\\[-4mm]
\end{itemize}
This choice of $F$ and $e$  and Claims~\ref{claim:2mechanism6} and \ref{claim:2K4} imply  that 
\begin{equation}\label{eq:noK4}
\text{${\rm cl}((E_0\cup F)+e)\cap K_u$ contains no copy of $K_4$.}
\end{equation}
  
 Suppose that ${\rm cl}(E_0)\cap K_u$ contains a cycle of length five, say 
 %$\{u_iu_{i+1 ({\rm mod } 5)}: 1\leq i\leq 5\}$.
 $u_1u_2u_3u_4u_5u_1$.
 We may assume  without loss of generality that $e=u_1u_3$.
 By (\ref{eq:noK4}), either
 $u_2u_4\notin {\rm cl}((E_0\cup F)+e)$ or $u_1u_4\notin {\rm cl}((E_0\cup F)+e)$ holds. Both alternatives lead to a  contradiction by applying 
 Claim~\ref{claim:2mechanism3}
and \ref{claim:2mechanism4}, respectively. 
 
 
 Suppose that ${\rm cl}(E_0)\cap K_u$ contains a cycle of length four, say 
 %$\{u_iu_{i+1 ({\rm mod } 4)}: 1\leq i\leq 4\}$.
$u_1u_2u_3u_4u_1$. 
If $e$ is a chord of the cycle, then the other chord is missing in ${\rm cl}((E_0\cup F)+e)$ by (\ref{eq:noK4}),
 and we can apply Claim~\ref{claim:2mechanism3} to get a contradiction.
 Hence $e$ is not a chord of the cycle.
Since  at least one diagonal of the cycle is missing in ${\rm cl}((E_0\cup F)+e)$ by (\ref{eq:noK4}),  we can again apply Claim~\ref{claim:2mechanism3} or Claim~\ref{claim:2mechanism4} to get a contradiction.


It remains to consider the case when  ${\rm cl}(E_0)\cap K_u$ contains a cycle of length three, say 
%on $\{u_1, u_2, u_3\}$.
$u_1u_2u_3u_1$.
Claim~\ref{claim:2mechanism9} and (\ref{eq:noK4}) tell us that there is exactly one edge in ${\rm cl}(E_0)\cap K_u$ from each of $u_4, u_5$ to $\{u_1, u_2, u_3\}$, and that both of these edges have a common end-vertex, say $u_1$.
By symmetry, we may assume that either $e=u_2u_4$ or $e=u_4u_5$ holds.
If $e=u_2u_4$, then $u_3u_5\in {\rm cl}((E_0\cup F)+e)$ by Claim~\ref{smallclaim2},
and $u_2u_5\notin {\rm cl}((E_0\cup F)+e)$ by (\ref{eq:noK4}).
Then $(E_0\cup F)+e+u_2u_5$ is independent, 
%satisfies (V1)(V2)(V3), 
contradicting Claim~\ref{claim:2mechanism4}.
Hence $e=u_4u_5$. 

Recall our selection of  $e$ at the beginning of the proof.
If $[F_v]\cap K_u=\emptyset$, then $e$ could have been chosen to be any edge in $K_u\setminus {\rm cl}(E_0)$. In particular we could choose $e=u_2u_4$, and obtain the contradiction in the previous paragraph.
Hence  $[F_v]\cap K_u\neq \emptyset$. Since $e$ can be any edge in $[F_v]\cap K_u$, we must have $[F_v]\cap K_u=\{u_4u_5\}$.

Choose any good pair $F'\in {F_v\choose 2}$, and consider $F'+u_2u_4$. 
Since $[F_v]\cap K_u=\{u_4u_5\}$, $F'+u_2u_4$ is independent.
Hence by Claims~\ref{claim:2mechanism3} and
% (X-replacement) and Claim~
\ref{claim:2mechanism4},
% (vertex-splitting), 
$u_2u_5, u_3u_5\in {\rm cl}((E_0\cup F')+u_2u_4)$.
Since $u_3u_5\notin {\rm cl}(E_0\cup F')$, we have ${\rm cl}((E_0\cup F')+u_2u_4)={\rm cl}((E_0\cup F')+u_3u_5)$.
Then by Claim~\ref{claim:2mechanism4},
%(vertex-splitting), 
${\rm cl}((E_0\cup F')+u_3u_5)$ also contains $u_3u_4$.
Summarizing, we have shown that ${\rm cl}((E_0\cup F')+u_2u_4)$ contains a $C_2^1$-rigid graph which spans $N_G(u_0)$. This contradicts Claim~\ref{claim:2mechanism5}.
\end{proof}

Combining Claim~\ref{claim:2mechanism9} and \ref{claim:2mechanism10}, we conclude that 
${\rm cl}(E_0)\cap K_u$ is a star on five vertices.
Without loss of generality, we may assume that 
\begin{equation}
\label{eq:star}
\text{${\rm cl}(E_0)\cap K_u$ is a star centered at $u_5$.}
\end{equation}

\subsubsection{\boldmath Further structural properties of $G$}\label{subsubsec:4}


%As in section \ref{sec:motion1dof}, 
We 
let $K$ be the edge set of the complete graph on $\{u_1, u_2, u_3, u_4\}$ and, 
for each edge $e\in K$,  we refer to the unique edge of $K$ which is not adjacent to $e$ as the {\em opposite edge to} $e$ and denote it by $\tilde{e}$. For $e\in K$ and $f\in F_v$, we say that   {\em $e$ is $f$-coupled} if $\tilde e\in [\{e,f\}]$.


\begin{claim}\label{claim:2opposite1}
Let $e\in [F_v]\cap K$. Then $\tilde{e}\in [F_v]$. 
\end{claim}
\begin{proof}
Since $e\in  [F_v]$, $e\notin {\rm cl}(E_0)$ and we can choose $F\in {F_v\choose 2}$ such that $(E_0\cup F)+e$ is independent. Together  with 
%${\rm cl}(E_0\cup F_v)={\rm cl}((E_0\cup F)+e)$. By 
Claim~\ref{smallclaim2}, this implies that $\tilde{e}\in {\rm cl}((E_0\cup F)+e)={\rm cl}(E_0\cup F_v)$. Since $\tilde e\not\in \cl(E_0)$ by (\ref{eq:star}), we have $\tilde e\in [F_v]$.
\end{proof}

\begin{claim}\label{claim:2opposite2}
Suppose $e$ is not $f$-coupled for some $e\in K$ and $f\in F_v$.
Then $e, \tilde{e}\in [F_v]$.
\end{claim}
\begin{proof}
Let $F_v=\{f_1, f_2, f_3\}$ where $f=f_1$.

Suppose $e\notin [F_v]$.
Then, by Lemma~\ref{claim:2mechanism1}, $E_0+f_i+f_j+e$ is independent for all distinct $i,j \in \{1,2,3\}$.
Hence, for each $i\in\{2,3\}$, Claim~\ref{smallclaim2} implies $\tilde{e}\in [\{f_1,f_i,e\}]$.
Since $\tilde{e}\notin [\{f_1,e\}]$ (as $e$ is not $f_1$-coupled), we have $f_i\in {\rm cl}(E_0+f_1+f_i+e)={\rm cl}(E_0+f_1+e+\tilde{e})$ for $i\in \{2,3\}$.
As $E_0\cup F_v$ is independent, this in turn implies that ${\rm cl}(E_0+f_1+e+\tilde{e})={\rm cl}(E_0\cup F_v)$, and
contradicts our initial assumption that $e\notin [F_v]$.

Hence $e\in [F_v]$.  Claim~\ref{claim:2opposite1} now implies that $\tilde{e}\in [F_v]$.
\end{proof}

\begin{claim}\label{claim:Fv}
Suppose $E_0+f+e+e'$ is independent for some 
$f\in F_v$ and distinct $e, e'\in [F_v]\cap K$. Then 
${\rm cl}(E_0+f+e+e')={\rm cl}(E_0+K_v)$.
\end{claim}
\begin{proof}
Recall that, by Claim~\ref{claim:2mechanism1},  $F_v$ is a base of $K_v\setminus {\rm cl}(E_0)$ in ${\cal C}_{n-1}/{\rm cl}(E_0)$.
%, which as rank three. 
Since $E_0+f+e+e'$ is independent and $f,e,e'\in [F_v]$, $\{f,e,e'\}$ %is an independent set of size three in ${\cal C}_{n-1}/{\rm cl}(E_0)$, which 
spans $F_v$ in ${\cal C}_{n-1}/{\rm cl}(E_0)$.
% by $e, e'\in [F_v]\cap K$ and $f\in F_v$.
This implies that ${\rm cl}(E_0+f+e+e')={\rm cl}(E_0\cup F_v)={\rm cl}(E_0\cup K_v)$.
\end{proof}

We will assume henceforth that  $F
=\{f_1, f_2\}
\in {F_v \choose 2}$ is a good pair. This is justified by Claim \ref{claim:good}.
We next categorize $G_0+f_i$ according to the properties of ${\rm cl}(E_0+f_i)$. We say that $G_0+f_i$  is:
\begin{description}
\item[Type 0] 
%$G_0+f_i$ is said to be {\em type 0} 
if $K_u\subseteq {\rm cl}(E_0+f_i+e_1+e_2)$ for some two edges $e_1, e_2\in K_u$.
%(In this case, $K_u\subseteq {\rm cl}(E(G)+f_i)$ holds, and a non-trivial motion of $(G+f_i, p)$ on $V_0$ is determined by $p(V_0)$. So it is an easy case...)

\item[Type A] 
%$G_0+f_i$ is said to be {\em type A} 
if the graphs
%there are three graphs $A_1^i, A_2^i, A_3^i$ having the following properties:
$A_1^i :=G_0+f_i+u_1u_2+u_2u_3$, $A_2^i:=G_0+f_i+u_2u_3+u_3u_1$, and $A_3^i:=G_0+f_i+u_3u_1+u_1u_2$ have the following properties.
%have the following properties: 
\begin{itemize}
\item[(1)] Each $A_j^i$ is $C^1_2$-independent and has one degree of freedom. 
\item[(2)] Each ${\rm cl}(A_j^i)\cap K_u$ is as shown in Figure~\ref{fig:A}.
\item[(3)] For some (or equivalently, every) non-trivial motion $\bq_j^i$ of $(A_j^i, \bp)$, $1\leq j\leq 3$, we have $Z(G_0+f_i, \bp)=Z_0(G_0+f_i,\bp)\oplus \langle \bq_1^i, \bq_2^i, \bq_3^i\rangle$. 
\end{itemize}

\item[Type B] 
%$G_0+f_i$ is said to be {\em type B} 
if the graphs
$B_1^i:=G_0+f_i+u_1u_2+u_3u_4$,  $B_2^i:=G_0+f_i+u_2u_3+u_3u_1$, and $B_3^i:=G_0+f_i+u_3u_1+u_1u_2$ have the following properties.
\begin{itemize}
\item[(1)] Each $B_j^i$ is $C^1_2$-independent and has one degree of freedom.  
\item[(2)] Each ${\rm cl}(B_j^i)\cap K_u$ is as shown in Figure~\ref{fig:B}.
\item[(3)] For some (or equivalently, every) non-trivial motion $\bq_j^i$ of $(B_j^i, \bp)$, $1\leq j\leq 3$, we have $Z(G_0+f_i, \bp)=Z_0(G_0+f_i,\bp)\oplus \langle \bq_1^i, \bq_2^i, \bq_3^i\rangle$.
\item[(4)] $K_v\subset {\rm cl}(B_1^i)$ and $\{u_1u_2,u_3u_4\}\subset [F_v]$.
\end{itemize}

\item[Type C] 
%$G_0+f_i$ is said to be {\em type C} 
if  the graphs 
$C_1^i:=G_0+f_i+u_1u_2+u_2u_3$, $C_2^i:=G_0+f_i+u_2u_3+u_3u_1$, and $C_3^i:=G_0+f_i+u_3u_1+u_1u_2$ have the following properties.
\begin{itemize}
\item[(1)] Each $C_j^i$ is $C^1_2$-independent and has one degree of freedom. 
\item[(2)] Each ${\rm cl}(C_j^i)\cap K_u$ is as  shown in Figure~\ref{fig:C}.
\item[(3)] For some (or equivalently, every) non-trivial motion $\bq_j^i$ of $(C_j^i, \bp)$, $1\leq j\leq 3$, we have $Z(G_0+f_i, \bp)=Z_0(G_0+f_i,\bp)\oplus \langle \bq_1^i, \bq_2^i, \bq_3^i\rangle$.
\item[(4)] $K_v\subset {\rm cl}(C_1^i)$.
\end{itemize}

\item[Type D] 
%$G_0+f_i$ is said to be {\em type D} 
if  the graphs
$D_1^i:=G_0+f_i+u_1u_2+u_3u_4$,  $D_2^i:=G_0+f_i+u_1u_3+u_3u_4$, and $D_3^i:=G_0+f_i+u_3u_1+u_1u_2$ have the following properties.
\begin{itemize}
\item[(1)] Each $D_j^i$ is $C^1_2$-independent and has one degree of freedom. 
\item[(2)] Each ${\rm cl}(D_j^i)\cap K_u$ is as  shown in Figure~\ref{fig:D}.
\item[(3)] For some (or equivalently, every) non-trivial motion $\bq_j^i$ of $(D_j^i, \bp)$, $1\leq j\leq 3$, we have $Z(G_0+f_i, \bp)=Z_0(G_0+f_i,\bp)\oplus \langle \bq_1^i, \bq_2^i, \bq_3^i\rangle$.
\item[(4)] $K_v\subset {\rm cl}(D_1^i)$.
\end{itemize}

\end{description}
In addition, for X,Y in $\{$A,B,C,D$\}$, we say that $(G_0,F)$ is {\em type} XY if $G_0+f_1$ is type X and $G_0+f_2$ is type Y.

\begin{figure}[p]
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{A1.pdf}
\par
(i) ${\rm cl}(A_1^i)\cap K_u$
\end{minipage}
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{A2.pdf}
\par
(ii) ${\rm cl}(A_2^i)\cap K_u$
\end{minipage}
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{A3.pdf}
\par
(iii) ${\rm cl}(A_3^i)\cap K_u$
\end{minipage}
\caption{${\rm cl}(A_j^i)\cap K_u$ for $1\leq j\leq 3$.}
\label{fig:A}
\end{figure}

\begin{figure}[p]
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{B1.pdf}
\par
(i) ${\rm cl}(B_1^i)\cap K_u$
\end{minipage}
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{B2.pdf}
\par
(ii) ${\rm cl}(B_2^i)\cap K_u$
\end{minipage}
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{B3.pdf}
\par
(iii) ${\rm cl}(B_3^i)\cap K_u$
\end{minipage}
\caption{${\rm cl}(B_j^i)\cap K_u$ for $1\leq j\leq 3$.}
\label{fig:B}
\end{figure}

\begin{figure}[p]
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{C1.pdf}
\par
(i) ${\rm cl}(C_1^i)\cap K_u$
\end{minipage}
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{C2.pdf}
\par
(ii) ${\rm cl}(C_2^i)\cap K_u$
\end{minipage}
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{C3.pdf}
\par
(iii) ${\rm cl}(C_3^i)\cap K_u$
\end{minipage}
\caption{${\rm cl}(C_j^i)\cap K_u$ for $1\leq j\leq 3$ (at most one dotted edge may exist in each graph).}
\label{fig:C}
\end{figure}

\begin{figure}[p]
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{D1.pdf}
\par
(i) ${\rm cl}(D_1^i)\cap K_u$
\end{minipage}
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{D2.pdf}
\par
(ii) ${\rm cl}(D_2^i)\cap K_u$
\end{minipage}
\begin{minipage}{0.32\textwidth}
\centering
\includegraphics[scale=0.8]{D3.pdf}
\par
(iii) ${\rm cl}(D_3^i)\cap K_u$
\end{minipage}
\caption{${\rm cl}(D_j^i)\cap K_u$ for $1\leq j\leq 3$ (at most one dotted edge may exist in each graph).}
\label{fig:D}
\end{figure}

\begin{claim}\label{claim:types}
Suppose $F=\{f_1,f_2\}$ is a good pair and $f_i\in F$. Then, 
up to a possible relabeling of 
%the indecies of 
$u_1,u_2,u_3, u_4$, 
$G_0+f_i$ is type 0, A, B, C, or D, and, if neither $G_0+f_1$ nor $G_0+f_2$ is type 0, then $(G_0,F)$ is type AA, AB, BA, BB, CC or DD.
\end{claim}
\begin{proof}
Since the claim holds trivially if $G_0+f_i$ is type 0 for some $i\in \{1,2\}$, we may assume that this is not the case. 
Recall that $K$ is the edge set of the complete graph on $\{u_1,u_2,u_3, u_4\}$. 
By Claim~\ref{claim:2opposite1}, $|[F_v]\cap K|$ is even.
We will consider the different alternatives for $|[F_v]\cap K|$. 

Suppose that $|[F_v]\cap K|=6$.
Since $F$ is a good pair, Claim \ref{claim:2mechanism2} implies there is an edge $e\in K$ such that $(E_0\cup F)+e$ is independent. Since  $e\in K=[F_v]\cap K$, this and \eqref{eq:star} give  $K_u\subset {\rm cl}(E_0\cup F_v)={\rm cl}((E_0\cup F)+e)$. %Since $F$ is a good pair, there is an edge $e\in K$ such that $(E_0\cup F)+e$ is independent by Claim~\ref{claim:2mechanism2}, and  $K_u\subset {\rm cl}(E_0\cup F_v)={\rm cl}((E_0\cup F)+e)$ now follows since  $e\in K=[F_v]\cap K$.
This contradicts Claim~\ref{claim:2mechanism5}.
Hence $|[F_v]\cap K|\in \{0, 2, 4\}$, and we split the proof accordingly.

\medskip

\noindent
\emph{Case 1:} $|[F_v]\cap K|=0$. 
We show $G_0+f_i$ is type A and hence $(G_0,F)$ is type AA.
%, assuming it is not type 0.
Note that Claim~\ref{claim:2opposite2} and the fact that $[F_v]\cap K=\emptyset$ imply that 
$\tilde{e}\in [\{f_i, e\}]$ for all $e\in K$, so every $e\in K$ is $f_i$-coupled.

Let $H^i:=G_0+f_i+u_1u_2+u_2u_3+u_3u_1$.
%We first show that $H^i$ is independent.
If $H^i$ is $C_2^1$-dependent then, by symmetry, we may assume  that $u_3u_1\in {\rm cl}(E_0+f_i+u_1u_2+u_2u_3)$.
Since each $e\in K$ is $f_i$-coupled, this gives $K\subset {\rm cl}(E_0+f_i+u_1u_2+u_2u_3)$, and contradicts our initial assumption that  $G_0+f_i$ is not type 0.
Hence $H^i$ is $C_2^1$-independent.

Since each $A_j^i$ is a subgraph of $H^i$, each $A_j^i$ is a $C_2^1$-independent 1-dof graph.
The $C_2^1$-independence of $H^i$ and the fact that each $e\in K$ is $f_i$-coupled imply that
 ${\rm cl}(A_j^i)\cap K_u$ is as shown in Figure~\ref{fig:A}. This in turn implies that
$Z(G_0+f_i,\bp)=Z_0(G_0+f_i,\bp)\oplus \langle \bq_1^i,\bq_2^i,\bq_3^i\rangle$ for any non-trivial motions $\bq_j^i$ of $(A_j^i, \bp)$, $1\leq j\leq 3$.

\medskip
\noindent
\emph{Case 2:} $|[F_v]\cap K|=2$. By relabeling $u_1,u_2,u_3,u_4$ if necessary, we may assume that $[F_v]\cap K=\{u_1u_2, u_3u_4\}$.
Then by Claim~\ref{claim:2opposite2}, each of  the edges in $K\setminus [F_v]$ is $f_i$-coupled.
We will show $G_0+f_i$ is type A or type B, and hence $(G_0,F)$ is type AA, AB, BA or BB.
%, assuming that $G_0+f_i$ is not type 0.
%

Let $H^i:=G_0+f_i+u_1u_2+u_2u_3+u_3u_1$.
Since $u_2u_3, u_3u_1$ are $f_i$-coupled and $G_0+f_i$ is not type 0, 
%if $H^i$ is dependent, $G_0+f_i$ would be type 0. Hence 
$H^i$ is $C_2^1$-independent.
% (by the assumption that $G_0+f_i$ is not type 0).
If 
%$u_3u_4\in [\{f_i, u_1u_2\}]$, 
$u_1u_2$ is $f_i$-coupled, then we may use  the same proof as in  Case 1 to show that $G_0+f_i$ is type A.
Hence we may assume that  $u_3u_4\notin [\{f_i, u_1u_2\}]$. 

%we consider $B_j^i \ (j=1,2,3)$.
Since $B_2^i$ and $B_3^i$ are subgraphs of $H^i$, they are $C_2^1$-independent 1-dof graphs.
The assumption that $G_0+f_i$ is not type 0 now implies that  ${\rm cl}(B_2^i)\cap K_u$ and ${\rm cl}(B_3^i)\cap K_u$ are as shown in Figure~\ref{fig:B}(ii)(iii). 
(The edge $u_3u_4$ does not exist in $\cl(B^i_2)\cap K_u$ since $G_0+f_i$ is not type 0. The reason why the edge $u_3u_4$ does not exist in $\cl(B^i_3)\cap K_u$ will be clarified later.)
The graph $B_1^i$ is $C^1_2$-independent since $u_3u_4\notin [\{f_i, u_1u_2\}]$.
Also, by Claim~\ref{claim:Fv}, ${\rm cl}(B_1^i)={\rm cl}(E_0+f_i+u_1u_2+u_3u_4)={\rm cl}(E_0+K_v)$.
This gives $K_v\subset {\rm cl}(B_1^i)$. Since $[F_v]\cap K=\{u_1u_2, u_3u_4\}$, it also implies  that 
${\rm cl}(B_1^i)\cap K_u$ is as shown in Figure~\ref{fig:B}(i).
The fact that ${\rm cl}(B_1^i)\cap K_u$ is as shown in Figure~\ref{fig:B}(i) now tells us that
$u_3u_4$ does not exist in $\cl(B^i_3)\cap K_u$.

The assertion that 
$Z(G_0+f_i,\bp)=Z_0(G_0+f_i,\bp)\oplus \langle \bq_1^i,\bq_2^i,\bq_3^i\rangle$ for any non-trivial motions $\bq_j^i$ of $(B_j^i, \bp)$ easily follows from
the fact that ${\rm cl}(B_j^i)\cap K_u$ is as in Figure~\ref{fig:B}.

\medskip
\noindent
\emph{Case 3:} $|[F_v]\cap K|=4$. 
By relabeling $u_1,u_2,u_3,u_4$ if necessary, we may assume that $[F_v]\cap K=\{u_1u_2, u_2u_3, u_3u_4, u_4u_1\}$.
Then by Claim~\ref{claim:2opposite2}, $u_1u_3$ and $u_2u_4$  are $f_i$-coupled.
We will show that $G_0+f_i$ is type C or type D.
If $|[\{f_i, u_1u_2\}]\cap \{u_2u_3, u_3u_4, u_1u_4\}|\geq 2$ then,  since $u_1u_3$ is coupled, ${\rm cl}(E_0+f_i+u_1u_2+u_1u_3)$ would contain at least five edges from $K$.  This in turn would imply that $K_u\subset {\rm cl}(E_0+f_i+u_1u_2+u_1u_3)$
and contradict our initial assumption that $G_0+f_i$ is not type 0. Hence
\begin{equation}\label{eq:type_case3}
\left|[\{f_i, u_1u_2\}]\cap \{u_2u_3, u_3u_4, u_1u_4\}\right|\leq 1.
\end{equation}

%
%
%We first claim  
%\begin{equation}\label{eq:type_case3}
%|[u_1u_2, f_i]\cap \{u_2u_3, u_3u_4, u_4u_1\}|\leq 1,
%\end{equation}
%where $[\{u_1u_2, f_i\}]$ is simply denoted by $[u_1u_2, f_i]$.
%Indeed, if this is not the case, then ${\rm cl}(E_0+f_i+u_1u_2+u_1u_3)$ would contain five edges among $K$ since $u_1u_3$ is coupled, which in turn implies $K_u\subset {\rm cl}(E_0+f_i+u_1u_2+u_1u_3)$.
%This contradicts that type 0 does not happen.

Consider the following two subcases:

\medskip
\noindent
\emph{Subcase 3-1:} $[\{f_1, u_1u_2\}]\cap \{u_2u_3, u_1u_4\}=\{u_1u_4\}$ and $[\{f_2, u_1u_2\}]
\cap \{u_2u_3, u_1u_4\}=\{u_2u_3\}$.
We will show that  $(G_0,F)$ is type DD. 
We first show that  $J^i:=G_0+f_i+u_1u_2+u_1u_3+u_3u_4$ is $C_2^1$-independent for both $i=1,2$.
To see this, observe that $E_0+f_i+u_1u_2+u_3u_4$ is independent by (\ref{eq:type_case3}) and the assumption of subcase 3-1.
Hence, by Claim~\ref{claim:Fv}, 
\begin{equation}\label{eq:type_case3_1}
{\rm cl}(E_0+f_i+u_1u_2+u_3u_4)={\rm cl}(E_0\cup F_v)={\rm cl}(E_0\cup K_v).
\end{equation} 
Since $[F_v]\cap K=\{u_1u_2, u_2u_3, u_3u_4, u_4u_1\}$ we have $u_1u_3\notin {\rm cl}(E_0+f_i+u_1u_2+u_3u_4)$ and hence 
$J^i$ is $C_2^1$-independent.

Since each $D_j^i$ is a subgraph of $J^i$, each $D_j^i$ is a $C_2^1$-independent 1-dof graph.
%By Claim~\ref{claim:F_v} and the fact that $u_1u_3$ is $f_i$-coupled, 
%${\rm cl}(D_j^i)\cap K_u$ is as in Figure~\ref{fig:D} 
%By $D_1^i=G_0+f_i+u_1u_2+u_3u_4$ and (\ref{eq:type_case3_1}), 
We have $K_v\subset {\rm cl}(D_1^i)$ by (\ref{eq:type_case3_1}).
The assumption that $G_0+f_i$ is not type 0 and (\ref{eq:type_case3_1}) also imply that 
${\rm cl}(D_j^i)\cap K_u$ is  as shown in Figure~\ref{fig:D}. The assertion that
$Z(G_0+f_i,\bp)=Z_0(G_0+f_i,\bp)\oplus \langle \bq_1^i,\bq_2^i,\bq_3^i\rangle$ for any non-trivial motions $\bq_j^i$ of $(D_j^i, \bp)$, $1\leq i\leq 3$,  follows easily from
the fact that ${\rm cl}(D_j^i)\cap K_u$ is as in Figure~\ref{fig:D}.

\medskip
\noindent
\emph{Subcase 3-2:} Either $[\{f_i, u_1u_2\}]\cap \{u_2u_3, u_1u_4\}\subseteq \{u_1u_4\}$ for both $i=1,2$, 
or\\ $[\{f_i, u_1u_2\}]\cap \{u_2u_3, u_1u_4\}\subseteq \{u_2u_3\}$ for both $i=1,2$.\\
Relabeling if necessary, we may assume that the first alternative holds.
We will show that  $(G_0,F)$ is type CC. 
%Let  $H^i:=G_0+u_1u_2+u_2u_3+u_3u_1$ (for $i=1,2$). 
We first show that  $H^i:=G_0+u_1u_2+u_2u_3+u_3u_1$  is $C_2^1$-independent (for both $i=1,2$).
To see this, observe that $E_0+f_i+u_1u_2+u_2u_3$ is independent since  $[\{f_i, u_1u_2\}]\cap \{u_2u_3, u_1u_4\}\subseteq \{u_1u_4\}$.
Hence, by Claim~\ref{claim:Fv}, 
\begin{equation}\label{eq:type_case3_2}
{\rm cl}(E_0+f_i+u_1u_2+u_2u_3)={\rm cl}(E_0\cup F_v)={\rm cl}(E_0\cup K_v).
\end{equation} 
Since  $[F_v]\cap K=\{u_1u_2, u_2u_3, u_3u_4, u_4u_1\}$, we have $u_1u_3\notin {\rm cl}(E_0+f_i+u_1u_2+u_2u_3)$ and hence 
$H^i$ is $C_2^1$-independent.

Since each $C_j^i$ is a subgraph of $H^i$, each $C_j^i$ is a $C_2^1$-independent  1-dof graph.
%By $C_1^i=G_0+f_i+u_1u_2+u_2u_3$ and, 
We have $K_v\subset {\rm cl}(C_1^i)$  by (\ref{eq:type_case3_2}).
The assumption that $G_0+f_i$ is not type 0 and  (\ref{eq:type_case3_2}) imply that 
${\rm cl}(C_j^i)\cap K_u$ is  as shown in Figure~\ref{fig:C}.
The assertion that 
$Z(G_0+f_i,\bp)=Z_0(G_0+f_i,\bp)\oplus \langle \bq_1^i,\bq_2^i,\bq_3^i\rangle$ for any non-trivial motions $\bq_j^i$ of $(C_j^i, \bp)$  follows easily from
the fact that ${\rm cl}(C_j^i)\cap K_u$ is as in Figure~\ref{fig:C}.
%
%This completes the proof. 
\end{proof}


\subsubsection{The motion spaces of $(G_0+f_i,p|_{V_0})$ and $(G+f_i,p)$}
\label{subsubsec:5}

%\subsubsection{The motion spaces of $(G_0+f_i,\bp|_{V_0})$ and $(G+f_i,\bp)$}
%\label{subsubsec:5}
We will obtain expressions for a non-trivial motion of each of the 1-dof frameworks $(A^i_j,\bp|_{V_0})$,
$(B^i_j,\bp|_{V_0})$, $(C^i_j,\bp|_{V_0})$ and  $(D^i_j,\bp|_{V_0})$. 
%As in Section \ref{sec:motion1dof}, w
We first apply a projective transformation to $(G,\bp)$ to ensure that
%,now analyze how a motion of $(G+f_i,\bp)$ is described in each type.
%Since $C_2^1$-rigidity is invariant under a projective transformation, in the subsequent discussion we assume that 
\begin{equation}\label{eq:quasi_generic}
\bp(u_1)=(1,0),\ \bp(u_2)=(0, 0),\ \bp(u_3)=(0,1),\ \bp(u_4)=(1,1),
\end{equation}
and all other points in $\bp(V_0)$ are generically placed.
%and the other points are generically placed.section 
%%(We could take such a configuration at the beginning of the proof. 
%(Note that a projective transformation does not change the underlying matroid.) 
Note that this transformation does not change the underlying $C_2^1$-cofactor matroid of $(G,\bp)$ by the projective invariance of $C_2^1$-rigidity~(see~\cite{Wsurvey} or Appendix~\ref{sec:projective}), and does not change the fact that $(G,\bp)$ has a bad motion at $v_0$ by Lemma \ref{lem:projective_bad}. 
%(We could take such a configuration at the beginning of the proof. 
%Note that a projective transformation does not change the underlying matroid.) 

For simplicity we use the notation 
$$D_{ij}=D(\bp(u_i),\bp(u_j)) \quad \text{ and } \quad \Delta_{ijk}=\Delta(\bp(u_i),\bp(u_j),\bp(u_k))$$ 
throughout the remainder of this section. 

Let $F=\{f_1,f_2\}$ be the fixed good pair, and suppose that $G_0+f_i$ is type A for some $i\in \{1,2\}$.
Since $(G,\bp)$ is 2-dof, $(G+f_i,\bp)$ is 1-dof.
Let $\bq^i$ be a non-trivial motion of  $(G+f_i,\bp)$. Then $\bq^i|_{V_0}$ is a motion of $(G_0+f_i,\bp|_{V_0})$ and 
property (3) in the definition of type A implies that $\bq^i|_{V_0}$ is a linear combination of $\bq_{1}^i,\bq_{2}^i,\bq_{3}^i$ and a trivial motion, where $\bq_j^i$ is a non-trivial motion of $(A_j^i, \bp|_{V_0})$.   By adding a suitable trivial motion to $\bq^i$, we may assume that  we have  
\begin{equation}\label{eq:uncoupled2}
\bq^i|_{V_0}=\sum_{j=1}^3\alpha_j^i \bq_j^i
\end{equation}
for some scalars $\alpha_j^i\in \mathbb{R}$.
%We may now apply Claim~\ref{claim:coupled1} to the 1-dof framework $(A^i_j,p|_{V_0})$ and then apply Claim \ref{claim:coupled3} to the motion $q^i$ of $(G+f_i,p)$ to deduce:
%In Claim~\ref{claim:coupled1} we have already seen how ${\rm cl}(A_j^i)$ can be used to determine the entries of each $q_j^i$. Moreover, in Claim~\ref{claim:coupled3} we have computed the value of each $\alpha_j^i$ explicitly. The following claim summarizes those facts.
\begin{claim}\label{claim:motionA}
Suppose that $G_0+f_i$ is type A. Then
for all $1\leq j\leq 3$, $(A_j^i,\bp|_{V_0})$ 
%is a 1-dof framework having 
has a non-trivial motion $\bq_j^i$ satisfying $\bq_j^i(w)\in\mathbb{Q}(\bp(V_0))$ for all $w\in V_0$,
 and 
\begin{itemize}
\item $\bq_1^i(u_5)=\bq_1^i(u_1)=\bq_1^i(u_2)=0, \bq_1^i(u_3)=D_{3,2} \times D_{3,5}$,  $\bq_1^i(u_4)=t_1 D_{4,1} \times D_{4,5}$;
\item $\bq_2^i(u_5)=\bq_2^i(u_2)=\bq_2^i(u_3)=0, \bq_2^i(u_1)=D_{1,3} \times D_{1,5}$, $\bq_2^i(u_4)=t_2 D_{4,2} \times D_{4,5}$;
\item $\bq_3^i(u_5)=\bq_3^i(u_1)=\bq_3^i(u_2)=0, \bq_3^i(u_3)=D_{3,1} \times D_{3,5}$,  $\bq_3^i(u_4)=t_3 D_{4,2} \times D_{4,5}$;
\end{itemize}
where 
%$s_1=s_2=s_3=1$, 
$t_1=\Delta_{523}/\Delta_{514}$, $t_2=-\Delta_{513}/\Delta_{524}$ and  $t_3=\Delta_{513}/\Delta_{524}$.
%$t_1=\left|\begin{array}{c} D_{34} \\ D_{32} \\ D_{35} \end{array}\right|/ \left|\begin{array}{c} D_{43} \\ D_{41} \\ D_{45} \end{array}\right|$,
%$t_2=\left|\begin{array}{c} D_{14} \\ D_{13} \\ D_{15} \end{array}\right|/ \left|\begin{array}{c} D_{41} \\ D_{42} \\ D_{45} \end{array}\right|$, and 
%$t_3=\left|\begin{array}{c} D_{34} \\ D_{31} \\ D_{35} \end{array}\right|/ \left|\begin{array}{c} D_{43} \\ D_{42} \\ D_{45} \end{array}\right|$.

In addition, $(G+f_i,\bp)$ has  a non-trivial motion $\bq^i$ such that 
$\bq^i|_{V_0}=\sum_{j=1}^3\alpha_j^i \bq_j^i$ where:
\begin{align*}
\alpha_1^i&=-\Delta_{012}\Delta_{013}\Delta_{024}\Delta_{135}\Delta_{245}t_2 - \Delta_{013}^2\Delta_{024}\Delta_{135}^2 + \Delta_{013}\Delta_{023}\Delta_{024}\Delta_{135}\Delta_{245}t_3; \\
\alpha_2^i&=\Delta_{012}\Delta_{013}\Delta_{014}\Delta_{135}\Delta_{145}t_1 - \Delta_{012}\Delta_{023}\Delta_{024}\Delta_{235}\Delta_{245}t_3;\\
\alpha_3^i&=\Delta_{012}\Delta_{023}\Delta_{024}\Delta_{235}\Delta_{245}t_2 - \Delta_{013}\Delta_{014}\Delta_{023}\Delta_{135}\Delta_{145}t_1 + \Delta_{013}\Delta_{023}\Delta_{024}\Delta_{135}\Delta_{235}.
\end{align*}
\end{claim}
\begin{proof}
We will suppress the superscript $i$ in $A^i_j,\bq^i_j,\bq^i,\alpha^i_j$ as it remains constant throughout the proof.




Consider $(A_1,\bp|_{V_0})$. Since $\cl(A_1)$ contains the triangle on $\{u_1, u_2, u_5\}$ and $u_1u_3\not\in \cl(A_1)$,  
$(A_1,\bp|_{V_0})$ has a non-trivial motion $\bq_1$ such that $\bq_1(u_1)=\bq_1(u_2)=\bq_1(u_5)=0$ and $\bq_1(u_3)\neq 0$. Since ${\rm cl}(A_1)$ contains $u_2u_3$ and $u_3u_5$, $\bq_1(u_3)=s_1 D_{2,3}\times D_{3,5}$ for some scalar $s_1$. Since $\bq_1(u_3)\neq 0$ we can scale $\bq_1$, so that $s_1=1$.
Since ${\rm cl}(A_1)$ contains $u_1u_4$ and $u_4u_5$, $\bq_1(v_4)=t_1 D_{1,4}\times D_{4,5}$ for some scalar $t_1$.
%By the edge constraint between $u_3$ and $u_4$, 
Since $u_3u_4\in \cl(A_1)$, we have 
$$0=D_{34}\cdot (\bq_1(u_3)-\bq_1(u_4))=\left|\begin{array}{c} D_{34} \\ D_{32} \\ D_{35} \end{array}\right|- \left|\begin{array}{c} D_{43} \\ D_{41} \\ D_{45} \end{array}\right|t_1 \mbox{ so } t_1=\left|\begin{array}{c} D_{34} \\ D_{32} \\ D_{35} \end{array}\right|/ \left|\begin{array}{c} D_{43} \\ D_{41} \\ D_{45} \end{array}\right|.$$ 
This can be simplified to $t_1=\Delta_{523}/\Delta_{514}$ by using (\ref{eq:Vandermonde}) and (\ref{eq:quasi_generic}).
%(and by the Vandermonde identity (\ref{eq:Vandermonde})).
Furthermore, since $(A_1,\bp|_{V_0})$ is a 1-dof framework and  $\bq_1(u_3)$ takes fixed non-zero values in $\mathbb{Q}(\bp(V_0))$, $\bq_1$ is  uniquely determined by Cramer's rule and will satisfy $\bq_1(w)\in\mathbb{Q}(\bp(V_0))$ for all $w\in V_0$.


We may apply the same argument, to deduce that  $(A_2,\bp|_{V_0})$  and $(A_3,\bp|_{V_0})$ have the non-trivial motions $\bq_2$ and $\bq_3$ given in the claim.

\medskip
We next prove the second part of the claim.
The existence of a non-trivial motion $\bq$ such that 
$\bq|_{V_0}=\sum_{j=1}^3 \alpha_j\bq_j$ is established in (\ref{eq:uncoupled2}).
Since $u_0u_k$ is an edge of $G$ for all $1\leq k\leq 5$, we have
$D_{0,k}\cdot [\bq(u_0)-\bq(u_k)]=0$ for all $1\leq k\leq 5$. 
Hence we obtain the system of equations
$$ D_{0,k}\cdot [\bq(u_0)-\alpha_1 \bq_1(u_k)-\alpha_2 \bq_2(u_k)-\alpha_3 \bq_3(u_k)]=0 \mbox{ for $1\leq k\leq 5$},$$
or in matrix form,
\begin{equation}
\label{eq:coupled1}
\left(
\begin{array}{cccc}
D_{0,1}\cdot \bq_1(u_1) & D_{0,1}\cdot \bq_2(u_1) &  D_{0,1}\cdot \bq_3(u_1) & D_{0,1} \\
D_{0,2}\cdot \bq_1(u_2) & D_{0,2}\cdot \bq_2(u_2) &  D_{0,2}\cdot \bq_3(u_2) & D_{0,2} \\
D_{0,3}\cdot \bq_1(u_3) & D_{0,3}\cdot \bq_2(u_3) &  D_{0,3}\cdot \bq_3(u_3) & D_{0,3} \\
D_{0,4}\cdot \bq_1(u_4) & D_{0,4}\cdot \bq_2(u_4) &  D_{0,4}\cdot \bq_3(u_4) & D_{0,4} \\
D_{0,5}\cdot \bq_1(u_5) & D_{0,5}\cdot \bq_2(u_5) &  D_{0,5}\cdot \bq_3(u_5) & D_{0,5} \\
\end{array}
\right) \left(
\begin{array}{c}
\alpha_1 \\ \alpha_2 \\ \alpha_3 \\ -a_0\\ -b_0\\ -c_0
\end{array}
\right) = 0,
\end{equation}
where  $(a_0,b_0,c_0)=\bq(u_0)$.
Substituting the zero values for $\bq_j(u_k)$ given in the first  part of the claim, we may rewrite this system  as: 
\begin{equation}
\label{eq:coupled2}
\left(
\begin{array}{cccc}
0 & D_{0,1}\cdot \bq_2(u_1) &  0 & D_{0,1} \\
0 & 0 &  0 & D_{0,2} \\
D_{0,3}\cdot \bq_1(u_3) & 0 &  D_{0,3}\cdot \bq_3(u_3) & D_{0,3} \\
D_{0,4}\cdot \bq_1(u_4) & D_{0,4}\cdot \bq_2(u_4) &  D_{0,4}\cdot \bq_3(u_4) & D_{0,4} \\
0 & 0 &  0 & D_{0,5} \\
\end{array}
\right) \left(
\begin{array}{c}
\alpha_1 \\ \alpha_2 \\ \alpha_3\\ -a_0\\ -b_0\\ -c_0 
\end{array}
\right) = 0.
\end{equation}
By scaling $\bq$, we may suppose that $\alpha_1+\alpha_2+\alpha_3=\mu$, 
where $\mu$ is a non-zero number which will be chosen later. 
%to simplify our computations. 
Let $M'$ be the matrix of coefficients in (\ref{eq:coupled2}) and  $M$ denote the square matrix $\left(\begin{array}{c}b\\M'\end{array}\right)$ where $b=(1,1,1,0,0,0)$. Then we may rewrite (\ref{eq:coupled2}) as $M(\alpha_1,\alpha_2,\alpha_3,-a_0,-b_0,-c_0)^\top=(\mu,0,0,0,0,0)^\top$ and Cramer's rule gives
\begin{align*}
\alpha_1&=\frac{\mu}{{\rm det} M}\left|
\begin{array}{cccc}
 D_{0,1}\cdot \bq_2(u_1) & 0  & D_{0,1} \\
 0 &  0 & D_{0,2} \\
 0 &  D_{0,3}\cdot \bq_3(u_3) & D_{0,3} \\
 D_{0,4}\cdot \bq_2(u_4) &  D_{0,4}\cdot \bq_3(u_4) & D_{0,4} \\
 0 &  0 & D_{0,5} \\
\end{array}
\right| \\
\alpha_2&=-\frac{\mu}{{\rm det} M}\left|
\begin{array}{cccc}
0  &  0 & D_{0,1} \\
0  &  0 & D_{0,2} \\
D_{0,3}\cdot \bq_1(u_3)  &  D_{0,3}\cdot \bq_3(u_3) & D_{0,3} \\
D_{0,4}\cdot \bq_1(u_4)  &  D_{0,4}\cdot \bq_3(u_4) & D_{0,4} \\
0 &  0 & D_{0,5} \\
\end{array}
\right| \\
\alpha_3&=\frac{\mu}{{\rm det} M}\left|
\begin{array}{cccc}
0 & D_{0,1}\cdot \bq_2(u_1) &   D_{0,1} \\
0 & 0 &   D_{0,2} \\
D_{0,3}\cdot \bq_1(u_3) & 0  & D_{0,3} \\
D_{0,4}\cdot \bq_1(u_4) & D_{0,4}\cdot \bq_2(u_4)  & D_{0,4} \\
0 & 0  & D_{0,5} \\
\end{array}
\right|
\end{align*}
%where $M$ denotes the block matrix $\left(\begin{array}{c}b\\M'\end{array}\right)$, $b=(1,1,1,0,0,0)$, and $M'$ is the matrix of coefficients in (\ref{eq:coupled2}).
Note  that each entry of the form $D_{0,k}\cdot \bq_j(u_k)$ in the above determinants can be written as 
a product of areas of three triangles.
%by Claim~\ref{claim:coupled1}.
For example, we have
$D_{01}\cdot \bq_2(u_1)=\left|\begin{array}{c} D_{10}\\ D_{13} \\ D_{15}  \end{array}\right|
=-\Delta_{103}\Delta_{135}\Delta_{150}$, 
where the first equation follows from the first part of the claim and the second equation follows from the Vadermonde identity (\ref{eq:Vandermonde}).

We may  expand the determinant in the formula for $\alpha_1$ to obtain
\begin{align*}
\frac{{\rm det} M}{\mu}\alpha_1 
&=  D_{0,1}\cdot \bq_2(u_1)\left(
-D_{0,3}\cdot \bq_3(u_3) 
\left|
\begin{array}{c}
D_{0,2} \\ D_{0,4} \\ D_{0,5}
\end{array}\right|
+
D_{0,4}\cdot \bq_3(u_4) 
\left|
\begin{array}{c}
D_{0,2} \\ D_{0,3} \\ D_{0,5}
\end{array}\right|\right) \\
&\quad -D_{0,4} \cdot \bq_2(u_4) D_{0,3}\cdot \bq_3(u_3) 
\left|
\begin{array}{c}
D_{0,1} \\ D_{0,2} \\ D_{0,5}
\end{array}\right| \\ 
%%%%%%%%
&= \left|
\begin{array}{c}
D_{1,0} \\ D_{1,3} \\ D_{1,5}
\end{array}\right|
\left(
-
\left|
\begin{array}{c}
D_{3,0} \\ D_{3,1} \\ D_{3,5}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,2} \\ D_{0,4} \\ D_{0,5}
\end{array}\right|
+t_3\left|
\begin{array}{c}
D_{4,0} \\ D_{4,2} \\ D_{4,5}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,2} \\ D_{0,3} \\ D_{0,5}
\end{array}\right|
\right)
-t_2
\left|
\begin{array}{c}
D_{4,0} \\ D_{4,2} \\ D_{4,5}
\end{array}\right|
\left|
\begin{array}{c}
D_{3,0} \\ D_{3,1} \\ D_{3,5}
\end{array}\right|
\left|
\begin{array}{c}
D_{0,1} \\ D_{0,2} \\ D_{0,5}
\end{array}\right|\\
%%%%%%%%%%%
&=
(\Delta_{013}\Delta_{135}\Delta_{015}\Delta_{035}\Delta_{024}\Delta_{045}\Delta_{025})
(-\Delta_{013}\Delta_{135} +t_3\Delta_{245}\Delta_{023} -t_2\Delta_{245}\Delta_{012}).
\end{align*}
%By a similar calculation, we also get the corresponding formulae for $\alpha_2$ and $\alpha_3$.
%For completeness, we will not skip it!!
%\begin{align*}
%&
%\frac{{\rm det} M}{k} \beta \\
%&= -D_{0,3}\cdot \bq_1(u_3)\left(
%-D_{0,2}\cdot \bq_3(u_2) 
%\left|
%\begin{array}{c}
%D_{0,1} \\ D_{0,4} \\ D_{0,5}
%\end{array}\right|
%+
%D_{0,4}\cdot \bq_3(u_4) 
%\left|
%\begin{array}{c}
%D_{0,1} \\ D_{0,2} \\ D_{0,5}
%\end{array}\right|\right)
%+D_{0,4} \cdot \bq_1(u_4) (-D_{0,2}\cdot \bq_3(u_2)) 
%\left|
%\begin{array}{c}
%D_{0,1} \\ D_{0,3} \\ D_{0,5}
%\end{array}\right| \\ 
%%%%%%%%%
%&=k_1 \left|
%\begin{array}{c}
%D_{3,0} \\ D_{3,1} \\ D_{3,5}
%\end{array}\right|
%\left(
%k_3
%\left|
%\begin{array}{c}
%D_{2,0} \\ D_{2,3} \\ D_{2,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,1} \\ D_{0,4} \\ D_{0,5}
%\end{array}\right|
%-k_3'\left|
%\begin{array}{c}
%D_{4,0} \\ D_{4,1} \\ D_{4,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,1} \\ D_{0,2} \\ D_{0,5}
%\end{array}\right|
%\right)
%-k_1'k_3
%\left|
%\begin{array}{c}
%D_{4,0} \\ D_{4,2} \\ D_{4,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{2,0} \\ D_{2,3} \\ D_{2,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,1} \\ D_{0,3} \\ D_{0,5}
%\end{array}\right|\\
%%%%%%%%%%%%
%&=-k_1k_3 \Delta_{3,0,1}\Delta_{3,1,5}\Delta_{3,5,0}\Delta_{2,0,3}\Delta_{2,3,5}\Delta_{2,5,0}\Delta_{0,1,4}\Delta_{0,4,5}\Delta_{0,5,1} \\
%& \hspace{1em} +k_1k_3' \Delta_{3,0,1}\Delta_{3,1,5}\Delta_{3,5,0}\Delta_{4,0,1}\Delta_{4,1,5}\Delta_{4,5,0}\Delta_{0,1,2}\Delta_{0,2,5}\Delta_{0,5,1} \\
%& \hspace{1em} +k_1'k_3 \Delta_{4,0,2}\Delta_{4,2,5}\Delta_{4,5,0}\Delta_{2,0,3}\Delta_{2,3,5}\Delta_{2,5,0}\Delta_{0,1,3}\Delta_{0,3,5}\Delta_{0,5,1}.
%\end{align*}
%
%\begin{align*}
%&\frac{{\rm det} M}{k}\gamma \\
%&= D_{0,3}\cdot \bq_1(u_3) \left( 
%D_{0,1}\cdot \bq_2(u_1) 
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{0,4} \\ D_{0,5}
%\end{array}\right|
%+
%D_{0,4}\cdot \bq_2(u_4) 
%\left|
%\begin{array}{c}
%D_{0,1} \\ D_{0,2} \\ D_{0,5}
%\end{array}\right|
%\right)
%-
%D_{0,4}\cdot \bq_1(u_4) 
%D_{0,1}\cdot \bq_2(u_1)
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{0,3} \\ D_{0,5}
%\end{array}\right| \\ 
%%%%%%%%%
%&=k_1 
%\left|
%\begin{array}{c}
%D_{3,0} \\ D_{3,1} \\ D_{3,5} 
%\end{array}\right| 
%\left(
%k_2
%\left|
%\begin{array}{c}
%D_{1,0} \\ D_{1,2} \\ D_{1,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{0,4} \\ D_{0,5}
%\end{array}\right|
%+
%k_2'
%\left|
%\begin{array}{c}
%D_{4,0} \\ D_{4,3} \\ D_{4,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,1} \\ D_{0,2} \\ D_{0,5}
%\end{array}\right|
%\right)
%-k_1'k_2 
%\left|
%\begin{array}{c}
%D_{4,0} \\ D_{4,2} \\ D_{4,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{1,0} \\ D_{1,2} \\ D_{1,5}
%\end{array}\right|
%\left|
%\begin{array}{c}
%D_{0,2} \\ D_{0,3} \\ D_{0,5}
%\end{array}\right|
%\\
%%%%%%%%%%%%
%&=-k_1k_2 \Delta_{3,0,1}\Delta_{3,1,5}\Delta_{3,5,0}\Delta_{1,0,2}\Delta_{1,2,5}\Delta_{1,5,0}\Delta_{0,2,4}\Delta_{0,4,5}\Delta_{0,5,2} \\
%& \hspace{1em} -k_1k_2' \Delta_{3,0,1}\Delta_{3,1,5}\Delta_{3,5,0}\Delta_{4,0,3}\Delta_{4,3,5}\Delta_{4,5,0}\Delta_{0,1,2}\Delta_{0,2,5}\Delta_{0,5,1} \\
%& \hspace{1em} +k_1'k_2 \Delta_{4,0,2}\Delta_{4,2,5}\Delta_{4,5,0}\Delta_{1,0,2}\Delta_{1,2,5}\Delta_{1,5,0}\Delta_{0,2,3}\Delta_{0,3,5}\Delta_{0,5,2}
%\end{align*}
The required expression for $\alpha_1$ follows by putting  $\mu={\rm det} M/ \Delta_{015}\Delta_{025}\Delta_{035}\Delta_{045}$. 

Similar calculations give the required formulae for $\alpha_2$ and $\alpha_3$ (using the same constant $\mu$).
\end{proof}



We next obtain an analogous claim for the case when $(G+f_i)$ is type B.
%Although the proof is identical, we shall give a proof for type B as this case requires an extra argument.  
%(We have double-checked by a computer if the values of the statements are correct.)

\begin{claim}\label{claim:motionB}
Suppose that $G_0+f_i$ is type B.
Then
for all $1\leq j\leq 3$, $(B_j^i,\bp|_{V_0})$ 
%is a 1-dof framework having 
has a non-trivial motion $\bq_j^i$ satisfying $\bq_j^i(w)\in \rat(\bp(V_0))$ for all $w\in V_0$, 
 and 
\begin{itemize}
\item $\bq_1^i(u_5)=\bq_1^i(u_1)=\bq_1^i(u_2)=0$, \\
$\bq_1^i(u_3)=D_{3,1} \times D_{3,5}+s_{12} D_{3,2}\times D_{3,5}$,  \\
$\bq_1^i(u_4)=t_{11}D_{4,1} \times D_{4,5}+ t_{12} D_{4,2}\times D_{4,5}$;
\item $\bq_2^i(u_5)=\bq_2^i(u_2)=\bq_2^i(u_3)=0, \bq_2^i(u_1)=D_{1,3} \times D_{1,5}$,  $\bq_2^i(u_4)=t_2 D_{4,2} \times D_{4,5}$;
\item $\bq_3^i(u_5)=\bq_3^i(u_1)=\bq_3^i(u_2)=0, \bq_3^i(u_3)=D_{1,3} \times D_{3,5}$, $\bq_3^i(u_4)=t_3^i D_{4,2} \times D_{4,5}$;
\end{itemize}
for $t_2=-\Delta_{513}/\Delta_{524}$ and some
non-zero constants $s_{12},t_{11},t_{12},t_3^i \in\mathbb{Q}(\bp(V_0))$, and we may take  $s_{12},t_{11},t_{12}$ to be the same constants for both $\bq_1^1$ and $\bq_1^2$ when $(G_0,F)$ is type BB.
%, $s_{11}=s_2=s_3=1$, and $t_2=-\Delta_{513}/\Delta_{524}$.
%and $t_2=\left|\begin{array}{c} D_{1,4} \\ D_{1,3} \\ D_{1,5}\end{array}\right|/\left|\begin{array}{c} D_{4,1} \\ D_{4,2} \\ D_{4,5}\end{array}\right|$.

In addition, $(G+f_i,\bp)$ has  a non-trivial motion $\bq^i$ such that 
$\bq^i|_{V_0}=\sum_{j=1}^3\beta_j^i \bq_j^i$ where: 
\begin{align*}
\beta_1^i&=-\Delta_{012}\Delta_{013}\Delta_{024}\Delta_{135}\Delta_{245}t_2
- \Delta_{013}^2 \Delta_{024} \Delta_{135}^2
%\\ &\hspace{1em}
+ \Delta_{013}\Delta_{023} \Delta_{024} \Delta_{135} \Delta_{245} t_3^i; \\
\beta_2^i&=\Delta_{012}\Delta_{013}\Delta_{014}\Delta_{135}\Delta_{145}t_{11}
-\Delta_{012}\Delta_{013}\Delta_{024}\Delta_{135}\Delta_{245}t_3^i \\
&\hspace{1em}+ \Delta_{012}\Delta_{013}\Delta_{024}\Delta_{135}\Delta_{245}t_{12} 
- \Delta_{012}\Delta_{023}\Delta_{024}\Delta_{235}\Delta_{245}s_{12}t_3^i; \\
\beta_3^i&=\Delta_{012}\Delta_{013}\Delta_{024}\Delta_{135}\Delta_{245}t_2  
+ \Delta_{012}\Delta_{023}\Delta_{024}\Delta_{235}\Delta_{245}s_{12}t_2 \\
&\hspace{1em}+ \Delta_{013}^2\Delta_{024}\Delta_{135}^2 
- \Delta_{013}\Delta_{014}\Delta_{023}\Delta_{135}\Delta_{145}t_{11}\\
&\hspace{1em}+ \Delta_{013}\Delta_{023}\Delta_{024}\Delta_{135}\Delta_{235}s_{12} 
- \Delta_{013}\Delta_{023}\Delta_{024}\Delta_{135}\Delta_{245}t_{12}.
\end{align*}
\end{claim}
\begin{proof}
We will suppress the superscript $i$ in $B^i_j,\bq^i_j,\beta^i_j, t_3^i$ as it remains constant throughout the proof.

We first consider $(B_2,\bp|_{V_0})$. Since $K(u_2,u_3,u_5)\subset \cl(B_2)$ and $u_1u_2\not\in \cl(B_2)$,  
$(B_2,\bp|_{V_0})$ has a non-trivial motion $\bq_2$ such that $\bq_2(u_2)=\bq_2(u_3)=\bq_2(u_5)=0$ and $\bq_2(u_1)\neq 0$. Since ${\rm cl}(B_2)$ contains $u_1u_3$ and $u_1u_5$, $\bq_2(u_1)=s_2 D_{1,3}\times D_{1,5}$ for some scalar $s_2$. Since $\bq_2(u_1)\neq 0$ we can scale $\bq_2$, so that $s_2=1$.
Since ${\rm cl}(B_2)$ contains $u_4u_2$ and $u_4u_5$, $\bq_2(v_4)=t_2 D_{4,2}\times D_{4,5}$ for some scalar $t_2$.
%By the edge constraint between $u_3$ and $u_4$, 
Since $u_1u_4\in \cl(B_2)$, we have 
$0=D_{14}\cdot (\bq_2(u_1)-\bq_2(u_4))$ and we can now use 
(\ref{eq:Vandermonde}) and (\ref{eq:quasi_generic}) to deduce that 
$t_2= -\Delta_{513}/\Delta_{524}$.
Furthermore, since $(B_2,\bp|_{V_0})$ is a 1-dof framework and $\bq_2(u_1)$ takes fixed non-zero values in $\mathbb{Q}(\bp(V_0))$, $\bq_2$ is  uniquely determined by Cramer's rule and will satisfy $\bq_2(w)\in\mathbb{Q}(\bp(V_0))$ for all $w\in V_0$.

%
%We first look at $(B_2, \bp)$ as this is an easier case.
%We consider pinning down triangle $\{u_2, u_3, u_5\}$ as shown in the white boxes in Figure~\ref{fig:B}(ii),
%and consider a non-trivial motion $q_2$ of $(B_2, \bp)$ with $q_2(u_5)=q_2(u_2)=q_2(u_3)=0$.
%Then by $u_1u_3, u_1u_5\in {\rm cl}(B_2)$, $q_2(u_1)=s_2 D_{1,3}\times D_{1,5}$ for some $s_2\in \mathbb{R}$.
%Similarly, by $u_4u_2, u_4u_5\in {\rm cl}(B_2)$, $q_2(u_4)=t_2 D_{4,2}\times D_{4,5}$ for some $t_2\in \mathbb{R}$.
%By the existence of edge $u_1u_2$ in $B_2$, we get 
%$t_2/s_2=-\Delta_{513}/\Delta_{524}$.
%By scaling $q_2$, we get $s_2=1:=s_2$ and $t_2= -\Delta_{513}/\Delta_{524}:=t_2$, as required.

We can apply the same argument to $(B_3, \bp|_{V_0})$ using the fact that $K(u_1,u_2,u_5)\subset B_3$ to obtain the formula for $\bq_3$. Note that $\bq_3(u_3)\neq 0\neq \bq_3(u_4)$ since $u_1u_4,u_2u_3\not\in \cl(B_3)$ and that we cannot obtain an explicit formula for $t_3$ because $u_3u_4\not\in \cl(B_3)$.



%We consider pinning down triangle $\{u_1, u_2, u_5\}$ as shown in the white boxes in Figure~\ref{fig:B}(iii),
%and consider a non-trivial motion $q_3$ of $(B_3, p)$ with $q_3(u_5)=q_3(u_2)=q_3(u_3)=0$.
%Then $q_3(u_1)=s_3 D_{1,3}\times D_{1,5}$ for some $s_3\in \mathbb{R}$
%and  $q_3(u_4)=t_3 D_{4,2}\times D_{4,5}$ for some $t_3\in \mathbb{R}$.
%Since $(B_3, p)$ is 1-dof with $V(B_3)=V_0$, by scaling, we can suppose that $s_3, t_3\in \mathbb{Q}(p(V_0))$.
%Also, both $s_3, t_3$ are non-zero since otherwise ${\rm cl}(B_3)\cap K_u$ would be different from that in Figure~\ref{fig:B}(iii).
%Hence by scaling we get $s_3=1:=s_3$ (but $t_3^1\neq t_3^2$ may hold).




We next consider $(B_1, \bp|_{V_0})$. Since $B_1-u_3u_4+u_3u_1=B_3$,
$\bq_3$ is a motion of $(B_1-u_3u_4,\bp|_{V_0})$ satisfying $\bq_3(u_5)=\bq_3(u_1)=\bq_3(u_2)=0, \bq_3(u_3)=D_{1,3} \times D_{3,5}$, $\bq_3(u_4)=t_3 D_{4,2} \times D_{4,5}$ and  $D_{3,4}\times (\bq_3(u_3)-\bq_3(u_4))\neq 0$. We may use the symmetry between $u_3$ and $u_4$ in type $B$, see Figure \ref{fig:B}, to deduce that $(B_1-u_3u_4,\bp|_{V_0})$ also has a nontrivial motion $\bar \bq_3$ satisfying $\bar\bq_3(u_5)=\bar\bq_3(u_1)=\bar\bq_3(u_2)=0, \bar\bq_3(u_3)=D_{2,3} \times D_{3,5}$, $\bar\bq_3(u_4)=\bar t_3 D_{4,1} \times D_{4,5}$ and
$D_{3,4}\times (\bar\bq_3(u_3)-\bar\bq_3(u_4))\neq 0$. (The motion $\bar \bq_3$ is a non-trivial motion of $\bar B_3:=B_1-u_3u_4+u_4u_1$ and we have ${\rm cl}(\bar B_3)\cap K_u={(\rm cl}(B_3)\cap K_u)-u_1u_3-u_2u_4+u_1u_4+u_2u_3$.)

%
%
%
% 
%We first show that 
%\begin{equation}
%\label{eq:B1}
%\begin{split}
%&\text{$B_1-u_3u_4+u_1u_3$ is a 1-dof graph with $u_2u_4\in \cl( B_1-u_3u_4+u_1u_3)$}\\
%&\text{and $u_1u_4, u_2u_3\notin \cl( B_1-u_3u_4+u_1u_3)$.}
%\end{split}
%\end{equation}
%Since ${\rm cl}(B_1)$ is as in Figure~\ref{fig:B}(i), $B_1+u_1u_3$ is $C_2^1$-rigid,
%and hence $B_1-u_3u_4+u_1u_3$ is a 1-dof graph.
%Also, by Property (4) of type B, $K_v\subset \cl(B_1)$, which, in particular, implies that $u_1u_3\notin [F_v]$.
%Hence, by Claim~\ref{claim:2opposite2}, $u_1u_3$ is $f_i$-coupled.
%In other words, $u_2u_4\in [\{f_i, u_1u_3\}]\subset \cl( B_1-u_3u_4+u_1u_3)$.
%To see the last property  in (\ref{eq:B1}),
%suppose that $u_1u_4\in \cl( B_1-u_3u_4+u_1u_3)$ or $u_2u_3\in \cl( B_1-u_3u_4+u_1u_3)$.
%Since $u_1u_4, u_2u_3\notin {\rm cl}(B_1)$, Property (4) of type B and Claim~\ref{claim:2opposite2} imply that both $u_1u_4$ and $u_2u_3$ are $f_i$-coupled.
%Therefore,  since $u_1u_4\in \cl( B_1-u_3u_4+u_1u_3)$ or $u_2u_3\in \cl( B_1-u_3u_4+u_1u_3)$, 
%$B_2\subset \cl( B_1-u_3u_4+u_1u_3)$ holds.
%Since both $B_2$ and $B_1-u_3u_4+u_1u_3$ are 1-dof graphs, 
%we get $u_1u_2\in \cl( B_1-u_3u_4+u_1u_3)=\cl(B_2)$.
%This contradicts that $\cl(B_2)$ is as in Figure~\ref{fig:B}(ii).
%This completes the proof of  (\ref{eq:B1}).
%
%By (\ref{eq:B1}), $(B_1-u_3u_4+u_1u_3,\bp|_{V_0})$ has a non-trivial motion $r$ satisfying 
%$r(u_1)=r(u_2)=r(u_5)=0$,
%$r(u_3)=a D_{3,1}\times D_{3,5}$, and 
%$r(u_4)=b D_{4,2}\times D_{4,5}$ for some non-zero $a, b\in \mathbb{R}$.
%As $u_3u_4\notin \cl(B_1-u_3u_4+u_1u_3)$, we also have $D_{3,4}\cdot (r(u_3)-r(u_4))\neq 0$.
%
%By changing the role of $u_3$ and $u_4$, we have  that 
%$B_1-u_3u_4+u_1u_4$ is a 1-dof graph and has a non-trivial motion $\tilde r$ satisfying 
%$\tilde r(u_1)=\tilde r(u_2)=\tilde r(u_5)=0$,
%$\tilde r(u_3)=c D_{3,2}\times D_{3,5}$,
%$\tilde r(u_4)=d D_{4,1}\times D_{4,5}$ for some non-zero $c, d\in \mathbb{R}$.
%Again $D_{3,4}\cdot (\tilde{r}(u_3)-\tilde{r}(u_4))\neq 0$.

%Combining those two motions, 
We can now obtain the  non-trivial motion $\bq_1$ of $(B_1,\bp|_{V_0})$ satisfying $\bq_1(u_5)=\bq_1(u_1)=\bq_1(u_2)=0$, 
$\bq_1(u_3)=s_{11}D_{3,1} \times D_{3,5}+s_{12} D_{3,2}\times D_{3,5}$ and 
$\bq_1(u_4)=t_{11}D_{4,1} \times D_{4,5}+ t_{12} D_{4,2}\times D_{4,5}$
by choosing a non-trivial linear combination of $\bq_3$ and $\bar \bq_3$ which will satisfy the constraint given by the edge $u_3u_4$. The constants $s_{11},s_{12},t_{11},t_{12}$ will all be non-zero since $u_3u_2,u_3u_1,u_4u_2,u_4u_1\not\in {\rm cl}(B_1)$, and so we can scale $\bq_1$ to ensure that $s_{11}=1$.

It remains to show that we can choose the same values for $s_{12}^i,t_{11}^i,t_{12}^i$ when $i=1,2$ and $G_0+f_1$ and $G_0+f_2$ are both type B.
Property (4) in the definition of type B gives $\{u_1u_2,u_3u_4\}\subset [F_v]$.
%$K_v\subset {\rm cl}(B_1)$.
Claim~\ref{claim:Fv} and the independence of $B_1$ now imply that ${\rm cl}(B_1^1)={\rm cl}(E_0+K_v)={\rm cl}(B_1^2)$.
This in turn implies that  $Z(B_1^1, \bp|_{V_0})=Z(B_1^2, \bp|_{V_0})$, so we can take
a common non-trivial motion that has the form stated in the claim.
This completes the proof of the first part of the claim.




%Hence by scaling $\bq_1$ we obtain the formulae as stated in the statement.
%(Note that $s_{11}, s_{12}, t_{11}, t_{12}$ are non-zero and independent from $i$ by $Z(B_1^1, p)=Z(B_1^2, p)$.)




\medskip

We next prove the second part of the claim. We can construct a non-trivial motion $\bq^i$ of $(G+f_i,\bp)$ with $\bq^i|_{V_0}=\sum_{j=1}^3 \beta^i_j \bq^i_j$ for some $\beta^i_j\in \R$ by adding a suitable trivial motion to an arbitrary non-trivial motion of $(G+f_i,\bp)$, as in the derivation of (\ref{eq:uncoupled2}). We need to show we can choose the $\beta^i_j$ to take the values stated in the claim.  
The proof is identical to that of the second part of Claim~\ref{claim:motionA} so we only give a sketch. 
As $i$ is fixed, we once more suppress the superscripts on $\beta^i, \bq^i$ and $\bq^i_j$.

Since $u_0u_k$ is an edge of $G$ for all $1\leq k\leq 5$, we have
$D_{0,k}\cdot [\bq(u_0)-\bq(u_k)]=0$ for all $1\leq k\leq 5$. 
Hence we obtain the system of equations
$$ D_{0,k}\cdot [\bq(u_0)-\beta_1 \bq_1(u_k)-\beta_2 \bq_2(u_k)-\beta_3 \bq_3(u_k)]=0 \mbox{ for $1\leq k\leq 5$}.$$
Putting $(a_0,b_0,c_0)=\bq(u_0)$ and
substituting the zero values for $\bq_j(u_k)$ given in the first  part of the claim, we may rewrite this system  as: 
\begin{equation}
\label{eq:beta1}
\left(
\begin{array}{cccc}
0 & D_{0,1}\cdot \bq_2(u_1) &  0 & D_{0,1} \\
0 & 0 &  0 & D_{0,2} \\
D_{0,3}\cdot \bq_1(u_3) & 0 &  D_{0,3}\cdot \bq_3(u_3) & D_{0,3} \\
D_{0,4}\cdot \bq_1(u_4) & D_{0,4}\cdot \bq_2(u_4) &  D_{0,4}\cdot \bq_3(u_4) & D_{0,4} \\
0 & 0 &  0 & D_{0,5} \\
\end{array}
\right) \left(
\begin{array}{c}
\beta_1 \\ \beta_2 \\ \beta_3\\ -a_0\\ -b_0\\ -c_0 
\end{array}
\right) = 0.
\end{equation}
Each entry of the form $D_{0,k}\cdot \bq_j(u_k)$ in the above matrix can be expressed as 
a product of areas of three triangles by using the non-zero values for $\bq_j(u_k)$ given in the first  part of the claim.
%For example, we have
%$$D_{01}\cdot q_2(u_1)=D_{01}\cdot (s_2D_{13}\times D_{15})= s_2\left|\begin{array}{c} D_{10}\\ D_{13} \\ D_{15}  \end{array}\right|
%=-\Delta_{103}\Delta_{135}\Delta_{150}.$$
By scaling $\bq$, we may suppose that $\beta_1+\beta_2+\beta_3=\mu$ for some constant $\mu$. 
We can now proceed as in the proof of Claim~\ref{claim:motionA} and obtain the stated formula for $\beta_j$ by setting $\mu={\rm det} M/ \Delta_{015}\Delta_{025}\Delta_{035}\Delta_{045}$, where $M=\left(
\begin{array}{c}
b\\M'
\end{array}
\right)$, $M'$ is the matrix of coefficients in (\ref{eq:beta1}) and $b=(1,1,1,0,0,0)$.
%
%
%set $c={\rm det} M/ \Delta_{015}\Delta_{025}\Delta_{035}\Delta_{045}$ for simplifying the resulting formulae as done in the proof of Claim~\ref{claim:coupled3}.
% Using Cramer's rule and expanding the determinants, one can get the formula of $\beta_j$ as written in the statement. A detailed calculation procedure is identical to the proof of Claim~\ref{claim:coupled3}.  
\end{proof}

We next state the analogous claims for the cases when $(G+f_i)$ is type C or D without proof as their proofs are identical to the proof of Claim~\ref{claim:motionA}.
%(We have double-checked by a computer if the formulae of the statements are correct.)
\begin{claim}\label{claim:motionC}
Suppose that $G_0+f_i$ is type C.
Then
for all $1\leq j\leq 3$, $(C_j^i,\bp|_{V_0})$ 
%is a 1-dof framework having 
has a non-trivial motion $\bq_j^i$ satisfying $\bq_j^i(w)\in \rat(\bp(V_0))$ for all $w\in V_0$,  and 
\begin{itemize}
\item $\bq_1^i(u_5)=\bq_1^i(u_1)=\bq_1^i(u_2)=0, \bq_1^i(u_3)= D_{3,2} \times D_{3,5}$, $\bq_1^i(u_4)=t_1 D_{4,1} \times D_{4,5}$;
\item $\bq_2^i(u_5)=\bq_2^i(u_2)=\bq_2^i(u_3)=0, \bq_2^i(u_1)= D_{1,3} \times D_{1,5}$, $\bq_2^i(u_4)=t_2^i D_{4,2} \times D_{4,5}$;
\item $\bq_3^i(u_5)=\bq_3^i(u_1)=\bq_3^i(u_2)=0, \bq_3^i(u_3)= D_{3,1} \times D_{3,5}$, $\bq_3^i(u_4)=t_3^i D_{4,2} \times D_{4,5}$;
\end{itemize}
for $t_1=\Delta_{523}/\Delta_{514}$ and some $t_2^i, t_3^i\in\mathbb{Q}(\bp(V_0))$. %$s_1=s_2=s_3=1$, and $t_1=\Delta_{523}/\Delta_{514}$.
%$t_1=\left|\begin{array}{c} D_{34} \\ D_{32} \\ D_{35} \end{array} \right| / \left|\begin{array}{c} D_{43} \\ D_{41} \\ D_{45} \end{array} \right|$.

In addition, $(G+f_i,\bp)$ has  a non-trivial motion $\bq^i$ such that 
$\bq^i|_{V_0}=\sum_{j=1}^3\gamma_j^i \bq_j^i$ where:
\begin{align*}
%\gamma_1^i&=-\Delta_{012}\Delta_{013}\Delta_{024}\Delta_{135}\Delta_{245}s_3t_2^i - \Delta_{013}^2\Delta_{024}\Delta_{135}^2s_2s_3 + \Delta_{013}\Delta_{023}\Delta_{024}\Delta_{135}\Delta_{245}s_2t_3^i; \\
\gamma_2^i&=\Delta_{012}\Delta_{013}\Delta_{014}\Delta_{135}\Delta_{145}t_1 - \Delta_{012}\Delta_{023}\Delta_{024}\Delta_{235}\Delta_{245}t_3^i;\\
\gamma_3^i&=\Delta_{012}\Delta_{023}\Delta_{024}\Delta_{235}\Delta_{245}t_2^i - \Delta_{013}\Delta_{014}\Delta_{023}\Delta_{135}\Delta_{145}t_1 + \Delta_{013}\Delta_{023}\Delta_{024}\Delta_{135}\Delta_{235}.
\end{align*}
\end{claim}

\begin{claim}\label{claim:motionD}
Suppose that $G_0+f_i$ is type D.
Then
for all $1\leq j\leq 3$, $(D_j^i,\bp|_{V_0})$ 
has
%is a 1-dof framework having 
a non-trivial motion $\bq_j^i$ satisfying $\bq_j^i(w)\in \rat(\bp(V_0))$ for all $w\in V_0$, 
 and 
\begin{itemize}
\item $\bq_1^i(u_5)=\bq_1^i(u_1)=\bq_1^i(u_2)=0, \bq_1^i(u_3)=D_{3,2} \times D_{3,5}$,  $\bq_1^i(u_4)=t_1 D_{4,1} \times D_{4,5}$;
\item $\bq_2^i(u_5)=\bq_2^i(u_3)=\bq_2^i(u_4)=0, \bq_2^i(u_1)=s_2^iD_{1,3} \times D_{1,5}$,  $\bq_2^i(u_2)=t_2^i D_{2,4} \times D_{2,5}$;
\item $\bq_3^i(u_5)=\bq_3^i(u_1)=\bq_3^i(u_2)=0, \bq_3^i(u_3)=s_3^iD_{3,1} \times D_{3,5}$, $\bq_3^i(u_4)=t_3^i D_{4,2} \times D_{4,5}$;
\end{itemize}
for $t_1=\Delta_{523}/\Delta_{514}$ and some $s_2^i, t_2^i, s_3^i, t_3^i\in\mathbb{Q}(\bp(V_0))$ 
with $\Delta_{513} s_j^i -\Delta_{524} t_j^i\neq 0$ for $j=2,3$.\footnote{The expression for $q_2^i$ contains two parameters $s^i_2,t^i_2$ because one of the edges $u_1u_4, u_2u_3$ may exist in $\cl(D^i_2)$, and hence we could have $q^i_2(u_1)=0$ or $q^i_2(u_2)=0$. We can deduce that $\Delta_{513}s^i_2-\Delta_{524}t^i_2\neq 0$ from the fact that the edge $u_1u_2$ is not in $\clo(D^i_2)$. A similar remark holds for $q_3^i$.}
%, $s_1=s_2=s_3=1$, and .
%$t_1=\left|\begin{array}{c} D_{34} \\ D_{32} \\ D_{35} \end{array} \right| / \left|\begin{array}{c} D_{43} \\ D_{41} \\ D_{45} \end{array} \right|$.

In addition, $(G+f_i,\bp)$ has  a non-trivial motion $\bq^i$ such that 
$\bq^i|_{V_0}=\sum_{j=1}^3\delta_j^i \bq_j^i$ where:
\begin{align*}
%\delta_2^i&=\Delta_{012}\Delta_{013}\Delta_{014}\Delta_{135}\Delta_{145}s_3t_1 - \Delta_{012}\Delta_{023}\Delta_{024}\Delta_{235}\Delta_{245}s_1t_3^i;\\
\delta_2^i=&\Delta_{012} \Delta_{013} \Delta_{014} \Delta_{135} \Delta_{145} s_3^it_1 - \Delta_{012} \Delta_{023} \Delta_{024} \Delta_{235} \Delta_{245}  t_3^i; \\
\delta_3^i=&-\Delta_{013} \Delta_{014} \Delta_{023} \Delta_{135} \Delta_{145} s_2^it_1 + \Delta_{013} \Delta_{014} \Delta_{024} \Delta_{145} \Delta_{245} t_1 t_2^i \\ 
&+\Delta_{013} \Delta_{023} \Delta_{024} \Delta_{135} \Delta_{235} s_2^i - \Delta_{014} \Delta_{023} \Delta_{024} \Delta_{235} \Delta_{245}  t_2^i.
\end{align*}
\end{claim}

We will show that each of the above expressions for a motion of $(G+f_i,p)$  
lead to a contradiction. We first show that the motion given by Claim \ref{claim:motionA} cannot occur.


\begin{claim}\label{claim:typeA}
$G_0+f_i$ cannot be of type A.
\end{claim}
\begin{proof}
Suppose, for a contradiction, that $G_0+f_i$ is type $A$. Let $\bq_j^i$ be the nontrivial motion of $(A^i_j,\bp|_{V_0})$ given by Claim \ref{claim:motionA}. 
We will omit the superscript $i$ from $\bq_j^i$ throughout the proof as it remains fixed. Let $\bp(u_0)=(x_0, y_0)$ and $\bp(u_5)=(x_5, y_5)$, and recall that the values of $\bp(u_k)$, $1\leq k\leq 4$, are given by (\ref{eq:quasi_generic}).
%(For $i\in \{1,\dots, 4\}$, $\bp(u_i)$ is given in (\ref{eq:quasi_generic}).)
We will contradict the choice of $G$ by showing that $(G+f_i,\bp)$ is a 1-dof framework with a bad motion at $u_0$.



%We first construct  a non-trivial motion $\bq^i$ of $(G+f_i, \bp)$ and a polynomial map $b:\hat{N}_G(u_0)\rightarrow \mathbb{Q}[X_0,Y_0,X_5, Y_5]^3$ such that 
%$\bq^i$ is a $b$-motion on $\hat{N}_G(u_0)$.
By Claim~\ref{claim:motionA}, $(G+f_i, \bp)$ has  a non-trivial motion $\bq^i$ such that
$\bq^i|_{V_0}=\sum_{j=1}^3 \alpha_j \bq_j$.
%, where $\beta_j$ and $\bq_j$ are as given in .
The formulae for $\alpha_j$, $j=1,2,3$,  and $\bq_j(u_k)$, $1\leq k\leq 5$, given in Claim~\ref{claim:motionB} imply that 
%we may express each coordinate of $\bq^i|_{V_0}$ as a polynomial in $x_0, y_0, x_5, y_5$ over $\mathbb{Q}$. Since $\bq^i|_{V_0}=\sum_{j=1}^3 \beta_j \bq_j$, 
each coordinate of $\bq^i(u_k)$, $1\leq k\leq 5$, can be expressed as a  polynomial in $x_0, y_0, x_5, y_5$ over $\mathbb{Q}$.  
We  show that the same is true for $\bq^i(u_0)$.

Let $\bq^i(u_0)=(a_0,b_0,c_0)$. 
%We may use the proof technique of Claim~\ref{claim:motionB}, to obtain:
We recall the the following linear system in the proof of  Claim~\ref{claim:motionA}:

\begin{equation}
\label{eq:Aq^i}
\left(
\begin{array}{cccc}
1 & 1 & 1 & 0  \\
0 & D_{0,1}\cdot \bq_2(u_1) &  0 & D_{0,1} \\
0 & 0 &  0 & D_{0,2} \\
D_{0,3}\cdot \bq_1(u_3) & 0 &  D_{0,3}\cdot \bq_3(u_3) & D_{0,3} \\
D_{0,4}\cdot \bq_1(u_4) & D_{0,4}\cdot \bq_2(u_4) &  D_{0,4}\cdot \bq_3(u_4) & D_{0,4} \\
0 & 0 &  0 & D_{0,5} \\
\end{array}
\right) \left(
\begin{array}{c}
\alpha_1 \\ \alpha_2 \\ \alpha_3\\ -a_0\\ -b_0\\ -c_0 
\end{array}
\right) = 
\left(
\begin{array}{c}
\mu \\ 0 \\ 0 \\ 0\\ 0\\ 0 
\end{array}
\right)
\end{equation}
where $\mu=\alpha_1+\alpha_2+\alpha_3\in \rat(\bp(\hat N_G(u_0)))$ takes the value given at the end of the proof of Claim~\ref{claim:motionA} so can be considered as a rational function of $x_0, y_0, x_5, y_5$ over $\rat$. 
Since each entry of the matrix of coefficients in (\ref{eq:Aq^i}) is a polynomial in  $x_0, y_0, x_5, y_5$, each of 
$a_0,b_0,c_0$ can be expressed as a rational function of $x_0, y_0, x_5, y_5$ over $\rat$.
Hence, by 
a further 
scaling 
%of 
$\bq^i$, we can suppose that each component of $\bq^i(u_k)$, $0\leq k\leq 5$, can be expressed as a polynomial in  $x_0, y_0, x_5, y_5$. 
This gives us a map $b:\hat{N}_G(u_0)\rightarrow \mathbb{Q}[X_0,Y_0,X_5, Y_5]^3$ such that 
$\bq^i$ is a $b$-motion on $\hat{N}_G(u_0)$.

We next show that $b$ satisfies (\ref{eq:bad}) i.e.
%For this it suffices to shows that 
the polynomial identity given by an edge $u_ku_\ell$, $1\leq k < \ell\leq 5$, 
%on $N(u_0)$ is deformed by $\bq$ 
is satisfied if and only if $\ell=5$. Since $x_0,y_0,x_5,y_5$ are generic, this is equivalent to showing that the motion $\bq^i$ satisfies the constraint  corresponding to the edge $u_ku_\ell$, %$1\leq k < \ell\leq 5$, 
%on $N(u_0)$ is deformed by $q$ 
if and only if $\ell=5$. 
Since the current motion $\bq^i$, is a non-zero scalar multiple of our original motion  
%$\bq^i=\sum_{j=1}\alpha_j \bq_j$ 
%over $N(u_0)$, 
it will suffice to show this for the original $\bq^i$. 
(More specifically, it will suffice to show $D_{k,\ell}\cdot (\bq^i(u_k)-\bq^i(u_{\ell}))\neq 0$ for $1\leq k<\ell\leq 4$ as $\bq^i$ is a motion of $(G+f_i,\bp)$ and ${\rm cl}(G+f_i)$ contains the star on $N_G(u_0)$ centered at $u_5$.) 
This follows since $\bq^i|_{V_0}=\sum_{j=1}^3\alpha_j \bq_j$ and each $u_ku_\ell$ is an edge of $\cl(A^i_j)$ for exactly two values $1\leq j\leq 3$.
% can be checked symbolically using the formulae for the $\alpha_j$ and $\bq_j(u_k)$ given in Claim~\ref{claim:motionA}.
%
%We have seen that each of $\beta_j$, $1\leq i\leq 3$ and each coordinate  of $q_j(u_k)$, $1\leq k\leq 5$ can be expressed as a polynomial in $x_0, y_0, x_5, y_5$. We can now  check symbolically that  
%$D_{k\ell} (q'(u_k)-q'(u_\ell))=0$ holds if and only if $\ell=5$.
%
%Since $\beta_j\neq 0$, from Figure~\ref{fig:B}, one can rapidly check that 
%$D_{kl} (q'(u_k)-q'(u_l))=0$ if $l=5$,
%and $D_{kl} (q'(u_k)-q'(u_l))\neq 0$ if $(k,l)\in \{(1,2), (1,3), (2,4)\}$.
%For the remaining three edges, one can check $D_{kl} (q'(u_k)-q'(u_l))\neq 0$ by a symbolic computation.
Thus $(G+f_i, \bp)$ has a bad motion at $u_0$.
%\end{proof}

%Note that $(G+f_i,p)$ is a 1-dof framework. 
Although $(G+f_i, \bp)$ is not generic as it satisfies (\ref{eq:quasi_generic}), Lemma~\ref{lem:projective_bad} ensures that we may use a projective transformation to construct a generic 1-dof framework $(G+f_i,\bp')$ which has a bad motion at $u_0$. This contradicts our  initial choice of $(G,\bp)$ to minimize $|V|$ and then $k$ since $k=2$ and $G+f_i$ is $1$-dof.
%In Section~\ref{subsec:1dof} we have already checked that a 
%no 1-dof generic framework with at most $|V|$ vertices has a bad motion.
\end{proof}

Our proof that the motions given by Claim \ref{claim:motionB}, \ref{claim:motionC} and \ref{claim:motionD}  cannot occur is more complicated because the expressions for the motions $\bq^i_j$ in these claims contain undetermined parameters. 
%
%The corresponding claim for type $B$ (Claim~\ref{claim:linear3} below) turns out to be substantially more difficult. 
We first give a preliminary claim which shows that 
%This claim is the unique part of our proof which requires the stronger induction hypothesis for $k$-dof parts with $k=1,2$. 
%We can reach this point in the proof by a much simpler argument if we restrict to $1$-dof parts, but we cannot rule out  the 
specific values of these parameters cannot occur when  
$G_0+f_i$ is type B. 
%(Analogous claims hold for types C and D but these are not needed in our proof.)
%$\bq_j^i$ which is forbidden by Claim~\ref{claim:bad_case}.


\begin{claim}\label{claim:bad_case}
Suppose that $G_0+f_i$ is type B.  Let $\bq^i$ and $\bq_j^i$ be the non-trivial motion of  $(G+f_i,\bp)$ and $(B_j^i,\bp|_{V_0})$, respectively,  given in Claim~\ref{claim:motionB}.
%Suppose further that 
Then 
%$\{s_{12},  t_{11}, t_{12}, t_2, t_3^i\}\not\subseteq \rat(\bp(\hat N_G(u_0)))$.
\[
 (s_{12},  t_{11}, t_{12}, t_2, t_3^i)\neq
\left( -\frac{\Delta_{513}}{\Delta_{523}}, \frac{\Delta_{513}}{\Delta_{514}}, 
-\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}\right).
\]
%
%We next use (\ref{eq:beta}) 
%to show that 
%Then $(G+f_i,\bp)$ has a bad motion at $u_0$.
\end{claim}
\begin{proof}
Suppose that $
 (s_{12},  t_{11}, t_{12}, t_2, t_3^i)=
\left( -\frac{\Delta_{513}}{\Delta_{523}}, \frac{\Delta_{513}}{\Delta_{514}}, 
-\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}\right)
$.
Then we can use the same argument as in the proof of Claim \ref{claim:typeA} to show that some scalar multiple of $\bq^i$ is a
  $b$-motion of $(G+f_i,\bp)$ on $\hat{N}_G(u_0)$ for some $b:\hat{N}_G(u_0)\rightarrow \mathbb{Q}[X_0,Y_0,X_5, Y_5]^3$. In order to
 verify that $b$ satisfies (\ref{eq:bad}) it suffices to show that 
$b$ satisfies
  $D_{k,\ell}\cdot (\bq^i(u_k)-\bq^i(u_{\ell}))\neq 0$ for all
  $u_ku_\ell\in K(u_1,u_2,u_3,u_4)$.  
This inequality holds for the edges $u_1u_2,u_1u_3,u_2u_4$ since they are  edges of $\cl(A^i_j)$ for exactly two values $1\leq j\leq 3$. We can verify the inequality holds for the remaining three edges by a direct computation using the expressions for the motions $\bq^i$ and $\bq^i_j$ given in Claim~\ref{claim:motionB}. For example, the facts that $u_1u_4$ is in $\cl(A^i_2)$, $q^i_1(u_1)=0=q^i_3(u_1)$ and $t_{12}=t_3^i$ give 
\begin{eqnarray*}
D_{1,4}\cdot (\bq^i(u_1)-\bq^i(u_{4}))&=&-D_{1,4}\cdot (\bq^i_1(u_4)+\bq^i_3(u_{4}))=t_{12}(\beta_1+\beta_3)
\left|
\begin{array}{c}
D_{4,1} \\ D_{4,2} \\ D_{4,3}
\end{array}\right|\\
&=&t_{12}\Delta_{513}^2 x_0(2x_0-1)(x_0-1)
\left|
\begin{array}{c}
D_{4,1} \\ D_{4,2} \\ D_{4,3}
\end{array}\right|
\neq 0.
\end{eqnarray*}
% can be checked symbolically using the formulae for the $\alpha_j$ and $\bq_j(u_k)$ given in Claim~\ref{claim:motionA}.
%
%We have seen that each of $\beta_j$, $1\leq i\leq 3$ and each coordinate  of $q_j(u_k)$, $1\leq k\leq 5$ can be expressed as a polynomial in $x_0, y_0, x_5, y_5$. We can now  check symbolically that  
%$D_{k\ell} (q'(u_k)-q'(u_\ell))=0$ holds if and only if $\ell=5$.
%
%Since $\beta_j\neq 0$, from Figure~\ref{fig:B}, one can rapidly check that 
%$D_{kl} (q'(u_k)-q'(u_l))=0$ if $l=5$,
%and $D_{kl} (q'(u_k)-q'(u_l))\neq 0$ if $(k,l)\in \{(1,2), (1,3), (2,4)\}$.
%For the remaining three edges, one can check $D_{kl} (q'(u_k)-q'(u_l))\neq 0$ by a symbolic computation.
Thus $(G+f_i, \bp)$ has a bad motion at $u_0$.

We can now use Lemma~\ref{lem:projective_bad}  to construct a generic 1-dof framework $(G+f_i,\bp')$ which has a bad motion at $u_0$. This contradicts our  initial choice of $(G,\bp)$ to minimize $|V|$ and then $k$ since $k=2$ and $G+f_i$ is $1$-dof.
\end{proof}

We can use Claim \ref{claim:bad_case} to obtain the following key result for handling the case when $G_0+f_i$ is type B.

\begin{claim}\label{claim:linear3}
Suppose that $G_0+f_i$ is type B, and, for $1\leq j\leq 3$, let $\bq_j^i$ be the non-trivial motion of  $(B_j^i,\bp|_{V_0})$ given in Claim~\ref{claim:motionB}.
%Suppose $\beta_2^i,\beta_3^i$ are as defined in Claim~\ref{claim:motionB} and 
If $\lambda_2\beta_2+\lambda_3\beta_3=0$ for some $\lambda_2,\lambda_3\in \mathbb{Q}(\bp(V_0))$, then $\lambda_2=\lambda_3=0$.
\end{claim}
\begin{proof}
 We will again omit the superscript $i$ from the proof since it stays fixed. We assume that  $\lambda_2\beta_2+\lambda_3\beta_3=0$ for some $\lambda_2,\lambda_3\in \mathbb{Q}(\bp(V_0))$ which are not both zero, and show that this contradicts Claim \ref{claim:bad_case}. 
% $$ (s_{12}^i,  t_{11}^i, t_{12}^i, t_2^i, t_3^i)=
%\left( -\frac{\Delta_{513}}{\Delta_{523}}, \frac{\Delta_{513}}{\Delta_{514}}, 
%-\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}\right)$$
%
%We first use the same proof technique as for Claims~\ref{claim:linear1} and (\ref{eq:quasi_generic}) to show that 
%\begin{equation}\label{eq:beta}
%(s_{12}, t_{11}, t_{12}, t_2, t_3^i)=
%\left( -\frac{\Delta_{513}}{\Delta_{523}}, \frac{\Delta_{513}}{\Delta_{514}}, 
%-\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}\right).
%\end{equation}

Let  $\bp(u_i)=(x_i, y_i)$ for $0\leq i\leq5$. 
By Claim~\ref{claim:motionB} we have an explicit formula for each $\beta_i$ in terms of $x_0,\dots, x_5, y_0, \dots, y_5$.
Since $V_0=V\setminus \{u_0\}$, 
 we may regard each $\beta_i$ as a polynomial in $x_0, y_0$ with coefficients in $\mathbb{Q}(\bp(V_0))$. 
If $\lambda_2\beta_2+\lambda_3\beta_3=0$ with $\lambda_i\in \mathbb{Q}(\bp(V_0))$, then $\lambda_2\beta_2+\lambda_3\beta_3$ is identically zero as a polynomial in $x_0, y_0$. 
In particular, the coefficient of each monomial is zero. 
%We show this cannot happen unless $\lambda_i=0$ for all $i$.
%

Using Claim~\ref{claim:motionB} and (\ref{eq:quasi_generic}),
a computation of the list of coefficients of the polynomial $\lambda_2\beta_2+\lambda_3\beta_3$ in $x_0, y_0$ over $\mathbb{Q}(\bp(V_0))$ gives:
\begin{itemize}
\item[$x_0^3$:] $-\Delta_{513}^2 \lambda_3 + \Delta_{513} \Delta_{514} \lambda_3 t_{11} - \Delta_{513} \Delta_{523} \lambda_3 s_{12} + \Delta_{513} \Delta_{524} \lambda_3 t_{12}$,
\item[$x_0^2y_0$:] $-\Delta_{513} \Delta_{514} \lambda_2 t_{11} + \Delta_{513} \Delta_{514} \lambda_3 t_{11} + \Delta_{513} \Delta_{523} \lambda_3 s_{12} - \Delta_{513} \Delta_{524} \lambda_2 t_{12}$ 

 $+ \Delta_{513} \Delta_{524} \lambda_2 t_3 +  \Delta_{523} \Delta_{524} \lambda_2 s_{12} t_3$,
\item[$x_0^2$:] $2 \Delta_{513}^2 \lambda_3 - 2 \Delta_{513} \Delta_{514} \lambda_3 t_{11} + \Delta_{513} \Delta_{523} \lambda_3 s_{12} - \Delta_{513} \Delta_{524} \lambda_3 t_{12}$,
\item[$x_0 y_0^2$:] $\Delta_{513}^2 \lambda_3 - \Delta_{513} \Delta_{514} \lambda_2 t_{11} - \Delta_{513} \Delta_{524} \lambda_3 t_{12} - \Delta_{523} \Delta_{524} \lambda_2 s_{12} t_3$,
\item[$x_0y_0$:] $-\Delta_{513}^2 \lambda_3 + 2 \Delta_{513} \Delta_{514} \lambda_2 t_{11} - \Delta_{513} \Delta_{514} \lambda_3 t_{11} - \Delta_{513} \Delta_{523} \lambda_3 s_{12} + \Delta_{513} \Delta_{524} \lambda_2 t_{12} - \Delta_{513} \Delta_{524} \lambda_2 t_3 +  \Delta_{513} \Delta_{524} \lambda_3 t_{12}$,
\item[$x_0$:] $-\Delta_{513}^2 \lambda_3 + \Delta_{513} \Delta_{514} \lambda_3 t_{11}$,
\item[$y_0^3$:] $\Delta_{513} \Delta_{524} \lambda_2 t_{12} - \Delta_{513} \Delta_{524} \lambda_2 t_3$,
\item[$y_0^2$:] $-\Delta_{513}^2 \lambda_3 + \Delta_{513} \Delta_{514} \lambda_2 t_{11} - \Delta_{513} \Delta_{524} \lambda_2 t_{12} + \Delta_{513} \Delta_{524} \lambda_2 t_3$,
\item[$y_0$:] $\Delta_{513}^2 \lambda_3 - \Delta_{513} \Delta_{514} \lambda_2 t_{11}$
\end{itemize}
where  $s_{12}, t_{11}, t_{12}, t_3$ are all  non-zero by Claim~\ref{claim:motionB}.
% if the coefficients are all zero with $a\neq 0$ or $b\neq 0$, then  $(s_{12}, t_{11}, t_{12}, t_3)$ takes the value as given in the statement.
%(Indeed, 
Since $\lambda_2\beta_2+\lambda_3\beta_3=0$, all coefficients are zero. The hypothesis that $\lambda_2,\lambda_3$ are not both zero and the expression for the coefficient of $y_0$ give $\lambda_2\neq 0$ and $\lambda_3\neq 0$.
The coefficient of $x_0$ now gives $t_{11}=\Delta_{513}/\Delta_{514}$, and
the coefficient of $y_0$ now gives $\lambda_2=\lambda_3$.
Then the coefficients of $x_0^3$ and $y_0^2$, give $s_{12}=\Delta_{524} t_{12}/ \Delta_{523}$ and $t_3=t_{12}$.
Finally, the coefficient of $x_0^2y_0$ gives $t_{12}=-\Delta_{513}/\Delta_{524}$.
Hence 
$$ (s_{12},  t_{11}, t_{12}, t_2, t_3)=
\left( -\frac{\Delta_{513}}{\Delta_{523}}, \frac{\Delta_{513}}{\Delta_{514}}, 
-\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}\right).$$
This contradicts Claim~\ref{claim:bad_case}.
\end{proof}



Our next result is key to handling the cases when $G_0+f_i$ is type C or D.

%We next give an analogous claim to Claim~\ref{claim:coupled2} for types A, C and D. 
%implies that no non-trivial linear combination of $\alpha_1^i, \alpha_2^i, \alpha_3$.
%By the same argument we have the following:
\begin{claim}\label{claim:linear1} Suppose  
%$\alpha_j^i, 
$\gamma_j^i,\delta_j^i, $ are as in Claims~\ref{claim:motionC} and \ref{claim:motionD}, respectively.\\
%(a) If $\lambda_1\alpha_1^i+\lambda_2\alpha_2^i+\lambda_3\alpha_3^i=0$ for some $\lambda_1,\lambda_2,\lambda_3\in \mathbb{Q}(\bp(V_0))$, then $\lambda_1=\lambda_2=\lambda_3=0$.\\
(a) If $\lambda_2\gamma_2^i+\lambda_3\gamma_3^i=0$ for some $\lambda_2,\lambda_3\in \mathbb{Q}(\bp(V_0))$, then $\lambda_2=\lambda_3=0$.
\\
(b) If $\lambda_2\delta_2^i+\lambda_3\delta_3^i=0$ for some $\lambda_2,\lambda_3\in \mathbb{Q}(\bp(V_0))$, then $\lambda_2=\lambda_3=0$.
\end{claim}
\begin{proof}
We first prove (a).
Let  $\bp(u_i)=(x_i, y_i)$ for $0\leq i\leq5$. 
As in the proof  of Claim~\ref{claim:linear3}, we regard each $\gamma_j^i$ as a polynomial in $x_0, y_0$ with coefficients in $\mathbb{Q}(\bp(V_0))$. 
Suppose $\sum_{2\leq j\leq 3} \lambda_j \gamma_j^i=0$ with $\lambda_j^i\in \mathbb{Q}(\bp(V_0))$. Then $P:=\sum_{2\leq j\leq 3} \lambda_j \gamma_j^i$ is identically zero as a polynomial in $x_0, y_0$. 
Using Claim~\ref{claim:motionC} and (\ref{eq:quasi_generic}), we find that the coefficient of $y_0^2$ in $P$ is $\Delta_{513}\Delta_{523} \lambda_2$,
and hence $\lambda_2=0$. This implies that the coefficient of $x_0y_0$ in $P$ is $-2\Delta_{513}\Delta_{523} \lambda_3$ and hence $\lambda_3=0$.

We next prove (b). 
If $\sum_{2\leq j\leq 3} \lambda_j \delta_j^i=0$ with $\lambda_j^i\in \mathbb{Q}(\bp(V_0))$, then $Q:=\sum_{2\leq j\leq 3} \lambda_j \delta_j^i$ is identically zero as a polynomial in $x_0, y_0$. 
Using Claim~\ref{claim:motionD} and (\ref{eq:quasi_generic}), 
we find that the coefficient of $x_0^2$ in $Q$ is $(-\Delta_{513} s_2^i + \Delta_{524}t_2^i)\Delta_{523} \lambda_3$.
Since  $\Delta_{513} s_2^i - \Delta_{524}t_2^i\neq 0$ by Claim~\ref{claim:motionD}, 
 $\lambda_3=0$. This implies that the coefficient of $x_0^2y_0$ in $Q$ is $(-\Delta_{513} s_3^i + \Delta_{524}t_3^i)\Delta_{523} \lambda_2$.
Since  $\Delta_{513} s_3^i - \Delta_{524}t_3^i\neq 0$ by Claim~\ref{claim:motionD}, 
 $\lambda_2=0$.
%Let  $\bp(u_i)=(x_i, y_i)$ for $0\leq i\leq5$. 
%By Claim~\ref{claim:motionA} we have an explicit formula for each $\alpha_i$ in terms of $x_0,\dots, x_5, y_0, \dots, y_5$.
%Since $V_0=V\setminus \{u_0\}$, 
% we may regard each $\alpha_i$ as a polynomial in $x_0, y_0$ with coefficients in $\mathbb{Q}(\bp(V_0))$. 
%If $\sum_{1\leq i\leq 3} \lambda_i \alpha_i=0$ with $\lambda_i\in \mathbb{Q}(\bp(V_0))$, then $\sum_{1\leq i\leq 3} \lambda_i \alpha_i$ is identically zero as a polynomial in $x_0, y_0$. 
%In particular, the coefficient of each monomial is zero. 
%We show this cannot happen unless $\lambda_i=0$ for all $i$.
%
%Using Claim~\ref{claim:motionA} and (\ref{eq:quasi_generic}) to compute $\sum_{1\leq i\leq 3} \lambda_i \alpha_i$ explicitly,
%%where $s_j$ and $t_j$ are given in  Claim~\ref{claim:coupled1}. 
%%By a computation (using (\ref{eq:semi-generic})) we obtain  
%we obtain the following list of coefficients of the monomials in $\sum_{1\leq i\leq 3} \lambda_i \alpha_i$.
%\begin{description}
%\item[$x_0^3:$] $\Delta_{513}^2\lambda_1 - \Delta_{524}^2\lambda_1$
%\item[$x_0^2y_0:$] $(-\Delta_{513}^2\Delta_{523}\lambda_2 + 2\Delta_{513}^2\Delta_{523}\lambda_3 + \Delta_{523}\Delta_{524}^2\lambda_2)/\Delta_{513}$ 
%\item[$x_0^2:$] $-2\Delta_{513}^2\lambda_1 - \Delta_{513}\Delta_{523}\lambda_3 + \Delta_{524}^2\lambda_1$ 
%\item[$x_0 y_0^2:$]  $(-\Delta_{513}^3\lambda_1 - \Delta_{513}^2\Delta_{523}\lambda_2 + \Delta_{513}\Delta_{524}^2\lambda_1 - \Delta_{523}\Delta_{524}^2\lambda_2)/\Delta_{513}$
%\item[$x_0y_0:$]  $\Delta_{513}^2\lambda_1 + 2\Delta_{513}\Delta_{523}\lambda_2 - 2\Delta_{513}\Delta_{523}\lambda_3 - \Delta_{524}^2\lambda_1$
%\item[$x_0:$] $\Delta_{513}^2\lambda_1 + \Delta_{513}\Delta_{523}\lambda_3$
%\item[$y_0^2:$] $\Delta_{513}^2\lambda_1 + \Delta_{513}\Delta_{523}\lambda_2$
%\item[$1:$] $-\Delta_{513}^2\lambda_1 - \Delta_{513}\Delta_{523}\lambda_2$
%\end{description}
%We can easily check  that  if all  eight coefficients are zero, then $\lambda_1=\lambda_2=\lambda_3=0$. 
\end{proof}




%Part (a) follows immediately from 
%Claim~\ref{claim:coupled2}. The proofs of (b) and (c) are identical to that of Claim~\ref{claim:coupled2}. We willl sketch the proof of (c) for completeness.
%
%$a\delta_2^i+b\delta_3^i=0$ for $a,b\in \mathbb{Q}(p(V_0))$.
%By Claim~\ref{claim:motionD}, each $\delta_j$ can be considered as a polynomial in $x_0, y_0$ over $\mathbb{Q}(p(V_0))$, where $p(u_0)=(x_0,y_0)$.
%Since $a,b\in \mathbb{Q}(p(V_0))$, $a\delta_2^i+b\delta_3^i$ is also a polynomial in $x_0, y_0$ over $\mathbb{Q}(p(V_0))$. Since $a\delta_2^i+b\delta_3^i=0$,  the coefficient of each monomial is zero. 
%The formulae given in Claim~\ref{claim:motionD} and (\ref{eq:quasi_generic}) now give the following  list of coefficients of $a\delta_2^i+b\delta_3^i$:
%\begin{itemize}
%\item[$x_0^2 y_0$:] $\Delta_{513} \Delta_{523} b + \Delta_{523} \Delta_{524} a t_3^i - \Delta_{523} \Delta_{524} b t_2^i$,
%\item[$x_0^2$:] $-\Delta_{513} \Delta_{523} b + \Delta_{523} \Delta_{524} b t_2^i$,
%\item[$x_0 y_0^2$:] $\Delta_{513} \Delta_{523} b - \Delta_{523} \Delta_{524} a t_3^i + \Delta_{523} \Delta_{524} b t_2^i$,
%\item[$x_0 y_0$:] $-\Delta_{513} \Delta_{523} \Delta_{524} a - 2 \Delta_{513} \Delta_{523} b$,
%\item[$x_0$:] $\Delta_{513} \Delta_{523} b - \Delta_{523} \Delta_{524} b t_2^i$,
%\item[$y_0^2$:] $-\Delta_{523} \Delta_{524} b t_2^i$,
%\item[$y_0$:]  $\Delta_{513} \Delta_{523} \Delta_{524} a + \Delta_{523} \Delta_{524} b t_2^i$.
% \end{itemize}
%It is straightforward to show that, if each coefficient is zero, then $a=b=0$.
%\end{proof}




%We next show that the conclusion of  Claim~\ref{claim:linear2} cannot hold.
% then $(G+f_i,p)$ has a bad motion at $u_0$.

%Hence Claim~\ref{claim:linear2} and Claim~\ref{claim:bad_case} imply the following:
%\begin{claim}\label{claim:linear3}
%If $a\beta_2^i+b\beta_3^i=0$ for $a,b\in \mathbb{Q}(\bp(V_0))$, then $a=b=0$.
%\end{claim}
%\end{proof}

We next 
%can use the same proof technique to 
obtain quadratic versions of Claims~\ref{claim:linear3} and \ref{claim:linear1}.
\begin{claim}\label{claim:quadratic}
Let 
%$\alpha_j^i, 
$\beta_j^i, 
\gamma_j^i, \delta_j^i$ be as defined in Claims~\ref{claim:motionB}, 
\ref{claim:motionC} and \ref{claim:motionD}, and  $\lambda_{h,j}\in \mathbb{Q}(\bp(V_0))$ for all $1\leq h,j\leq 3$. 
\begin{description}
%\item[AA:] If $\sum_{1\leq h\leq 3}\sum_{1\leq j\leq 3} \lambda_{h,j} \alpha_h^1\alpha_j^2=0$, then $\lambda_{k,k}=0$ for some $k\in \{1,2,3\}$.
%
%\item[A-B:] If $\sum_{1\leq h\leq 3}\sum_{2\leq j\leq 3} \lambda_{h,j} \alpha_h^1\beta_j^2=0$, then $\lambda_{k,k}=0$ for some $k\in \{2,3\}$.
%
\item[BB:] If $\sum_{2\leq h\leq 3}\sum_{2\leq j\leq 3} \lambda_{h,j} \beta_h^1\beta_j^2=0$, then $\lambda_{k,k}=0$ for some $k\in \{2,3\}$.

\item[CC:] If $\sum_{2\leq h\leq 3}\sum_{2\leq j\leq 3} \lambda_{h,j} \gamma_h^1\gamma_j^2=0$, then $\lambda_{k,k}=0$ for some $k\in \{2,3\}$.

\item[DD:] If $\sum_{2\leq h\leq 3}\sum_{2\leq j\leq 3} \lambda_{h,j} \delta_h^1\delta_j^2=0$, then $\lambda_{k,k}=0$ for some $k\in \{2,3\}$.
\end{description}
\end{claim}
\begin{proof}
We first check case (CC).
Suppose $\sum_{2\leq i\leq 3}\sum_{2\leq j\leq 3} \lambda_{i,j} \gamma_i^1\gamma_j^2=0$. 
We may regard this as a polynomial identity with indeterminates  $x_0, y_0$ and hence the coefficient of each monomial must be zero.
If we compute the formula for $\sum_{2\leq i\leq 3}\sum_{2\leq j\leq 3} \lambda_{i,j} \gamma_i^1\gamma_j^2$ explicitly using Claim~\ref{claim:motionC} and (\ref{eq:quasi_generic}), we find that
the coefficient of $y_0^4$  is 
$\Delta_{513}^2\Delta_{523}^2 \lambda_{2,2}$.
Since $\Delta_{513}\neq 0$ and $\Delta_{523}\neq 0$, we obtain $\lambda_{2,2}=0$.

We next check case (DD).
Suppose $\sum_{2\leq i\leq 3}\sum_{2\leq j\leq 3} \lambda_{i,j} \delta_i^1\delta_j^2=0$. 
%We may regard this as a polynomial identity with indeterminates  $x_0, y_0$ and hence the coefficient of each monomial must be zero.
If we compute the formula for $\sum_{2\leq i\leq 3}\sum_{2\leq j\leq 3} \lambda_{i,j} \delta_i^1\delta_j^2$ explicitly using Claim~\ref{claim:motionD} and (\ref{eq:quasi_generic}), we find that
the coefficient of $x_0^4$  is $\Delta_{523}^2 \lambda_{3,3}(\Delta_{524}t_2^1-T_{513}s_2^1)(\Delta_{524}t_2^2-\Delta_{513}s_2^2)$.
Since $\Delta_{524}t_2^i-\Delta_{513}s_2^i\neq 0$ by Claim~\ref{claim:motionD}, we obtain $\lambda_{3,3}=0$.

Case (BB) can be verified in  the same way by using (\ref{eq:quasi_generic}), Claim~\ref{claim:motionB},  and Claim~\ref{claim:bad_case}. The main steps are as follows. We suppose that $P:=\sum_{2\leq h\leq 3}\sum_{2\leq j\leq 3} \lambda_{h,j} \beta_h^1\beta_j^2=0$ and $\lambda_{k,k}\neq 0$ for $k\in\{2,3\}$. 
The coefficient of $x_0^2$ in $P$  implies that $t_{11}=\Delta_{513}/\Delta_{514}$, and the coefficient of $y_0^6$ implies that either $t_{12}=t_{3}^1$ or $t_{12}=t_{3}^2$. By symmetry we may assume that $t_{12}=t_{3}^1$. Then 
%the coefficient of $x_0^2$ gives $t_{11}=\Delta_{135}/\Delta_{145}$, 
the coefficient of $x_0^4$ gives $s_{12}=t_{3}^1\Delta_{524}/\Delta_{523}$, and the coefficient of $y_0^2$ gives $\lambda_{3,2}=\lambda_{2,2}+\lambda_{3,3}-\lambda_{2,3}$. 
The coefficient of $x_0y_0^2$ now implies that either $\lambda_{3,3}=\lambda_{2,3}$ or $t_3^1=t_3^2$. 
If $t_3^1\neq t_3^2$ then we have $\lambda_{3,3}=\lambda_{2,3}$, the coefficient of $x_0y^5$ now implies that $t_{3}^1=-\Delta_{513}/\Delta_{524}$   and the resulting values of $t_{12},s_{12}$ contradict Claim \ref{claim:bad_case}. Hence $t_3^1=t_3^2$. The coefficient of $x_0y_0^3$ and the fact that $t_{3}^1\neq -\Delta_{513}/\Delta_{524}$ by Claim \ref{claim:bad_case} then give $\lambda_{2,2}=\lambda_{3,3}$. The coefficient of $x_0^2y_0^4$ now gives $t_{3}^1=-\Delta_{513}/\Delta_{524}$ and this again contradicts Claim \ref{claim:bad_case}.
%}
%In Case (C-C), the coefficient of $y_0^2$ is $\Delta_{513}^2 \Delta_{523}^2 \lambda_{22}$.
%Hence $\lambda_{22}=0$ follows.
 \end{proof}

%\begin{claim}\label{claim:quadraticB}
%Suppose that $(G_0,F)$ is type AB or BB. 
%For $1\leq j\leq 3$, let $\alpha^i_j$ be as given in Claim~\ref{claim:motionA}, let $\beta_j^i$ be as given in Claim~\ref{claim:motionB},
%%Let $\alpha_h^1$, for $1\leq h\leq 3$, and $\beta_h^1$, for $1\leq h\leq 2$, be as defined in Claims~\ref{claim:motionA} and \ref{claim:motionB}, respectively 
%and let $\lambda_{h,j}\in \mathbb{Q}(\bp(V_0))$ for all $1\leq h,j\leq 3$. 
%\begin{description}
%\item[AB:] If $\sum_{1\leq h\leq 3}\sum_{2\leq j\leq 3} \lambda_{h,j} \alpha_h^1\beta_j^2=0$, then $\lambda_{k,k}=0$ for some $k\in \{2,3\}$.
%
%\item[BB:] If $\sum_{2\leq h\leq 3}\sum_{2\leq j\leq 3} \lambda_{h,j} \beta_h^1\beta_j^2=0$, then $\lambda_{k,k}=0$ for some $k\in \{2,3\}$.
%\end{description}
%\end{claim}
%\begin{proof}
%We may apply the same proof technique as Claim \ref{claim:quadratic} to deduce that either $\lambda_{k,k}=0$ for some $k\in \{2,3\}$ or 
%\[
%(s_{12}, t_{11}, t_{12}, t_2, t_3^i)=
%\left(-\frac{\Delta_{513}}{\Delta_{523}}, \frac{\Delta_{513}}{\Delta_{514}}, 
%-\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}, -\frac{\Delta_{513}}{\Delta_{524}}\right)
%\]
%for some $i\in \{1,2\}$.
%The second alternative cannot happen by  Claim~\ref{claim:bad_case}.
%\end{proof}

We  close this section with an observation on the type 0 case.
\begin{claim}\label{claim:motion0}
Suppose that $G_0+f_i$ is type 0. Then 
$(G+f_i, \bp)$ has a non-trivial motion $\bq^i$ such that 
$\bq^i|_{V_0}$ is a non-trivial motion of $(G_0+f_i+K_u,\bp|_{V_0})$, $\bq^i(v_0)=\bq^i(v_1)=\bq^i(v_5)=0$, and
$\bq^i(w)\in \mathbb{Q}(\bp(V_0))$ for all $w\in V_0$.
\end{claim}
\begin{proof}
Since $G_0+f_i$ is type 0, there are two edges $e_1, e_2\in K$ such that 
$K_u\subseteq {\rm cl}(E_0+f_i+e_1+e_2)$.
Since $G+f_i$ is $C_2^1$-independent, we have ${\rm cl}(G+f_i+e_1+e_2-u_0u_4-u_0u_5)={\rm cl}(G+f_i)$ and hence $K_u\subseteq {\rm cl}(G+f_i)$.
This implies that  every non-trivial motion of $(G_0+f_i+e_1+e_2, \bp|_{V_0})$ is extendable to a non-trivial motion $\bq^i$ of $(G+f_i,\bp)$. Since $K(v_0,v_1,v_5)\subset G$ by (\ref{eq:Kv}), we may combine $\bq^i$ with a suitable trivial motion to ensure that $\bq^i(v_0)=\bq^i(v_1)=\bq^i(v_5)=0$. By scaling, we may also assume that some component of $\bq_i|_{V_0}$ is equal to one. Since $(G_0+f_i+e_1+e_2, \bp|_{V_0})$ is a 1-dof framework, we may now use Cramer's rule to deduce that $\bq^i(w)\in \mathbb{Q}(\bp(V_0))$ for all $w\in V_0$.
\end{proof}


\subsubsection{Completing the proof of Theorem \ref{thm:well-behaved}}\label{subsubsec:6}

We are now ready to complete the proof of Theorem \ref{thm:well-behaved}. 
Recall that $(G,\bp)$ is a minimal counterexample to Theorem \ref{thm:well-behaved}, and  has a motion $\bq_{\rm bad}$ which is bad at $v_0$, and $F=\{f_1,f_2\}\in {{F_v}\choose{2}}$ is a good pair.
Since  $K(v_0, v_1, v_5)\subset G$ by (\ref{eq:Kv}),
we may combine $\bq_{\rm bad}$ with a suitable trivial motion $\bt$ so that the resulting motion 
\begin{equation}\label{eq:q+t}
\hat{\bq}_{\rm bad}:=\bq_{\rm bad}+\bt
\end{equation}
 satisfies 
$\hat{\bq}_{\rm bad}(v_0)=\hat{\bq}_{\rm bad}(v_1)=\hat{\bq}_{\rm bad}(v_5)=0$.
Similarly, if $G_0+f_i$ is type X for some X in $\{$B,C,D$\}$,
%for all $1\leq i\leq 3$, 
we may combine the motion $\bq_j^i$ of $(X_j^i,\bp|_{V_0})$ given in Claims~\ref{claim:motionA}-\ref{claim:motionD} with a suitable trivial motion $\bt_j^i$ so that the resulting motion 
\begin{equation}\label{eq:q_j^i+t_j^i}
\hat{\bq}_j^i:=\bq_j^i+\bt_j^i
\end{equation}
 satisfies  
$\hat{\bq}_j^i(v_0)=\hat{\bq}_j^i(v_1)=\hat{\bq}_j^i(v_5)=0$.
Since all entries of ${\bq}_{\rm bad}(v_k)$ and ${\bq}_j^i(v_k)$ are contained in $\mathbb{Q}(\bp(V_0))$ for each $v_k\in \hat{N}_G(v_0)$, we may deduce that all entries of 
$\hat{\bq}_{\rm bad}(v_k)$ and $\hat{\bq}_j^i(v_k)$ are contained in $\mathbb{Q}(\bp(V_0))$ for each $v_k\in \hat{N}_G(v_0)$.


%
%As in the proof for the 1-dof case, the proof is done by pinning down three points to eliminate trivial motions.
%We shall first set up this for completeness.
%Since $(G,p)$ is a counterexample to Theorem \ref{thm:well-behaved}, it has a $b$-motion $q^*$ which is bad on  $\hat{N}(v_0)$. 
%Consider triangle $\{v_0, v_1, v_5\}$ in $G_0$.
%By adding some trivial motion $q^{\rm tri}$ to $q^*$, $\hat{q}^*:=q^*+q^{\rm tri}$ satisfies 
%$\hat{q}^*(v_0)=\hat{q}^*(v_1)=\hat{q}^*(v_5)=0$.
%Also let $q^i_j$ be a non-trivial motion discussed in  Claim~\ref{claim:motionA}-Claim~\ref{claim:motionD}.
%Adding some trivial motion
%$q_{{\rm tri},j}^i$ to $q_j^i$, $\hat{q}_j^i:=q_j^i+q_{{\rm tri},j}^i$ satisfies 
%$\hat{q}_j^i(v_0)=\hat{q}_j^i(v_1)=\hat{q}_j^i(v_5)=0$.
%Note that all entries of ${q}^*(v_k)$ are contained in $\mathbb{Q}(p(V_0))$ for each $v_k\in \hat{N}_G(v_0)$ by ${q}^*(v_k)=b_{v_k}$.
%Similarly, by Claim~\ref{claim:motionA}-Claim~\ref{claim:motionD}, all entries of ${q}_j^i(v_k)$ are contained in $\mathbb{Q}(p(V_0))$ for each $v_k\in \hat{N}_G(v_0)$.
%Hence all entries of $\hat{q}^*(v_k)$ and $\hat{q}_j^i(v_k)$ are contained in $\mathbb{Q}(p(V_0))$ for each $v_k\in \hat{N}_G(v_0)$. 

We will use the following parameterization of the motion space of $(G,\bp)$ over $\hat{N}_G(v_0)$. Let $G_v$ be the subgraph of $G$ induced by $\hat N_G(v_0)$. Then (\ref{eq:Kv}) implies that $G_v$ is isomorphic to the graph obtained from a complete bipartite graph $K_{2,4}$ by adding an edge between the two vertices in the 2-set $\{v_0,v_5\}$ of the bipartition. See Figure~\ref{fig:K24plus}.
\begin{figure}[h]
\centering
\includegraphics[scale=0.6]{K24plus}
\caption{$G_v$.}
\label{fig:K24plus}
\end{figure}
%Recall by (\ref{eq:Kv}) that $G$ has $K_{2,4}^+$ on $\hat{N}(v_0)$, where $\{v_0,v_5\}$ is one side and $\{v_1,v_2,v_3,v_4\}$ is the other side. 
Let 
%$(G_v,p|_{\hat{N}(v_0)})$ be the restriction of $(G,p)$ to $\hat{N}(v_0)$, and let 
$Z'$ be the space of all motions $\bq'$ of $(G_v,\bp|_{\hat{N}(v_0)})$ with $\bq'(v_0)=\bq'(v_1)=\bq'(v_5)=0$.
As $G_v$ is a 3-dof graph, $Z'$ is a 3-dimensional linear space.
Since $u_0\not\in V(G_v)$ we may choose a base $B$ for $Z'$ in which the coordinates of each vector lie in $\rat(\bp(V_0))$, and let $\psi:Z'\rightarrow \mathbb{R}^3$ be the linear bijection which maps $B$ onto the standard base of $\R^3$. Note that $\psi$ can be represented by a matrix over $\mathbb{Q}(\bp(V_0))$.
%
%Since $\hat{q}^*(v_0)=\hat{q}^*(v_1)=\hat{q}^*(v_5)$, we can write
%\begin{align*}
%&\hat{q}^*(v_2)=k_2 D_{20}\times D_{25}, \\
%&\hat{q}^*(v_3)=k_3 D_{30}\times D_{35}, \\
%&\hat{q}^*(v_4)=k_4 D_{40}\times D_{45}
%\end{align*}
% by some $k_2, k_3, k_4\in \mathbb{Q}(\bp(V_0))$. 
%Denote $k^*=(k_2, k_3, k_4)^{\top}\in \mathbb{R}^3$.
%By the same manner $k_j^i\in \mathbb{R}^3$ is defined from $\hat{q}_j^i$.

Using  Claims \ref{claim:types} and \ref{claim:typeA}, and relabeling $u_1,u_2,u_3,u_4$ and $f_1,f_2$ if necessary, we may assume that each $G_0+f_i$ is type 0, B, C or D, and that $(G_0,F)$ is type  BB, CC or DD if neither $G_0+f_1$ nor $G_0+f_2$ is type 0.
The proof is completed by considering the following three cases, depending on the type of each $G+f_i$.  %the following case analysis depending on the type of $G+f_i$.

\medskip
\noindent \emph{Case 1:} Neither $G_0+f_1$ nor $G_0+f_2$ is type 0. \\
%We shall first consider the case when neither $G_0+f_1$  nor $G_0+f_1$ are type 0.
%
Let $\bq^i$ be the non-trivial motion of $(G+f_i,\bp)$ given in Claims~\ref{claim:motionB}-\ref{claim:motionD}. Then $\bq^i|_{V_0}=\sum_{j=1}^3\chi_j^i\bq_j^i$ for some appropriate $\chi\in \{\beta,\gamma,\delta\}$  and we put 
\begin{equation}\label{eq:58.1}
\hat \bq^i=\bq^i+\sum_{j=1}^3\chi_j^i \bt_j^i
\end{equation}
where $\bt_j^i$ is the trivial motion given in (\ref{eq:q_j^i+t_j^i}) 
(and we are abusing notation by using the same symbol $\bt_j^i$ for a trivial motion of $(G+f_i,\bp)$ and its restriction to $V_0$). 
%By (\ref{eq:coupled1}), 
Then, by  $\bq^i|_{V_0}=\sum_{j=1}^3\chi_j^i\bq_j^i$  and (\ref{eq:q_j^i+t_j^i}), 
$$\hat \bq^i|_{V_0}=\bq^i|_{V_0}+\sum_{j=1}^3\chi_j^i \bt_j^i=\sum_{j=1}^3\chi_j^i \bq_j^i+\sum_{j=1}^3\chi_j^i \bt_j^i=\sum_{j=1}^3\chi_j^i (\bq_j^i+\bt_j^i)=\sum_{j=1}^3\chi_j^i \hat{\bq}_j^i.$$ 
%
%
%$\sum_{j=1}^3\alpha_j^i \hat{q}_j$ (resp., $\sum_{j=1}^3\beta_j^i \hat{q}_j$, $\sum_{j=1}^3\gamma_j^i \hat{q}_j$, $\sum_{j=1}^3\delta_j^i \hat{q}_j$ depending on the type) is the restriction of $\hat q^i$  to $V_0$.
As $(f_1, f_2)$ is a good pair, $Z(G,\bp)=Z_0(G,\bp)\oplus \langle \hat{\bq}^1, \hat{\bq}^2\rangle$ holds.
Hence, by Lemma~\ref{lem:canonical}, 
\begin{equation}\label{eq:58.5}
\hat{\bq}_{\rm bad}\in \langle \hat{\bq}^1, \hat{\bq}^2\rangle.
\end{equation}
%
%Suppose that $(G_0,F)$  is type AA. Since $\hat{\bq}_{\rm bad}\in \langle \hat{\bq}^1, \hat{\bq}^2\rangle$ we have 
%\begin{equation}\label{eq:AA1}
%\hat{\bq}_{\rm bad}|_{V_0}\in \left\langle \sum_{j=1}^3\alpha_j^1 \,\hat{\bq}_j^1|_{V_0}, \sum_{j=1}^3\alpha_j^2 \,\hat{\bq}_j^2|_{V_0}\right\rangle.
%\end{equation}
%By restricting our attention to $\hat{N}(v_0)$ in $G$, we obtain
%\begin{equation}\label{eq:AA2}
%\hat{\bq}_{\rm bad}|_{\hat{N}(v_0)}\in \left\langle \sum_{j=1}^3\alpha_j^1\, \hat{\bq}_j^1|_{\hat{N}(v_0)}, \sum_{j=1}^3\alpha_j^2\, \hat{\bq}_j^2|_{\hat{N}(v_0)}\right\rangle.
%\end{equation}
% 
%
%Let $k$ and $k_j^i$ denote the images of $\hat{\bq}_{\rm bad}|_{\hat{N}(v_0)}$ and $\hat{\bq}_j^i|_{\hat{N}(v_0)}$,  respectively, under $\psi$. Then (\ref{eq:AA2}) implies that 
%\[
%{\rm det} 
%\left(\begin{array}{c|c|c}
% & & \\
% k& \sum_{j=1}^3\alpha_j^1 k_j^1 & \sum_{j=1}^3\alpha_j^2 k_j^2 \\
% & & 
% \end{array}\right)=0,
%\]
%%where $k^*$ and $k_j^i$ denotes the image of $\hat{\bq}^*|_{\hat{N}(v_0)}$ and $(\hat{\bq}_j^i)|_{\hat{N}(v_0)}$ by $\psi$, respectively.
%and the bilinearity of the determinant gives
%\[
%\sum_{1\leq i\leq 3}\sum_{1\leq j\leq 3}{\rm det} 
%\left(\begin{array}{c|c|c}
% & & \\
% k &  k_i^1 &  k_j^2 \\
% & & 
% \end{array}\right)\alpha_i^1\alpha_j^2=0.
%\]
%Since all of the entries of $k,k_i^1,k_j^2$ lie in $\rat(\bp(V_0))$ by our choice of $\psi$, Claim~\ref{claim:quadratic} now gives
%\[
%{\rm det} 
%\left(\begin{array}{c|c|c}
% & & \\
% k &  k_j^1 &  k_j^2 \\
% & & 
% \end{array}\right)=0
%\]
%for some $j\in \{1,2,3\}$. Without loss of generality we may assume $j=1$. Then
%$k$ is a linear combination of $k_1^1$ and $k_1^2$ so $\hat{\bq}_{\rm bad}|_{\hat{N}(v_0)}=a\,\hat{\bq}_1^1|_{\hat{N}(v_0)}+b\,\hat{\bq}_1^2|_{\hat{N}(v_0)}$
%for some $a,b\in \R$. 
%Let 
%\[
%\bar \bq :=a\,\hat{\bq}_1^1+b\,\hat{\bq}_1^2.
%\]
%%This in turn implies that  a linear combination of 
%%$\hat{\bq}_1^1$ and $\hat{\bq}_1^2$ is a $b$-motion.
%Since $\hat{\bq}_1^i$ is  a non-trivial motion of $(A_1^i, \bp|_{V_0})$ and $A_1^i=G_0+f_i+u_1u_2+u_2u_3$,
%%Hence, any linear combination of $\hat{\bq}_1^1$ and $\hat{\bq}_1^2$  
%$\bar \bq$ is a motion of $(G_0+u_1u_2+u_2u_3,\bp|_{V_0})$. 
%%Recall that $\hat \bq_{\rm bad}|_{V_0}=\bq_{\rm bad}|_{V_0}+\bt|_{V_0}$ for some trivial motion $\bt$. 
%Let 
%\[
%\tilde \bq:=\bar \bq- \bt,
%\] 
%where $\bt$ is the trivial motion given in (\ref{eq:q+t}).
%Then $\tilde\bq$ is a motion of 
%the 2-dof framework $(G_0+u_1u_2+u_2u_3,\bp|_{V_0})$ and 
%$$\tilde \bq|_{\hat{N}(v_0)}=\bar \bq|_{\hat{N}(v_0)}- \bt|_{\hat{N}(v_0)}=\hat \bq_{\rm bad}|_{\hat{N}(v_0)}- \bt|_{\hat{N}(v_0)}=\bq_{\rm bad}|_{\hat{N}(v_0)}.$$
%Hence $\tilde \bq$ is bad at $v_0$ on the framework $(G_0+u_1u_2+u_2u_3,\bp|_{V_0})$.
%% of the 2-dof framework $(G_0+u_1u_2+u_2u_3,\bp|_{V_0})$.  
%This contradicts the fact that $(G,\bp)$ is a minimal counterexample.

%Next we consider the case when 
Suppose $(G_0,F)$  is type BB. Since $\hat{\bq}_{\rm bad}\in \langle \hat{\bq}^1, \hat{\bq}^2\rangle$ by (\ref{eq:58.1}), we have 
\begin{equation}\label{eq:BB1}
\hat{\bq}_{\rm bad}|_{V_0}\in \left\langle \sum_{j=1}^3\beta_j^1 \,\hat{\bq}_j^1|_{V_0}, \sum_{j=1}^3\beta_j^2 \,\hat{\bq}_j^2|_{V_0}\right\rangle.
\end{equation}
We also have $K_v\subseteq {\rm cl}(B_1^i)$ by Property (4) of the definition of type B, so
$\hat{\bq}_1^i|_{\hat{N}(v_0)}=0$ for both $i=1,2$.
Hence the restriction of (\ref{eq:BB1}) to $\hat{N}(v_0)$ gives
\begin{equation}\label{eq:BB2}
\hat{\bq}_{\rm bad}|_{\hat{N}(v_0)}\in \left\langle \sum_{j=2}^3\beta_j^1 \,\hat{\bq}_j^1|_{\hat{N}(v_0)}, \sum_{j=2}^3\beta_j^2 \,\hat{\bq}_j^2|_{\hat{N}(v_0)}\right\rangle.
\end{equation}

Let $k$ and $k_j^i$ denote the images of $\hat{\bq}_{\rm bad}|_{\hat{N}(v_0)}$ and $\hat{\bq}_j^i|_{\hat{N}(v_0)}$,  respectively, under $\psi$. Then (\ref{eq:BB2}) implies that 
\[
{\rm det} 
\left(\begin{array}{c|c|c}
 & & \\
 k& \sum_{j=2}^3\beta_j^1 k_j^1 & \sum_{j=2}^3\beta_j^2 k_j^2 \\
 & & 
 \end{array}\right)=0,
\]
%where $k^*$ and $k_j^i$ denotes the image of $\hat{\bq}^*|_{\hat{N}(v_0)}$ and $(\hat{\bq}_j^i)|_{\hat{N}(v_0)}$ by $\psi$, respectively.
and the bilinearity of the determinant gives
\[
\sum_{i=2}^3\sum_{j=2}^3{\rm det} 
\left(\begin{array}{c|c|c}
 & & \\
 k &  k_i^1 &  k_j^2 \\
 & & 
 \end{array}\right)\beta_i^1\beta_j^2=0.
\]
%
%
%
%
%
%and we may deduce as above that
%\[
%{\rm det} 
%\left(\begin{array}{c|c|c}
% & & \\
% k & \sum_{j=2}^3\beta_j^1 k_j^1 & \sum_{j=2}^3\beta_j^2 k_j^2, \\
% & & 
% \end{array}\right)=0
%\]
%where $k$ and $k_j^i$ denote the images of $\hat{\bq}_{\rm bad}|_{\hat{N}(v_0)}$ and $\hat{\bq}_j^i|_{\hat{N}(v_0)}$,  respectively, under $\psi$.
%The bilinearity of the determinant now gives 
%\[
%\sum_{2\leq i\leq 3}\sum_{2\leq j\leq 3}{\rm det} 
%\left(\begin{array}{c|c|c}
% & & \\
% k &  k_i^1 &  k_j^2 \\
% & & 
% \end{array}\right)\beta_i^1\beta_j^2=0,
%\]
Claim~\ref{claim:quadratic} now implies that
\[
{\rm det} 
\left(\begin{array}{c|c|c}
 & & \\
 k &  k_j^1 &  k_j^2 \\
 & & 
 \end{array}\right)=0
\]
for some $j\in \{2,3\}$. We may assume without loss of generality that $j=2$.
Then
$k$ is a linear combination of $k_2^1$ and $k_2^2$ so $\hat{\bq}_{\rm bad}|_{\hat{N}(v_0)}=a\,\hat{\bq}_2^1|_{\hat{N}(v_0)}+b\,\hat{\bq}_2^2|_{\hat{N}(v_0)}$
for some $a,b\in \R$. 
Let 
\[
\bar \bq :=a\,\hat{\bq}_2^1+b\,\hat{\bq}_2^2.
\]
%This in turn implies that  a linear combination of 
%$\hat{\bq}_1^1$ and $\hat{\bq}_1^2$ is a $b$-motion.
Since $\hat{\bq}_2^i$ is  a non-trivial motion of $(B_2^i, \bp|_{V_0})$ and $B_2^i=G_0+f_i+u_1u_3+u_2u_3$,
%Hence, any linear combination of $\hat{\bq}_1^1$ and $\hat{\bq}_1^2$  
$\bar \bq$ is a motion of $(G_0+u_1u_3+u_2u_3,\bp|_{V_0})$. 
%Recall that $\hat \bq_{\rm bad}|_{V_0}=\bq_{\rm bad}|_{V_0}+\bt|_{V_0}$ for some trivial motion $\bt$. 
Let 
\[
\tilde \bq:=\bar \bq- \bt,
\] 
where $\bt$ is the trivial motion given in (\ref{eq:q+t}).
Then $\tilde\bq$ is a motion of 
the 2-dof framework $(G_0+u_1u_3+u_2u_3,\bp|_{V_0})$ and 
$$\tilde \bq|_{\hat{N}(v_0)}=\bar \bq|_{\hat{N}(v_0)}- \bt|_{\hat{N}(v_0)}=\hat \bq_{\rm bad}|_{\hat{N}(v_0)}- \bt|_{\hat{N}(v_0)}=\bq_{\rm bad}|_{\hat{N}(v_0)}.$$
Hence $\tilde \bq$ is bad a bad motion at $v_0$ for the framework $(G_0+u_1u_3+u_2u_3,\bp|_{V_0})$.
% of the 2-dof framework $(G_0+u_1u_2+u_2u_3,\bp|_{V_0})$.  
This contradicts the fact that $(G,\bp)$ is a minimal counterexample.




%
%We can now use a similar argument to the case when $(G_0,F)$ is type AA to deduce that the 2-dof framework 
%$(G_0+u_2u_3+u_3u_1,\bp|_{V_0})$ has a bad motion at $v_0$, contradicting the fact that
%%This in turn implies that  a linear combination of 
%%$\hat{q}_2^1$ and $\hat{q}_2^2$ is a $b$-motion.
%%Recall that $\hat{q}_2^i$ is  a non-trivial motion of $(B_2^i, p|_{V_0})$ with $B_1^i=G_0+f_i+u_2u_3+u_3u_1$.
%%Hence, any linear combination of 
%%$\hat{q}_2^1$ and $\hat{q}_2^2$  is a motion of  $(G_0+u_2u_3+u_3u_1,p|_{V_0})$, and in particular the 2-dof framework $(G_0+u_2u_3+u_3u_1,p|_{V_0})$ has the $b$-motion.
%%This contradicts that 
%$(G,\bp)$ is a minimal counterexample.

The remaining cases when $(G_0,F)$ is type  CC or DD can be solved similarly.
% using Claims~\ref{claim:quadratic} and \ref{claim:quadraticB}.


\medskip
\noindent \emph{Case 2:} $G_0+f_1$ is type 0 and $G_0+f_2$ is not. \\
%Suppose that $G_0+f_1$ is type 0 and  $G_0+f_2$ is type X for some ${\rm X}\in \{\rm  A, B, C, D\}$. 
We only give a proof for the case when $G_0+f_2$ is type B since the other cases can be solved in an identical manner.

By Claim~\ref{claim:motion0}, $(G+f_1,\bp)$ has a non-trivial motion $\bq^1$ such that $\bq^1|_{V_0}$ is a motion of $(G_0+f_1+K_u, \bp|_{V_0})$, $\bq^1(v_0)=\bq^1(v_1)=\bq^1(v_5)=0$ and $\bq^1(w)\in \mathbb{Q}(\bp(V_0))$ for all $w\in V_0$. 
%By adding non-trivial motions, we may suppose that $\bq^i(v_0)=\bq^i(v_1)=\bq^i(v_5)=0$.

Let $\hat{\bq}^2=\bq^2+\sum_{j=1}^3\beta^2_j \bt^2_j$ be as defined in (\ref{eq:58.1}). 
Since  $(f_1, f_2)$ is a good pair, $Z(G,\bp)=Z_0(G,\bp)\oplus \langle {\bq}^1, \hat{\bq}^2\rangle$ holds.
Hence, by Lemma~\ref{lem:canonical},   $\hat{\bq}_{\rm bad}\in \langle {\bq}^1, \hat{\bq}^2\rangle$.
Since $K_v\subseteq {\rm cl}(B_1^2)$ by Property (4) of the definition of type B, this gives
\begin{equation}\label{eq:0B1}
\hat{\bq}_{\rm bad}|_{\hat{N}(v_0)}\in \left\langle \bq^1|_{\hat{N}(v_0)}, \sum_{j=2}^3\beta_j^2 \,\hat{\bq}_j^2|_{\hat{N}(v_0)}\right\rangle.
\end{equation}
As in the previous case, this implies that 
\[
{\rm det} 
\left(\begin{array}{c|c|c}
 & & \\
 k & k^1 & \sum_{j=2}^3\beta_j^2 k_j^2 \\
 & & 
 \end{array}\right)=0,
\]
where $k$, $ k^1$, $k_j^2$ are the image of $\hat \bq_{\rm bad}|_{\hat{N}(v_0)}$, $\bq^1|_{\hat{N}(v_0)}$, $\hat{\bq}_j^2|_{\hat{N}(v_0)}$, respectively, under $\psi$.
The bilinearity of the determinant now gives 
\[
\sum_{2\leq j\leq 3}{\rm det} 
\left(\begin{array}{c|c|c}
 & & \\
 k &  k^1 &  k_j^2 \\
 & & 
 \end{array}\right)\beta_j^2=0,
\]
and Claim~\ref{claim:linear3} implies that 
\[
{\rm det} 
\left(\begin{array}{c|c|c}
 & & \\
 k &  k^1 &  k_j^2 \\
 & & 
 \end{array}\right)=0
\]
for each $j\in \{2,3\}$. In particular, we have that
$k$ is a linear combination of $k^1$ and $k_2^2$ so $\hat{\bq}_{\rm bad}|_{\hat{N}(v_0)}=a{\bq}^1|_{\hat{N}(v_0)}+b\hat{\bq}_2^2|_{\hat{N}(v_0)}$
for some $a,b\in \R$. Let $\bar \bq :=a{\bq}^1|_{V_0}+b\hat{\bq}_2^2$.
%This in turn implies that  a linear combination of 
%$\hat{\bq}_1^1$ and $\hat{\bq}_1^2$ is a $b$-motion.
Since
$\bq^1|_{V_0}$ is a motion of $(G_0+f_1+K_u, \bp|_{V_0})$ and
$\hat{\bq}_2^2$ is  a  motion of $(B_2^2, \bp|_{V_0})$ where $B_2^2=G_0+f_2+u_2u_3+u_3u_1$,
$\bar \bq$ is a motion of $(G_0+u_2u_3+u_3u_1,\bp|_{V_0})$. 
%Recall that $\hat \bq_{\rm bad}|_{V_0}=\bq|_{V_0}+\bt$ for some trivial motion $\bt$. 
Let $\tilde \bq:=\bar \bq- \bt$, where $\bt$ is the trivial motion given in (\ref{eq:q+t}).
Then $\tilde \bq$ is a motion of the 2-dof framework $(G_0+u_2u_3+u_3u_1,\bp|_{V_0})$ and 
$$\tilde \bq|_{\hat{N}(v_0)}=\bar \bq|_{\hat{N}(v_0)}- \bt|_{\hat{N}(v_0)}=\hat \bq_{\rm bad}|_{\hat{N}(v_0)}- \bt|_{\hat{N}(v_0)}=\bq_{\rm bad}|_{\hat{N}(v_0)}.$$
Hence $\tilde \bq$ is bad at $v_0$.
% of the 2-dof framework $(G_0+u_1u_2+u_2u_3,\bp|_{V_0})$.  
This contradicts the fact that $(G,\bp)$ is a minimal counterexample.





%
%
%This in turn implies that  a linear combination of 
%$q^1|_{V_0}$ and $\hat{q}_2^2$ is a $b$-motion.
%Recall that 
%$q^1|_{V_0}$ is a motion of $(G_0+f_1+K_u, p|_{V_0})$ whereas
%$\hat{q}_2^2$ is  a  motion of $(B_2^i, p|_{V_0})$ with $B_2^2=G_0+f_2+u_2u_3+u_3u_1$.
%Hence, any linear combination of $q^1|_{V_0}$ and $\hat{q}_2^2$ is a  motion of $(G_0+u_2u_3+u_3u_1,p|_{V_0})$, and in particular the 2-dof framework $(G_0+u_2u_3+u_3u_1,p|_{V_0})$ has the $b$-motion.
%This contradicts that $(G,p)$ is a minimal counterexample.

\medskip
\noindent \emph{Case 3:} Both $G_0+f_1$ and $G_0+f_2$ are type 0. \\ 
%Suppose that both $G_0+f_i$ are type 0.
By Claim~\ref{claim:motion0}, $(G+f_i, \bp)$ has a motion $\bq^i$ such that $\bq^i|_{V_0}$ is a motion of $(G_0+f_i+K_u, \bp|_{V_0})$, $\bq^i(v_0)=\bq^i(v_1)=\bq^i(v_5)=0$ and $\bq^i(w)\in \mathbb{Q}(\bp(V_0))$ for all $w\in V_0$. 

As $(f_1, f_2)$ is a good pair, $Z(G,\bp)=Z_0(G,\bp)\oplus \langle \bq^1, \bq^2\rangle$ holds.
Hence, by Lemma~\ref{lem:canonical},  $\hat{\bq}_{\rm bad}\in \langle \bq^1, \bq^2\rangle$.
This gives
\begin{equation}\label{eq:001}
\hat{\bq}_{\rm bad}|_{\hat{N}(v_0)}\in \left\langle \bq^1|_{\hat{N}(v_0)}, \bq^2|_{\hat{N}(v_0)}\right\rangle.
\end{equation}
and hence
\[
{\rm det} 
\left(\begin{array}{c|c|c}
 & & \\
 k & k^1 &  k^2 \\
 & & 
 \end{array}\right)=0,
\]
where $k$, $k^1$, $k^2$ are the image of $\hat \bq_{\rm bad}|_{\hat{N}(v_0)}$, $\bq^1|_{\hat{N}(v_0)}$, $\bq^2|_{\hat{N}(v_0)}$respectively, under $\psi$.
This in turn implies that  $\hat \bq_{\rm bad}|_{\hat{N}(v_0)}$ is a linear combination of  $\bq^1|_{\hat{N}(v_0)}$ and $\bq^2|_{\hat{N}(v_0)}$.
We can now use a similar argument to the previous case to deduce that 
$(G_0+K_u,\bp|_{V_0})$ has a bad motion at $v_0$. Since $(G_0+K_u,\bp|_{V_0})$ is a $k$-dof framework for some $k=1,2$, this  contradicts the minimality of $(G,\bp)$.

This completes the proof of Theorem~\ref{thm:well-behaved}.
%
%
%
%a linear combination of 
%$\bq^1|_{V_0}$ and $\bq^2|_{V_0}$ is a $b$-motion.
%Recall that $\bq^i|_{V_0}$ is a motion of $(G_0+f_i+K_u, p|_{V_0})$.
%Hence, any linear combination of $\bq^1|_{V_0}$ and $q^2|_{V_0}$ is a  motion of $(G_0+K_u,p|_{V_0})$, and in particular  $(G_0+K_u,p|_{V_0})$ has the $b$-motion.
%Since $(G_0+K_u,p|_{V_0})$ is 1-dof or 2-dof, this contradicts that $(G,p)$ is a minimal counterexample.





